Tractable Inference in Credal Sentential Decision Diagrams

Probabilistic sentential decision diagrams are logic circuits where the inputs of disjunctive gates are annotated by probability values. They allow for a compact representation of joint probability mass functions defined over sets of Boolean variables, that are also consistent with the logical constraints defined by the circuit. The probabilities in such a model are usually learned from a set of observations. This leads to overconfident and prior-dependent inferences when data are scarce, unreliable or conflicting. In this work, we develop the credal sentential decision diagrams, a generalisation of their probabilistic counterpart that allows for replacing the local probabilities with (so-called credal) sets of mass functions. These models induce a joint credal set over the set of Boolean variables, that sharply assigns probability zero to states inconsistent with the logical constraints. Three inference algorithms are derived for these models, these allow to compute: (i) the lower and upper probabilities of an observation for an arbitrary number of variables; (ii) the lower and upper conditional probabilities for the state of a single variable given an observation; (iii) whether or not all the probabilistic sentential decision diagrams compatible with the credal specification have the same most probable explanation of a given set of variables given an observation of the other variables. These inferences are tractable, as all the three algorithms, based on bottom-up traversal with local linear programming tasks on the disjunctive gates, can be solved in polynomial time with respect to the circuit size. For a first empirical validation, we consider a simple application based on noisy seven-segment display images. The credal models are observed to properly distinguish between easy and hard-to-detect instances and outperform other generative models not able to cope with logical constraints.

==> pgfcirc.defines.tex <==
%% Key managements

\long\def\pgf@circ@comment#1{}

\def\circuitikzbasekey{/tikz/circuitikz}

\pgfkeys{\circuitikzbasekey/.is family}

\def\circuitikzset#1{\pgfkeys{\circuitikzbasekey,#1}}
\let\ctikzset\circuitikzset
\def\ctikzvalof#1{\pgfkeysvalueof{\circuitikzbasekey/#1}}
\def\ctikzsetvalof#1#2{\pgfkeyssetvalue{\circuitikzbasekey/#1}{#2}}

%% Temporary Counters

\newcount\pgf@circ@count@a
\newcount\pgf@circ@count@b
\newcount\pgf@circ@count@c
%%%%%%%%%%%%
%% Dimensions

% coordinates
\newdimen\pgf@circ@res@up
\newdimen\pgf@circ@res@down
\newdimen\pgf@circ@res@zero
\newdimen\pgf@circ@res@left
\newdimen\pgf@circ@res@right
\newdimen\pgf@circ@res@other
\newdimen\pgf@circ@res@step
\newdimen\pgf@circ@res@temp
% inital thickness
\newdimen \pgfstartlinewidth

% arrow tips, ported over old arrows library (deprecated)
% see https://tex.stackexchange.com/questions/234084/latex-arrow-tip-with-arrows-meta-library
% this was the original definition of latex' tips, renamed to avoid clashes
%
\pgfarrowsdeclare{latexslim}{latexslim}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{+-4\pgfutil@tempdima}
  \pgfarrowsrightextend{+6\pgfutil@tempdima}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfpathmoveto{\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{3.5\pgfutil@tempdima}{.5\pgfutil@tempdima}}
  {\pgfqpoint{-1\pgfutil@tempdima}{1.5\pgfutil@tempdima}}
  {\pgfqpoint{-4\pgfutil@tempdima}{3.75\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-1.5\pgfutil@tempdima}{1\pgfutil@tempdima}}
  {\pgfqpoint{-1.5\pgfutil@tempdima}{-1\pgfutil@tempdima}}
  {\pgfqpoint{-4\pgfutil@tempdima}{-3.75\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-1\pgfutil@tempdima}{-1.5\pgfutil@tempdima}}
  {\pgfqpoint{3.5\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
  {\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfill
}

\pgfarrowsdeclarereversed{latexslim reversed}{latexslim reversed}{latexslim}{latexslim}

\def\pgf@circ@setifdefinedfill#1#2{%
    % if \ctikzclass is defined and \ctikzclass/fill is defined and is not none:
    % set the fill color and execute \pgfusepath{#1}, else execute \pgfusepath{#2}
    \ifdefined\ctikzclass
        \pgfkeysifdefined{\circuitikzbasekey/\ctikzclass/fill}%
        {% yes, it's defined
            \edef\@@tmp{\ctikzvalof{\ctikzclass/fill}}\edef\@@none{none}%
            \ifx\@@tmp\@@none % but it's none
                \pgfusepath{#2}%
            \else
                \pgfsetfillcolor{\@@tmp}%
                \pgfusepath{#1}%
            \fi
        }{% the class is defined but the fill key not; use  #2
            \pgfusepath{#2}%
        }
    \else
    \pgfusepath{#2}%
    \fi
}

%% Macro to fill or draw

\def\pgf@circ@draworfill{%
    \ifx\tikz@fillcolor\pgfutil@empty
        \pgf@circ@setifdefinedfill{draw,fill}{draw}
    \else
        \pgfsetfillcolor{\tikz@fillcolor}
        \pgfusepath{draw, fill}
    \fi
}

\def\pgf@circ@draworfillandclip{%
    \ifx\tikz@fillcolor\pgfutil@empty
        \pgf@circ@setifdefinedfill{draw, clip, fill}{draw, clip}
        \pgfusepath{draw, clip}
    \else
        \pgfsetfillcolor{\tikz@fillcolor}
        \pgfusepath{draw, clip, fill}
    \fi
}

\def\pgf@circ@maybefill{%
    \ifx\tikz@fillcolor\pgfutil@empty
        \pgf@circ@setifdefinedfill{fill}{discard}
    \else
        \pgfsetfillcolor{\tikz@fillcolor}
        \pgfusepath{fill}
    \fi
}

%% Macros for setting linewidth
% #1 is the legacy class (bipoles, tripoles) etc
% #2 is the reference linewidth
\def\pgf@circ@setlinewidth#1#2{%
    \ifdefined\ctikzclass
        \pgfkeysifdefined{\circuitikzbasekey/\ctikzclass/thickness}%
        {% yes, it's defined
        \edef\@@tmp{\ctikzvalof{\ctikzclass/thickness}}\edef\@@none{none}%
        \ifx\@@tmp\@@none % but it's none
            \pgfsetlinewidth{\ctikzvalof{#1/thickness}#2}% passthrough legacy class
        \else
            \pgfsetlinewidth{\@@tmp #2}%
        \fi
        }{ % key not defined, do the legacy thing
            \pgfsetlinewidth{\ctikzvalof{#1/thickness}#2}%
        }% Ok, do nothing
    \else % no class
        \pgfsetlinewidth{\ctikzvalof{#1/thickness}#2}%
    \fi
}
% use \pgf@circ@setlinewidth{none}{\pgflinewidth} if there is no legacy case
\ctikzset{none/thickness/.initial=1.0} % do not touch

%% font changes compatible with plain/LaTeX/ConTeXt
%% thanks to Henri Menke https://github.com/circuitikz/circuitikz/issues/285#issuecomment-537224605

\ifpgfutil@format@is@latex
    \long\def\pgf@circ@font@tiny{\tiny}
    \long\def\pgf@circ@font@small{\small}
    \long\def\pgf@circ@font@bold{\textbf}
    \long\def\pgf@circ@font@boldmath{\boldmath}
    \long\def\pgf@circ@font@sixbm{\fontsize{6}{7}\selectfont\boldmath}
    \long\def\pgf@circ@font@tenbm{\fontsize{10}{12}\selectfont\boldmath}
    \long\def\pgf@circ@font@twelve{\fontsize{12}{14}\selectfont}
\else\ifpgfutil@format@is@plain
    \long\def\pgf@circ@font@tiny{\fiverm}
    \long\def\pgf@circ@font@small{\sevenrm}
    \long\def\pgf@circ@font@bold#1{{\bf#1}}
    \long\def\pgf@circ@font@boldmath{\bf}       % to be tested
    \long\def\pgf@circ@font@sixbm{\sevenrm\bf}  %
    \long\def\pgf@circ@font@tenbm{\tenrm\bf}    %
    \long\def\pgf@circ@font@twelve{\twelverm}   %
\else\ifpgfutil@format@is@context
    \long\def\pgf@circ@font@tiny{\tfxx}
    \long\def\pgf@circ@font@small{\tfx}
    \long\def\pgf@circ@font@bold{\bold}
    \long\def\pgf@circ@font@boldmath{\bold}    % to be tested
    \long\def\pgf@circ@font@sixbm{\tfx\bold}   %
    \long\def\pgf@circ@font@tenbm{\normal\bold}%
    \long\def\pgf@circ@font@twelve{\tfa}       %
\fi\fi\fi


% voltage options

\newif\ifpgf@circ@siunitx
\newif\ifpgf@circuit@compat
\newif\ifpgf@circ@oldvoltagedirection % default false
\newif\ifpgf@circ@explicitvdir
\newif\ifpgf@circ@fixbatteries

\ctikzset{voltage dir/.is choice}
\ctikzset{voltage dir/old/.code={\pgf@circ@oldvoltagedirectiontrue\pgf@circ@fixbatteriesfalse}}
\ctikzset{voltage dir/noold/.code={\pgf@circ@oldvoltagedirectionfalse\pgf@circ@fixbatteriesfalse}}
\ctikzset{voltage dir/RP/.code={\pgf@circ@oldvoltagedirectiontrue\pgf@circ@fixbatteriestrue}}
\ctikzset{voltage dir/EF/.code={\pgf@circ@oldvoltagedirectionfalse\pgf@circ@fixbatteriestrue}}
\tikzset{voltage dir/.style={circuitikz/voltage dir=#1}}

% Option ">" for twoports
\newif\ifpgf@circuit@inputarrow
\ctikzset{>/.add code={}{\pgf@circuit@inputarrowtrue}}
\ctikzset{inputarrow/.is choice}
\ctikzset{inputarrow/true/.code={\pgf@circuit@inputarrowtrue}}
\ctikzset{inputarrow/false/.code={\pgf@circuit@inputarrowfalse}}

% Option "boxed" for nodes and twoports
\newif\ifpgf@circuit@boxed
\pgfkeys{/tikz/boxed/.add code={}{\pgf@circuit@boxedtrue}}
\ctikzset{boxed/.add code={}{\pgf@circuit@boxedtrue}}
\pgfkeys{/tikz/box/.add code={}{\pgf@circuit@boxedtrue}}
\ctikzset{box/.add code={}{\pgf@circuit@boxedtrue}}

% Option "dashed" for nodes and twoports
\newif\ifpgf@circuit@dashed
\pgfkeys{/tikz/dashed/.add code={}{\pgf@circuit@dashedtrue}}
\ctikzset{dashed/.add code={}{\pgf@circuit@dashedtrue}}

% Option "t=*" for nodes
\pgfkeys{/tikz/t/.add code={}{\ctikzset{text=#1}}}

\ctikzset{current arrow scale/.initial=16}

\ctikzset{bipoles/.is family}
\ctikzset{bipoles/border margin/.initial=1.1}
\ctikzset{bipoles/thickness/.initial=2}
\ctikzset{tripoles/thickness/.initial=2}
\ctikzset{quadpoles/thickness/.initial=2}
\ctikzset{nodes width/.initial=.04}

% Base len for all circuitikz
\newdimen\pgf@circ@Rlen
% scaled length for internal use in scalable shapes
\newdimen\pgf@circ@scaled@Rlen
\ctikzset{bipoles/length/.code={\pgf@circ@Rlen = #1\pgf@circ@scaled@Rlen=\pgf@circ@Rlen}}
\pgf@circ@Rlen = 1.4cm
% by default scale is 1.0
\pgf@circ@scaled@Rlen=\pgf@circ@Rlen

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% main style definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% load a style file: search ctikzstyle-NAME.tex in path
\def\ctikzloadstyle#1{%
    \edef\pgf@temp{#1}%
    % guard against re-loading
    \expandafter\ifx\csname pgf@circ@style@\pgf@temp @loaded\endcsname\relax%
    \expandafter\global\expandafter\let\csname pgf@circ@style@\pgf@temp @loaded\endcsname=\pgfutil@empty
    \pgfutil@InputIfFileExists{ctikzstyle-#1}{}{%
        \tikzerror{I did not find the circuitikz style #1}}%
    \fi
}

% load and enact a style
\def\ctikzsetstyle#1{%
    \ctikzloadstyle{#1}%
    \tikzset{#1 circuit style}%
}

% global style parameters
\ctikzset{default/scale/.initial=1.0}   % do not touch
\ctikzset{default/fill/.initial=none}   % do not touch
\ctikzset{default/thickness/.initial=none}   % do not touch
% default is use as the generic default style for bipoles

% mostly bipoles:

\ctikzset{resistors/scale/.initial=1.0}
\ctikzset{resistors/fill/.initial=none}
\ctikzset{resistors/thickness/.initial=none}

\ctikzset{capacitors/scale/.initial=1.0}
\ctikzset{capacitors/fill/.initial=none}
\ctikzset{capacitors/thickness/.initial=none}

\ctikzset{inductors/scale/.initial=1.0}
\ctikzset{inductors/fill/.initial=none}
\ctikzset{inductors/thickness/.initial=none}

\ctikzset{diodes/scale/.initial=1.0}
\ctikzset{diodes/fill/.initial=none}
\ctikzset{diodes/thickness/.initial=none}

\ctikzset{batteries/scale/.initial=1.0}
\ctikzset{batteries/fill/.initial=none}
\ctikzset{batteries/thickness/.initial=none}

\ctikzset{sources/scale/.initial=1.0}
\ctikzset{sources/fill/.initial=none}
\ctikzset{sources/thickness/.initial=none}

\ctikzset{csources/scale/.initial=1.0}
\ctikzset{csources/fill/.initial=none}
\ctikzset{csources/thickness/.initial=none}

\ctikzset{instruments/scale/.initial=1.0}
\ctikzset{instruments/fill/.initial=none}
\ctikzset{instruments/thickness/.initial=none}

\ctikzset{mechanicals/scale/.initial=1.0}
\ctikzset{mechanicals/fill/.initial=none}
\ctikzset{mechanicals/thickness/.initial=none}

\ctikzset{misc/scale/.initial=1.0}
\ctikzset{misc/fill/.initial=none}
\ctikzset{misc/thickness/.initial=none}

\ctikzset{blocks/scale/.initial=1.0}
\ctikzset{blocks/fill/.initial=none}
\ctikzset{blocks/thickness/.initial=none}

% mostly nodes

\ctikzset{grounds/scale/.initial=1.0}
\ctikzset{grounds/fill/.initial=none}
\ctikzset{grounds/thickness/.initial=none}

\ctikzset{power supplies/scale/.initial=1.0}
\ctikzset{power supplies/fill/.initial=none}
\ctikzset{power supplies/thickness/.initial=none}

\ctikzset{transistors/scale/.initial=1.0}
\ctikzset{transistors/fill/.initial=none}
\ctikzset{transistors/thickness/.initial=none}

\ctikzset{tubes/scale/.initial=1.0}
\ctikzset{tubes/fill/.initial=none}
\ctikzset{tubes/thickness/.initial=none}

\ctikzset{RF/scale/.initial=1.0}
\ctikzset{RF/fill/.initial=none}
\ctikzset{RF/thickness/.initial=none}

\ctikzset{electromechanicals/scale/.initial=1.0}
\ctikzset{electromechanicals/fill/.initial=none}
\ctikzset{electromechanicals/thickness/.initial=none}

% transformers go with inductors
\ctikzset{amplifiers/scale/.initial=1.0}
\ctikzset{amplifiers/fill/.initial=none}
\ctikzset{amplifiers/thickness/.initial=none}

\ctikzset{switches/scale/.initial=1.0}
\ctikzset{switches/fill/.initial=none}
\ctikzset{switches/thickness/.initial=none}

\ctikzset{logic ports/scale/.initial=1.0}
\ctikzset{logic ports/fill/.initial=none}
\ctikzset{logic ports/thickness/.initial=none}

\ctikzset{chips/scale/.initial=1.0}
\ctikzset{chips/fill/.initial=none}
\ctikzset{chips/thickness/.initial=none}

\ctikzset{displays/scale/.initial=1.0}
\ctikzset{displays/fill/.initial=none}
\ctikzset{displays/thickness/.initial=none}

% grounds and power supplies

\ctikzset{monopoles/.is family}
\ctikzset{monopoles/ground/width/.initial=.25}
\ctikzset{monopoles/ground/connectionthickness/.initial=1}
\ctikzset{monopoles/ground/thickness/.initial=2}
\ctikzset{monopoles/rground/thickness/.initial=2}
\ctikzset{monopoles/tground/thickness/.initial=3}
\ctikzset{monopoles/vcc/width/.initial=.2}
\ctikzset{monopoles/vcc/arrow/.initial=legacy}
\ctikzset{monopoles/vee/arrow/.initial=legacy}
\ctikzset{monopoles/match/width/.initial=.4}
\ctikzset{monopoles/chassis/width/.initial=.25}
\ctikzset{monopoles/alternative chassis/width/.initial=.25}
\ctikzset{monopoles/equipotentiality/width/.initial=.25}
\ctikzset{monopoles/antenna/width/.initial=.25}
\ctikzset{monopoles/antenna/label/xanchor/.initial=.4}
\ctikzset{monopoles/antenna/label/yanchor/.initial=.75}
\ctikzset{monopoles/txantenna/label/xanchor/.initial=.4}
\ctikzset{monopoles/txantenna/label/yanchor/.initial=.75}
\ctikzset{monopoles/txantenna/width/.initial=.25}
\ctikzset{monopoles/rxantenna/label/xanchor/.initial=.4}
\ctikzset{monopoles/rxantenna/label/yanchor/.initial=.75}
\ctikzset{monopoles/rxantenna/width/.initial=.25}
\ctikzset{monopoles/bareantenna/width/.initial=.25}
\ctikzset{monopoles/bareantenna/label/xanchor/.initial=1}
\ctikzset{monopoles/bareantenna/label/yanchor/.initial=0.5}
\ctikzset{monopoles/waves/width/.initial=0.5}

% microstrips
\ctikzset{bipoles/mstline/height/.initial=0.3}
\ctikzset{bipoles/mstline/width/.initial=1.2}
\pgfkeys{/tikz/mstlinelen/.add code={}{\ctikzset{bipoles/mstline/width=#1}}}
\ctikzset{monopoles/msport/width/.initial=.5}
\ctikzset{monopoles/msrstub/height/.initial=1.0}
\ctikzset{monopoles/msrstub/width/.initial=0.6}

% microphone and loudspeaker
\ctikzset{bipoles/loudspeaker/height/.initial=.8}
\ctikzset{bipoles/loudspeaker/depth/.initial=.3}
\ctikzset{bipoles/loudspeaker/width/.initial=.8}
\ctikzset{bipoles/mic/height/.initial=1.2}
\ctikzset{bipoles/mic/depth/.initial=.0}
\ctikzset{bipoles/mic/width/.initial=.8}

% Zig Zag resistors
\ctikzset{resistors/zigs/.initial=3}
\ctikzset{resistors/width/.code={%
    \ctikzset{bipoles/resistor/width=#1}%
    \ctikzset{bipoles/vresistor/width=#1}%
    \ctikzset{bipoles/potentiometer/width=#1}%
    \ctikzset{bipoles/resistivesens/width=#1}%
    \ctikzset{bipoles/photoresistor/width=#1}%
    \ctikzset{bipoles/thermistor/width=#1}%
    \ctikzset{bipoles/thermistorntc/width=#1}%
    \ctikzset{bipoles/thermistorptc/width=#1}%
    \ctikzset{bipoles/varistor/width=#1}%
    \ctikzset{bipoles/generic/width=#1}%
    \ctikzset{bipoles/generic potentiometer/width=#1}%
    \ctikzset{bipoles/ageneric/width=#1}%
    \ctikzset{bipoles/tgeneric/width=#1}%
}}
\ctikzset{wiper pos/.code={%
    \ctikzset{bipoles/potentiometer/wiper pos=#1}%
    \ctikzset{bipoles/generic potentiometer/wiper pos=#1}%
}}
% zigzag resistor
\ctikzset{bipoles/resistor/height/.initial=.3}
\ctikzset{bipoles/resistor/width/.initial=.8}
\ctikzset{bipoles/potentiometer/height/.initial=.8}
\ctikzset{bipoles/potentiometer/height 2/.initial=.3}
\ctikzset{bipoles/potentiometer/width/.initial=.8}
\ctikzset{bipoles/potentiometer/wiper pos/.initial=.5}
\ctikzset{bipoles/vresistor/height/.initial=.6}
\ctikzset{bipoles/vresistor/width/.initial=.8}
\ctikzset{bipoles/resistivesens/height/.initial=.6}
\ctikzset{bipoles/resistivesens/width/.initial=.8}
% square resistors
\ctikzset{bipoles/photoresistor/height/.initial=.6}
\ctikzset{bipoles/photoresistor/height 2/.initial=.3}
\ctikzset{bipoles/photoresistor/width/.initial=.8}
\ctikzset{bipoles/thermistor/main/.initial=.7}
\ctikzset{bipoles/thermistor/height/.initial=.428}%.3/.7
\ctikzset{bipoles/thermistorntc/width/.initial=.8}
\ctikzset{bipoles/thermistorntc/main/.initial=.7}
\ctikzset{bipoles/thermistorntc/height/.initial=.428}%.3/.7
\ctikzset{bipoles/thermistorntc/height 2/.initial=.75}%.3/.7
\ctikzset{bipoles/thermistorptc/width/.initial=.8}
\ctikzset{bipoles/thermistorptc/main/.initial=.7}
\ctikzset{bipoles/thermistorptc/height/.initial=.428}%.3/.7
\ctikzset{bipoles/thermistorptc/height 2/.initial=.75}%.3/.7
\ctikzset{bipoles/thermistor/width/.initial=.8}
\ctikzset{bipoles/varistor/main/.initial=.7}
\ctikzset{bipoles/varistor/height/.initial=.428}%.3/.7
\ctikzset{bipoles/varistor/width/.initial=.8}
\ctikzset{bipoles/generic/height/.initial=.30}
\ctikzset{bipoles/generic/width/.initial=.80}
\ctikzset{bipoles/generic potentiometer/height/.initial=.80}
\ctikzset{bipoles/generic potentiometer/height 2/.initial=.30}
\ctikzset{bipoles/generic potentiometer/width/.initial=.80}
\ctikzset{bipoles/generic potentiometer/wiper pos/.initial=.5}
\ctikzset{bipoles/ageneric/height/.initial=.30}
\ctikzset{bipoles/tgeneric/height/.initial=.70}
\ctikzset{bipoles/tgeneric/width/.initial=.80}
\ctikzset{bipoles/ageneric/width/.initial=.80}

%% Capacitors
\ctikzset{bipoles/capacitor/height/.initial=.6}
\ctikzset{bipoles/capacitor/width/.initial=.2}
\ctikzset{bipoles/ecapacitor/height/.initial=.5}
\ctikzset{bipoles/ecapacitor/width/.initial=.2}
\ctikzset{bipoles/ecapacitor/font/.initial=\pgf@circ@font@sixbm}
%%% pcapacitor is deprecated
\ctikzset{bipoles/pcapacitor/height/.initial=.6}
\ctikzset{bipoles/pcapacitor/width/.initial=.2}
\ctikzset{bipoles/pcapacitor/bend width/.initial=1.1}
\ctikzset{bipoles/ccapacitor/height/.initial=.6}
\ctikzset{bipoles/ccapacitor/width/.initial=.12}
\ctikzset{bipoles/ccapacitor/bend width/.initial=1.1}
\ctikzset{bipoles/vcapacitor/height/.initial=.6}
\ctikzset{bipoles/vcapacitor/width/.initial=.5}
\ctikzset{bipoles/vcapacitor/capacitor width/.initial=.4}
\ctikzset{bipoles/piezoelectric/height/.initial=.7}
\ctikzset{bipoles/piezoelectric/width/.initial=.5}

% Inductors
\ctikzset{inductors/coils/.code={%
    \ctikzset{bipoles/cuteinductor/coils=#1}%
    \ctikzset{bipoles/cutechoke/coils=#1}%
    \ctikzset{bipoles/americaninductor/coils=#1}%
    \ctikzset{bipoles/vcuteinductor/coils=#1}%
    \ctikzset{bipoles/vamericaninductor/coils=#1}%
}}
\ctikzset{inductors/width/.code={%
    \ctikzset{bipoles/cuteinductor/width=#1}%
    \ctikzset{bipoles/cutechoke/width=#1}%
    \ctikzset{bipoles/americaninductor/width=#1}%
    \ctikzset{bipoles/vcuteinductor/width=#1}%
    \ctikzset{bipoles/vamericaninductor/width=#1}%
    \ctikzset{bipoles/fullgeneric/width=#1}%
    \ctikzset{bipoles/tfullgeneric/width=#1}%
}}
\ctikzset{bipoles/cuteinductor/height/.initial=.3}
\ctikzset{bipoles/cuteinductor/lower coil height/.initial=.15}
\ctikzset{bipoles/cuteinductor/width/.initial=.6}
\ctikzset{bipoles/cuteinductor/coils/.initial=5}
\ctikzset{bipoles/cuteinductor/coil aspect/.initial=.5}%percentage of inductor width, which is covered by lower coil
%% Cute choke settings
\ctikzset{bipoles/cutechoke/height/.initial=.3}
\ctikzset{bipoles/cutechoke/lower coil height/.initial=.15}
\ctikzset{bipoles/cutechoke/width/.initial=.6}
\ctikzset{bipoles/cutechoke/coils/.initial=5}
\ctikzset{bipoles/cutechoke/coil aspect/.initial=.5}%percentage of choke width, which is covered by lower coil
\ctikzset{bipoles/cutechoke/cstep/.initial=.3}
\ctikzset{bipoles/cutechoke/cdist/.initial=1.3}
\ctikzset{bipoles/cutechoke/cthick/.initial=1}
\newif\ifpgf@circuit@bipole@twolineschoke
\pgf@circuit@bipole@twolineschokefalse
\pgfkeys{/tikz/onelinechoke/.add code={}{\pgf@circuit@bipole@twolineschokefalse}}
\ctikzset{onelinechoke/.add code={}{\pgf@circuit@bipole@twolineschokefalse}}
\pgfkeys{/tikz/twolineschoke/.add code={}{\pgf@circuit@bipole@twolineschoketrue}}
\ctikzset{twolineschoke/.add code={}{\pgf@circuit@bipole@twolineschoketrue}}
%
\ctikzset{bipoles/americaninductor/height/.initial=.3}
\ctikzset{bipoles/americaninductor/height 2/.initial=.1}
\ctikzset{bipoles/americaninductor/width/.initial=.8}
\ctikzset{bipoles/americaninductor/coils/.initial=4}
\ctikzset{bipoles/americaninductor/coil height/.initial=.15}
\ctikzset{bipoles/vcuteinductor/height/.initial=.6}
\ctikzset{bipoles/vcuteinductor/lower coil height/.initial=.3}
\ctikzset{bipoles/vcuteinductor/width/.initial=.6}
\ctikzset{bipoles/vcuteinductor/coils/.initial=5}
\ctikzset{bipoles/vcuteinductor/coil aspect/.initial=.5}%percentage of inductor width, which is covered by lower coil
\ctikzset{bipoles/vamericaninductor/height/.initial=.6}
\ctikzset{bipoles/vamericaninductor/height 2/.initial=.2}
\ctikzset{bipoles/vamericaninductor/width/.initial=.8}
\ctikzset{bipoles/vamericaninductor/coils/.initial=4}
\ctikzset{bipoles/vamericaninductor/coil height/.initial=.15}
\ctikzset{bipoles/tfullgeneric/height/.initial=.70}
\ctikzset{bipoles/tfullgeneric/width/.initial=.80}
\ctikzset{bipoles/fullgeneric/height/.initial=.30}
\ctikzset{bipoles/fullgeneric/width/.initial=.80}

% Sources

\ctikzset{bipoles/esource/height/.initial=.60}
\ctikzset{bipoles/esource/width/.initial=.60}
\ctikzset{bipoles/pvsource/height/.initial=.60}
\ctikzset{bipoles/pvsource/width/.initial=.60}
\ctikzset{bipoles/isource/height/.initial=.60}
\ctikzset{bipoles/isource/width/.initial=.60}
\ctikzset{bipoles/oosource/height/.initial=.60}
\ctikzset{bipoles/oosource/width/.initial=.60}
\ctikzset{bipoles/oosource/circlesize/.initial=.65}%circlesize+circleoffset should be =1
\ctikzset{bipoles/oosource/circleoffset/.initial=.35}%circlesize+circleoffset should be =1
\ctikzset{bipoles/dcisource/angle/.initial=80}
\ctikzset{bipoles/dcisource/height/.initial=.60}
\ctikzset{bipoles/dcisource/width/.initial=.60}
\ctikzset{bipoles/dcvsource/height/.initial=.60}
\ctikzset{bipoles/dcvsource/width/.initial=.60}
\ctikzset{bipoles/vsourcetri/height/.initial=.60}
\ctikzset{bipoles/vsourcetri/width/.initial=.60}
\ctikzset{bipoles/isourceam/height/.initial=.60}
\ctikzset{bipoles/isourceam/width/.initial=.60}
\ctikzset{bipoles/vsource/height/.initial=.60}
\ctikzset{bipoles/vsource/width/.initial=.60}
\ctikzset{bipoles/vsourceam/height/.initial=.60}
\ctikzset{bipoles/vsourceam/width/.initial=.60}
\ctikzset{bipoles/vsourceam/margin/.initial=.7}
\ctikzset{bipoles/isourcesin/height/.initial=.60}
\ctikzset{bipoles/isourcesin/width/.initial=.60}
\ctikzset{bipoles/vsourcesin/height/.initial=.60}
\ctikzset{bipoles/vsourcesin/width/.initial=.60}
\ctikzset{bipoles/vsourcesquare/height/.initial=.60}
\ctikzset{bipoles/vsourcesquare/width/.initial=.60}
\ctikzset{bipoles/cisource/height/.initial=.7}
\ctikzset{bipoles/cisource/width/.initial=.7}
\ctikzset{bipoles/cisourceam/height/.initial=.7}
\ctikzset{bipoles/cisourceam/width/.initial=.7}
\ctikzset{bipoles/ecsource/height/.initial=.7}
\ctikzset{bipoles/ecsource/width/.initial=.7}
\ctikzset{bipoles/cvsource/height/.initial=.7}
\ctikzset{bipoles/cvsource/width/.initial=.7}
\ctikzset{bipoles/cvsourceam/height/.initial=.7}
\ctikzset{bipoles/cvsourceam/width/.initial=.7}
\ctikzset{bipoles/cvsourceam/margin/.initial=.7}
\ctikzset{bipoles/cvsourceam/text scale/.initial=1}
\ctikzset{bipoles/cisourcesin/width/.initial=.7}
\ctikzset{bipoles/cvsourcesin/height/.initial=.7}
\ctikzset{bipoles/cvsourcesin/width/.initial=.7}
\ctikzset{bipoles/battery/height/.initial=.6}
\ctikzset{bipoles/battery/width/.initial=.3}
\ctikzset{bipoles/battery1/height/.initial=.6}
\ctikzset{bipoles/battery1/width/.initial=.3}
\ctikzset{bipoles/battery2/height/.initial=.6}
\ctikzset{bipoles/battery2/width/.initial=.3}

% diodes

\ctikzset{bipoles/diode/height/.initial=.50}
\ctikzset{bipoles/diode/width/.initial=.40}
\ctikzset{bipoles/bidirectionaldiode/height/.initial=1.1}
\ctikzset{bipoles/bidirectionaldiode/width/.initial=1}
\ctikzset{bipoles/bidirectionaldiode/diode width left/.initial=.3}
\ctikzset{bipoles/bidirectionaldiode/diode width right/.initial=.3}
\ctikzset{bipoles/varcap/height/.initial=.50}
\ctikzset{bipoles/varcap/width/.initial=.45}

% switches

\ctikzset{bipoles/spst/height/.initial=.35}
\ctikzset{bipoles/spst/width/.initial=.35}
\ctikzset{bipoles/spst/depth/.initial=.2}
\ctikzset{bipoles/nos/height/.initial=.3}
\ctikzset{bipoles/nos/width/.initial=.35}
\ctikzset{bipoles/nos/depth/.initial=.2}
\ctikzset{bipoles/ncs/height/.initial=.35}
\ctikzset{bipoles/ncs/width/.initial=.35}
\ctikzset{bipoles/ncs/depth/.initial=.2}

% misc

\ctikzset{bipoles/european gas filled surge arrester/height/.initial=.30}
\ctikzset{bipoles/european gas filled surge arrester/width/.initial=.80}
\ctikzset{bipoles/european gas filled surge arrester/inside/.initial=.30}
\ctikzset{bipoles/american gas filled surge arrester/height/.initial=.60}
\ctikzset{bipoles/american gas filled surge arrester/width/.initial=.60}
\ctikzset{bipoles/american gas filled surge arrester/inside/.initial=.15}
\ctikzset{bipoles/american gas filled surge arrester/dot x/.initial=.25}
\ctikzset{bipoles/american gas filled surge arrester/dot y/.initial=.45}
\ctikzset{bipoles/american gas filled surge arrester/size/.initial=.1}
\ctikzset{bipoles/fuse/height/.initial=.20}
\ctikzset{bipoles/fuse/width/.initial=.50}
\ctikzset{bipoles/afuse/height/.initial=.20}
\ctikzset{bipoles/afuse/width/.initial=.50}
\ctikzset{bipoles/memristor/height/.initial=.30}
\ctikzset{bipoles/memristor/wave height/.initial=.5}
\ctikzset{bipoles/memristor/width/.initial=.80}
\ctikzset{bipoles/open/height/.initial=.3} %necessary for curly voltages
\ctikzset{bipoles/open/width/.initial=.3} %necessary for curly voltages
\ctikzset{bipoles/open/voltage/straight label distance/.initial=0}
\ctikzset{bipoles/open/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/short/height/.initial=0} %dummy height for voltage positioning
\ctikzset{bipoles/short/width/.initial=0} %dummy width for voltage positioning
%\ctikzset{bipoles/short/voltage/straight label distance/.initial=.2}
%\ctikzset{bipoles/short/voltage/distance from node/.initial=.5}
\ctikzset{bipoles/ammeter/height/.initial=.60}
\ctikzset{bipoles/ammeter/width/.initial=.60}
\ctikzset{bipoles/ohmmeter/height/.initial=.60}
\ctikzset{bipoles/ohmmeter/width/.initial=.60}
\ctikzset{bipoles/voltmeter/height/.initial=.60}
\ctikzset{bipoles/voltmeter/width/.initial=.60}
\ctikzset{bipoles/smeter/height/.initial=.60}
\ctikzset{bipoles/smeter/width/.initial=.60}
\ctikzset{bipoles/qmeter/depth/.initial=.40}
\ctikzset{bipoles/qmeter/height/.initial=.80}
\ctikzset{bipoles/qmeter/width/.initial=.60}
\ctikzset{bipoles/iloop/width/.initial=.40}
\ctikzset{bipoles/iloop/height/.initial=.60}
\ctikzset{bipoles/oscope/height/.initial=.60}
\ctikzset{bipoles/oscope/width/.initial=.60}
\ctikzset{bipoles/buffer/height/.initial=1}
\ctikzset{bipoles/buffer/width/.initial=1}
\ctikzset{bipoles/not port/width/.initial=1}
\ctikzset{bipoles/not port/height/.initial=.8}
\ctikzset{bipoles/not port/circle width/.initial=.15}
\ctikzset{bipoles/lamp/height/.initial=.60}
\ctikzset{bipoles/lamp/width/.initial=.60}
\ctikzset{bipoles/bulb/height/.initial=.8}
\ctikzset{bipoles/bulb/width/.initial=.8}
\ctikzset{bipoles/tline/height/.initial=.3}
\ctikzset{bipoles/tline/width/.initial=.8}
\ctikzset{bipoles/squid/height/.initial=.60}
\ctikzset{bipoles/squid/width/.initial=.60}
\ctikzset{bipoles/barrier/height/.initial=.60}
\ctikzset{bipoles/barrier/width/.initial=.60}
\ctikzset{bipoles/thermocouple/height/.initial=.250}
\ctikzset{bipoles/thermocouple/height 2/.initial=.60}
\ctikzset{bipoles/thermocouple/width/.initial=.140}
\ctikzset{bipoles/pushbutton/height/.initial=.5}
\ctikzset{bipoles/pushbutton/height 2/.initial=.2}
\ctikzset{bipoles/pushbutton/width/.initial=.50}

\ctikzset{bipoles/twoport/width/.initial=.7}
\ctikzset{bipoles/twoport/height/.initial=.7}
\ctikzset{bipoles/twoport/text/.initial=}
\ctikzset{bipoles/vco/width/.initial=.7}
\ctikzset{bipoles/bandpass/width/.initial=.7}
\ctikzset{bipoles/bandstop/width/.initial=.7}
\ctikzset{bipoles/highpass/width/.initial=.7}
\ctikzset{bipoles/lowpass/width/.initial=.7}
\ctikzset{bipoles/adc/width/.initial=.7}
\ctikzset{bipoles/dac/width/.initial=.7}
\ctikzset{bipoles/dsp/width/.initial=.7}
\ctikzset{bipoles/fft/width/.initial=.7}
\ctikzset{bipoles/amp/width/.initial=.7}
\ctikzset{bipoles/vamp/width/.initial=.7}
\ctikzset{bipoles/piattenuator/width/.initial=.7}
\ctikzset{bipoles/vpiattenuator/width/.initial=.7}
\ctikzset{bipoles/tattenuator/width/.initial=.7}
\ctikzset{bipoles/vtattenuator/width/.initial=.7}
\ctikzset{bipoles/phaseshifter/width/.initial=.7}
\ctikzset{bipoles/vphaseshifter/width/.initial=.7}
\ctikzset{bipoles/detector/width/.initial=.7}

% crossing wires
\ctikzset{bipoles/crossing/size/.initial=.2}

% Transistors starts here

\newif\ifpgf@circuit@trans@depletiontype
\pgf@circuit@trans@depletiontypefalse

\newif\ifpgf@circuit@mos@arrows
\ctikzset{tripoles/mos style/.is choice}
\ctikzset{tripoles/mos style/no arrows/.code={\pgf@circuit@mos@arrowsfalse}}
\ctikzset{tripoles/mos style/arrows/.code={\pgf@circuit@mos@arrowstrue}}
\pgfkeys{/tikz/arrowmos/.add code={}{\pgf@circuit@mos@arrowstrue}}
\pgfkeys{/tikz/noarrowmos/.add code={}{\pgf@circuit@mos@arrowsfalse}}

% Fixed label positions
\newif\ifpgf@circuit@transisors@fixlabels
\pgf@circuit@transisors@fixlabelstrue
\pgfkeys{/tikz/center transistors text/.add code={}{\pgf@circuit@transisors@fixlabelstrue}}
\ctikzset{fix transistors text/.add code={}{\pgf@circuit@transisors@fixlabelstrue}}
\pgfkeys{/tikz/legacy transistors text/.add code={}{\pgf@circuit@transisors@fixlabelsfalse}}
\ctikzset{legacy transistors text/.add code={}{\pgf@circuit@transisors@fixlabelsfalse}}

% Option solderdot for fet
\newif\ifpgf@circuit@fet@solderdot
\pgfkeys{/tikz/solderdot/.add code={}{\pgf@circuit@fet@solderdottrue}}
\ctikzset{solderdot/.add code={}{\pgf@circuit@fet@solderdottrue}}
\pgfkeys{/tikz/nosolderdot/.add code={}{\pgf@circuit@fet@solderdotfalse}}
\ctikzset{nosolderdot/.add code={}{\pgf@circuit@fet@solderdotfalse}}

% Option bodydiode for fet
\newif\ifpgf@circuit@fet@bodydiode
\pgfkeys{/tikz/bodydiode/.add code={}{\pgf@circuit@fet@bodydiodetrue}}
\ctikzset{bodydiode/.add code={}{\pgf@circuit@fet@bodydiodetrue}}
\pgfkeys{/tikz/nobodydiode/.add code={}{\pgf@circuit@fet@bodydiodefalse}}
\ctikzset{nobodydiode/.add code={}{\pgf@circuit@fet@bodydiodefalse}}

% Option draw fet without gate connection
\newif\ifpgf@circuit@bpt@drawgate
\pgf@circuit@bpt@drawgatetrue
\pgfkeys{/tikz/nogate/.add code={}{\pgf@circuit@bpt@drawgatefalse}}
\ctikzset{nogate/.add code={}{\pgf@circuit@bpt@drawgatefalse}}
\pgfkeys{/tikz/nobase/.add code={}{\pgf@circuit@bpt@drawgatefalse}}
\ctikzset{nobase/.add code={}{\pgf@circuit@bpt@drawgatefalse}}

% Option draw bpt without base connection
\newif\ifpgf@circuit@bpt@drawbase
\pgf@circuit@bpt@drawbasetrue
\pgfkeys{/tikz/nobase/.add code={}{\pgf@circuit@bpt@drawbasefalse}}
\ctikzset{nobase/.add code={}{\pgf@circuit@bpt@drawbasefalse}}
\pgfkeys{/tikz/nogate/.add code={}{\pgf@circuit@bpt@drawbasefalse}}
\ctikzset{nogate/.add code={}{\pgf@circuit@bpt@drawbasefalse}}

% Option draw bpt with optical input
\newif\ifpgf@circuit@bpt@drawphoto
\pgf@circuit@bpt@drawphotofalse
\pgfkeys{/tikz/photo/.add code={}{\pgf@circuit@bpt@drawphototrue}}
\ctikzset{photo/.add code={}{\pgf@circuit@bpt@drawphototrue}}
\pgfkeys{/tikz/photo/.add code={}{\pgf@circuit@bpt@drawphototrue}}
\ctikzset{photo/.add code={}{\pgf@circuit@bpt@drawphototrue}}

% Option draw fet without bulk connection -- Added by Burak Kelleci
\newif\ifpgf@circuit@bpt@drawbulk
\pgfkeys{/tikz/bulk/.add code={}{\pgf@circuit@bpt@drawbulktrue}}
\ctikzset{bulk/.add code={}{\pgf@circuit@bpt@drawbulktrue}}
\pgfkeys{/tikz/nobulk/.add code={}{\pgf@circuit@bpt@drawbulkfalse}}
\ctikzset{nobulk/.add code={}{\pgf@circuit@bpt@drawbulkfalse}}

% Option draw pmos with empty circle
\newif\ifpgf@circuit@pmos@emptycircle
\pgf@circuit@pmos@emptycirclefalse
\ctikzset{tripoles/pmos style/.is choice}
\pgfkeys{/tikz/emptycircle/.add code={}{\pgf@circuit@pmos@emptycircletrue}}
\ctikzset{tripoles/pmos style/emptycircle/.add code={}{\pgf@circuit@pmos@emptycircletrue}}
% Option draw pmos with no circle
\newif\ifpgf@circuit@pmos@nocircle
\pgf@circuit@pmos@nocirclefalse
\pgfkeys{/tikz/nocircle/.add code={}{\pgf@circuit@pmos@nocircletrue}}
\ctikzset{tripoles/pmos style/nocircle/.add code={}{\pgf@circuit@pmos@nocircletrue}}
% back to normal
\pgfkeys{/tikz/fullcircle/.add code={}{\pgf@circuit@pmos@emptycirclefalse\pgf@circuit@pmos@nocirclefalse}}
\ctikzset{tripoles/pmos style/fullcircle/.add code={}{\pgf@circuit@pmos@emptycirclefalse\pgf@circuit@pmos@nocirclefalse}}
% arrows at the end, the correct way
\newif\ifpgf@circuit@trans@arrowatend
\pgf@circuit@trans@arrowatendfalse
\ctikzset{transistors/arrow pos/.is choice}
\ctikzset{transistors/arrow pos/legacy/.code={\pgf@circuit@trans@arrowatendfalse}}
\ctikzset{transistors/arrow pos/end/.code={\pgf@circuit@trans@arrowatendtrue}}

\newif\ifpgf@circuit@trans@ntype
\pgf@circuit@trans@ntypetrue %default true
%\newif\ifpgf@circuit@trans@ptype
%\ctikzset{tripoles/nmos/.add code={\pgf@circuit@trans@ntypetrue}}
\ctikzset{tripoles/nmos/width/.initial=.7}
\ctikzset{tripoles/nmos/gate height/.initial=.35}
\ctikzset{tripoles/nmos/base height/.initial=.5}
\ctikzset{tripoles/nmos/conn height/.initial=0}
\ctikzset{tripoles/nmos/height/.initial=1.1}
\ctikzset{tripoles/nmos/base width/.initial=.5}
\ctikzset{tripoles/nmos/gate width/.initial=.62}
\ctikzset{tripoles/nmos/arrow pos/.initial=.6}
\ctikzset{tripoles/nmos/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nmos/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nmos/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nmos/curr direction/.initial=1}

\ctikzset{tripoles/pmos/width/.initial=.7}
\ctikzset{tripoles/pmos/gate height/.initial=.35}
\ctikzset{tripoles/pmos/base height/.initial=.5}
\ctikzset{tripoles/pmos/conn height/.initial=0}
\ctikzset{tripoles/pmos/height/.initial=1.1}
\ctikzset{tripoles/pmos/base width/.initial=.5}
\ctikzset{tripoles/pmos/gate width/.initial=.62}
\ctikzset{tripoles/pmos/arrow pos/.initial=.4}
\ctikzset{tripoles/pmos/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pmos/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pmos/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pmos/curr direction/.initial=-1}

\ctikzset{tripoles/hemt/width/.initial=.7}
\ctikzset{tripoles/hemt/gate height/.initial=.35}
\ctikzset{tripoles/hemt/base height/.initial=.5}
\ctikzset{tripoles/hemt/conn height/.initial=0}
\ctikzset{tripoles/hemt/height/.initial=1.1}
\ctikzset{tripoles/hemt/base width/.initial=.5}
\ctikzset{tripoles/hemt/gate width/.initial=.62}
\ctikzset{tripoles/hemt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/hemt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/hemt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/hemt/curr direction/.initial=1}

\ctikzset{tripoles/nfet/width/.initial=.7}
\ctikzset{tripoles/nfet/gate height/.initial=.35}
\ctikzset{tripoles/nfet/base height/.initial=.5}
\ctikzset{tripoles/nfet/conn height/.initial=0}
\ctikzset{tripoles/nfet/height/.initial=1.1}
\ctikzset{tripoles/nfet/base width/.initial=.5}
\ctikzset{tripoles/nfet/gate width/.initial=.62}
\ctikzset{tripoles/nfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nfet/curr direction/.initial=1}

\ctikzset{tripoles/pfet/width/.initial=.7}
\ctikzset{tripoles/pfet/gate height/.initial=.35}
\ctikzset{tripoles/pfet/base height/.initial=.5}
\ctikzset{tripoles/pfet/conn height/.initial=0}
\ctikzset{tripoles/pfet/height/.initial=1.1}
\ctikzset{tripoles/pfet/base width/.initial=.5}
\ctikzset{tripoles/pfet/gate width/.initial=.62}
\ctikzset{tripoles/pfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pfet/curr direction/.initial=-1}

\ctikzset{tripoles/nigfete/width/.initial=.7}
\ctikzset{tripoles/nigfete/gate height/.initial=.35}
\ctikzset{tripoles/nigfete/base height/.initial=.5}
\ctikzset{tripoles/nigfete/conn height/.initial=.35}
\ctikzset{tripoles/nigfete/height/.initial=1.1}
\ctikzset{tripoles/nigfete/base width/.initial=.5}
\ctikzset{tripoles/nigfete/gate width/.initial=.62}
\ctikzset{tripoles/nigfete/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nigfete/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nigfete/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nigfete/curr direction/.initial=1}

\ctikzset{tripoles/nigfetd/width/.initial=.7}
\ctikzset{tripoles/nigfetd/gate height/.initial=.35}
\ctikzset{tripoles/nigfetd/base height/.initial=.5}
\ctikzset{tripoles/nigfetd/conn height/.initial=.35}
\ctikzset{tripoles/nigfetd/height/.initial=1.1}
\ctikzset{tripoles/nigfetd/base width/.initial=.5}
\ctikzset{tripoles/nigfetd/gate width/.initial=.62}
\ctikzset{tripoles/nigfetd/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nigfetd/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nigfetd/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nigfetd/curr direction/.initial=1}

\ctikzset{tripoles/nigfetebulk/width/.initial=.7}
\ctikzset{tripoles/nigfetebulk/gate height/.initial=.35}
\ctikzset{tripoles/nigfetebulk/base height/.initial=.5}
\ctikzset{tripoles/nigfetebulk/conn height/.initial=.35}
\ctikzset{tripoles/nigfetebulk/height/.initial=1.1}
\ctikzset{tripoles/nigfetebulk/base width/.initial=.5}
\ctikzset{tripoles/nigfetebulk/gate width/.initial=.62}
\ctikzset{tripoles/nigfetebulk/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nigfetebulk/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nigfetebulk/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nigfetebulk/curr direction/.initial=1}

\ctikzset{tripoles/pigfete/width/.initial=.7}
\ctikzset{tripoles/pigfete/gate height/.initial=.35}
\ctikzset{tripoles/pigfete/base height/.initial=.5}
\ctikzset{tripoles/pigfete/conn height/.initial=.35}
\ctikzset{tripoles/pigfete/height/.initial=1.1}
\ctikzset{tripoles/pigfete/base width/.initial=.5}
\ctikzset{tripoles/pigfete/gate width/.initial=.62}
\ctikzset{tripoles/pigfete/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pigfete/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pigfete/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pigfete/curr direction/.initial=-1}

\ctikzset{tripoles/pigfetd/width/.initial=.7}
\ctikzset{tripoles/pigfetd/gate height/.initial=.35}
\ctikzset{tripoles/pigfetd/base height/.initial=.5}
\ctikzset{tripoles/pigfetd/conn height/.initial=.35}
\ctikzset{tripoles/pigfetd/height/.initial=1.1}
\ctikzset{tripoles/pigfetd/base width/.initial=.5}
\ctikzset{tripoles/pigfetd/gate width/.initial=.62}
\ctikzset{tripoles/pigfetd/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pigfetd/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pigfetd/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pigfetd/curr direction/.initial=-1}

\ctikzset{tripoles/pigfetebulk/width/.initial=.7}
\ctikzset{tripoles/pigfetebulk/gate height/.initial=.35}
\ctikzset{tripoles/pigfetebulk/conn height/.initial=.35}
\ctikzset{tripoles/pigfetebulk/base height/.initial=.5}
\ctikzset{tripoles/pigfetebulk/height/.initial=1.1}
\ctikzset{tripoles/pigfetebulk/base width/.initial=.5}
\ctikzset{tripoles/pigfetebulk/gate width/.initial=.62}
\ctikzset{tripoles/pigfetebulk/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pigfetebulk/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pigfetebulk/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pigfetebulk/curr direction/.initial=-1}

\ctikzset{tripoles/npn/width/.initial=.6}
\ctikzset{tripoles/npn/base height/.initial=.45}
\ctikzset{tripoles/npn/base height 2/.initial=.15}
\ctikzset{tripoles/npn/base height/.initial=.4}
\ctikzset{tripoles/npn/conn height/.initial=0}
\ctikzset{tripoles/npn/height/.initial=1.1}
\ctikzset{tripoles/npn/base width/.initial=.5}
\ctikzset{tripoles/npn/arrow pos/.initial=.5}
\ctikzset{tripoles/npn/bodydiode scale/.initial=.3}
\ctikzset{tripoles/npn/bodydiode distance/.initial=.3}
\ctikzset{tripoles/npn/bodydiode conn/.initial=.6}
\ctikzset{tripoles/npn/curr direction/.initial=1}

\ctikzset{tripoles/pnp/width/.initial=.6}
\ctikzset{tripoles/pnp/base height/.initial=.45}
\ctikzset{tripoles/pnp/base height 2/.initial=.15}
\ctikzset{tripoles/pnp/base height/.initial=.4}
\ctikzset{tripoles/pnp/conn height/.initial=0}
\ctikzset{tripoles/pnp/height/.initial=1.1}
\ctikzset{tripoles/pnp/base width/.initial=.5}
\ctikzset{tripoles/pnp/arrow pos/.initial=.5}
\ctikzset{tripoles/pnp/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pnp/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pnp/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pnp/curr direction/.initial=-1}

\ctikzset{tripoles/pigbt/width/.initial=.6}
\ctikzset{tripoles/pigbt/gate height/.initial=.45}
\ctikzset{tripoles/pigbt/gate height 2/.initial=.15}
\ctikzset{tripoles/pigbt/base height/.initial=.4}
\ctikzset{tripoles/pigbt/conn height/.initial=0}
\ctikzset{tripoles/pigbt/height/.initial=1.1}
\ctikzset{tripoles/pigbt/gate width/.initial=.62}
\ctikzset{tripoles/pigbt/base width/.initial=.5}
\ctikzset{tripoles/pigbt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pigbt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pigbt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pigbt/curr direction/.initial=-1}

\ctikzset{tripoles/nigbt/width/.initial=.6}
\ctikzset{tripoles/nigbt/gate height/.initial=.45}
\ctikzset{tripoles/nigbt/gate height 2/.initial=.15}
\ctikzset{tripoles/nigbt/base height/.initial=.4}
\ctikzset{tripoles/nigbt/conn height/.initial=0}
\ctikzset{tripoles/nigbt/height/.initial=1.1}
\ctikzset{tripoles/nigbt/gate width/.initial=.62}
\ctikzset{tripoles/nigbt/base width/.initial=.5}
\ctikzset{tripoles/nigbt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nigbt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nigbt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nigbt/curr direction/.initial=1}

\ctikzset{tripoles/Lpigbt/width/.initial=.6}
\ctikzset{tripoles/Lpigbt/gate height/.initial=.45}
\ctikzset{tripoles/Lpigbt/gate height 2/.initial=.15}
\ctikzset{tripoles/Lpigbt/base height/.initial=.4}
\ctikzset{tripoles/Lpigbt/conn height/.initial=.4}
\ctikzset{tripoles/Lpigbt/height/.initial=1.1}
\ctikzset{tripoles/Lpigbt/gate width/.initial=.62}
\ctikzset{tripoles/Lpigbt/base width/.initial=.5}
\ctikzset{tripoles/Lpigbt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/Lpigbt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/Lpigbt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/Lpigbt/curr direction/.initial=-1}

\ctikzset{tripoles/Lnigbt/width/.initial=.6}
\ctikzset{tripoles/Lnigbt/gate height/.initial=.45}
\ctikzset{tripoles/Lnigbt/gate height 2/.initial=.15}
\ctikzset{tripoles/Lnigbt/base height/.initial=.4}
\ctikzset{tripoles/Lnigbt/conn height/.initial=.4}
\ctikzset{tripoles/Lnigbt/height/.initial=1.1}
\ctikzset{tripoles/Lnigbt/gate width/.initial=.62}
\ctikzset{tripoles/Lnigbt/base width/.initial=.5}
\ctikzset{tripoles/Lnigbt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/Lnigbt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/Lnigbt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/Lnigbt/curr direction/.initial=1}

\ctikzset{tripoles/njfet/width/.initial=.7}
\ctikzset{tripoles/njfet/gate height/.initial=.5}
\ctikzset{tripoles/njfet/gate height 2/.initial=.35}
\ctikzset{tripoles/njfet/gate width/.initial=.5}
\ctikzset{tripoles/njfet/conn height/.initial=.35}
\ctikzset{tripoles/njfet/height/.initial=1.1}
\ctikzset{tripoles/njfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/njfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/njfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/njfet/curr direction/.initial=1}

\ctikzset{tripoles/pjfet/width/.initial=.7}
\ctikzset{tripoles/pjfet/gate height/.initial=.5}
\ctikzset{tripoles/pjfet/gate height 2/.initial=.35}
\ctikzset{tripoles/pjfet/gate width/.initial=.5}
\ctikzset{tripoles/pjfet/conn height/.initial=.35}
\ctikzset{tripoles/pjfet/height/.initial=1.1}
\ctikzset{tripoles/pjfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pjfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pjfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pjfet/curr direction/.initial=-1}

\ctikzset{tripoles/isfet/width/.initial=1}
\ctikzset{tripoles/isfet/gate height/.initial=.35}
\ctikzset{tripoles/isfet/base height/.initial=.5}
\ctikzset{tripoles/isfet/height/.initial=1.1}
\ctikzset{tripoles/isfet/base width/.initial=.3}
\ctikzset{tripoles/isfet/gate width/.initial=.5}
\ctikzset{tripoles/isfet/conn height/.initial=0}
\ctikzset{tripoles/isfet/wave width/.initial=.16}
\ctikzset{tripoles/isfet/wave amp/.initial=.06}
\ctikzset{tripoles/isfet/waves y sep/.initial=.22}
\ctikzset{tripoles/isfet/waves x sep/.initial=.8}
\ctikzset{tripoles/isfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/isfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/isfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/isfet/curr direction/.initial=1}
%
% multi-emitter and multi-collector BJTs by Romano Giannetti
%
\ctikzset{tripoles/bjt/emitters/.initial=1}
\ctikzset{tripoles/bjt/collectors/.initial=1}
\pgfkeys{/tikz/emitters/.add code={}{\ctikzset{tripoles/bjt/emitters=#1}}}
\pgfkeys{/tikz/collectors/.add code={}{\ctikzset{tripoles/bjt/collectors=#1}}}
\ctikzset{tripoles/bjt/pins width/.initial=0.3}
\pgfkeys{/tikz/bjt pins width/.add code={}{\ctikzset{tripoles/bjt/pins width=#1}}}
\ctikzset{tripoles/bjt/multi height/.initial=.5}
\pgfkeys{/tikz/bjt multi height/.add code={}{\ctikzset{tripoles/bjt/multi height/.initial=#1}}}
%
\ctikzset{tripoles/bjt/width/.initial=.3}
\ctikzset{tripoles/bjt/base height 2/.initial=.4}
\ctikzset{tripoles/bjt/base height/.initial=1.1}
\ctikzset{tripoles/bjt/height/.initial=.4}
\ctikzset{tripoles/bjt/base width/.initial=1}
\ctikzset{tripoles/bjt/arrow pos/.initial=.5}
% do NOT touch these two!
\ctikzset{tripoles/bjt/npn/curr direction/.initial=1}
\ctikzset{tripoles/bjt/pnp/curr direction/.initial=-1}

%% transistors stop here

%% Logic ports

\newif\ifpgf@circuit@europeanlogicport
\ctikzset{logic ports/.is choice}
\ctikzset{logic ports/european/.code= {\pgf@circuit@europeanlogicporttrue
    \tikzset{and port/.style={shape=european and port}}%
    \tikzset{or port/.style={shape=european or port}}%
    \tikzset{xor port/.style={shape=european xor port}}%
    \tikzset{buffer port/.style={shape=european buffer port}}%
    \tikzset{not port/.style={shape=european not port}}%
    \tikzset{nand port/.style={shape=european nand port}}%
    \tikzset{nor port/.style={shape=european nor port}}%
    \tikzset{xnor port/.style={shape=european xnor port}}%
}}
\ctikzset{logic ports/american/.code= {\pgf@circuit@europeanlogicportfalse
    \tikzset{and port/.style={shape=american and port}}%
    \tikzset{or port/.style={shape=american or port}}%
    \tikzset{xor port/.style={shape=american xor port}}%
    \tikzset{buffer port/.style={shape=american buffer port}}%
    \tikzset{not port/.style={shape=american not port}}%
    \tikzset{nand port/.style={shape=american nand port}}%
    \tikzset{nor port/.style={shape=american nor port}}%
    \tikzset{xnor port/.style={shape=american xnor port}}%
}}

\ctikzset{logic ports origin/.is choice}
\ctikzset{logic ports origin/legacy/.code={
    \ctikzset{tripoles/american and port/origin/.initial=0.8}%
    \ctikzset{tripoles/american nand port/origin/.initial=0.8}%
    \ctikzset{tripoles/american nor port/origin/.initial=0.8}%
    \ctikzset{tripoles/american or port/origin/.initial=0.8}%
    \ctikzset{tripoles/american xor port/origin/.initial=0.8}%
    \ctikzset{tripoles/american xnor port/origin/.initial=0.8}%
    \ctikzset{tripoles/european and port/origin/.initial=0.8}%
    \ctikzset{tripoles/european nand port/origin/.initial=0.8}%
    \ctikzset{tripoles/european or port/origin/.initial=0.8}%
    \ctikzset{tripoles/european nor port/origin/.initial=0.8}%
    \ctikzset{tripoles/european xor port/origin/.initial=0.8}%
    \ctikzset{tripoles/european xnor port/origin/.initial=0.8}%
    \ctikzset{tripoles/european buffer port/origin/.initial=0.8}%
    \ctikzset{tripoles/european not port/origin/.initial=0.8}%
    }%
}
\ctikzset{logic ports origin/center/.code={%
    \ctikzset{tripoles/american and port/origin/.initial=0}%
    \ctikzset{tripoles/american nand port/origin/.initial=0}%
    \ctikzset{tripoles/american nor port/origin/.initial=0}%
    \ctikzset{tripoles/american or port/origin/.initial=0}%
    \ctikzset{tripoles/american xor port/origin/.initial=0}%
    \ctikzset{tripoles/american xnor port/origin/.initial=0}%
    \ctikzset{tripoles/european and port/origin/.initial=0}%
    \ctikzset{tripoles/european nand port/origin/.initial=0}%
    \ctikzset{tripoles/european or port/origin/.initial=0}%
    \ctikzset{tripoles/european nor port/origin/.initial=0}%
    \ctikzset{tripoles/european xor port/origin/.initial=0}%
    \ctikzset{tripoles/european xnor port/origin/.initial=0}%
    \ctikzset{tripoles/european buffer port/origin/.initial=0}%
    \ctikzset{tripoles/european not port/origin/.initial=0}%
    }%
}


\ctikzset{tripoles/american and port/width/.initial=1.1}
\ctikzset{tripoles/american and port/height/.initial=.8}
\ctikzset{tripoles/american and port/port width/.initial=.7}
\ctikzset{tripoles/american and port/input height/.initial=.5}
\ctikzset{tripoles/american nand port/width/.initial=1.1}
\ctikzset{tripoles/american nand port/height/.initial=.8}
\ctikzset{tripoles/american nand port/port width/.initial=.7}
\ctikzset{tripoles/american nand port/circle width/.initial=.15}
\ctikzset{tripoles/american nand port/input height/.initial=.5}
\ctikzset{tripoles/american or port/width/.initial=1.1}
\ctikzset{tripoles/american or port/height/.initial=.8}
\ctikzset{tripoles/american or port/port width/.initial=.7}
\ctikzset{tripoles/american or port/input height/.initial=.5}
\ctikzset{tripoles/american or port/input skip/.initial=.25}
\ctikzset{tripoles/american or port/aaa/.initial=.6}
\ctikzset{tripoles/american or port/bbb/.initial=.4}
\ctikzset{tripoles/american or port/ccc/.initial=.5}
\ctikzset{tripoles/american or port/ddd/.initial=.0}
\ctikzset{tripoles/american nor port/width/.initial=1.1}
\ctikzset{tripoles/american nor port/height/.initial=.8}
\ctikzset{tripoles/american nor port/port width/.initial=.7}
\ctikzset{tripoles/american nor port/input height/.initial=.5}
\ctikzset{tripoles/american nor port/input skip/.initial=.25}
\ctikzset{tripoles/american nor port/circle width/.initial=.15}
\ctikzset{tripoles/american nor port/aaa/.initial=.6}
\ctikzset{tripoles/american nor port/bbb/.initial=.4}
\ctikzset{tripoles/american nor port/ccc/.initial=.5}
\ctikzset{tripoles/american nor port/ddd/.initial=.0}
\ctikzset{tripoles/american xor port/width/.initial=1.1}
\ctikzset{tripoles/american xor port/height/.initial=.8}
\ctikzset{tripoles/american xor port/port width/.initial=.7}
\ctikzset{tripoles/american xor port/input height/.initial=.5}
\ctikzset{tripoles/american xor port/input skip/.initial=.15}
\ctikzset{tripoles/american xor port/distance/.initial=.1}
\ctikzset{tripoles/american xnor port/width/.initial=1.1}
\ctikzset{tripoles/american xnor port/height/.initial=.8}
\ctikzset{tripoles/american xnor port/port width/.initial=.7}
\ctikzset{tripoles/american xnor port/input height/.initial=.5}
\ctikzset{tripoles/american xnor port/input skip/.initial=.15}
\ctikzset{tripoles/american xnor port/distance/.initial=.1}
\ctikzset{tripoles/american xnor port/circle width/.initial=.15}
\ctikzset{tripoles/american and port/origin/.initial=0.8}
\ctikzset{tripoles/american and port/inputs/.initial=2}
% variable number of inputs
\ctikzset{tripoles/american nand port/origin/.initial=0.8}
\ctikzset{tripoles/american nand port/inputs/.initial=2}
\ctikzset{tripoles/american nor port/origin/.initial=0.8}
\ctikzset{tripoles/american nor port/inputs/.initial=2}
\ctikzset{tripoles/american nor port/angle/.initial=70}
\ctikzset{tripoles/american nor port/inner/.initial=0.3}
\ctikzset{tripoles/american or port/origin/.initial=0.8}
\ctikzset{tripoles/american or port/inputs/.initial=2}
\ctikzset{tripoles/american or port/angle/.initial=70}
\ctikzset{tripoles/american or port/inner/.initial=0.3}
\ctikzset{tripoles/american xor port/origin/.initial=0.8}
\ctikzset{tripoles/american xor port/inputs/.initial=2}
\ctikzset{tripoles/american xor port/angle/.initial=70}
\ctikzset{tripoles/american xor port/inner/.initial=0.3}
\ctikzset{tripoles/american xnor port/origin/.initial=0.8}
\ctikzset{tripoles/american xnor port/inputs/.initial=2}
\ctikzset{tripoles/american xnor port/angle/.initial=70}
\ctikzset{tripoles/american xnor port/inner/.initial=0.3}

\ctikzset{tripoles/european and port/width/.initial=1.4}
\ctikzset{tripoles/european and port/height/.initial=.65}
\ctikzset{tripoles/european and port/reserved/.initial=.6}
\ctikzset{tripoles/european and port/input height/.initial=.6}
\ctikzset{tripoles/european or port/width/.initial=1.4}
\ctikzset{tripoles/european or port/height/.initial=.65}
\ctikzset{tripoles/european or port/reserved/.initial=.6}
\ctikzset{tripoles/european or port/input height/.initial=.6}
\ctikzset{tripoles/european xor port/width/.initial=1.4}
\ctikzset{tripoles/european xor port/height/.initial=.65}
\ctikzset{tripoles/european xor port/reserved/.initial=.6}
\ctikzset{tripoles/european xor port/input height/.initial=.6}
\ctikzset{tripoles/european nand port/width/.initial=1.4}
\ctikzset{tripoles/european nand port/not height/.initial=.3}
\ctikzset{tripoles/european nand port/not width/.initial=.8}
\ctikzset{tripoles/european nand port/height/.initial=.65}
\ctikzset{tripoles/european nand port/reserved/.initial=.6}
\ctikzset{tripoles/european nand port/input height/.initial=.6}
\ctikzset{tripoles/european buffer port/width/.initial=1.4}
\ctikzset{tripoles/european buffer port/not height/.initial=.3}
\ctikzset{tripoles/european buffer port/not width/.initial=.8}
\ctikzset{tripoles/european buffer port/height/.initial=.65}
\ctikzset{tripoles/european buffer port/reserved/.initial=.6}
\ctikzset{tripoles/european buffer port/input height/.initial=0}
\ctikzset{tripoles/european not port/width/.initial=1.4}
\ctikzset{tripoles/european not port/not height/.initial=.3}
\ctikzset{tripoles/european not port/not width/.initial=.8}
\ctikzset{tripoles/european not port/height/.initial=.65}
\ctikzset{tripoles/european not port/reserved/.initial=.6}
\ctikzset{tripoles/european not port/input height/.initial=0}
\ctikzset{tripoles/european xnor port/width/.initial=1.4}
\ctikzset{tripoles/european xnor port/not height/.initial=.3}
\ctikzset{tripoles/european xnor port/not width/.initial=.8}
\ctikzset{tripoles/european xnor port/height/.initial=.65}
\ctikzset{tripoles/european xnor port/reserved/.initial=.6}
\ctikzset{tripoles/european xnor port/input height/.initial=.6}
\ctikzset{tripoles/european nor port/width/.initial=1.4}
\ctikzset{tripoles/european nor port/not height/.initial=.3}
\ctikzset{tripoles/european nor port/not width/.initial=.8}
\ctikzset{tripoles/european nor port/height/.initial=.65}
\ctikzset{tripoles/european nor port/reserved/.initial=.6}
\ctikzset{tripoles/european nor port/input height/.initial=.6}
% variable number of inputs
\ctikzset{tripoles/european and port/origin/.initial=0.8}
\ctikzset{tripoles/european and port/inputs/.initial=2}
\ctikzset{tripoles/european nand port/origin/.initial=0.8}
\ctikzset{tripoles/european nand port/inputs/.initial=2}
\ctikzset{tripoles/european or port/origin/.initial=0.8}
\ctikzset{tripoles/european or port/inputs/.initial=2}
\ctikzset{tripoles/european nor port/origin/.initial=0.8}
\ctikzset{tripoles/european nor port/inputs/.initial=2}
\ctikzset{tripoles/european xor port/origin/.initial=0.8}
\ctikzset{tripoles/european xor port/inputs/.initial=2}
\ctikzset{tripoles/european xnor port/origin/.initial=0.8}
\ctikzset{tripoles/european xnor port/inputs/.initial=2}
\ctikzset{tripoles/european buffer port/origin/.initial=0.8}
\ctikzset{tripoles/european buffer port/inputs/.initial=1}%
\ctikzset{tripoles/european not port/origin/.initial=0.8}
\ctikzset{tripoles/european not port/inputs/.initial=1}%
%%% parameters that are not used anymore after multi-input
%%% gates --- left for compatibility of source code.
\ctikzset{tripoles/american xor port/aaa/.initial=.6}
\ctikzset{tripoles/american xor port/bbb/.initial=.4}
\ctikzset{tripoles/american xor port/ccc/.initial=.5}
\ctikzset{tripoles/american xor port/ddd/.initial=.0}
\ctikzset{tripoles/american xnor port/aaa/.initial=.6}
\ctikzset{tripoles/american xnor port/bbb/.initial=.4}
\ctikzset{tripoles/american xnor port/ccc/.initial=.5}
\ctikzset{tripoles/american xnor port/ddd/.initial=.0}
% switches for logic gates
%
\pgfkeys{/tikz/number inputs/.initial=0}
\pgfkeys{/tikz/number inputs/.default=0}
%
% switches for op amps
% changing input polarity
%
\newif\ifpgf@circuit@oa@iplusup\pgf@circuit@oa@iplusupfalse
\pgfkeys{/tikz/noinv input up/.add code={}{\pgf@circuit@oa@iplusuptrue}}
\ctikzset{noinv input up/.add code={}{\pgf@circuit@oa@iplusuptrue}}
\pgfkeys{/tikz/noinv input down/.add code={}{\pgf@circuit@oa@iplusupfalse}}
\ctikzset{noinv input down/.add code={}{\pgf@circuit@oa@iplusupfalse}}
%
% changing output polarity (for fully diff objects)
%
\newif\ifpgf@circuit@oa@oplusup\pgf@circuit@oa@oplusuptrue
\pgfkeys{/tikz/noinv output up/.add code={}{\pgf@circuit@oa@oplusuptrue}}
\ctikzset{noinv output up/.add code={}{\pgf@circuit@oa@oplusuptrue}}
\pgfkeys{/tikz/noinv output down/.add code={}{\pgf@circuit@oa@oplusupfalse}}
\ctikzset{noinv output down/.add code={}{\pgf@circuit@oa@oplusupfalse}}

% Operational amplifier
\ctikzset{tripoles/op amp/width/.initial=1.7}              % Total width
\ctikzset{tripoles/op amp/port width/.initial=.7}          % Terminals length
\ctikzset{tripoles/op amp/height/.initial=1.4}             % Total height
\ctikzset{tripoles/op amp/input height/.initial=.5}        % Input port vertical separation
\ctikzset{tripoles/op amp/up pos/.initial=.45}             % Top and bottom anchor position
\ctikzset{tripoles/op amp/font/.initial=\pgf@circ@font@tenbm}  % Absolute font size needed!

% Fully differential operational amplifier
\ctikzset{tripoles/fd op amp/width/.initial=1.7}           % Total width
\ctikzset{tripoles/fd op amp/port width/.initial=.7}       % Terminals length
\ctikzset{tripoles/fd op amp/height/.initial=1.4}          % Total height
\ctikzset{tripoles/fd op amp/input height/.initial=.5}     % Input port vertical separation
\ctikzset{tripoles/fd op amp/output height/.initial=.5}    % Output port vertical separation
\ctikzset{tripoles/fd op amp/up pos/.initial=.45}          % Top and bottom anchor position
\ctikzset{tripoles/fd op amp/font/.initial=\pgf@circ@font@tenbm}  % Absolute font size needed!

\ctikzset{tripoles/en amp/width/.initial=1.7}
\ctikzset{tripoles/en amp/port width/.initial=.7}
\ctikzset{tripoles/en amp/height/.initial=1.6}
\ctikzset{tripoles/en amp/input height/.initial=.3}
\ctikzset{tripoles/en amp/up pos/.initial=.45}
\ctikzset{tripoles/en amp/font/.initial=\pgf@circ@font@tenbm}   % Absolute font size needed!
\ctikzset{tripoles/en amp/font2/.initial=\pgf@circ@font@twelve}  % Absolute font size needed!
\ctikzset{tripoles/en amp/text/.initial={$\mathstrut{\triangleright}\,{\infty}$}}
\tikzset{
    en amp text/.code = {%
        \ctikzsetvalof{tripoles/en amp/text}{#1}%
    },
    en amp text A/.code = {%
        \ctikzsetvalof{tripoles/en amp/text}{$\mathstrut{\triangleright}\,\mathrm{A}$}%
    },
}

% Transconductance amplifier
\ctikzset{tripoles/gm amp/width/.initial=1.7}              % Total width
\ctikzset{tripoles/gm amp/port width/.initial=.7}          % Terminals length
\ctikzset{tripoles/gm amp/height/.initial=1.4}             % Left side of the trapezoid
\ctikzset{tripoles/gm amp/height 2/.initial=0.5}           % Right side of the trapezoid
\ctikzset{tripoles/gm amp/input height/.initial=.5}        % Input port vertical separation
\ctikzset{tripoles/gm amp/up pos/.initial=.45}             % Top and bottom anchor position
\ctikzset{tripoles/gm amp/font/.initial=\pgf@circ@font@tenbm}  % Absolute font size needed!

% Instrumentation amplifier
\ctikzset{tripoles/inst amp/width/.initial=1.7}            % Total width
\ctikzset{tripoles/inst amp/port width/.initial=.7}        % Terminals length
\ctikzset{tripoles/inst amp/height/.initial=1.4}           % Left side of the trapezoid
\ctikzset{tripoles/inst amp/height 2/.initial=0.6}         % Right side of the trapezoid
\ctikzset{tripoles/inst amp/input height/.initial=.5}      % Input ports vertical separation
\ctikzset{tripoles/inst amp/up pos/.initial=.4}            % Top and bottom anchor position
\ctikzset{tripoles/inst amp/refv pos/.initial=.7}          % Top and bottom voltage reference position
\ctikzset{tripoles/inst amp/font/.initial=\pgf@circ@font@tenbm}  % Absolute font size needed!

% Instrumentation amplifier with differential output
\ctikzset{tripoles/fd inst amp/width/.initial=1.7}         % Total width
\ctikzset{tripoles/fd inst amp/port width/.initial=.7}     % Terminals length
\ctikzset{tripoles/fd inst amp/height/.initial=1.4}        % Left side of the trapezoid
\ctikzset{tripoles/fd inst amp/height 2/.initial=0.6}      % Right side of the trapezoid
\ctikzset{tripoles/fd inst amp/input height/.initial=.5}   % Input ports vertical separation
\ctikzset{tripoles/fd inst amp/output height/.initial=.5}  % Output ports vertical separation
\ctikzset{tripoles/fd inst amp/up pos/.initial=.4}         % Top and bottom anchor position
\ctikzset{tripoles/fd inst amp/refv pos/.initial=.7}       % Top and bottom voltage reference position
\ctikzset{tripoles/fd inst amp/font/.initial=\pgf@circ@font@tenbm}  % Absolute font size needed!

% Instrumentation amplifier with gain resistor terminals
\ctikzset{tripoles/inst amp ra/width/.initial=2.4}         % Total width
\ctikzset{tripoles/inst amp ra/port width/.initial=.7}     % Terminals length
\ctikzset{tripoles/inst amp ra/height/.initial=2.9}        % Left side of the trapezoid
\ctikzset{tripoles/inst amp ra/height 2/.initial=0.4}      % Right side of the trapezoid
\ctikzset{tripoles/inst amp ra/input height/.initial=.7}   % Input ports vertical separation
\ctikzset{tripoles/inst amp ra/up pos/.initial=.4}         % Top and bottom anchor position
\ctikzset{tripoles/inst amp ra/refv pos/.initial=.7}       % Top and bottom voltage reference position
\ctikzset{tripoles/inst amp ra/ra pos/.initial=.6}         % Gain resistor terminals vertical separation
\ctikzset{tripoles/inst amp ra/font/.initial=\pgf@circ@font@tenbm}  % Absolute font size needed!

% Plain amplifier
\ctikzset{tripoles/plain amp/width/.initial=1.7}           % Total width
\ctikzset{tripoles/plain amp/port width/.initial=.7}       % Terminals length
\ctikzset{tripoles/plain amp/height/.initial=1.4}          % Total height
\ctikzset{tripoles/plain amp/input height/.initial=.5}     % Input ports vertical separation
\ctikzset{tripoles/plain amp/up pos/.initial=.45}          % Top and bottom anchor position

\ctikzset{tripoles/thyristor/height/.initial=1.10}
\ctikzset{tripoles/thyristor/height 2/.initial=.5}
\ctikzset{tripoles/thyristor/width/.initial=1.0}
\ctikzset{tripoles/thyristor/diode height/.initial=.5}
\ctikzset{tripoles/thyristor/diode width left/.initial=.4}
\ctikzset{tripoles/thyristor/diode width right/.initial=.3}

\ctikzset{tripoles/triac/height/.initial=1.1}
\ctikzset{tripoles/triac/width/.initial=1}
\ctikzset{tripoles/triac/diode width left/.initial=.3}
\ctikzset{tripoles/triac/diode width right/.initial=.3}

%% Cute switches
\ctikzset{bipoles/cuteswitch/shape/.initial={ocirc}}
\ctikzset{bipoles/cuteswitch/height/.initial=.6}
\ctikzset{bipoles/cuteswitch/height 2/.initial=.2}
\ctikzset{bipoles/cuteswitch/width/.initial=.50}
\ctikzset{bipoles/cuteswitch/thickness/.initial=1}

\ctikzset{tripoles/spdt/width/.initial=.85}
\ctikzset{tripoles/spdt/height/.initial=.45}
\ctikzset{tripoles/spdt/margin/.initial=.45}

\ctikzset{tripoles/toggleswitch/height/.initial=.8}
\ctikzset{tripoles/toggleswitch/height 2/.initial=.0}
\ctikzset{tripoles/toggleswitch/width/.initial=.80}

\ctikzset{tripoles/mixer/width/.initial=0.7}
\ctikzset{tripoles/adder/width/.initial=0.7}
\ctikzset{tripoles/circulator/width/.initial=.7}
\ctikzset{tripoles/oscillator/width/.initial=.7}


\ctikzset{tripoles/wilkinson/height/.initial=1.3}
\ctikzset{tripoles/wilkinson/width/.initial=1.3}

\ctikzset{quadpoles/transformer/inner/.initial=0.4}
\ctikzset{quadpoles/transformer/width/.initial=1.5}
\ctikzset{quadpoles/transformer/width1/.initial=.4}
\ctikzset{quadpoles/transformer/height/.initial=1.5}
\ctikzset{quadpoles/transformer/height1/.initial=.8}
\ctikzset{quadpoles/transformer core/inner/.initial=0.4}
\ctikzset{quadpoles/transformer core/width/.initial=1.5}
\ctikzset{quadpoles/transformer core/height/.initial=1.5}
\ctikzset{quadpoles/transformer core/core height/.initial=.5}
\ctikzset{quadpoles/transformer core/core width/.initial=.05}
\ctikzset{quadpoles/gyrator/inner/.initial=0.4}
\ctikzset{quadpoles/gyrator/width/.initial=1.5}
\ctikzset{quadpoles/gyrator/height/.initial=1.5}
\ctikzset{quadpoles/fourport/width/.initial=1.3}
\ctikzset{quadpoles/fourport/height/.initial=1.3}
\ctikzset{quadpoles/coupler/width/.initial=1.3}
\ctikzset{quadpoles/coupler/height/.initial=1.3}
\ctikzset{quadpoles/coupler2/width/.initial=1.3}
\ctikzset{quadpoles/coupler2/height/.initial=1.3}

\ctikzset{/tikz/circuitikz/tripoles/magnetron/width/.initial=1}

\ctikzset{quadpoles style/.is choice}
\ctikzset{quadpoles style/inward/.code={% default value
        \ctikzset{quadpoles/transformer/inner=0.4}%
        \ctikzset{quadpoles/transformer/width=1.5}%
        \ctikzset{quadpoles/transformer core/inner=0.4}%
        \ctikzset{quadpoles/transformer core/width=1.5}%
        \ctikzset{quadpoles/gyrator/inner=0.4}%
        \ctikzset{quadpoles/gyrator/width=1.5}%
    }%
}
\ctikzset{quadpoles style/inline/.code={% now horizontal baffle
        \ctikzset{quadpoles/transformer/inner=1}%
        \ctikzset{quadpoles/transformer/width=0.6}%
        \ctikzset{quadpoles/transformer core/inner=1}%
        \ctikzset{quadpoles/transformer core/width=0.6}%
        \ctikzset{quadpoles/gyrator/inner=1} % FIXME
        \ctikzset{quadpoles/gyrator/width=0.6}%
    }%
}

%
% multipoles
%
\ctikzset{multipoles/thickness/.initial=2}
\ctikzset{multipoles/font/.initial=\pgf@circ@font@tiny}
% DIP (dual in line package) chips
\ctikzset{multipoles/dipchip/width/.initial=1.2}
\ctikzset{multipoles/dipchip/num pins/.initial=8}
\ctikzset{multipoles/dipchip/pin spacing/.initial=0.4}
\pgfkeys{/tikz/num pins/.add code={}{\ctikzset{multipoles/dipchip/num pins=#1}}}
% QFP (quad flat package) chips
\ctikzset{multipoles/qfpchip/num pins/.initial=8}
\ctikzset{multipoles/qfpchip/pin spacing/.initial=0.4}
\pgfkeys{/tikz/num pins/.add code={}{\ctikzset{multipoles/qfpchip/num pins=#1}}}
% chip numbers
\newif\ifpgf@circuit@chip@shownumbers\pgf@circuit@chip@shownumberstrue
\pgfkeys{/tikz/show numbers/.add code={}{\pgf@circuit@chip@shownumberstrue}}
\ctikzset{show numbers/.add code={}{\pgf@circuit@chip@shownumberstrue}}
\pgfkeys{/tikz/hide numbers/.add code={}{\pgf@circuit@chip@shownumbersfalse}}
\ctikzset{hide numbers/.add code={}{\pgf@circuit@chip@shownumbersfalse}}
\newif\ifpgf@circuit@chip@straightnumbers\pgf@circuit@chip@straightnumberstrue
\pgfkeys{/tikz/straight numbers/.add code={}{\pgf@circuit@chip@straightnumberstrue}}
\ctikzset{straight numbers/.add code={}{\pgf@circuit@chip@straightnumberstrue}}
\pgfkeys{/tikz/rotated numbers/.add code={}{\pgf@circuit@chip@straightnumbersfalse}}
\ctikzset{rotated numbers/.add code={}{\pgf@circuit@chip@straightnumbersfalse}}
% external chip pins
\ctikzset{multipoles/external pins thickness/.initial=1}
\ctikzset{multipoles/external pins width/.initial=0.2}
\ctikzset{multipoles/external pad fraction/.initial=0}
\pgfkeys{/tikz/external pins width/.add code={}{\ctikzset{multipoles/external pins width=#1}}}
\pgfkeys{/tikz/external pad fraction/.add code={}{\ctikzset{multipoles/external pad fraction=#1}}}
% topmarks
\newif\ifpgf@circuit@chip@topmark\pgf@circuit@chip@topmarktrue
\pgfkeys{/tikz/topmark/.add code={}{\pgf@circuit@chip@topmarktrue}}
\ctikzset{topmark/.add code={}{\pgf@circuit@chip@topmarktrue}}
\pgfkeys{/tikz/no topmark/.add code={}{\pgf@circuit@chip@topmarkfalse}}
\ctikzset{no topmark/.add code={}{\pgf@circuit@chip@topmarkfalse}}

% rotary switch by Romano
\ctikzset{multipoles/rotary/thickness/.initial=1}
\ctikzset{multipoles/rotary/shape/.initial=ocirc}
\ctikzset{multipoles/rotary/channels/.initial=5}
\ctikzset{multipoles/rotary/angle/.initial=60}
\ctikzset{multipoles/rotary/wiper/.initial=20}
\ctikzset{multipoles/rotary/arrow/.is choice}
\newif\ifpgf@circ@rotaryarrow\pgf@circ@rotaryarrowfalse
\newif\ifpgf@circ@rotaryarrow@cw\pgf@circ@rotaryarrow@cwfalse
\newif\ifpgf@circ@rotaryarrow@ccw\pgf@circ@rotaryarrow@ccwfalse
\ctikzset{multipoles/rotary/arrow/none/.code={\pgf@circ@rotaryarrowfalse\pgf@circ@rotaryarrow@cwfalse\pgf@circ@rotaryarrow@ccwfalse}}
\ctikzset{multipoles/rotary/arrow/both/.code={\pgf@circ@rotaryarrowtrue\pgf@circ@rotaryarrow@cwtrue\pgf@circ@rotaryarrow@ccwtrue}}
\ctikzset{multipoles/rotary/arrow/cw/.code={\pgf@circ@rotaryarrowtrue\pgf@circ@rotaryarrow@cwtrue\pgf@circ@rotaryarrow@ccwfalse}}
\ctikzset{multipoles/rotary/arrow/ccw/.code={\pgf@circ@rotaryarrowtrue\pgf@circ@rotaryarrow@cwfalse\pgf@circ@rotaryarrow@ccwtrue}}

\tikzset{%
    rotary switch/.style args={#1in#2wiper#3}{%
        shape=rotaryswitch,
        /tikz/circuitikz/multipoles/rotary/channels=#1,
        /tikz/circuitikz/multipoles/rotary/angle=#2,
        /tikz/circuitikz/multipoles/rotary/wiper=#3,
    },
    rotary switch -/.style args={#1in#2wiper#3}{
        rotary switch=#1 in #2 wiper #3,
        /tikz/circuitikz/multipoles/rotary/arrow=none,
    },
    rotary switch <-/.style args={#1in#2wiper#3}{
        rotary switch=#1 in #2 wiper #3,
        /tikz/circuitikz/multipoles/rotary/arrow=ccw,
    },
    rotary switch ->/.style args={#1in#2wiper#3}{
        rotary switch=#1 in #2 wiper #3,
        /tikz/circuitikz/multipoles/rotary/arrow=cw,
    },
    rotary switch <->/.style args={#1in#2wiper#3}{
        rotary switch=#1 in #2 wiper #3,
        /tikz/circuitikz/multipoles/rotary/arrow=both,
    },
    % Notice that these should be the same as the initial values of the keys
    rotary switch/.default={5 in 60 wiper 20},
    rotary switch -/.default={5 in 60 wiper 20},
    rotary switch <-/.default={5 in 60 wiper 20},
    rotary switch ->/.default={5 in 60 wiper 20},
    rotary switch <->/.default={5 in 60 wiper 20},
}

% %Mechanical section
\ctikzset{/tikz/circuitikz/tripoles/elmech/height/.initial=.8}
\ctikzset{/tikz/circuitikz/tripoles/elmech/width/.initial=.6}
\ctikzset{bipoles/spring/height/.initial=.5}
\ctikzset{bipoles/spring/width/.initial=.5}
\ctikzset{bipoles/mass/height/.initial=.55}
\ctikzset{bipoles/mass/box height/.initial=.4}
\ctikzset{bipoles/mass/width/.initial=.5}

\ctikzset{bipoles/damper/height/.initial=.35}
\ctikzset{bipoles/damper/length/.initial=.3}
\ctikzset{bipoles/damper/width/.initial=.4}


\ctikzset{bipole/.is family}
\ctikzset{bipole/kind/.initial=}
\ctikzset{bipole/name/.initial=}
\newif\ifpgf@circuit@bipole@isvoltage
\ctikzset{bipole/is voltage/.is if=pgf@circuit@bipole@isvoltage}
\newif\ifpgf@circuit@bipole@voltageoutsideofsymbol
\ctikzset{bipole/is voltageoutsideofsymbol/.is if=pgf@circuit@bipole@voltageoutsideofsymbol}
\newif\ifpgf@circuit@bipole@strokedsymbol
\ctikzset{bipole/is strokedsymbol/.is if=pgf@circuit@bipole@strokedsymbol}
\newif\ifpgf@circuit@bipole@iscurrent
\ctikzset{bipole/is current/.is if=pgf@circuit@bipole@iscurrent}

\ctikzset{bipole/voltage/.is family}
\newif\ifpgf@circuit@bipole@voltage@backward
\ctikzset{bipole/voltage/direction/.is choice}
\ctikzset{bipole/voltage/direction/forward/.code={\pgf@circuit@bipole@voltage@backwardfalse}}
\ctikzset{bipole/voltage/direction/backward/.code={\pgf@circuit@bipole@voltage@backwardtrue}}
\newif\ifpgf@circuit@bipole@voltage@below
\ctikzset{bipole/voltage/position/.is choice}
\ctikzset{bipole/voltage/position/above/.code={\pgf@circuit@bipole@voltage@belowfalse}}
\ctikzset{bipole/voltage/position/below/.code={\pgf@circuit@bipole@voltage@belowtrue}}

\ctikzset{bipole/voltage/label/unit/.initial=}
\ctikzset{bipole/voltage/label/name/.initial=}

\ctikzset{bipole/current/.is family}
\newif\ifpgf@circuit@bipole@current@backward
\ctikzset{bipole/current/direction/.is choice}
\ctikzset{bipole/current/direction/forward/.code={\pgf@circuit@bipole@current@backwardfalse}}
\ctikzset{bipole/current/direction/backward/.code={\pgf@circuit@bipole@current@backwardtrue}}
\newif\ifpgf@circuit@bipole@current@before
\ctikzset{bipole/current/x position/.is choice}
\ctikzset{bipole/current/x position/after/.code={\pgf@circuit@bipole@current@beforefalse}}
\ctikzset{bipole/current/x position/before/.code={\pgf@circuit@bipole@current@beforetrue}}
\newif\ifpgf@circuit@bipole@current@below
\ctikzset{bipole/current/y position/.is choice}
\ctikzset{bipole/current/y position/above/.code={\pgf@circuit@bipole@current@belowfalse}}
\ctikzset{bipole/current/y position/below/.code={\pgf@circuit@bipole@current@belowtrue}}
\ctikzset{bipole/current/label/unit/.initial=}
\ctikzset{bipole/current/label/name/.initial=}

\ctikzset{bipole/flow/.is family}
\newif\ifpgf@circuit@bipole@flow@backward
\ctikzset{bipole/flow/direction/.is choice}
\ctikzset{bipole/flow/direction/forward/.code={\pgf@circuit@bipole@flow@backwardfalse}}
\ctikzset{bipole/flow/direction/backward/.code={\pgf@circuit@bipole@flow@backwardtrue}}
\newif\ifpgf@circuit@bipole@flow@before
\ctikzset{bipole/flow/x position/.is choice}
\ctikzset{bipole/flow/x position/after/.code={\pgf@circuit@bipole@flow@beforefalse}}
\ctikzset{bipole/flow/x position/before/.code={\pgf@circuit@bipole@flow@beforetrue}}
\newif\ifpgf@circuit@bipole@flow@below
\ctikzset{bipole/flow/y position/.is choice}
\ctikzset{bipole/flow/y position/above/.code={\pgf@circuit@bipole@flow@belowfalse}}
\ctikzset{bipole/flow/y position/below/.code={\pgf@circuit@bipole@flow@belowtrue}}
\ctikzset{bipole/flow/label/unit/.initial=}
\ctikzset{bipole/flow/label/name/.initial=}
\ctikzset{flow/distance/.initial = .5}
\ctikzset{flow/offset/.initial = .2}%distance between flow-arrow and conductor

\ctikzset{bipole/label/.is family}
\ctikzset{bipole/label/position/.initial=90}
\ctikzset{bipole/label/unit/.initial=}
\ctikzset{bipole/label/name/.initial=}
\ctikzset{bipole/annotation/.is family}
\ctikzset{bipole/annotation/position/.initial=-90}
\ctikzset{bipole/annotation/unit/.initial=}
\ctikzset{bipole/annotation/name/.initial=}

\newif\ifpgf@circuit@europeanresistor
\ctikzset{resistor/.is choice}
\ctikzset{resistor/american/.code = \pgf@circuit@europeanresistorfalse }
\ctikzset{resistor/european/.code = \pgf@circuit@europeanresistortrue }

\ctikzset{inductor/.is choice}
\ctikzset{inductor/cute/.code={\ctikzsetvalof{inductor}{cute}}}
\ctikzset{inductor/european/.code={\ctikzsetvalof{inductor}{european}}}
\ctikzset{inductor/american/.code={\ctikzsetvalof{inductor}{american}}}

\newif\ifpgf@circuit@strokediode
\newif\ifpgf@circuit@fulldiode
\pgf@circuit@strokediodefalse
\pgf@circuit@fulldiodefalse

\ctikzset{diode/.is choice}
\ctikzset{diode/empty/.code = \pgf@circuit@fulldiodefalse\pgf@circuit@strokediodefalse}%default
\ctikzset{diode/full/.code = \pgf@circuit@fulldiodetrue }
\ctikzset{diode/stroke/.code = \pgf@circuit@strokediodetrue}

\tikzset{full diodes/.style = { \circuitikzbasekey/diode = full}}
\tikzset{empty diodes/.style = { \circuitikzbasekey/diode = empty}}
\tikzset{stroke diodes/.style = { \circuitikzbasekey/diode = stroke}}

\ctikzset{thickness/.initial=2}
\ctikzset{color/.initial=black}
\pgfkeys{/tikz/color/.add code={}{\ctikzset{color={#1}}}}

\newif\ifpgf@circ@siunitx
\newif\ifpgf@circ@siunitx@res

\ctikzset{straight/.is choice}
\ctikzset{straightvoltage value/.initial=true}
\ctikzset{straight/true/.code = {\pgf@circuit@bipole@voltage@straighttrue}}
\ctikzset{straight/false/.code = {\pgf@circuit@bipole@voltage@straightfalse}}
\ctikzset{straightvoltage/.style = {/tikz/circuitikz/straight=true}}
\newif\ifpgf@circuit@bipole@voltage@straight
\ctikzset{bipole/straight/.is if=pgf@circuit@bipole@voltage@straight}


\ctikzset{voltage/.is family}
\ctikzset{voltage/distance from node/.initial=.5} %\pgf@circ@Rlen units
\ctikzset{voltage/distance from line/.initial=.08} % pos, tra 0 e 1
\ctikzset{voltage/bump a/.initial=1.2}
\ctikzset{voltage/bump b/.initial=1.5}
\ctikzset{voltage/shift/.initial=0.0} % shift form the cable of voltage symbols
\ctikzset{voltage shift/.style={voltage/shift=#1}}
\tikzset{voltage shift/.style={\circuitikzbasekey/voltage/shift=#1}}
\ctikzset{voltage/european label distance/.initial=1.4}
\ctikzset{voltage/american label distance/.initial=1.1}
% shaping the +/- sign, see pgfcircvoltage.tex
\ctikzset{voltage/american font/.initial={}}
\ctikzset{voltage/american plus/.initial={$+$}}
\ctikzset{voltage/american minus/.initial={$-$}}

% special cases
\ctikzset{bipoles/generic/voltage/distance from node/.initial=.4}
\ctikzset{bipoles/generic/voltage/bump b/.initial=2}
\ctikzset{bipoles/generic/voltage/european label distance/.initial=1.8}
%\ctikzset{bipoles/thermocouple/voltage/distance from node/.initial=.3}
\ctikzset{bipoles/thermocouple/voltage/bump b/.initial=2.2}
\ctikzset{bipoles/thermocouple/voltage/european label distance/.initial=1.5}
\ctikzset{bipoles/ageneric/voltage/distance from node/.initial=.4}
\ctikzset{bipoles/ageneric/voltage/bump b/.initial=2}
\ctikzset{bipoles/ageneric/voltage/european label distance/.initial=1.8}
\ctikzset{bipoles/fullgeneric/voltage/distance from node/.initial=.4}
\ctikzset{bipoles/fullgeneric/voltage/bump b/.initial=2}
\ctikzset{bipoles/fullgeneric/voltage/european label distance/.initial=1.8}
\ctikzset{bipoles/memristor/voltage/distance from node/.initial=.4}
\ctikzset{bipoles/memristor/voltage/bump b/.initial=2}
\ctikzset{bipoles/memristor/voltage/european label distance/.initial=1.8}
%\ctikzset{bipoles/tline/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/tline/voltage/bump b/.initial=2.4}
\ctikzset{bipoles/tline/voltage/european label distance/.initial=2.1}
%\ctikzset{bipoles/varistor/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/varistor/voltage/bump b/.initial=2.4}
\ctikzset{bipoles/varistor/voltage/european label distance/.initial=2}
%\ctikzset{bipoles/photoresistor/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/photoresistor/voltage/bump b/.initial=2}
\ctikzset{bipoles/photoresistor/voltage/european label distance/.initial=1.8}
%\ctikzset{bipoles/thermistor/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/thermistor/voltage/bump b/.initial=2.4}
\ctikzset{bipoles/thermistor/voltage/european label distance/.initial=2}
%\ctikzset{bipoles/thermistorntc/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/thermistorntc/voltage/bump b/.initial=1.6}
%\ctikzset{bipoles/thermistorptc/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/thermistorptc/voltage/bump b/.initial=1.6}

\ctikzset{current/.is family}
\ctikzset{current/distance/.initial = .5}


\tikzset{american currents/.style = {\circuitikzbasekey/current = american}}
\tikzset{european currents/.style = {\circuitikzbasekey/current = european}}
\tikzset{american voltages/.style = {\circuitikzbasekey/voltage = american}}
\tikzset{european voltages/.style = {\circuitikzbasekey/voltage = european}}
\tikzset{american resistors/.style = {\circuitikzbasekey/resistor = american}}
\tikzset{european resistors/.style = {\circuitikzbasekey/resistor = european}}

\newif\ifpgf@circuit@europeangfsurgearrester
\ctikzset{gas filled surge arrester choice/.is choice}
\ctikzset{gas filled surge arrester choice/european/.code= {\pgf@circuit@europeangfsurgearrestertrue}}
\ctikzset{gas filled surge arrester choice/american/.code= {\pgf@circuit@europeangfsurgearresterfalse}}

\tikzset{american gas filled surge arrester set/.style = {\circuitikzbasekey/gas filled surge arrester choice=american}}
\tikzset{european gas filled surge arrester set/.style = {\circuitikzbasekey/gas filled surge arrester choice=european}}
\tikzset{american inductors/.style = {\circuitikzbasekey/inductor = american}}
\tikzset{european inductors/.style = {\circuitikzbasekey/inductor = european}}
\tikzset{cute inductors/.style = {\circuitikzbasekey/inductor = cute}}
\tikzset{american ports/.style = {\circuitikzbasekey/logic ports = american}}
\tikzset{european ports/.style = {\circuitikzbasekey/logic ports = european}}
\tikzset{european/.style = {european currents, european voltages, european resistors, european inductors, european ports, european gas filled surge arrester set}}
\tikzset{american/.style = {american currents, american voltages, american resistors, american inductors, american ports, american gas filled surge arrester set}}
\tikzset{cute/.style = {european currents, european voltages, american resistors, cute inductors, american ports}}

% I should try to make the tree clearer (this voltage conflicts with the options above)

\newif\ifpgf@circuit@europeanvoltage
\ctikzset{voltage/.is choice}
\ctikzset{voltage/american/.code = {\pgf@circuit@europeanvoltagefalse}}
\ctikzset{voltage/european/.code = {\pgf@circuit@europeanvoltagetrue}}

\newif\ifpgf@circuit@europeancurrent
\ctikzset{current/.is choice}
\ctikzset{current/american/.code = \pgf@circuit@europeancurrentfalse}
\ctikzset{current/european/.code = \pgf@circuit@europeancurrenttrue}

% noise sources
\ctikzset{bipoles/noise sources/fillcolor/.initial=gray!50}

\ctikzset{label/align/.is choice}
\ctikzset{label/align/straight/.code={\ctikzsetvalof{label/align}{straight}}}
\ctikzset{label/align/rotate/.code={\ctikzsetvalof{label/align}{rotate}}}
\ctikzset{label/align/smart/.code={\ctikzsetvalof{label/align}{smart}}}

% seven segment displays by RGtti

\newif\ifpgf@circ@sevenseg@dot
\newif\ifpgf@circ@sevenseg@box
\def\pgf@circ@sevenseg@dotstate{empty}
\ctikzset{seven seg/.is family}
\ctikzset{seven seg/dot/.is choice}
% none means no dot, not space for it. Empty means no dot, but space
\ctikzset{seven seg/dot/none/.code={\pgf@circ@sevenseg@dotfalse}}
\ctikzset{seven seg/dot/empty/.code={\pgf@circ@sevenseg@dottrue\def\pgf@circ@sevenseg@dotstate{empty}}}
\ctikzset{seven seg/dot/off/.code={\pgf@circ@sevenseg@dottrue\def\pgf@circ@sevenseg@dotstate{off}}}
\ctikzset{seven seg/dot/on/.code={\pgf@circ@sevenseg@dottrue\def\pgf@circ@sevenseg@dotstate{on}}}
%
\ctikzset{seven seg/width/.initial=0.4}% relative to \pgf@circ@Rlen
\ctikzset{seven seg/thickness/.initial=4pt}% segment thickness
\ctikzset{seven seg/segment sep/.initial=0.2pt}% gap between segments
\ctikzset{seven seg/box sep/.initial=1pt}% external box gap
\ctikzset{seven seg/color on/.initial=red}% color for segment "on"
\ctikzset{seven seg/color off/.initial=gray!20!white} % ...and "off"
\ctikzset{seven seg/box/.is choice}
\ctikzset{seven seg/box/off/.code={\pgf@circ@sevenseg@boxfalse}}
\ctikzset{seven seg/box/on/.code={\pgf@circ@sevenseg@boxtrue}}

\ctikzset{seven seg/bits/.initial=0000000}

\ctikzset{seven seg/value/.code={%
    \edef\@@tmp{#1}%
    \edef\@@n{0} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1111110}\fi
    \edef\@@n{1} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=0110000}\fi
    \edef\@@n{2} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1101101}\fi
    \edef\@@n{3} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1111001}\fi
    \edef\@@n{4} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=0110011}\fi
    \edef\@@n{5} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1011011}\fi
    \edef\@@n{6} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1011111}\fi
    \edef\@@n{7} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1110000}\fi
    \edef\@@n{8} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1111111}\fi
    \edef\@@n{9} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1111011}\fi
    \edef\@@n{10}\ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1110111}\fi
    \edef\@@n{11}\ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=0011111}\fi
    \edef\@@n{12}\ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1001110}\fi
    \edef\@@n{13}\ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=0111101}\fi
    \edef\@@n{14}\ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1001111}\fi
    \edef\@@n{15}\ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1000111}\fi
    \edef\@@n{A} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1110111}\fi
    \edef\@@n{B} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=0011111}\fi
    \edef\@@n{C} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1001110}\fi
    \edef\@@n{D} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=0111101}\fi
    \edef\@@n{E} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1001111}\fi
    \edef\@@n{F} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1000111}\fi
    \edef\@@n{a} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1110111}\fi
    \edef\@@n{b} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=0011111}\fi
    \edef\@@n{c} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1001110}\fi
    \edef\@@n{d} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=0111101}\fi
    \edef\@@n{e} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1001111}\fi
    \edef\@@n{f} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=1000111}\fi
    \edef\@@n{-} \ifx\@@tmp\@@n\relax\ctikzset{seven seg/bits=0000001}\fi
}}

\tikzset{%
    seven segment val/.style args={#1dot#2box#3}{%
        shape=bare7seg,
        /tikz/circuitikz/seven seg/value=#1,
        /tikz/circuitikz/seven seg/dot=#2,
        /tikz/circuitikz/seven seg/box=#3,
    },
    seven segment bits/.style args={#1dot#2box#3}{%
        shape=bare7seg,
        /tikz/circuitikz/seven seg/bits=#1,
        /tikz/circuitikz/seven seg/dot=#2,
        /tikz/circuitikz/seven seg/box=#3,
    },
}


%%%%%%%%%% new
\pgfkeys{\circuitikzbasekey/.search also={/tikz}}

% Electronic tubes: diodetube, triode, tetrode and pentode
\ctikzset{tubes/width/.initial=1}                    % relative width
\ctikzset{tubes/height/.initial=1.4}                 % relative height
\ctikzset{tubes/tube radius/.initial=0.40}           % radius of tube circle
\ctikzset{tubes/anode distance/.initial=0.40}        % distance from center
\ctikzset{tubes/anode width/.initial=0.40}           % width of an anode/plate
\ctikzset{tubes/grid protrusion/.initial=0.25}       % distance from center
\ctikzset{tubes/grid dashes/.initial=5}              % number of grid dashes
\ctikzset{tubes/grid separation/.initial=0.2}        % separation between grids
\ctikzset{tubes/grid shift/.initial=0.0}             % y shift grids from center
\ctikzset{tubes/cathode distance/.initial=0.40}      % distance from grid
\ctikzset{tubes/cathode width/.initial=0.40}         % width of an cathode
\ctikzset{tubes/cathode corners/.initial=0.06}       % corners of the cathode wire
\ctikzset{tubes/cathode right extend/.initial=0.075} % extension at the right side
\ctikzset{tubes/filament distance/.initial=0.1}      % distance from cathode
\ctikzset{tubes/filament angle/.initial=15}          % Angle from centerpoint

\newif\ifpgf@circuit@tubes@filament\pgf@circuit@tubes@filamentfalse
\pgfkeys{/tikz/filament/.add code={}{\pgf@circuit@tubes@filamenttrue}}
\ctikzset{tubes/filament/.add code={}{\pgf@circuit@tubes@filamenttrue}}
\newif\ifpgf@circuit@tubes@nocathode\pgf@circuit@tubes@nocathodefalse
\pgfkeys{/tikz/nocathode/.add code={}{\pgf@circuit@tubes@nocathodetrue}}
\ctikzset{tubes/nocathode/.add code={}{\pgf@circuit@tubes@nocathodetrue}}
\newif\ifpgf@circuit@tubes@fullcathode\pgf@circuit@tubes@fullcathodefalse
\pgfkeys{/tikz/fullcathode/.add code={}{\pgf@circuit@tubes@fullcathodetrue}}
\ctikzset{tubes/fullcathode/.add code={}{\pgf@circuit@tubes@fullcathodetrue}}

\endinput


==> pgfcircbipoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%% Generic macro for defining a bipole shape
% #1 - additional anchors
% #2 - lower y-size of the bipole (from the center).
% #3 - #shape is the name of the shape
% #4 - upper y-size of the bipole (from the center)
% #5 - width of the bipole
% #6 - macros drawing the bipole
%
\long\def\pgfcircdeclarebipole{%
    \pgfcircdeclarebipolescaled{default}}

%% Generic macro for defining a bipole shape
% #1 - scale factor
% #2 - additional anchors
% #3 - lower y-size of the bipole (from the center).
% #4 - #shape is the name of the shape
% #5 - upper y-size of the bipole (from the center)
% #6 - width of the bipole
% #7 - macros drawing the bipole
%
\long\def\pgfcircdeclarebipolescaled#1#2#3#4#5#6#7{
    \pgfdeclareshape{#4shape}{
        \savedmacro{\ctikzclass}{\edef\ctikzclass{#1}}
        \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
        \savedanchor{\northeast}{
            \pgf@circ@scaled@Rlen=\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen
            \pgf@y=#5\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=#6\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
        }
        \savedanchor{\northeastborder}{
            \pgf@circ@scaled@Rlen=\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen
            \pgf@y=#5\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@y=\ctikzvalof{bipoles/border margin}\pgf@y
            \pgf@x=#6\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
            \pgf@x=\ctikzvalof{bipoles/border margin}\pgf@x
        }
        \savedanchor{\southwestborder}{
            \pgf@circ@scaled@Rlen=\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen
            \pgf@y=-#3\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@y=\ctikzvalof{bipoles/border margin}\pgf@y
            \pgf@x=-#6\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
            \pgf@x=\ctikzvalof{bipoles/border margin}\pgf@x
        }
        \savedanchor{\southwest}{
            \pgf@circ@scaled@Rlen=\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen
            \pgf@y=-#3\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-#6\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
        }
        \savedanchor{\centerpoint}{
            \pgf@circ@scaled@Rlen=\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen
            \pgf@circ@res@down=-#3\pgf@circ@scaled@Rlen
            \pgf@circ@res@up=#5\pgf@circ@scaled@Rlen
            \pgfpointorigin
            \pgf@y=\pgf@circ@res@up
            \advance\pgf@y by\pgf@circ@res@down
            \pgf@y=.5\pgf@y
        }
        \anchor{center}{\pgfpointorigin}
        \anchor{n}{
            \northeast
            \pgf@x=0cm
        }
        \anchor{north east}{
            \northeast
        }
        \anchor{north west}{
            \northeast
            \pgf@x=-\pgf@x
        }
        \anchor{ne}{
            \northeast
        }
        \anchor{nw}{
            \northeast
            \pgf@x=-\pgf@x
        }
        \anchor{e}{
            \northeast
            \pgf@y=0cm
        }
        \anchor{s}{
            \southwest
            \pgf@x=0cm
        }
        \anchor{south east}{
            \southwest
            \pgf@x=-\pgf@x
        }
        \anchor{south west}{
            \southwest
        }
        \anchor{se}{
            \southwest
            \pgf@x=-\pgf@x
        }
        \anchor{sw}{
            \southwest
        }
        \anchor{w}{
            \southwest
            \pgf@y=0cm
        }
        \anchor{north}{
            \northeast
            \pgf@x=0cm
        }
        \anchor{east}{
            \northeast
            \pgf@y=0cm
        }
        \anchor{south}{
            \southwest
            \pgf@x=0cm
        }
        \anchor{west}{
            \southwest
            \pgf@y=0cm
        }
        \anchor{right}{
            \northeast
            \pgf@y=0cm
        }
        \anchor{above}{
            \northeast
            \pgf@x=0cm
        }
        \anchor{left}{
            \southwest
            \pgf@y=0cm
        }
        \anchor{below}{
            \southwest
            \pgf@x=0cm
        }
        \anchor{a}{
            \northeast
            \pgf@y=0cm
        }
        \anchor{b}{
            \southwest
            \pgf@y=0cm
        }
        \savedanchor{\textanchor}{%
            \pgf@y=\ht\pgfnodeparttextbox
            \pgf@x=-.5\wd\pgfnodeparttextbox
        }
        \anchor{text}{
            \textanchor
        }
        \anchorborder{%
            \ifpgf@circuit@bipole@inverted
                \pgf@circ@res@left=-\pgf@x
                \pgf@circ@res@right=-\pgf@y
            \else
                \pgf@circ@res@left=\pgf@x
                \pgf@circ@res@right=\pgf@y
            \fi
            \ifdim\pgf@circ@res@right>0cm
                \pgfpointborderrectangle{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@right}}{\northeastborder}
            \else
                \southwestborder
                \pgfpointborderrectangle{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@right}}{\pgfpoint{-\pgf@x}{-\pgf@y}}
            \fi
        }

        #2

        \backgroundpath{
            \pgfsetcolor{\ctikzvalof{color}}

            \northeast
            \pgf@circ@res@up = \pgf@y
            \pgf@circ@res@zero = 0cm
            \pgf@circ@res@left = -\pgf@x
            \pgf@circ@res@right = \pgf@x
            \southwest
            \pgf@circ@res@down = \pgf@y
            \pgf@circ@scaled@Rlen=\scaledRlen
            \pgfstartlinewidth=\pgflinewidth
            \pgfsetcornersarced{\pgfpointorigin}% do not use rounded corners!
            #7

            \pgfsetlinewidth{\pgfstartlinewidth}
        }
    }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Standard bipole shapes declarations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%
% Resistive components
%%%%%%%%%%%%%%%%%%%%%%%%

%% Short circuit

%%% NOTICE that the short is really NOT drawn; we trust the fact that its
%%% natural length is zero.
\pgfcircdeclarebipole
{}
{0}
{short}
{0}
{0}
{ }

%% Open circuit
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/open/height}}
{open}
{\ctikzvalof{bipoles/open/height}}
{\ctikzvalof{bipoles/open/width}}
{ }

%% Generic bipole - used as resistor by some (bleah)
\pgfcircdeclarebipolescaled{resistors}
{}
{\ctikzvalof{bipoles/generic/height}}
{generic}
{\ctikzvalof{bipoles/generic/height}}
{\ctikzvalof{bipoles/generic/width}}
{
    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgf@circ@draworfill
}

%% Generic empty tunable
\pgfcircdeclarebipolescaled{resistors}
{}
{\ctikzvalof{bipoles/tgeneric/height}}
{tgeneric}
{\ctikzvalof{bipoles/tgeneric/height}}
{\ctikzvalof{bipoles/tgeneric/width}}
{
    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{.4\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{.4\pgf@circ@res@down}}
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgf@circ@draworfill
    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{.5\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-.5\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Generic asymmetric bipole
\pgfcircdeclarebipolescaled{resistors}
{}
{\ctikzvalof{bipoles/ageneric/height}}
{ageneric}
{\ctikzvalof{bipoles/ageneric/height}}
{\ctikzvalof{bipoles/ageneric/width}}
{
    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope

    \pgfpathrectanglecorners{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{stroke,fill}
}

%% Memristor
\pgfcircdeclarebipolescaled{resistors}
{}
{\ctikzvalof{bipoles/memristor/height}}
{memristor}
{\ctikzvalof{bipoles/memristor/height}}
{\ctikzvalof{bipoles/memristor/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 14

    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.72*\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.72*\pgf@circ@res@left}{\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.35*\pgf@circ@res@left}{\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.35*\pgf@circ@res@left}{-\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{-.05*\pgf@circ@res@left}{-\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{-.05*\pgf@circ@res@left}{\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.42*\pgf@circ@res@right}{\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.42*\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.8*\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}

    \pgfpathrectanglecorners{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{stroke,fill}
}

%% Photoresistor
\pgfcircdeclarebipolescaled{resistors}
{}
{\ctikzvalof{bipoles/photoresistor/height 2}}
{photoresistor}
{\ctikzvalof{bipoles/photoresistor/height}}
{\ctikzvalof{bipoles/photoresistor/width}}
{
    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{-\pgf@circ@res@down}}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.3\pgf@circ@res@right}{-1.2\pgf@circ@res@down}}
        \pgfusepath{draw}
        \pgfpathmoveto{\pgfpoint{.45\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.05\pgf@circ@res@right}{-1.2\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Thermistor
\pgfcircdeclarebipolescaled{resistors}
{{% anchor for labelling the type of dependency
    \anchor{label}{%
        \southwest
        \pgf@x=0.4\pgf@x
        \pgf@y=1.2\pgf@y
    }%
}}
{\ctikzvalof{bipoles/thermistor/height}}
{thermistor}
{\ctikzvalof{bipoles/thermistor/height}}
{\ctikzvalof{bipoles/thermistor/width}}
{
    \pgfscope
    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\ctikzvalof{bipoles/thermistor/main}\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{-\ctikzvalof{bipoles/thermistor/main}\pgf@circ@res@up}}
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgf@circ@draworfill
    \endpgfscope

    %\pgfscope
    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{-\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{1.2\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{1.2\pgf@circ@res@down}}
    \pgfusepath{draw}
    %\endpgfscope
}

%% Thermistor PTC
\pgfcircdeclarebipolescaled{resistors}
{}
{\ctikzvalof{bipoles/thermistorptc/height 2}}
{thermistorptc}
{\ctikzvalof{bipoles/thermistorptc/height}}
{\ctikzvalof{bipoles/thermistorptc/width}}
{
    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\ctikzvalof{bipoles/thermistorptc/main}\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{-\ctikzvalof{bipoles/thermistorptc/main}\pgf@circ@res@up}}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{-\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgftext[top,x=.85\pgf@circ@res@left,y=.75\pgf@circ@res@down]{\pgf@circ@font@tiny$\vartheta$}
    \pgfsetarrowsend{latexslim}
    \pgfpathmoveto{\pgfpoint{.62\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.62\pgf@circ@res@left}{.7\pgf@circ@res@down}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{.45\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.45\pgf@circ@res@left}{.7\pgf@circ@res@down}}
    \pgfusepath{draw}
}

%% Thermistor NTC
\pgfcircdeclarebipolescaled{resistors}
{}
{\ctikzvalof{bipoles/thermistorntc/height 2}}
{thermistorntc}
{\ctikzvalof{bipoles/thermistorntc/height}}
{\ctikzvalof{bipoles/thermistorntc/width}}
{
    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\ctikzvalof{bipoles/thermistorntc/main}\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{-\ctikzvalof{bipoles/thermistorntc/main}\pgf@circ@res@up}}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{-\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgftext[top,x=.85\pgf@circ@res@left,y=.75\pgf@circ@res@down]{\pgf@circ@font@tiny$\vartheta$}
    \pgfsetarrowsend{latexslim}
    \pgfpathmoveto{\pgfpoint{.62\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.62\pgf@circ@res@left}{.7\pgf@circ@res@down}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{.45\pgf@circ@res@left}{.7\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.45\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfusepath{draw}
}

%% Generic tunable
\pgfcircdeclarebipolescaled{resistors}
{
    \savedanchor{\wiper}{
            \pgf@circ@scaled@Rlen=\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen
            \pgf@ya=\ctikzvalof{bipoles/generic potentiometer/height}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@ya
            \pgf@xa=\ctikzvalof{bipoles/generic potentiometer/width}\pgf@circ@scaled@Rlen
            \pgfmathsetlength{\pgf@x}{(\ctikzvalof{bipoles/generic potentiometer/wiper pos}-0.5)*\pgf@xa}
        }
    \anchor{wiper}{\wiper}
    \anchor{W}{\wiper}
}
{\ctikzvalof{bipoles/generic potentiometer/height 2}}
{genericpotentiometer}
{\ctikzvalof{bipoles/generic potentiometer/height}}
{\ctikzvalof{bipoles/generic potentiometer/width}}
{

    \pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 14

    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope
    \pgfscope
        %\pgfsetlinewidth{\pgfstartlinewidth}
        \pgfsetarrowsend{latexslim}
        \pgfextractx{\pgf@circ@res@other}{\wiper}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Zig zag resistores
\def\pgf@circ@zigzag#1{%
    \divide \pgf@circ@res@step by \numexpr4*\zigs\relax

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \pgf@circ@count@a=\zigs\relax
    % first half zig
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-#1\pgf@circ@res@down}}
    \pgfmathloop%
    \advance\pgf@circ@count@a by -1\relax% Loop zigs -1 times
    \ifnum\pgf@circ@count@a>0
        \advance\pgf@circ@res@other by 2\pgf@circ@res@step
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{#1\pgf@circ@res@down}}
        \advance\pgf@circ@res@other by 2\pgf@circ@res@step
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-#1\pgf@circ@res@down}}
    \repeatpgfmathloop%
    % last zig and a half
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{#1\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
    \pgfsetbeveljoin
    \pgfusepath{draw}
}

%% Resistor
\pgfcircdeclarebipolescaled{resistors}
{
\savedmacro{\zigs}{\edef\zigs{\ctikzvalof{resistors/zigs}}}
}
{\ctikzvalof{bipoles/resistor/height}}
{resistor}
{\ctikzvalof{bipoles/resistor/height}}
{\ctikzvalof{bipoles/resistor/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments
    \pgfmathsetlength{\pgf@circ@res@step}{\ctikzvalof{bipoles/resistor/width}*\scaledRlen+\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}
    \pgf@circ@zigzag{1}
}


%% Variable resistor
\pgfcircdeclarebipolescaled{resistors}
{
\savedmacro{\zigs}{\edef\zigs{\ctikzvalof{resistors/zigs}}}
}
{\ctikzvalof{bipoles/vresistor/height}}
{vresistor}
{\ctikzvalof{bipoles/vresistor/height}}
{\ctikzvalof{bipoles/vresistor/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments
    \pgfmathsetlength{\pgf@circ@res@step}{\ctikzvalof{bipoles/vresistor/width}*\scaledRlen+\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}
    \pgf@circ@zigzag{.5}

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@other}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-.4\pgf@circ@res@other}{\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Potentiometer
\pgfcircdeclarebipolescaled{resistors}
{
    \savedanchor{\wiper}{
            \pgf@circ@scaled@Rlen=\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen
            \pgf@ya=\ctikzvalof{bipoles/potentiometer/height}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@ya
            \pgf@xa=\ctikzvalof{bipoles/potentiometer/width}\pgf@circ@scaled@Rlen
            \pgfmathsetlength{\pgf@x}{(\ctikzvalof{bipoles/potentiometer/wiper pos}-0.5)*\pgf@xa}
        }
    \anchor{wiper}{\wiper}
    \anchor{W}{\wiper}
    \savedmacro{\zigs}{\edef\zigs{\ctikzvalof{resistors/zigs}}}
}
{\ctikzvalof{bipoles/potentiometer/height 2}}
{potentiometer}
{\ctikzvalof{bipoles/potentiometer/height}}
{\ctikzvalof{bipoles/potentiometer/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments
    \pgfmathsetlength{\pgf@circ@res@step}{\ctikzvalof{bipoles/potentiometer/width}*\scaledRlen+\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}
    \pgf@circ@zigzag{1}

    \pgfscope
        %\pgfsetlinewidth{\pgfstartlinewidth}
        \pgfsetarrowsend{latexslim}
        \pgfextractx{\pgf@circ@res@other}{\wiper}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Resistive sensor
\pgfcircdeclarebipolescaled{resistors}
{% anchor for labelling the type of dependency
    \anchor{label}{\southwest\pgf@x=0.4\pgf@x}%
    \savedmacro{\zigs}{\edef\zigs{\ctikzvalof{resistors/zigs}}}
}
{\ctikzvalof{bipoles/resistivesens/height}}
{resistivesens}
{\ctikzvalof{bipoles/resistivesens/height}}
{\ctikzvalof{bipoles/resistivesens/width}}
{%
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments
    \pgfmathsetlength{\pgf@circ@res@step}{\ctikzvalof{bipoles/resistivesens/width}*\scaledRlen+\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}
    \pgf@circ@zigzag{.5}

    \pgfscope
        \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@other}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-.4\pgf@circ@res@other}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-.9\pgf@circ@res@other}{\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%%%%%%%%%%%%%%
%% Capacitors
%%%%%%%%%%%%%

%% Plain Capacitor
\pgfcircdeclarebipolescaled{capacitors}
{}
{\ctikzvalof{bipoles/capacitor/height}}
{capacitor}
{\ctikzvalof{bipoles/capacitor/height}}
{\ctikzvalof{bipoles/capacitor/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}

}

%% Capacitive sensor
\pgfcircdeclarebipolescaled{capacitors}
{
    \anchor{label}{\southwest\pgf@x=2.6\pgf@x\pgf@y=1.2\pgf@y}%
}
{\ctikzvalof{bipoles/capacitor/height}}
{capacitivesens}
{\ctikzvalof{bipoles/capacitor/height}}
{\ctikzvalof{bipoles/capacitor/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}
    \pgfscope
        \pgfpathmoveto{\pgfpoint{2.6\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-2.6\pgf@circ@res@right}{1.2\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-4.4\pgf@circ@res@right}{1.2\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Polar Capacitor (DEPRECATED)
\pgfcircdeclarebipolescaled{capacitors}
{}
{\ctikzvalof{bipoles/pcapacitor/height}}
{polarcapacitor}
{\ctikzvalof{bipoles/pcapacitor/height}}
{\ctikzvalof{bipoles/pcapacitor/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfscope
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left+ \ctikzvalof{bipoles/pcapacitor/bend width}\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgftransformrotate{-90}
        \pgfpathsine{\pgfpoint{\pgf@circ@res@up}{-\ctikzvalof{bipoles/pcapacitor/bend width}\pgf@circ@res@left}}
        \pgfpathcosine{\pgfpoint{\pgf@circ@res@up}{\ctikzvalof{bipoles/pcapacitor/bend width}\pgf@circ@res@left}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}
}


%% Curved capacitor
% see https://tex.stackexchange.com/questions/509594/polar-capacitor-orientation-in-circuitikz-seems-wrong
% for a rationale
%
\pgfcircdeclarebipolescaled{capacitors}
{}
{\ctikzvalof{bipoles/ccapacitor/height}}
{ccapacitor}
{\ctikzvalof{bipoles/ccapacitor/height}}
{\ctikzvalof{bipoles/ccapacitor/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfscope
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right+ \ctikzvalof{bipoles/ccapacitor/bend width}\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgftransformrotate{-90}
        \pgfpathsine{\pgfpoint{\pgf@circ@res@up}{-\ctikzvalof{bipoles/ccapacitor/bend width}\pgf@circ@res@right}}
        \pgfpathcosine{\pgfpoint{\pgf@circ@res@up}{\ctikzvalof{bipoles/ccapacitor/bend width}\pgf@circ@res@right}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfusepath{draw}
}




%% Electrolytic Capacitor
\pgfcircdeclarebipolescaled{capacitors}
{}
{\ctikzvalof{bipoles/ecapacitor/height}}
{ecapacitor}
{\ctikzvalof{bipoles/ecapacitor/height}}
{\ctikzvalof{bipoles/ecapacitor/width}}
{
    \pgfsetrectcap
    % % % Draw plus pole
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgf@circ@draworfill
    % % Draw minus pole
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfsetfillcolor{\ctikzvalof{color}}
    \pgfusepath{draw,fill}
    \pgfsetfillcolor{\ctikzvalof{color}}
    % % plus pole annotation
    \pgftext[right,at=\pgfpoint{1.2\pgf@circ@res@left}{.6\pgf@circ@res@up}]
    {\ctikzvalof{bipoles/ecapacitor/font} $+$}
}

%% Variable Capacitor
\pgfcircdeclarebipolescaled{capacitors}
{}
{\ctikzvalof{bipoles/vcapacitor/height}}
{vcapacitor}
{\ctikzvalof{bipoles/vcapacitor/height}}
{\ctikzvalof{bipoles/vcapacitor/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/vcapacitor/capacitor width} \pgf@circ@res@right

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}
    \pgfusepath{draw}

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{0pt}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfusepath{draw}
}


%% Piezoelectric Element

\pgfcircdeclarebipolescaled{capacitors}
{}
{\ctikzvalof{bipoles/piezoelectric/height}}
{piezoelectric}
{\ctikzvalof{bipoles/piezoelectric/height}}
{\ctikzvalof{bipoles/piezoelectric/width}}
{
    % \pgf@circ@res@step = \ctikzvalof{bipoles/piezoelectric/width}\pgf@circ@Rlen
    % \divide \pgf@circ@res@step by 5

    %% Outer markings
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}

    %% Inner Box
    \pgf@circ@res@step = \pgf@circ@res@right \divide \pgf@circ@res@step by 10
    \pgfscope
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfpathrectanglecorners
            {\pgfpoint{\pgf@circ@res@left+4*\pgf@circ@res@step}{\pgf@circ@res@up-\pgf@circ@res@step}}
            {\pgfpoint{\pgf@circ@res@right-4*\pgf@circ@res@step}{\pgf@circ@res@down+\pgf@circ@res@step}}
        \pgf@circ@draworfill
    \endpgfscope
}

%%%%%%%%%%%%%%%
%% Inductors
%%%%%%%%%%%%%%%

%% cute inductor
\pgfcircdeclarebipolescaled{inductors}
{
    \savedanchor{\midtap}{%
        \pgf@x=0pt\relax
        \pgfmathsetlength{\pgf@y}{%
            (mod(\ctikzvalof{bipoles/cuteinductor/coils},2) ?%
            \ctikzvalof{bipoles/cuteinductor/height} :% even
            -\ctikzvalof{bipoles/cuteinductor/lower coil height}) %odd
            *\pgf@circ@scaled@Rlen/2
        }
    }
    \anchor{midtap}{\midtap}
}
{\ctikzvalof{bipoles/cuteinductor/lower coil height}}
{cuteinductor}
{\ctikzvalof{bipoles/cuteinductor/height}}
{\ctikzvalof{bipoles/cuteinductor/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments

    \pgfmathsetlength{\pgf@circ@res@other}%width of small coil
    {0.5*\ctikzvalof{bipoles/cuteinductor/coil aspect}*\ctikzvalof{bipoles/cuteinductor/width}*\scaledRlen/(\ctikzvalof{bipoles/cuteinductor/coils}-1)}


    \pgfmathsetlength{\pgf@circ@res@step}
    {(\ctikzvalof{bipoles/cuteinductor/width}*\scaledRlen+\pgfhorizontaltransformationadjustment\pgflinewidth+(\ctikzvalof{bipoles/cuteinductor/coils}-1)*2*\pgf@circ@res@other)/\ctikzvalof{bipoles/cuteinductor/coils}/2}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {2,...,\ctikzvalof{bipoles/cuteinductor/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
        \pgfpatharc{0}{-180}{\pgf@circ@res@other and -\pgf@circ@res@down}
    }
    \pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}
}

%% cute inductive sensor
\pgfcircdeclarebipolescaled{inductors}
{% anchor for labelling the type of dependency
    \anchor{label}{\southwest\pgf@x=0.8\pgf@x\pgf@y=2.6\pgf@y}%
    \savedanchor{\midtap}{%
        \pgf@x=0pt\relax
        \pgfmathsetlength{\pgf@y}{%
            (mod(\ctikzvalof{bipoles/cuteinductor/coils},2) ?%
            \ctikzvalof{bipoles/cuteinductor/height} :% even
            -\ctikzvalof{bipoles/cuteinductor/lower coil height}) %odd
            *\pgf@circ@scaled@Rlen/2
        }
    }
    \anchor{midtap}{\midtap}
}
{\ctikzvalof{bipoles/cuteinductor/lower coil height}}
{scuteinductor}
{\ctikzvalof{bipoles/cuteinductor/height}}
{\ctikzvalof{bipoles/cuteinductor/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments

    \pgfmathsetlength{\pgf@circ@res@other}%width of small coil
    {0.5*\ctikzvalof{bipoles/cuteinductor/coil aspect}*\ctikzvalof{bipoles/cuteinductor/width}*\scaledRlen/(\ctikzvalof{bipoles/cuteinductor/coils}-1)}


    \pgfmathsetlength{\pgf@circ@res@step}
    {(\ctikzvalof{bipoles/cuteinductor/width}*\scaledRlen+\pgfhorizontaltransformationadjustment\pgflinewidth+(\ctikzvalof{bipoles/cuteinductor/coils}-1)*2*\pgf@circ@res@other)/\ctikzvalof{bipoles/cuteinductor/coils}/2}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {2,...,\ctikzvalof{bipoles/cuteinductor/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
        \pgfpatharc{0}{-180}{\pgf@circ@res@other and -\pgf@circ@res@down}
    }
    \pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}
    \pgfscope
        \pgfpathmoveto{\pgfpoint{.8\pgf@circ@res@right}{2\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-.8\pgf@circ@res@right}{2.6\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-1.6\pgf@circ@res@right}{2.6\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% cute choke
\pgfcircdeclarebipolescaled{inductors}
{
    \savedanchor{\midtap}{%
        \pgf@x=0pt\relax
        \pgfmathsetlength{\pgf@y}{%
            (mod(\ctikzvalof{bipoles/cuteinductor/coils},2) ?%
            \ctikzvalof{bipoles/cuteinductor/height} :% even
            -\ctikzvalof{bipoles/cuteinductor/lower coil height}) %odd
            *\pgf@circ@scaled@Rlen/2
        }
    }
    \anchor{midtap}{\midtap}
}
{\ctikzvalof{bipoles/cutechoke/lower coil height}}
{cutechoke}
{\ctikzvalof{bipoles/cutechoke/height}}
{\ctikzvalof{bipoles/cutechoke/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments

    \pgfmathsetlength{\pgf@circ@res@other}%width of small coil
    {0.5*\ctikzvalof{bipoles/cutechoke/coil aspect}*\ctikzvalof{bipoles/cutechoke/width}*\scaledRlen/(\ctikzvalof{bipoles/cutechoke/coils}-1)}


    \pgfmathsetlength{\pgf@circ@res@step}
    {(\ctikzvalof{bipoles/cutechoke/width}*\scaledRlen+\pgfhorizontaltransformationadjustment\pgflinewidth+(\ctikzvalof{bipoles/cutechoke/coils}-1)*2*\pgf@circ@res@other)/\ctikzvalof{bipoles/cutechoke/coils}/2}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {2,...,\ctikzvalof{bipoles/cutechoke/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
        \pgfpatharc{0}{-180}{\pgf@circ@res@other and -\pgf@circ@res@down}
    }
    \pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth+\ctikzvalof{bipoles/cutechoke/cdist}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth+\ctikzvalof{bipoles/cutechoke/cdist}\pgf@circ@res@up}}
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfsetlinewidth{\ctikzvalof{bipoles/cutechoke/cthick}\pgflinewidth}
    \pgfusepath{stroke}

    \ifpgf@circuit@bipole@twolineschoke
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth+\ctikzvalof{bipoles/cutechoke/cdist}\pgf@circ@res@up+\ctikzvalof{bipoles/cutechoke/cstep}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth+\ctikzvalof{bipoles/cutechoke/cdist}\pgf@circ@res@up+\ctikzvalof{bipoles/cutechoke/cstep}\pgf@circ@res@up}}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfsetlinewidth{\ctikzvalof{bipoles/cutechoke/cthick}\pgflinewidth}
        \pgfusepath{stroke}
    \fi
}

%% variable cute inductor
\pgfcircdeclarebipolescaled{inductors}
{
    \savedanchor{\midtap}{%
        \pgf@x=0pt\relax
        \pgfmathsetlength{\pgf@y}{%
            (mod(\ctikzvalof{bipoles/cuteinductor/coils},2) ?%
            \ctikzvalof{bipoles/cuteinductor/height} :% even
            -\ctikzvalof{bipoles/cuteinductor/lower coil height}) %odd
            *\pgf@circ@scaled@Rlen/2
        }
    }
    \anchor{midtap}{\midtap}
}
{\ctikzvalof{bipoles/vcuteinductor/lower coil height}}
{vcuteinductor}
{\ctikzvalof{bipoles/vcuteinductor/height}}
{\ctikzvalof{bipoles/vcuteinductor/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments

    \pgfmathsetlength{\pgf@circ@res@other}%width of small coil
    {0.5*\ctikzvalof{bipoles/vcuteinductor/coil aspect}*\ctikzvalof{bipoles/vcuteinductor/width}*\scaledRlen/(\ctikzvalof{bipoles/vcuteinductor/coils}-1)}


    \pgfmathsetlength{\pgf@circ@res@step}
    {(\ctikzvalof{bipoles/vcuteinductor/width}*\scaledRlen+\pgfhorizontaltransformationadjustment\pgflinewidth+(\ctikzvalof{bipoles/vcuteinductor/coils}-1)*2*\pgf@circ@res@other)/\ctikzvalof{bipoles/vcuteinductor/coils}/2}

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {2,...,\ctikzvalof{bipoles/vcuteinductor/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and .5\pgf@circ@res@up}
        \pgfpatharc{0}{-180}{\pgf@circ@res@other and -.5\pgf@circ@res@down}
    }
    \pgfpatharc{180}{0}{\pgf@circ@res@step and .5\pgf@circ@res@up}
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}
}

%% american inductor
\pgfcircdeclarebipolescaled{inductors}
{
    \savedanchor{\midtap}{%
        \pgf@x=0pt\relax
        \pgfmathsetlength{\pgf@y}{%
            (mod(\ctikzvalof{bipoles/americaninductor/coils},2) ?%
            2*\ctikzvalof{bipoles/americaninductor/coil height} :% even
            0) %odd
            *\pgf@circ@scaled@Rlen/2
        }
    }
    \anchor{midtap}{\midtap}
}
{\ctikzvalof{bipoles/americaninductor/height 2}}
{americaninductor}
{\ctikzvalof{bipoles/americaninductor/height}}
{\ctikzvalof{bipoles/americaninductor/width}}
{
    \pgf@circ@res@step=\ctikzvalof{bipoles/americaninductor/width}\pgf@circ@scaled@Rlen
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments
    \advance \pgf@circ@res@step by \pgfhorizontaltransformationadjustment\pgflinewidth
    \divide \pgf@circ@res@step by \ctikzvalof{bipoles/americaninductor/coils}
    \divide \pgf@circ@res@step by 2
    \pgf@circ@res@other = \ctikzvalof{bipoles/americaninductor/coil height}\pgf@circ@scaled@Rlen

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {1,...,\ctikzvalof{bipoles/americaninductor/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and  \pgf@circ@res@other}
    }
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}
}


%% american inductive sensor
\pgfcircdeclarebipolescaled{inductors}
{% anchor for labelling the type of dependency
    \anchor{label}{\southwest\pgf@x=0.8\pgf@x\pgf@y=2.6\pgf@y}%
    \savedanchor{\midtap}{%
        \pgf@x=0pt\relax
        \pgfmathsetlength{\pgf@y}{%
            (mod(\ctikzvalof{bipoles/americaninductor/coils},2) ?%
            2*\ctikzvalof{bipoles/americaninductor/coil height} :% even
            0) %odd
            *\pgf@circ@scaled@Rlen/2
        }
    }
    \anchor{midtap}{\midtap}
}
{\ctikzvalof{bipoles/americaninductor/height 2}}
{samericaninductor}
{\ctikzvalof{bipoles/americaninductor/height}}
{\ctikzvalof{bipoles/americaninductor/width}}
{
    \pgf@circ@res@step=\ctikzvalof{bipoles/americaninductor/width}\pgf@circ@scaled@Rlen
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments
    \advance \pgf@circ@res@step by \pgfhorizontaltransformationadjustment\pgflinewidth
    \divide \pgf@circ@res@step by \ctikzvalof{bipoles/americaninductor/coils}
    \divide \pgf@circ@res@step by 2
    \pgf@circ@res@other = \ctikzvalof{bipoles/americaninductor/coil height}\pgf@circ@scaled@Rlen

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {1,...,\ctikzvalof{bipoles/americaninductor/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and  \pgf@circ@res@other}
    }
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}
    \pgfscope
        \pgfpathmoveto{\pgfpoint{.8\pgf@circ@res@right}{2\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-.8\pgf@circ@res@right}{2.6\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-1.6\pgf@circ@res@right}{2.6\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% variable american inductor
\pgfcircdeclarebipolescaled{inductors}
{
    \savedanchor{\midtap}{%
        \pgf@x=0pt\relax
        \pgfmathsetlength{\pgf@y}{%
            (mod(\ctikzvalof{bipoles/vamericaninductor/coils},2) ?%
            2*\ctikzvalof{bipoles/vamericaninductor/coil height} :% even
            0) %odd
            *\pgf@circ@scaled@Rlen/2
        }
    }
    \anchor{midtap}{\midtap}
}
{\ctikzvalof{bipoles/vamericaninductor/height 2}}
{vamericaninductor}
{\ctikzvalof{bipoles/vamericaninductor/height}}
{\ctikzvalof{bipoles/vamericaninductor/width}}
{
    \pgf@circ@res@step=\ctikzvalof{bipoles/vamericaninductor/width}\pgf@circ@scaled@Rlen
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments
    \advance \pgf@circ@res@step by \pgfhorizontaltransformationadjustment\pgflinewidth
    \divide \pgf@circ@res@step by \ctikzvalof{bipoles/vamericaninductor/coils}
    \divide \pgf@circ@res@step by 2
    \pgf@circ@res@other = \ctikzvalof{bipoles/vamericaninductor/coil height}\pgf@circ@scaled@Rlen

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {1,...,\ctikzvalof{bipoles/vamericaninductor/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and  \pgf@circ@res@other}
    }
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-.4\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Generic bipole, filled - used as inductor by some
\pgfcircdeclarebipolescaled{inductors}
{
    \anchor{midtap}{\northeast\pgf@x=0pt\relax}
}
{\ctikzvalof{bipoles/fullgeneric/height}}
{fullgeneric}
{\ctikzvalof{bipoles/fullgeneric/height}}
{\ctikzvalof{bipoles/fullgeneric/width}}
{
    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfusepath{draw,fill}
}

%% Generic sensor, filled - used as inductive sensor by some
\pgfcircdeclarebipolescaled{inductors}
{% anchor for labelling the type of dependency
    \anchor{label}{\southwest\pgf@x=0.4\pgf@x\pgf@y=2\pgf@y}%
    \anchor{midtap}{\northeast\pgf@x=0pt\relax}
}
{\ctikzvalof{bipoles/fullgeneric/height}}
{sfullgeneric}
{\ctikzvalof{bipoles/fullgeneric/height}}
{\ctikzvalof{bipoles/fullgeneric/width}}
{

    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfusepath{draw,fill}
    %\pgfscope
    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{-2\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{2\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{2\pgf@circ@res@down}}
    \pgfusepath{draw}
    %\endpgfscope
}

%% Generic full tunable
\pgfcircdeclarebipolescaled{inductors}
{
    \anchor{midtap}{\northeast\pgf@x=0pt\relax}
}
{\ctikzvalof{bipoles/tfullgeneric/height}}
{tfullgeneric}
{\ctikzvalof{bipoles/tfullgeneric/height}}
{\ctikzvalof{bipoles/tfullgeneric/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 14

    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{.4\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{.4\pgf@circ@res@down}}
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfusepath{draw,fill}

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{.5\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-.5\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%%%%%%%%%%%
%% Battery
%%%%%%%%%%%

%% Battery
\pgfcircdeclarebipolescaled{batteries}
{}
{\ctikzvalof{bipoles/battery/height}}
{battery}
{\ctikzvalof{bipoles/battery/height}}
{\ctikzvalof{bipoles/battery/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/battery/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 6

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \ifpgf@circ@fixbatteries
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{.5\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \else
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{.5\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@down}}
    \fi
    \pgfusepath{draw}
}


%% Battery 1 % poles with equl thickness

\pgfcircdeclarebipolescaled{batteries}
{}
{\ctikzvalof{bipoles/battery1/height}}
{battery1}
{\ctikzvalof{bipoles/battery1/height}}
{\ctikzvalof{bipoles/battery1/width}}
{
    \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
    \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfusepath{draw}

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \ifpgf@circ@fixbatteries
        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@right}{\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@left}{.5\pgf@circ@res@down}}
    \else
        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@right}{.5\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@left}{\pgf@circ@res@down}}
    \fi
    \pgfusepath{draw}
}

%% Battery 2 % negative pole thicker

\pgfcircdeclarebipolescaled{batteries}
{}
{\ctikzvalof{bipoles/battery2/height}}
{battery2}
{\ctikzvalof{bipoles/battery2/height}}
{\ctikzvalof{bipoles/battery2/width}}
{
    \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
    \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfusepath{draw}

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \ifpgf@circ@fixbatteries
        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgfusepath{draw}
        \pgfsetlinewidth{3\pgflinewidth}
        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@left}{.5\pgf@circ@res@down}}
    \else
        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfusepath{draw}
        \pgfsetlinewidth{3\pgflinewidth}
        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@right}{.5\pgf@circ@res@down}}
    \fi
    \pgfusepath{draw}
}

%%%%%%%%%%%
%% Round and diamond sources
%%%%%%%%%%%

%% Independent voltage source
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/vsource/height}}
{vsource}
{\ctikzvalof{bipoles/vsource/height}}
{\ctikzvalof{bipoles/vsource/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
}

%% Independent voltage source - American style
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/vsourceam/height}}
{vsourceAM}
{\ctikzvalof{bipoles/vsourceam/height}}
{\ctikzvalof{bipoles/vsourceam/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfsetcolor{\ctikzvalof{color}}
    \ifpgf@circ@oldvoltagedirection
        \pgftext[bottom,rotate=90,y=\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@down]{$+$}
        \pgftext[top,rotate=90,y=\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@up]{$-$}
    \else
        \pgftext[bottom,rotate=90,y=\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@down]{$-$}
        \pgftext[top,rotate=90,y=\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@up]{$+$}
    \fi
}

%% Independent sinusoidal voltage source
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/vsourcesin/height}}
{vsourcesin}
{\ctikzvalof{bipoles/vsourcesin/height}}
{\ctikzvalof{bipoles/vsourcesin/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill

    \pgf@circ@res@up = .5\pgf@circ@res@up
    \pgfscope
        \pgftransformrotate{90}
        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@up}{0cm}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

% Square Voltage source -  contributed by Alistair Kwan
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/vsourcesquare/height}}
{vsourcesquare}
{\ctikzvalof{bipoles/vsourcesquare/height}}
{\ctikzvalof{bipoles/vsourcesquare/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgf@circ@res@up = .5\pgf@circ@res@up
    \pgfscope
        \pgftransformrotate{90}
        \pgfpathmoveto{\pgfpoint{-1\pgf@circ@res@up}{0cm}}
        \pgfpathlineto{\pgfpoint{-1\pgf@circ@res@up}{1\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0\pgf@circ@res@up}{1\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0\pgf@circ@res@up}{-1\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{1\pgf@circ@res@up}{-1\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{1\pgf@circ@res@up}{0\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

% Triangle Voltage source - contributed by Ralf Farkas
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/vsourcetri/height}}
{vsourcetri}
{\ctikzvalof{bipoles/vsourcetri/height}}
{\ctikzvalof{bipoles/vsourcetri/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill

    \pgf@circ@res@up = .5\pgf@circ@res@up
    \pgfscope
        \pgftransformrotate{90}
        \pgfpathmoveto{\pgfpoint{-1\pgf@circ@res@up}{0cm}}
        \pgfpathlineto{\pgfpoint{-0.5\pgf@circ@res@up}{0.75\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@up}{-0.75\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{1\pgf@circ@res@up}{0\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}


%% PV Source
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/pvsource/height}}
{pvsource}
{\ctikzvalof{bipoles/pvsource/height}}
{\ctikzvalof{bipoles/pvsource/width}}
{
    \pgfpointorigin
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
    \pgf@circ@draworfill

    \pgfpathmoveto{\pgfpoint{.15\pgf@circ@res@right}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
    \pgfpathmoveto{\pgfpoint{.15\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfusepath{draw}

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{.15\pgf@circ@res@left}{.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.15\pgf@circ@res@left}{.4\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{.15\pgf@circ@res@right}{.6\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.15\pgf@circ@res@right}{.6\pgf@circ@res@down}}
    \pgfusepath{draw}

    %Arrow Part
    \pgfscope
        \pgfsetarrowsend{latex}
        \pgfpathmoveto{\pgfpointadd{\pgfpoint{.3\pgf@circ@res@left}{0}}{\pgfpointpolar{-45}{2.2\pgf@circ@res@up}}}
        \pgfpathlineto{\pgfpointadd{\pgfpoint{.3\pgf@circ@res@left}{0}}{\pgfpointpolar{-45}{1.3\pgf@circ@res@up}}}
        \pgfusepath{draw}
        \pgfpathmoveto{\pgfpointadd{\pgfpoint{0}{0.3\pgf@circ@res@up}}{\pgfpointpolar{-45}{2.2\pgf@circ@res@up}}}
        \pgfpathlineto{\pgfpointadd{\pgfpoint{0}{0.3\pgf@circ@res@up}}{\pgfpointpolar{-45}{1.3\pgf@circ@res@up}}}
        \pgfusepath{draw}
    \endpgfscope

}

%% Empty Source
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/esource/height}}
{esource}
{\ctikzvalof{bipoles/esource/height}}
{\ctikzvalof{bipoles/esource/width}}
{
    \pgfpointorigin
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
}

%% DC Current Source with open shape
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/dcisource/height}}
{dcisource}
{\ctikzvalof{bipoles/dcisource/height}}
{\ctikzvalof{bipoles/dcisource/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@maybefill
    \edef\@@angle{\ctikzvalof{bipoles/dcisource/angle}}
    \pgfpathmoveto{\pgfpointpolar{\@@angle}{\pgf@circ@res@up}}
    \pgfpatharc{\@@angle}{-\@@angle}{\pgf@circ@res@up}
    \pgfpathmoveto{\pgfpointpolar{180-\@@angle}{\pgf@circ@res@up}}
    \pgfpatharc{180-\@@angle}{180+\@@angle}{\pgf@circ@res@up}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{.7\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
    \pgfscope
        \pgftransformshift{\pgfpoint{.5\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
    \endpgfscope
}

%% DC-Voltage source
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/dcvsource/height}}
{dcvsource}
{\ctikzvalof{bipoles/dcvsource/height}}
{\ctikzvalof{bipoles/dcvsource/width}}
{
    \pgfpointorigin
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@up}{.5\pgf@circ@res@left}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@up}{.5\pgf@circ@res@right}}
    \pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@down}{.5\pgf@circ@res@left}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@down}{.5\pgf@circ@res@right}}
    \pgfusepath{draw}
}

%% Independent current source
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/isource/height}}
{isource}
{\ctikzvalof{bipoles/isource/height}}
{\ctikzvalof{bipoles/isource/width}}
{
    \pgfpointorigin
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}
    \pgf@circ@draworfill
}

%% Independent double oo source
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/oosource/height}}
{oosource}
{\ctikzvalof{bipoles/oosource/height}}
{\ctikzvalof{bipoles/oosource/width}}
{
    \pgfpointorigin
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathcircle{\pgfpoint{\ctikzvalof{bipoles/oosource/circleoffset}\pgf@circ@res@left}{0}}
        {\ctikzvalof{bipoles/oosource/circlesize}\pgf@circ@res@left}
    \pgf@circ@maybefill
    \pgfpathcircle{\pgfpoint{\ctikzvalof{bipoles/oosource/circleoffset}\pgf@circ@res@right}{0}}
        {\ctikzvalof{bipoles/oosource/circlesize}\pgf@circ@res@right}
    \pgf@circ@draworfill
    \pgfpathcircle{\pgfpoint{\ctikzvalof{bipoles/oosource/circleoffset}\pgf@circ@res@left}{0}}
        {\ctikzvalof{bipoles/oosource/circlesize}\pgf@circ@res@left}
    \pgfusepath{draw}
}

%% Independent current source - American
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/isourceam/height}}
{isourceAM}
{\ctikzvalof{bipoles/isourceam/height}}
{\ctikzvalof{bipoles/isourceam/width}}
{
    \pgfpointorigin
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill

    \pgfpathmoveto{\pgfpoint{.7\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
    \pgfscope
        \pgftransformshift{\pgfpoint{.5\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
    \endpgfscope
}

%% Independent sinusoidal current source
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/isource/height}}
{isourcesin}
{\ctikzvalof{bipoles/isource/height}}
{\ctikzvalof{bipoles/isource/width}}
{
    \pgfpointorigin
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill

    \pgf@circ@res@up = .5\pgf@circ@res@up
    \pgfscope
        \pgftransformrotate{90}
        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@up}{0cm}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Empty controlled source
\pgfcircdeclarebipolescaled{csources}
{}
{\ctikzvalof{bipoles/ecsource/height}}
{ecsource}
{\ctikzvalof{bipoles/ecsource/height}}
{\ctikzvalof{bipoles/ecsource/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathclose
    \pgf@circ@draworfill
}

%% Controlled voltage source
\pgfcircdeclarebipolescaled{csources}
{}
{\ctikzvalof{bipoles/cvsource/height}}
{cvsource}
{\ctikzvalof{bipoles/cvsource/height}}
{\ctikzvalof{bipoles/cvsource/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathclose
    \pgf@circ@draworfill

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
}

%% Controlled voltage source - American
\pgfcircdeclarebipolescaled{csources}
{}
{\ctikzvalof{bipoles/cvsourceam/height}}
{cvsourceAM}
{\ctikzvalof{bipoles/cvsourceam/height}}
{\ctikzvalof{bipoles/cvsourceam/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathclose
    \pgf@circ@draworfill

    \pgfsetcolor{\ctikzvalof{color}}
    \ifpgf@circ@oldvoltagedirection
        \pgftext[bottom,rotate=90,y=\ctikzvalof{bipoles/cvsourceam/margin}\pgf@circ@res@left]{$+$}
        \pgftext[top,rotate=90,y=\ctikzvalof{bipoles/cvsourceam/margin}\pgf@circ@res@right]{$-$}
    \else
        \pgftext[bottom,rotate=90,y=\ctikzvalof{bipoles/cvsourceam/margin}\pgf@circ@res@left]{$-$}
        \pgftext[top,rotate=90,y=\ctikzvalof{bipoles/cvsourceam/margin}\pgf@circ@res@right]{$+$}
    \fi
}

%% Controlled sinusoidal voltage source
\pgfcircdeclarebipolescaled{csources}
{}
{\ctikzvalof{bipoles/cvsourcesin/height}}
{cvsourcesin}
{\ctikzvalof{bipoles/cvsourcesin/height}}
{\ctikzvalof{bipoles/cvsourcesin/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfscope
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
        \pgfpathclose
        \pgf@circ@draworfill
    \endpgfscope

    \pgf@circ@res@up = .5\pgf@circ@res@up
    \pgfscope
        \pgftransformrotate{90}
        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@up}{0cm}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Controlled sinusoidal current source
\pgfcircdeclarebipolescaled{csources}
{}
{\ctikzvalof{bipoles/cvsourcesin/height}}
{cisourcesin}
{\ctikzvalof{bipoles/cvsourcesin/height}}
{\ctikzvalof{bipoles/cvsourcesin/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfscope
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
        \pgfpathclose
        \pgf@circ@draworfill
    \endpgfscope

    \pgf@circ@res@up = .5\pgf@circ@res@up
    \pgfscope
        \pgftransformrotate{90}
        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@up}{0cm}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Controlled current source
\pgfcircdeclarebipolescaled{csources}
{}
{\ctikzvalof{bipoles/cisource/height}}
{cisource}
{\ctikzvalof{bipoles/cisource/height}}
{\ctikzvalof{bipoles/cisource/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathclose
    \pgf@circ@draworfill

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfusepath{draw}
}

%% Controlled current source - American
\pgfcircdeclarebipolescaled{csources}
{}
{\ctikzvalof{bipoles/cisourceam/height}}
{cisourceAM}
{\ctikzvalof{bipoles/cisourceam/height}}
{\ctikzvalof{bipoles/cisourceam/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathclose
    \pgf@circ@draworfill
    \pgfpathmoveto{\pgfpoint{.7\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
    \pgfscope
        \pgftransformshift{\pgfpoint{.5\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
    \endpgfscope
}

%% Cute Independent voltage source
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/vsource/height}}
{vsourceC}
{\ctikzvalof{bipoles/vsource/height}}
{\ctikzvalof{bipoles/vsource/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfmathsetmacro{\@@thicker}{3*\ctikzvalof{bipoles/thickness}}
    \pgfsetlinewidth{\@@thicker\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfsetroundcap\pgfusepath{draw}
}

%% Cute Independent current source
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/isource/height}}
{isourceC}
{\ctikzvalof{bipoles/isource/height}}
{\ctikzvalof{bipoles/isource/width}}
{
    \pgfpointorigin
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfmathsetmacro{\@@thicker}{3*\ctikzvalof{bipoles/thickness}}
    \pgfsetlinewidth{\@@thicker\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{.6\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{.6\pgf@circ@res@down}}
    \pgfsetroundcap\pgfusepath{draw}
}

%% Cute Controlled voltage source
\pgfcircdeclarebipolescaled{csources}
{}
{\ctikzvalof{bipoles/cvsource/height}}
{cvsourceC}
{\ctikzvalof{bipoles/cvsource/height}}
{\ctikzvalof{bipoles/cvsource/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@draworfill
    \pgfmathsetmacro{\@@thicker}{3*\ctikzvalof{bipoles/thickness}}
    \pgfsetlinewidth{\@@thicker\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfsetroundcap\pgfusepath{draw}
}

%% Cute Controlled current source
\pgfcircdeclarebipolescaled{csources}
{}
{\ctikzvalof{bipoles/cisource/height}}
{cisourceC}
{\ctikzvalof{bipoles/cisource/height}}
{\ctikzvalof{bipoles/cisource/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@draworfill
    \pgfmathsetmacro{\@@thicker}{3*\ctikzvalof{bipoles/thickness}}
    \pgfsetlinewidth{\@@thicker\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@zero}{.6\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{.6\pgf@circ@res@down}}
    \pgfsetroundcap\pgfusepath{draw}
}

%%  Noise voltage source
\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/vsource/height}}
{vsourceN}
{\ctikzvalof{bipoles/vsource/height}}
{\ctikzvalof{bipoles/vsource/width}}
{
    \pgfscope
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
        %
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step=0.125\pgf@circ@scaled@Rlen\relax
        \edef\pgf@noise@temp{dashed}
        \edef\pgf@noise@fill{\ctikzvalof{bipoles/noise sources/fillcolor}}
        \ifx\pgf@noise@temp\pgf@noise@fill
            % fillable in this case
            \pgf@circ@draworfillandclip
            \pgfmathsetmacro{\@@thinner}{.5*\ctikzvalof{bipoles/thickness}}
            \pgfsetlinewidth{\@@thinner\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by \pgf@circ@res@step\advance\pgf@circ@res@down by \pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by \pgf@circ@res@step\advance\pgf@circ@res@down by \pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by \pgf@circ@res@step\advance\pgf@circ@res@down by \pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            %
            \advance\pgf@circ@res@up by -4\pgf@circ@res@step \advance\pgf@circ@res@down by -4\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by -\pgf@circ@res@step\advance\pgf@circ@res@down by -\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by -\pgf@circ@res@step\advance\pgf@circ@res@down by -\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgfusepath{draw}
        \else
            \pgfsetfillcolor{\pgf@noise@fill}
            \pgfusepath{draw,fill}
        \fi
    \endpgfscope
    \pgfmathsetmacro{\@@thicker}{3*\ctikzvalof{bipoles/thickness}}
    \pgfsetlinewidth{\@@thicker\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfsetroundcap\pgfusepath{draw}
}
%% Noise current source

\pgfcircdeclarebipolescaled{sources}
{}
{\ctikzvalof{bipoles/isource/height}}
{isourceN}
{\ctikzvalof{bipoles/isource/height}}
{\ctikzvalof{bipoles/isource/width}}
{
    \pgfpointorigin
    \pgfscope
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
        %
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step=0.125\pgf@circ@scaled@Rlen\relax
        \edef\pgf@noise@temp{dashed}
        \edef\pgf@noise@fill{\ctikzvalof{bipoles/noise sources/fillcolor}}
        \ifx\pgf@noise@temp\pgf@noise@fill
            % fillable in this case
            \pgf@circ@draworfillandclip
            \pgfmathsetmacro{\@@thinner}{.5*\ctikzvalof{bipoles/thickness}}
            \pgfsetlinewidth{\@@thinner\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by \pgf@circ@res@step\advance\pgf@circ@res@down by \pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by \pgf@circ@res@step\advance\pgf@circ@res@down by \pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by \pgf@circ@res@step\advance\pgf@circ@res@down by \pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            %
            \advance\pgf@circ@res@up by -4\pgf@circ@res@step \advance\pgf@circ@res@down by -4\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by -\pgf@circ@res@step\advance\pgf@circ@res@down by -\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by -\pgf@circ@res@step\advance\pgf@circ@res@down by -\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgfusepath{draw}
        \else
            \pgfsetfillcolor{\pgf@noise@fill}
            \pgfusepath{draw,fill}
        \fi
    \endpgfscope
    \pgfmathsetmacro{\@@thicker}{3*\ctikzvalof{bipoles/thickness}}
    \pgfsetlinewidth{\@@thicker\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{.6\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{.6\pgf@circ@res@down}}
    \pgfsetroundcap\pgfusepath{draw}
}

%%%%%%%%%%%%%%
%% Diodes
%%%%%%%%%%%%%%

%% Black generic diode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{fulldiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Black Zener diode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{fullzdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Black alternative zigzag Zener diode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{fullzzdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-1.8\pgf@circ@res@left}{\pgf@circ@res@down-0.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-0.2\pgf@circ@res@left}{\pgf@circ@res@up-0.5\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Black Schottky diode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{fullsdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{.6\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-1.4\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-1.4\pgf@circ@res@left}{.6\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

}

%% Black tunnel diode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{fulltdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Black light emitting diode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{fulllediode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfsetarrowsend{latexslim}
    \pgfpathmoveto{\pgfpoint{-0.4\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{2\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.2\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@right}{1.8\pgf@circ@res@up}}
    \pgfusepath{draw}

}

%% Black photodiode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{fullpdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfsetarrowsstart{latexslim}
    \pgfpathmoveto{\pgfpoint{-0.4\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{2\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.2\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@right}{1.8\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Black varcap
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/varcap/height}}
{fullvarcap}
{\ctikzvalof{bipoles/varcap/height}}
{\ctikzvalof{bipoles/varcap/width}}
{
    \pgf@circ@res@temp=\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
    \pgfsetlinewidth{\pgf@circ@res@temp}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
    \pgfusepath{draw,fill}
    %
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Code for the diode triangle
\def\pgf@circ@basicdiodeshape{
    % \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathclose
        \pgf@circ@draworfill
        \pgfscope
            % to allow filling, we need to draw explicitly the stroke here.
            \pgfsetlinewidth{\pgfstartlinewidth}
            \ifpgf@circuit@bipole@strokedsymbol
                \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
                \pgfpathlineto{\pgfpoint{0pt}{0pt}}
                \pgfusepath{draw}
            \fi
        \endpgfscope
    % \endpgfscope
}

%% Empty generic diode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{emptydiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfscope
        \pgf@circ@basicdiodeshape
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Empty Zener diode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{emptyzdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfscope
        \pgf@circ@basicdiodeshape
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-0.6\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Empty alternative zigzag Zener diode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{emptyzzdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfscope
        \pgf@circ@basicdiodeshape
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-1.8\pgf@circ@res@left}{\pgf@circ@res@down-0.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-0.2\pgf@circ@res@left}{\pgf@circ@res@up-0.5\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}
%% Empty Schottky diode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{emptysdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfscope
        \pgf@circ@basicdiodeshape
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{.6\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-1.4\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-1.4\pgf@circ@res@left}{.6\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

}

%% Empty tunnel diode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{emptytdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfscope
        \pgf@circ@basicdiodeshape
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Empty light emitting diode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{emptylediode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfscope
        \pgf@circ@basicdiodeshape
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfsetarrowsend{latexslim}
    \pgfpathmoveto{\pgfpoint{-0.4\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{2\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.2\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@right}{1.8\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Empty photodiode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/diode/height}}
{emptypdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfscope
        \pgf@circ@basicdiodeshape
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfsetarrowsstart{latexslim}
    \pgfpathmoveto{\pgfpoint{-0.4\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{2\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.2\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@right}{1.8\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Empty varcap
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/varcap/height}}
{emptyvarcap}
{\ctikzvalof{bipoles/varcap/height}}
{\ctikzvalof{bipoles/varcap/width}}
{
    \pgf@circ@res@temp=\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
    \pgfsetlinewidth{\pgf@circ@res@temp}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    % \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
    \pgfpathclose
    \pgf@circ@draworfill
    \pgfscope
        % to allow filling, we need to draw explicitily the stroke here.
        \pgfsetlinewidth{\pgfstartlinewidth}
        \ifpgf@circuit@bipole@strokedsymbol
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfusepath{draw}
        \fi
    \endpgfscope
    %
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Empty bidirectionaldiode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/bidirectionaldiode/height}}
{emptybidirectionaldiode}
{\ctikzvalof{bipoles/bidirectionaldiode/height}}
{\ctikzvalof{bipoles/bidirectionaldiode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgf@circ@res@other = \ctikzvalof{bipoles/bidirectionaldiode/diode width left}\pgf@circ@res@left
    \pgf@circ@res@step = \ctikzvalof{bipoles/bidirectionaldiode/diode width right}\pgf@circ@res@right

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@step}{0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@other}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgf@circ@draworfill

    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}
}

%% Full bidirectionaldiode
\pgfcircdeclarebipolescaled{diodes}
{}
{\ctikzvalof{bipoles/bidirectionaldiode/height}}
{fullbidirectionaldiode}
{\ctikzvalof{bipoles/bidirectionaldiode/height}}
{\ctikzvalof{bipoles/bidirectionaldiode/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgf@circ@res@other = \ctikzvalof{bipoles/bidirectionaldiode/diode width left}\pgf@circ@res@left
    \pgf@circ@res@step = \ctikzvalof{bipoles/bidirectionaldiode/diode width right}\pgf@circ@res@right

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@step}{0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@other}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgfusepath{draw, fill}

    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}
}

%% Black thyristor
\pgfcircdeclarebipolescaled{diodes}
{
    \anchor{gate}{\northeast}
    \anchor{anode}{\southwest\pgf@y=0cm}
    \anchor{G}{\northeast}
    \anchor{cathode}{\northeast\pgf@y=0cm }
}
{\ctikzvalof{tripoles/thyristor/height 2}}
{fullthyristor}
{\ctikzvalof{tripoles/thyristor/height}}
{\ctikzvalof{tripoles/thyristor/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgf@circ@res@other = \ctikzvalof{tripoles/thyristor/diode width left}\pgf@circ@res@left
    \pgf@circ@res@step = \ctikzvalof{tripoles/thyristor/diode width right}\pgf@circ@res@right

    \pgfscope
        \pgftransformxshift{\pgf@circ@res@other}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}

        \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
        \pgfusepath{draw,fill}

        \pgfsetlinewidth{\pgfstartlinewidth}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
        \pgfpathlineto{\pgfpoint{2*\pgf@circ@res@step-2*\pgf@circ@res@other}{\ctikzvalof{tripoles/thyristor/diode height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{2*\pgf@circ@res@step-2*\pgf@circ@res@other}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@down}}

    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}

}

%% Empty thyristor

\pgfcircdeclarebipolescaled{diodes}
{
    \anchor{gate}{\northeast}
    \anchor{anode}{\southwest\pgf@y=0cm}
    \anchor{G}{\northeast}
    \anchor{cathode}{\northeast\pgf@y=0cm }
}
{\ctikzvalof{tripoles/thyristor/height 2}}
{emptythyristor}
{\ctikzvalof{tripoles/thyristor/height}}
{\ctikzvalof{tripoles/thyristor/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgf@circ@res@other = \ctikzvalof{tripoles/thyristor/diode width left}\pgf@circ@res@left
    \pgf@circ@res@step = \ctikzvalof{tripoles/thyristor/diode width right}\pgf@circ@res@right

    \pgfscope
        \pgftransformxshift{\pgf@circ@res@other}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}

        \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathclose
        \pgf@circ@draworfill
        \pgfscope
            % to allow filling, we need to draw explicitily the stroke here.
            \pgfsetlinewidth{\pgfstartlinewidth}
            \ifpgf@circuit@bipole@strokedsymbol
                \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
                \pgfpathlineto{\pgfpoint{0pt}{0pt}}
                \pgfusepath{draw}
            \fi
        \endpgfscope

        \pgfsetlinewidth{\pgfstartlinewidth}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
        \pgfpathlineto{\pgfpoint{2*\pgf@circ@res@step-2*\pgf@circ@res@other}{\ctikzvalof{tripoles/thyristor/diode height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{2*\pgf@circ@res@step-2*\pgf@circ@res@other}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@down}}

    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}
}

%% Empty triac
\pgfcircdeclarebipolescaled{diodes}
{
    \anchor{gate}{\northeast}
    \anchor{anode}{\southwest\pgf@y=0cm}
    \anchor{G}{\northeast}
    \anchor{cathode}{\northeast\pgf@y=0cm }
}
{\ctikzvalof{tripoles/triac/height}}
{emptytriac}
{\ctikzvalof{tripoles/triac/height}}
{\ctikzvalof{tripoles/triac/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgf@circ@res@other = \ctikzvalof{tripoles/triac/diode width left}\pgf@circ@res@left
    \pgf@circ@res@step = \ctikzvalof{tripoles/triac/diode width right}\pgf@circ@res@right

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@step}{0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@other}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgf@circ@draworfill

    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}} % sqrt(1/2)

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}
}

%% Full triac
\pgfcircdeclarebipolescaled{diodes}
{
    \anchor{gate}{\northeast}
    \anchor{anode}{\southwest\pgf@y=0cm}
    \anchor{G}{\northeast}
    \anchor{cathode}{\northeast\pgf@y=0cm }
}
{\ctikzvalof{tripoles/triac/height}}
{fulltriac}
{\ctikzvalof{tripoles/triac/height}}
{\ctikzvalof{tripoles/triac/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgf@circ@res@other = \ctikzvalof{tripoles/triac/diode width left}\pgf@circ@res@left
    \pgf@circ@res@step = \ctikzvalof{tripoles/triac/diode width right}\pgf@circ@res@right

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@step}{0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@other}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgfusepath{draw,fill}

    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}} % sqrt(1/2)

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}
}

%%%%%%%%%%%%%
%% switches
%%%%%%%%%%%%%

%% (Closing) SPST
\pgfcircdeclarebipolescaled{switches}
{}
{\ctikzvalof{bipoles/spst/depth}}
{cspst}
{\ctikzvalof{bipoles/spst/height}}
{\ctikzvalof{bipoles/spst/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathmoveto{\pgfpointpolar{90}{1.2\pgf@circ@res@right}}
        \pgfpatharc{90}{-20}{1.2\pgf@circ@res@right}
        \pgfsetarrowsend{latexslim}
        \pgfsetbeveljoin
        \pgfusepath{draw}
    \endpgfscope
}

%% Opening SPST
\pgfcircdeclarebipolescaled{switches}
{}
{\ctikzvalof{bipoles/spst/depth}}
{ospst}
{\ctikzvalof{bipoles/spst/height}}
{\ctikzvalof{bipoles/spst/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathmoveto{\pgfpointpolar{-10}{1.2\pgf@circ@res@right}}
        \pgfpatharc{-10}{90}{1.2\pgf@circ@res@right}
        \pgfsetarrowsend{latexslim}
        \pgfsetbeveljoin
        \pgfusepath{draw}
    \endpgfscope
}

%% Normal open Switch
\pgfcircdeclarebipolescaled{switches}
{}
{\ctikzvalof{bipoles/nos/depth}}
{nos}
{\ctikzvalof{bipoles/nos/height}}
{\ctikzvalof{bipoles/nos/width}}
{

    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.9\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfsetbuttcap
    \pgfusepath{draw}
}

%% Normal closed Switch
\pgfcircdeclarebipolescaled{switches}
{}
{\ctikzvalof{bipoles/ncs/depth}}
{ncs}
{\ctikzvalof{bipoles/ncs/height}}
{\ctikzvalof{bipoles/ncs/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.9\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Push Button
\pgfcircdeclarebipolescaled{switches}
{}
{\ctikzvalof{bipoles/pushbutton/height 2}}
{pushbutton}
{\ctikzvalof{bipoles/pushbutton/height}}
{\ctikzvalof{bipoles/pushbutton/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{0}{.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfnode{ocirc}{center}{}{}{\pgfusepath{draw}}
    \pgftransformshift{\pgfpoint{2\pgf@circ@res@right}{0pt}}
    \pgfnode{ocirc}{center}{}{}{\pgfusepath{draw}}
}

%% Normally closed Push Button
\pgfcircdeclarebipolescaled{switches}
{}
{\ctikzvalof{bipoles/pushbutton/height 2}}
{ncpushbutton}
{\ctikzvalof{bipoles/pushbutton/height}}
{\ctikzvalof{bipoles/pushbutton/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    % This is the radius of the "ocirc" shape (see pgfcircshapes.tex)
    % Warning, if the nodes will have a class, we have to touch this.
    \pgf@circ@res@temp=\ctikzvalof{nodes width}\pgf@circ@Rlen
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@temp}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-\pgf@circ@res@temp}}
    \pgfpathmoveto{\pgfpoint{0}{-\pgf@circ@res@temp}}
    \pgfpathlineto{\pgfpoint{0}{\pgf@circ@res@up}}
    \pgfusepath{draw}
    %
    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfnode{ocirc}{center}{}{}{\pgfusepath{draw}}
    \pgftransformshift{\pgfpoint{2\pgf@circ@res@right}{0pt}}
    \pgfnode{ocirc}{center}{}{}{\pgfusepath{draw}}
}
% cute switch "to" shapes help function
% #1 -> name
% #2 -> barposition
% #3 -> arrowcode
\long\def\pgfcircdeclarecutesw#1#2#3{
    \pgfcircdeclarebipolescaled{switches}
    {
        \savedanchor\midlever{
            % these values are calculated when we create the definition of the shape.
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@y=\ctikzvalof{bipoles/cuteswitch/height}\pgf@circ@scaled@Rlen
            \pgf@circ@res@temp=\ctikzvalof{nodes width}\pgf@circ@scaled@Rlen
            \pgf@circ@res@temp=\ctikzvalof{bipoles/cuteswitch/thickness}\pgf@circ@res@temp
            \pgf@circ@res@down = -.5\pgf@y
            \pgf@circ@res@up = .5\pgf@y
            \pgfextracty{\pgf@circ@res@other}{#2}
            \pgf@x=0pt
            \pgf@y=.5\pgf@circ@res@other
        }
        % radius of the connector
        % This is the radius of the "ocirc" shape (see pgfcircshapes.tex)
        % If cnnecting nodes are scaled, we have to modify this
        \saveddimen{\radius}{\pgfmathsetlength\pgf@x{\pgf@circ@Rlen*\ctikzvalof{nodes width}}}
        % shapename
        \savedmacro{\thisshape}{\def\thisshape{\tikz@fig@name}}
        % shape type
        \savedmacro{\cshape}{\def\cshape{\ctikzvalof{bipoles/cuteswitch/shape}}}
        % mid of the lever, to stack switches
        \anchor{mid}{\midlever}
        \anchor{cout}{\northeast \pgf@y=0cm}
        \anchor{cin}{\southwest\pgf@y=0cm}
        \anchor{out}{\northeast \pgf@y=0cm\advance\pgf@x by \radius}
        \anchor{in}{\southwest\pgf@y=0cm\advance\pgf@x by -\radius}
    }
    {\ctikzvalof{bipoles/cuteswitch/height 2}}
    {#1}
    {\ctikzvalof{bipoles/cuteswitch/height}}
    {\ctikzvalof{bipoles/cuteswitch/width}}{
        \pgfscope
        % This is the radius of the "ocirc" shape (see pgfcircshapes.tex)
        % If cnnecting nodes are scaled, we have to modify this
        \pgf@circ@res@temp=\ctikzvalof{nodes width}\pgf@circ@Rlen
        \pgf@circ@res@temp=\ctikzvalof{bipoles/cuteswitch/thickness}\pgf@circ@res@temp
        \pgfsetlinewidth{2\pgf@circ@res@temp}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{#2}
        \pgfsetroundcap\pgfusepath{draw}
        \endpgfscope
        \pgfscope % arrow
        #3
        \endpgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfnode{\cshape}{center}{}{\thisshape-in}{\pgfusepath{draw}}
        \pgftransformshift{\pgfpoint{2\pgf@circ@res@right}{0pt}}
        \pgfnode{\cshape}{center}{}{\thisshape-out}{\pgfusepath{draw}}
    }
}

%% closed cute switch
\pgfcircdeclarecutesw{cuteclosedswitch}
    {\pgfpoint{\pgf@circ@res@right}{1.5\pgf@circ@res@temp}}
    {}

%% open cute switch
\pgfcircdeclarecutesw{cuteopenswitch}
    {\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    {}

%% closing cute switch
\pgfcircdeclarecutesw{cuteclosingswitch}
    {\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    {
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}} % in node
    \pgfpathmoveto{\pgfpointpolar{70}{1.2\pgf@circ@res@right}}
    \pgfpatharc{70}{-10}{1.2\pgf@circ@res@right}
    \pgfsetarrowsend{latexslim}
    \pgfusepath{draw}
    }

%% opening cute switch
\pgfcircdeclarecutesw{cuteopeningswitch}
    {\pgfpoint{\pgf@circ@res@right}{1.5\pgf@circ@res@temp}}
    {
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}} % in node
    \pgfpathmoveto{\pgfpointpolar{-10}{1.2\pgf@circ@res@right}}
    \pgfpatharc{-10}{60}{1.2\pgf@circ@res@right}
    \pgfsetarrowsend{latexslim}
    \pgfusepath{draw}
    }

%%%%%%%%%%%%%%%%%
%% Instruments
%%%%%%%%%%%%%%%%%

% % METERINGSHAPE
\long\def\drawmeteringcircle{
    \def\pgf@circ@temp{right}
    \ifx\tikz@res@label@pos\pgf@circ@temp
        \pgf@circ@res@step=-1.2\pgf@circ@res@up
    \else
        \def\pgf@circ@temp{below}
        \ifx\tikz@res@label@pos\pgf@circ@temp
            \pgf@circ@res@step=-1.2\pgf@circ@res@up
        \else
            \pgf@circ@res@step=1.2\pgf@circ@res@up
        \fi
    \fi
    %draw connections to circle
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.9\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathmoveto{\pgfpoint{.9\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
    %draw circle
    \pgfscope
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfpathcircle{\pgfpointorigin}{.9\pgf@circ@res@up}
        \pgf@circ@draworfill
    \endpgfscope
    %draw arrow
    \pgfscope
        \pgfsetarrowsend{latex}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%AMPEREMETER
\pgfcircdeclarebipolescaled{instruments}
{}
{\ctikzvalof{bipoles/ammeter/height}}
{ammeter}
{\ctikzvalof{bipoles/ammeter/height}}
{\ctikzvalof{bipoles/ammeter/width}}
{
    \drawmeteringcircle
    \pgfnode{circle}{center}{\pgf@circ@font@bold{A}}{}{}
}
%OHMMETER
\pgfcircdeclarebipolescaled{instruments}
{}
{\ctikzvalof{bipoles/ohmmeter/height}}
{ohmmeter}
{\ctikzvalof{bipoles/ohmmeter/height}}
{\ctikzvalof{bipoles/ohmmeter/width}}
{
    \drawmeteringcircle
    \pgfnode{circle}{center}{\boldmath$\Omega$}{}{}
}
%VOLTMETER
\pgfcircdeclarebipolescaled{instruments}
{}
{\ctikzvalof{bipoles/voltmeter/height}}
{voltmeter}
{\ctikzvalof{bipoles/voltmeter/height}}
{\ctikzvalof{bipoles/voltmeter/width}}
{
    \drawmeteringcircle
    \pgfnode{circle}{center}{\pgf@circ@font@bold{V}}{}{}

}

% oscilloscope, suggested by @nobrl https://github.com/circuitikz/circuitikz/issues/176
\pgfcircdeclarebipolescaled{instruments}
{
    \anchor{in 1}{\southwest\pgf@y=0.75\pgf@y\pgf@x=0.4\pgf@x}
    \anchor{in 2}{\southwest\pgf@y=0.75\pgf@y\pgf@x=-0.4\pgf@x}
    % put the node text above and centered
    \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
}
{\ctikzvalof{bipoles/oscope/height}}
{oscope}
{\ctikzvalof{bipoles/oscope/height}}
{\ctikzvalof{bipoles/oscope/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfextracty{\pgf@circ@res@up}{\northeast}
    \pgfextractx{\pgf@circ@res@right}{\northeast}
    \pgfextractx{\pgf@circ@res@left}{\southwest}
    \pgfextracty{\pgf@circ@res@down}{\southwest}
    \pgfmathsetlength{\pgf@circ@res@step}{0.25*\pgf@circ@res@up}
    \pgfscope
        \pgfsetcornersarced{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@step}}
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
        % this would create a round (analog?) scope...
        % \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
        \pgf@circ@draworfill
    \endpgfscope
    % get the rotation
    \pgfgettransformentries\a\b\temp\temp\temp\temp
    \pgfmathsetmacro{\rot}{-atan2(\b,\a)}
    % and unrotate the scope
    \pgfscope
        \pgftransformrotate{\rot}
        % grid
        \pgfscope
            \pgfsetlinewidth{0.5\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpoint{0.75\pgf@circ@res@left}{0.25\pgf@circ@res@down}}
            \pgfpathgrid[stepx=\pgf@circ@res@step, stepy=\pgf@circ@res@step]%
            {\pgfpoint{0.75\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
            {\pgfpoint{0.75\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
            \pgfsetstrokeopacity{0.5}
            \pgfusepath{draw}
        \endpgfscope
        % function displayed, thanks to
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{0.75\pgf@circ@res@left}{0.25\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{0.05\pgf@circ@res@left}{0.25\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0.05\pgf@circ@res@left}{0.25\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{0.65\pgf@circ@res@right}{0.25\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0.65\pgf@circ@res@right}{0.25\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

% generic round meter with always horizontal text, no arrow
\pgfcircdeclarebipolescaled{instruments}
{}
{\ctikzvalof{bipoles/esource/height}}
{rmeter}
{\ctikzvalof{bipoles/esource/height}}
{\ctikzvalof{bipoles/esource/width}}
{
    \pgfpointorigin
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    % draw the text label
    % get the rotation
    \pgfgettransformentries\a\b\temp\temp\temp\temp
    \pgfmathsetmacro{\rot}{-atan2(\b,\a)}
    % and unrotate the scope
    \pgfscope
        \pgfsetcolor{\ctikzvalof{color}}
        \pgftransformrotate{\rot}
        \pgftext[center,x=0,y=0]{\ctikzvalof{bipoles/twoport/text}}
    \endpgfscope
}

% generic round meter with always horizontal text, with arrow
\pgfcircdeclarebipolescaled{instruments}
{}
{\ctikzvalof{bipoles/esource/height}}
{rmeterwa}
{\ctikzvalof{bipoles/esource/height}}
{\ctikzvalof{bipoles/esource/width}}
{
    \pgfpointorigin
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    % draw the text label
    % get the rotation
    \pgfgettransformentries\a\b\temp\temp\temp\temp
    \pgfmathsetmacro{\rot}{-atan2(\b,\a)}
    % and unrotate the scope
    \pgfscope
        \pgftransformrotate{\rot}
        \pgfsetcolor{\ctikzvalof{color}}
        \pgfsetlinewidth{\pgfstartlinewidth}
        % arrow: create  a center hole to have better visual
        \pgfscope
            % clipping path: first a rectangle bigger then the shape
            % to avoid problems with the line thickness
            \pgfpathrectanglecorners{\pgfpoint{2\pgf@circ@res@left}{2\pgf@circ@res@down}}
            {\pgfpoint{2\pgf@circ@res@right}{2\pgf@circ@res@up}}
            % next open a circle into it
            \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{.6\pgf@circ@res@up}}{\pgfpoint{.6\pgf@circ@res@left}{0}}
            % do the difference and clip before drawing
            \pgfseteorule
            \pgfusepath{clip}
            \pgfsetarrowsend{latexslim}
            % the arrow is better if it has a bit of breath and it's not 45º
            \pgfpathmoveto{\pgfpoint{.8\pgf@circ@res@left}{1.2\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{.8\pgf@circ@res@right}{1.2\pgf@circ@res@up}}
            \pgfusepath{draw}
        \endpgfscope
        \pgftext[center]{\ctikzvalof{bipoles/twoport/text}}
    \endpgfscope
}

% generic square meter with always horizontal text
\pgfcircdeclarebipolescaled{instruments}
{
    \anchor{in 1}{\southwest\pgf@y=0.75\pgf@y\pgf@x=0.4\pgf@x}
    \anchor{in 2}{\southwest\pgf@y=0.75\pgf@y\pgf@x=-0.4\pgf@x}
    % put the node text above and centered
    \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
}
{\ctikzvalof{bipoles/smeter/height}}
{smeter}
{\ctikzvalof{bipoles/smeter/height}}
{\ctikzvalof{bipoles/smeter/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfextracty{\pgf@circ@res@up}{\northeast}
    \pgfextractx{\pgf@circ@res@right}{\northeast}
    \pgfextractx{\pgf@circ@res@left}{\southwest}
    \pgfextracty{\pgf@circ@res@down}{\southwest}
    \pgfmathsetlength{\pgf@circ@res@step}{0.25*\pgf@circ@res@up}
    \pgfscope
        \pgfsetcornersarced{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@step}}
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgf@circ@draworfill
    \endpgfscope
    % get the rotation
    \pgfgettransformentries\a\b\temp\temp\temp\temp
    \pgfmathsetmacro{\rot}{-atan2(\b,\a)}
    % and unrotate the scope
    \pgfscope
        \pgftransformrotate{\rot}
        % the metering window
        \pgfscope
            \def\@starta{105}\def\@stopa{75}
            \pgfsetlinewidth{\pgfstartlinewidth}
            \pgftransformshift{\pgfpoint{0pt}{-1.8\pgf@circ@res@up}}
            \pgfpathmoveto{\pgfpointpolar{\@starta}{2\pgf@circ@res@up}}
            \pgfpatharc{\@starta}{\@stopa}{2\pgf@circ@res@up}
            \pgfpathlineto{\pgfpointpolar{\@stopa}{2.5\pgf@circ@res@up}}
            \pgfpatharc{\@stopa}{\@starta}{2.5\pgf@circ@res@up}
            \pgfclosepath
            \pgfpathmoveto{\pgfpointpolar{80}{2\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpointpolar{80}{2.4\pgf@circ@res@up}}
            \pgfusepath{draw}
        \endpgfscope
        \pgftext[center, y=0.5\pgf@circ@res@down]{\ctikzvalof{bipoles/twoport/text}}
    \endpgfscope
}

% probes qucs style:
% #1 : name
% #2 : extra code
\long\def\pgfcirc@qucsprobe#1#2{
    \pgfcircdeclarebipolescaled{instruments}
    {
        \anchor{v+}{\southwest\pgf@x=0.6\pgf@x}
        \anchor{v-}{\southwest\pgf@x=-0.6\pgf@x}
        % put the node text above and centered
        \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northeast}
            \pgfpoint{-.5\wd\pgfnodeparttextbox}{
                \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
            }
        }
    }
    {\ctikzvalof{bipoles/qmeter/depth}}
    {#1}
    {\ctikzvalof{bipoles/qmeter/height}}
    {\ctikzvalof{bipoles/qmeter/width}}
    {
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfextractx{\pgf@circ@res@right}{\northeast}
        \pgfextractx{\pgf@circ@res@left}{\southwest}
        \pgfextracty{\pgf@circ@res@down}{\southwest}
        \pgfmathsetlength{\pgf@circ@res@step}{0.25*\pgf@circ@res@up}
        \pgfscope
            \pgfscope
                \pgfsetcornersarced{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@step}}
                \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
            \pgf@circ@draworfill
            \endpgfscope
            \def\@starta{103}\def\@stopa{77}
            \pgfsetlinewidth{\pgfstartlinewidth}
            \pgfscope
                \pgftransformshift{\pgfpoint{0pt}{-1.7\pgf@circ@res@up}}
                \pgfpathmoveto{\pgfpointpolar{\@starta}{2.1\pgf@circ@res@up}}
                \pgfpatharc{\@starta}{\@stopa}{2.1\pgf@circ@res@up}
                \pgfpathlineto{\pgfpointpolar{\@stopa}{2.5\pgf@circ@res@up}}
                \pgfpatharc{\@stopa}{\@starta}{2.5\pgf@circ@res@up}
                \pgfclosepath
                \pgfpathmoveto{\pgfpointpolar{83}{2.1\pgf@circ@res@up}}
                \pgfpathlineto{\pgfpointpolar{83}{2.4\pgf@circ@res@up}}
                \pgfusepath{draw}
                \pgf@circ@draworfill
            \endpgfscope
            #2
        \endpgfscope
    }
}

\pgfcirc@qucsprobe{qiprobe}{
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfusepath{draw}
    \pgfnode{currarrow}{center}{}{}{}
}

\pgfcirc@qucsprobe{qvprobe}{
    \pgfmathsetlength{\pgf@circ@res@other}{\ctikzvalof{nodes width}*\pgf@circ@scaled@Rlen}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@left}{0pt}}
    \pgfpathcircle{\pgfpoint{.6\pgf@circ@res@left+\pgf@circ@res@other}{0pt}}{\pgf@circ@res@other}
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathcircle{\pgfpoint{.6\pgf@circ@res@right-\pgf@circ@res@other}{0pt}}{\pgf@circ@res@other}
    \pgfusepath{draw}
    \pgfscope
        % "+" and "-", drawn so that they scale correctly
        \pgfsetlinewidth{2\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left+\pgf@circ@res@other}{-1.5\pgf@circ@res@other}}
        \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@left+\pgf@circ@res@other}{-3.5\pgf@circ@res@other}}
        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left+0\pgf@circ@res@other}{-2.5\pgf@circ@res@other}}
        \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@left+2\pgf@circ@res@other}{-2.5\pgf@circ@res@other}}
        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@right+0\pgf@circ@res@other}{-2.5\pgf@circ@res@other}}
        \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right-2\pgf@circ@res@other}{-2.5\pgf@circ@res@other}}
        \pgfusepath{draw}
    \endpgfscope
}

\pgfcirc@qucsprobe{qpprobe}{
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfusepath{draw}
    \pgfnode{currarrow}{center}{}{}{}
    \pgfmathsetlength{\pgf@circ@res@other}{\ctikzvalof{nodes width}*\pgf@circ@scaled@Rlen}
    \pgfpathcircle{\pgfpoint{.6\pgf@circ@res@left}{-3\pgf@circ@res@other}}{\pgf@circ@res@other}
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{-4\pgf@circ@res@other}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathcircle{\pgfpoint{.6\pgf@circ@res@right}{-3\pgf@circ@res@other}}{\pgf@circ@res@other}
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@right}{-4\pgf@circ@res@other}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}
    \pgfscope
        % "+" and "-", drawn so that they scale correctly
        \pgfsetlinewidth{2\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left+3\pgf@circ@res@other}{-2\pgf@circ@res@other}}
        \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@left+3\pgf@circ@res@other}{-4\pgf@circ@res@other}}
        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left+2\pgf@circ@res@other}{-3\pgf@circ@res@other}}
        \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@left+4\pgf@circ@res@other}{-3\pgf@circ@res@other}}
        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@right-4\pgf@circ@res@other}{-3\pgf@circ@res@other}}
        \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right-2\pgf@circ@res@other}{-3\pgf@circ@res@other}}
        \pgfusepath{draw}
    \endpgfscope
}

% current loop for oscope and similar: stylized
\pgfcircdeclarebipolescaled{instruments}
{
    \anchor{i}{\northeast\pgf@x=0pt\relax}
    \anchor{text}{
        \pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfextractx{\pgf@circ@res@left}{\northeast}
        \pgfpoint{-.5\wd\pgfnodeparttextbox+\pgf@circ@res@left}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
}
{\ctikzvalof{bipoles/iloop/height}}
{iloop}
{\ctikzvalof{bipoles/iloop/height}}
{\ctikzvalof{bipoles/iloop/width}}
{
    \pgfextracty{\pgf@circ@res@up}{\northeast}
    \pgfextractx{\pgf@circ@res@right}{\northeast}
    \pgf@circ@res@down=-\pgf@circ@res@up
    \pgf@circ@res@left=-\pgf@circ@res@right
    \pgfscope
        \pgfstartlinewidth=\pgflinewidth
        \pgfsetcolor{\ctikzvalof{color}}
        % external ellipse
        \pgfscope
            \pgf@circ@setlinewidth{bipoles}{\pgflinewidth}
            % clipping path: first a rectangle bigger then the shape
            % to avoid problems with the line thickness
            \pgfpathrectanglecorners{\pgfpoint{2\pgf@circ@res@left}{2\pgf@circ@res@down}}
            {\pgfpoint{2\pgf@circ@res@right}{2\pgf@circ@res@up}}
            % next the opening to the left
            \pgfpathrectanglecorners{\pgfpoint{2\pgf@circ@res@left}{.1\pgf@circ@res@down}}
            {\pgfpoint{0pt}{.1\pgf@circ@res@up}}
            % do the difference and clip before drawing
            \pgfseteorule
            \pgfusepath{clip}
            \pgfpathellipse{\pgfpointorigin}{
                \pgfpoint{0pt}{0.8\pgf@circ@res@up}}{
            \pgfpoint{0.4\pgf@circ@res@right}{0pt}}
            \pgfusepath{draw}
        \endpgfscope
        % internal wire
        \pgfsetlinewidth{\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0.3\pgf@circ@res@right}{0pt}}
        \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        % and the contact line up
        \pgfpathmoveto{\pgfpoint{0pt}{0.8\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

% current loop for oscope and similar: real (double connection)
\pgfcircdeclarebipolescaled{instruments}
{
    \anchor{i+}{
        \pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfextractx{\pgf@circ@res@right}{\northeast}
        \pgf@circ@res@step=0.4\pgf@circ@res@right
        \pgf@circ@res@other=0.8\pgf@circ@res@up
        \pgfpointpolar{105}{\pgf@circ@res@step and \pgf@circ@res@other}
        \pgf@y=\pgf@circ@res@up
    }
    \anchor{i-}{
        \pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfextractx{\pgf@circ@res@right}{\northeast}
        \pgf@circ@res@step=0.4\pgf@circ@res@right
        \pgf@circ@res@other=0.8\pgf@circ@res@up
        \pgfpointpolar{75}{\pgf@circ@res@step and \pgf@circ@res@other}
        \pgf@y=\pgf@circ@res@up
    }
    \anchor{text}{
        \pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfextractx{\pgf@circ@res@left}{\northeast}
        \pgfpoint{-.5\wd\pgfnodeparttextbox+\pgf@circ@res@left}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
}
{\ctikzvalof{bipoles/iloop/height}}
{iloop2}
{\ctikzvalof{bipoles/iloop/height}}
{\ctikzvalof{bipoles/iloop/width}}
{
    \pgfextracty{\pgf@circ@res@up}{\northeast}
    \pgfextractx{\pgf@circ@res@right}{\northeast}
    \pgf@circ@res@down=-\pgf@circ@res@up
    \pgf@circ@res@left=-\pgf@circ@res@right
    % must be the same than internal i+ and i- anchors definition
    \pgf@circ@res@step=0.4\pgf@circ@res@right
    \pgf@circ@res@other=0.8\pgf@circ@res@up
    \def\@plus{\pgfpointpolar{105}{\pgf@circ@res@step and \pgf@circ@res@other}}
    \def\@minus{\pgfpointpolar{75}{\pgf@circ@res@step and \pgf@circ@res@other}}
    \pgfscope
        \pgfstartlinewidth=\pgflinewidth
        \pgfsetcolor{\ctikzvalof{color}}
        % external ellipse
        \pgfscope
            \pgf@circ@setlinewidth{bipoles}{\pgflinewidth}
            % clipping path: first a rectangle bigger then the shape
            % to avoid problems with the line thickness
            \pgfpathrectanglecorners{\pgfpoint{2\pgf@circ@res@left}{2\pgf@circ@res@down}}
            {\pgfpoint{2\pgf@circ@res@right}{2\pgf@circ@res@up}}
            % next the opening to the left
            \pgfpathrectanglecorners{\pgfpoint{2\pgf@circ@res@left}{.1\pgf@circ@res@down}}
            {\pgfpoint{0pt}{.1\pgf@circ@res@up}}
            % do the difference and clip before drawing
            \pgfseteorule
            \pgfusepath{clip}
            \pgfpathmoveto{\@plus}
            \pgfpatharc{105}{435}{\pgf@circ@res@step and \pgf@circ@res@other}
            \pgfusepath{draw}
        \endpgfscope
        % internal wire
        \pgfsetlinewidth{\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0.3\pgf@circ@res@right}{0pt}}
        \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        % and the contact line up
        % I use ...left and ---right as temporal lengths here to avoid defining more
        \pgfextractx{\pgf@circ@res@left}{\@plus}
        \pgfextractx{\pgf@circ@res@right}{\@minus}
        \pgfpathmoveto{\@plus}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathmoveto{\@minus}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}


%% Varistor
\pgfcircdeclarebipolescaled{resistors}
{}
{\ctikzvalof{bipoles/varistor/height}}
{varistor}
{\ctikzvalof{bipoles/varistor/height}}
{\ctikzvalof{bipoles/varistor/width}}
{
    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\ctikzvalof{bipoles/varistor/main}\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{-\ctikzvalof{bipoles/varistor/main}\pgf@circ@res@up}}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{-\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfusepath{draw}

    \pgftext[top,x=.65\pgf@circ@res@left,y=1.2\pgf@circ@res@down]{{\pgf@circ@font@tiny\textsf{U}}}
}

%%%%%%%%%%%%%%
%% RF bipoles
%%%%%%%%%%%%%%

% transmission line
\pgfcircdeclarebipolescaled{RF}
{}
{\ctikzvalof{bipoles/tline/height}}
{tline}
{\ctikzvalof{bipoles/tline/height}}
{\ctikzvalof{bipoles/tline/width}}
{
    \pgf@circ@res@step=.2\pgf@circ@res@right % half x axis
    \begin{pgftransparencygroup}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@step}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left+\pgf@circ@res@step}{\pgf@circ@res@up}}
        \pgfpatharc{-90}{90}{-\pgf@circ@res@step and -\pgf@circ@res@up}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@step}{\pgf@circ@res@down}}
        \pgf@circ@draworfill
        \pgfpathellipse{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@step}{0pt}}
        {\pgfpoint{\pgf@circ@res@step}{0pt}}{\pgfpoint{0pt}{-\pgf@circ@res@up}}
        \pgf@circ@draworfill
    \end{pgftransparencygroup}
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfusepath{stroke}
}

% microstrip transmission line
\pgfcircdeclarebipolescaled{RF}
{}
{\ctikzvalof{bipoles/mstline/height}}
{mstline}
{\ctikzvalof{bipoles/mstline/height}}
{\ctikzvalof{bipoles/mstline/width}}
{
    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgf@circ@draworfill
}

%%%%%%%%%%%%%%%%%%%
%% Block diagrams
%%%%%%%%%%%%%%%%%%%

%% Draw the two-port fillable box
\def\pgf@circ@twoportbox{
    \pgfscope
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgf@circ@draworfill
    \endpgfscope
}

%% Generic two port box
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/twoport/height}}
{twoport}
{\ctikzvalof{bipoles/twoport/height}}
{\ctikzvalof{bipoles/twoport/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/twoport/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi
    % draw outer box
    \pgf@circ@twoportbox
    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgftext[center,x=0,y=0]{\ctikzvalof{bipoles/twoport/text}}

}

%% voltage controled oscillator
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/vco/width}}
{vco}
{\ctikzvalof{bipoles/twoport/width}}
{\ctikzvalof{bipoles/vco/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/vco/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi
    % draw circle
    \pgfscope
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfpathcircle{\pgfpoint{0}{0}} {\pgf@circ@res@step}
        \pgf@circ@draworfill
    \endpgfscope
    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner sine waves
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-.5\pgf@circ@res@step}{0\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
}

%% bandpass filter
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/bandpass/width}}
{bandpass}
{\ctikzvalof{bipoles/bandpass/width}}
{\ctikzvalof{bipoles/bandpass/width}}
{

    \pgf@circ@res@step = \ctikzvalof{bipoles/bandpass/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{0.35\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.65\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.65\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{-0.35\pgf@circ@res@step}}
    \pgfusepath{draw}
}

%% bandstop filter
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/bandstop/width}}
{bandstop}
{\ctikzvalof{bipoles/bandstop/width}}
{\ctikzvalof{bipoles/bandstop/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/bandstop/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225% 134 degree, because >= 135 is not possible
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}% always draw solid line for inner symbol
    \pgfsetarrows{-}%never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.15\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.15\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
}

%% highpass filter
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/highpass/width}}
{highpass}
{\ctikzvalof{bipoles/highpass/width}}
{\ctikzvalof{bipoles/highpass/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/highpass/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.15\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.15\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.65\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{-0.35\pgf@circ@res@step}}
    \pgfusepath{draw}
}

%% lowpass filter
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/lowpass/width}}
{lowpass}
{\ctikzvalof{bipoles/lowpass/width}}
{\ctikzvalof{bipoles/lowpass/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/lowpass/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{0.35\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.65\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.15\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.15\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
}

%% ADC
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/adc/width}}
{adc}
{\ctikzvalof{bipoles/adc/width}}
{\ctikzvalof{bipoles/adc/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/adc/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\texti{A}
    \def\textii{D}
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \def\texti{D}
        \def\textii{A}
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
        \def\texti{D}
        \def\textii{A}
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
        \def\texti{A}
        \def\textii{D}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgftext[center,x=0.45\pgf@circ@res@left,y=0.45\pgf@circ@res@up]{\textsf{\texti}}
    \pgftext[center,x=0.45\pgf@circ@res@right,y=0.45\pgf@circ@res@down]{\textsf{\textii}}
}

%% DAC
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/dac/width}}
{dac}
{\ctikzvalof{bipoles/dac/width}}
{\ctikzvalof{bipoles/dac/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/dac/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\texti{D}
    \def\textii{A}
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \def\texti{A}
        \def\textii{D}
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
        \def\texti{A}
        \def\textii{D}
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
        \def\texti{D}
        \def\textii{A}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgftext[center,x=0.45\pgf@circ@res@left,y=0.45\pgf@circ@res@up]{\textsf{\texti}}
    \pgftext[center,x=0.45\pgf@circ@res@right,y=0.45\pgf@circ@res@down]{\textsf{\textii}}
}

%% DSP
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/dsp/width}}
{dsp}
{\ctikzvalof{bipoles/dsp/width}}
{\ctikzvalof{bipoles/dsp/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/dsp/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgftext[center,x=0,y=0]{\textsf{DSP}}
}

%% FFT
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/fft/width}}
{fft}
{\ctikzvalof{bipoles/fft/width}}
{\ctikzvalof{bipoles/fft/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/fft/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgftext[center,x=0,y=0]{\textsf{FFT}}
}

%% Amplifier
\pgfcircdeclarebipolescaled{blocks}
{}
{
    \ifpgf@circuit@boxed
        \ctikzvalof{bipoles/twoport/width}
    \else
        \ctikzvalof{bipoles/amp/width}
    \fi
}
{amp}
{
    \ifpgf@circuit@boxed
        \ctikzvalof{bipoles/twoport/width}
    \else
        \ctikzvalof{bipoles/amp/width}
    \fi
}
{
    \ifpgf@circuit@boxed
        \ctikzvalof{bipoles/twoport/width}
    \else
        \ctikzvalof{bipoles/amp/width}
    \fi
}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/amp/width}\pgf@circ@scaled@Rlen

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \ifpgf@circuit@boxed
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfnode{blockbox}{center}{}{pgf@box}{\pgfusepath{draw}}
        \pgf@circ@draworfill
    \fi

    % draw input arrow
    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    \ifpgf@circuit@boxed
        \pgfsetlinewidth{\pgfstartlinewidth}
        \pgfsetdash{}{0pt}	% draw solid line for inner symbol if no box is drawn
        \pgf@circ@res@step=.7\pgf@circ@res@step % scale amp symbol when inside a box
    \else
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \fi

    \pgfsetarrows{-} %never draw arrows

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.55\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{0}}
    \pgfpathlineto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.55\pgf@circ@res@step}}

    \pgfpathclose
    \pgf@circ@draworfill

    % draw inner text
    \pgftext[center,x=-0.12\pgf@circ@res@step,y=0]{\ctikzvalof{bipoles/twoport/text}}
}


%% variable amplifier
\pgfcircdeclarebipolescaled{blocks}
{}
{
    \ifpgf@circuit@boxed
        \ctikzvalof{bipoles/twoport/width}
    \else
        \ctikzvalof{bipoles/amp/width}
    \fi
}
{vamp}
{
    \ifpgf@circuit@boxed
        \ctikzvalof{bipoles/twoport/width}
    \else
        \ctikzvalof{bipoles/amp/width}
    \fi
}
{
    \ifpgf@circuit@boxed
        \ctikzvalof{bipoles/twoport/width}
    \else
        \ctikzvalof{bipoles/amp/width}
    \fi
}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/amp/width}\pgf@circ@scaled@Rlen

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \ifpgf@circuit@boxed
        \pgfnode{blockbox}{center}{}{pgf@box}{\pgfusepath{draw}}
    \fi

    % draw input arrow
    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    \ifpgf@circuit@boxed
        \pgfsetlinewidth{\pgfstartlinewidth}
        \pgfsetdash{}{0pt}	% draw solid line for inner symbol if no box is drawn
        \pgf@circ@res@step=.7\pgf@circ@res@step % scale amp symbol when inside a box
    \else
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \fi


    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.55\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{0}}
    \pgfpathlineto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.55\pgf@circ@res@step}}

    \pgfpathclose
    \pgf@circ@draworfill

    % draw inner text
    \pgftext[center,x=-0.12\pgf@circ@res@step,y=0]{\ctikzvalof{bipoles/twoport/text}}

    % draw arrow
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfsetarrowsend{latex}
    \pgfpathmoveto{\pgfpoint{-0.8\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@step}{0.6\pgf@circ@res@step}}
    \pgfusepath{draw}
}

%% pi attenuator
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/piattenuator/width}}
{piattenuator}
{\ctikzvalof{bipoles/piattenuator/width}}
{\ctikzvalof{bipoles/piattenuator/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/piattenuator/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@left}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@right}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.6\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% variable pi attenuator
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/vpiattenuator/width}}
{vpiattenuator}
{\ctikzvalof{bipoles/vpiattenuator/width}}
{\ctikzvalof{bipoles/vpiattenuator/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/vpiattenuator/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@left}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@right}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.6\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetarrowsend{latex}
    \pgfpathmoveto{\pgfpoint{0.7\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% T attenuator
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/tattenuator/width}}
{tattenuator}
{\ctikzvalof{bipoles/tattenuator/width}}
{\ctikzvalof{bipoles/tattenuator/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/tattenuator/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{0pt}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0pt}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.6\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% variable T attenuator
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/vtattenuator/width}}
{vtattenuator}
{\ctikzvalof{bipoles/vtattenuator/width}}
{\ctikzvalof{bipoles/vtattenuator/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/vtattenuator/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{0pt}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0pt}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.6\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetarrowsend{latex}
    \pgfpathmoveto{\pgfpoint{0.7\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% phase shifter
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/phaseshifter/width}}
{phaseshifter}
{\ctikzvalof{bipoles/phaseshifter/width}}
{\ctikzvalof{bipoles/phaseshifter/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/phaseshifter/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % inner symbol
    \pgftext[center,x=0,y=0]{\Large$\varphi$}
}

%% variable phase shifter
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/phaseshifter/width}}
{vphaseshifter}
{\ctikzvalof{bipoles/vphaseshifter/width}}
{\ctikzvalof{bipoles/vphaseshifter/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/vphaseshifter/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % inner symbol
    \pgftext[center,x=0,y=0]{\Large$\varphi$}

    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfsetarrowsend{latex}
    \pgfpathmoveto{\pgfpoint{0.75\pgf@circ@res@left}{0.65\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.65\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% detector
\pgfcircdeclarebipolescaled{blocks}
{}
{\ctikzvalof{bipoles/detector/width}}
{detector}
{\ctikzvalof{bipoles/detector/width}}
{\ctikzvalof{bipoles/detector/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/detector/width}\pgf@circ@scaled@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\ctikzvalof{bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % draw inner stuff
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{0.8\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{0.75\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@right}{0}}
    \pgfusepath{draw}

    \ifpgf@circuit@fulldiode
        \pgfmathparse{2\pgf@circ@res@up / \pgf@circ@scaled@Rlen / \ctikzvalof{bipoles/generic/width}}
        \pgftransformscale{\pgfmathresult}
        \pgfnode{fulldiodeshape}{center}{}{pgf@fulldiode}{\pgfusepath{fill}}
    \else
        \pgfmathparse{2\pgf@circ@res@up / \pgf@circ@scaled@Rlen / \ctikzvalof{bipoles/resistor/width}}
        \pgftransformscale{\pgfmathresult}
        \pgfnode{emptydiodeshape}{center}{}{pgf@emptydiode}{\pgfusepath{fill}}
    \fi

}

%%%%%%%%%%%%%%%%%%%%%%%
%% MECHANICAL SYMBOLS
%%%%%%%%%%%%%%%%%%%%%%%

%% mechanical capacitance - stiffness/spring

\pgfcircdeclarebipolescaled{mechanicals}
{}
{\ctikzvalof{bipoles/spring/height}}
{spring}
{\ctikzvalof{bipoles/spring/height}}
{\ctikzvalof{bipoles/spring/width}}{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments

    \pgfmathsetlength{\pgf@circ@res@step}
    {(\ctikzvalof{bipoles/spring/width}*\pgf@circ@scaled@Rlen+\pgfhorizontaltransformationadjustment*.5*\pgflinewidth)/16}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{\pgf@circ@res@zero}}
    \pgfsetcornersarced{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}
}

%% mechanical inductance - mass
\pgfcircdeclarebipolescaled{mechanicals}
{}
{\ctikzvalof{bipoles/mass/box height}}
{mass}
{\ctikzvalof{bipoles/mass/height}}
{\ctikzvalof{bipoles/mass/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgftransformationadjustments
    \pgfpathrectangle{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
        {\pgfpoint{-2\pgf@circ@res@down}{-2\pgf@circ@res@down}}
    \pgf@circ@draworfill

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfsetrectcap
    \pgfsetmiterjoin
    \pgfusepath{stroke}
}

%% mechanical resistor - damper
\pgfcircdeclarebipolescaled{mechanicals}
{}
{\ctikzvalof{bipoles/damper/height}}
{damper}
{\ctikzvalof{bipoles/damper/height}}
{\ctikzvalof{bipoles/damper/width}}
{
    \pgfpathrectanglecorners{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgf@circ@maybefill

    % line into the damper
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
        {\pgf@circ@res@zero}}
    \pgfusepath{stroke}

    % damper box
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}

    \pgfsetrectcap
    \pgfsetmiterjoin
    \pgfusepath{stroke}

    % damper vertical element
    \pgfpathmoveto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
        {.8\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
        {.8\pgf@circ@res@up}}
    \pgfsetbuttcap
    \pgfusepath{stroke}

}
%% mechanical viscoelastic element, suggested by @alex
%% in https://tex.stackexchange.com/questions/484268/combined-spring-damper-in-circuitikz
\pgfcircdeclarebipolescaled{mechanicals}
{}                                   % extra anchors
{\ctikzvalof{bipoles/damper/height}} % depth (under the path line)
{viscoe}                             % name
{\ctikzvalof{bipoles/damper/height}} % height (above the path line)
{\ctikzvalof{bipoles/damper/width}}  % width
{ % draw the bipole
    \pgfpathrectanglecorners{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgf@circ@maybefill

    % spring into the damper
    \pgfscope
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfsetcornersarced{\pgfpoint{.25\pgf@circ@res@up}{.25\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.75\pgf@circ@res@left}{.75\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.5\pgf@circ@res@left}{-.75\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.75\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{-.75\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}{.75\pgf@circ@res@up}}
        \pgfusepath{stroke}
    \endpgfscope
    % damper box
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}

    \pgfsetrectcap
    \pgfsetmiterjoin
    \pgfusepath{stroke}

    % damper vertical element
    \pgfpathmoveto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
        {.8\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
        {.8\pgf@circ@res@up}}
    \pgfsetbuttcap
    \pgfusepath{stroke}

}

%%%%%%%%%%%%%%%%
%% Crossing
%%%%%%%%%%%%%%%%

%% crossing bipole (but see also nodes)
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/crossing/size}}
{crossing}
{\ctikzvalof{bipoles/crossing/size}}
{\ctikzvalof{bipoles/crossing/size}}{
    \pgfscope
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfpatharc{0}{-180}{0.4*\pgf@circ@res@left}
        \pgfsetbeveljoin
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfusepath{draw}
    \endpgfscope
}

%%%%%%%%%%%%%%%%%%%%%%%%%
%% Miscellaneous bipoles
%%%%%%%%%%%%%%%%%%%%%%%%%

%% loudspeaker and microphone

\pgfcircdeclarebipolescaled{misc}
{}
{\ctikzvalof{bipoles/loudspeaker/depth}}
{loudspeaker}
{\ctikzvalof{bipoles/loudspeaker/height}}
{\ctikzvalof{bipoles/loudspeaker/width}}{

    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{.4\pgf@circ@res@up}}
    {\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@left}{.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.8\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.8\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{.4\pgf@circ@res@up}}
    \pgfpathclose
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgf@circ@draworfill
}

\pgfcircdeclarebipolescaled{misc}
{}
{\ctikzvalof{bipoles/mic/depth}}
{mic}
{\ctikzvalof{bipoles/mic/height}}
{\ctikzvalof{bipoles/mic/width}}{

    \pgfscope
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathcircle{\pgfpoint{0pt}{.6\pgf@circ@res@up}}{.4\pgf@circ@res@up}
    \pgf@circ@draworfill
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
    \endpgfscope
    \pgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{-.2\pgf@circ@res@up}{0pt}}
    % 0.25358 is 0.6-0.4*cos(30)
    \pgfpathlineto{\pgfpoint{-.2\pgf@circ@res@up}{.25358\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@up}{.25358\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@up}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfusepath{draw}

    \pgfusepath{draw}
    \endpgfscope
}

%% european gas filled surge arrester
\pgfcircdeclarebipolescaled{misc}
{}
{\ctikzvalof{bipoles/european gas filled surge arrester/height}}
{european gas filled surge arrester}
{\ctikzvalof{bipoles/european gas filled surge arrester/height}}
{\ctikzvalof{bipoles/european gas filled surge arrester/width}}
{

    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgf@circ@draworfill

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/european gas filled surge arrester/inside}\pgf@circ@res@left}{0pt}}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfusepath{draw}

    \endpgfscope
}

%% american gas filled surge arrester
\pgfcircdeclarebipolescaled{misc}
{}
{\ctikzvalof{bipoles/american gas filled surge arrester/height}}
{american gas filled surge arrester}
{\ctikzvalof{bipoles/american gas filled surge arrester/height}}
{\ctikzvalof{bipoles/american gas filled surge arrester/width}}{

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpointorigin	\pgf@circ@res@other =  \pgf@x  \advance \pgf@circ@res@other by -\pgf@circ@res@up
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
    \pgfusepath{draw}

    \pgfscope
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfpathcircle{\pgfpointorigin}{.9\pgf@circ@res@up}
        \pgf@circ@draworfill
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}

    \pgfscope
        \pgfsetarrowsend{latex}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/american gas filled surge arrester/inside}\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfusepath{draw}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/american gas filled surge arrester/inside}\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfusepath{draw}
    \endpgfscope{}

    \pgfcircle{\pgfpoint{\ctikzvalof{bipoles/american gas filled surge arrester/dot x}\pgf@circ@res@left}{\ctikzvalof{bipoles/american gas filled surge arrester/dot y}\pgf@circ@res@down}}{\ctikzvalof{bipoles/american gas filled surge arrester/size}\pgf@circ@res@down}
    \pgfusepath{fill}
}

%% thermocouple
\pgfcircdeclarebipolescaled{misc}
{}
{\ctikzvalof{bipoles/thermocouple/height 2}}
{thermocouple}
{\ctikzvalof{bipoles/thermocouple/height}}
{\ctikzvalof{bipoles/thermocouple/width}}
{
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@down}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@down}}
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathlineto{\pgfpoint{0}{\pgf@circ@res@down}}
    \pgfusepath{draw}
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{0}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
    \pgfusepath{draw}
}

%% fuse
\pgfcircdeclarebipolescaled{misc}
{}
{\ctikzvalof{bipoles/fuse/height}}
{fuse}
{\ctikzvalof{bipoles/fuse/height}}
{\ctikzvalof{bipoles/fuse/width}}
{
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
    \pgfusepath{draw}

    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgf@circ@draworfill
}

%% asymmetric fuse
\pgfcircdeclarebipolescaled{misc}
{}
{\ctikzvalof{bipoles/afuse/height}}
{afuse}
{\ctikzvalof{bipoles/afuse/height}}
{\ctikzvalof{bipoles/afuse/width}}
{
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
    \pgfusepath{draw}

    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope

    \pgfpathrectanglecorners{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{stroke,fill}
}

%% SQUID added by Cor Molenaar 5 March 2010
\pgfcircdeclarebipolescaled{misc}
{}
{\ctikzvalof{bipoles/squid/height}}
{squid}
{\ctikzvalof{bipoles/squid/height}}
{\ctikzvalof{bipoles/squid/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{1.35*\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{0.65*\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{0.65*\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{1.35*\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{1.35*\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{0.65*\pgf@circ@res@down}}
    \pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{0.65*\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{1.35*\pgf@circ@res@down}}

    \pgfusepath{draw}
}

% Generic barrier added by Cor Molenaar 5 March 2010
\pgfcircdeclarebipolescaled{misc}
{}
{\ctikzvalof{bipoles/barrier/height}}
{barrier}
{\ctikzvalof{bipoles/barrier/height}}
{\ctikzvalof{bipoles/barrier/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{0.35*\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{0.35*\pgf@circ@res@down}}
    \pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{0.35*\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{0.35*\pgf@circ@res@up}}

    \pgfusepath{draw}
}

%% Lamp
\pgfcircdeclarebipolescaled{misc}
{}
{\ctikzvalof{bipoles/lamp/height}}
{lamp}
{\ctikzvalof{bipoles/lamp/height}}
{\ctikzvalof{bipoles/lamp/width}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfpathmoveto{\pgfpoint{.7071*\pgf@circ@res@left}{.7071*\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.7071*\pgf@circ@res@right}{.7071*\pgf@circ@res@down}}
    \pgfpathmoveto{\pgfpoint{.7071*\pgf@circ@res@left}{.7071*\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.7071*\pgf@circ@res@right}{.7071*\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% bulb
\pgfcircdeclarebipolescaled{misc}
{}
{\ctikzvalof{bipoles/bulb/height}}
{bulb}
{\ctikzvalof{bipoles/bulb/height}}
{\ctikzvalof{bipoles/bulb/width}}
{%
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{0.8\pgf@circ@res@up}}{\pgfpoint{0.8\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpatharc{0}{-180}{0.4*\pgf@circ@res@left}
    \pgfsetbeveljoin
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
}


% end of pgfcircbipoles.tex


==> pgfcirccurrent.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Current handling

%% styles
\ctikzset{bipole current style/.style={}}
\tikzset{bipole current style/.code={
        \ctikzset{bipole current style/.style={#1}}
}}
\tikzset{bipole current append style/.code={
        \ctikzset{bipole current style/.append style={#1}}
}}

%% Options
\ctikzset{i^>/.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = forward,
        \circuitikzbasekey/bipole/current/x position = after,
        \circuitikzbasekey/bipole/current/y position = above
    }
}

\ctikzset{i_>/.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = forward,
        \circuitikzbasekey/bipole/current/x position = after,
        \circuitikzbasekey/bipole/current/y position = below
    }
}

\ctikzset{i>^/.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = forward,
        \circuitikzbasekey/bipole/current/x position = before,
        \circuitikzbasekey/bipole/current/y position = above
    }
}

\ctikzset{i>_/.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = forward,
        \circuitikzbasekey/bipole/current/x position = before,
        \circuitikzbasekey/bipole/current/y position = below
    }
}

\ctikzset{i^</.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = backward,
        \circuitikzbasekey/bipole/current/x position = after,
        \circuitikzbasekey/bipole/current/y position = above
    }
}

\ctikzset{i_</.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = backward,
        \circuitikzbasekey/bipole/current/x position = after,
        \circuitikzbasekey/bipole/current/y position = below
    }
}

\ctikzset{i<^/.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = backward,
        \circuitikzbasekey/bipole/current/x position = before,
        \circuitikzbasekey/bipole/current/y position = above
    }
}

\ctikzset{i<_/.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = backward,
        \circuitikzbasekey/bipole/current/x position = before,
        \circuitikzbasekey/bipole/current/y position = below
    }
}

\ctikzset{i/.code = {
        \pgfkeys{\circuitikzbasekey/bipole/current/direction = forward,
            \circuitikzbasekey/bipole/current/x position = after,
        \circuitikzbasekey/bipole/current/y position = above }
        \pgfkeys{/tikz/circuitikz/bipole/current/label/name=#1}
        \ctikzsetvalof{bipole/current/label/unit}{}
        \ifpgf@circ@siunitx
            \pgf@circ@handleSI{#1}
            \ifpgf@circ@siunitx@res
                \edef\pgf@temp{\pgf@circ@handleSI@val}
                \pgfkeyslet{/tikz/circuitikz/bipole/current/label/name}{\pgf@temp}
                \edef\pgf@temp{\pgf@circ@handleSI@unit}
                \pgfkeyslet{/tikz/circuitikz/bipole/current/label/unit}{\pgf@temp}
            \else
        \fi
        \else
    \fi
    %reverse current direction for voltage sources
    \ifpgf@circ@oldvoltagedirection\else
        \ifpgf@circuit@bipole@isvoltage
            \ifpgf@circuit@bipole@voltage@backward
                \pgfkeys{\circuitikzbasekey/bipole/current/direction = forward,
                    \circuitikzbasekey/bipole/current/x position = after,
                \circuitikzbasekey/bipole/current/y position = below }
            \else
                \pgfkeys{\circuitikzbasekey/bipole/current/direction = backward,
                    \circuitikzbasekey/bipole/current/x position = before,
                \circuitikzbasekey/bipole/current/y position = above }
            \fi\fi\fi
    }
}

\ifpgf@circ@oldvoltagedirection
    \ctikzset{i</.style = { i = #1, \circuitikzbasekey/bipole/current/direction = backward } }
\else
    \ctikzset{i</.style = { i = #1, \circuitikzbasekey/bipole/current/direction = backward, \circuitikzbasekey/bipole/current/x position = before } }
\fi
\ctikzset{i_/.style = { i = #1, \circuitikzbasekey/bipole/current/y position = below } }
\ctikzset{i>/.style = {i = #1, \circuitikzbasekey/bipole/current/direction = forward } }
\ctikzset{i^/.style = { i= #1, \circuitikzbasekey/bipole/current/y position = above } }

%% Output routine
\def\pgf@circ@drawcurrent{
    \pgfextra{
        \edef\pgf@circ@ffffff{\pgf@circ@direction}
        \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@ffffff\pgf@nil}

        \ifnum\pgfcircmathresult >4 \ifnum\pgfcircmathresult <86
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{north west} \else \def\pgf@circ@dir{south east}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >85 \ifnum\pgfcircmathresult <95
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{west} \else \def\pgf@circ@dir{east}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >94 \ifnum\pgfcircmathresult <176
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{south west}\else \def\pgf@circ@dir{north east}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >175 \ifnum\pgfcircmathresult <185
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{south}\else\def\pgf@circ@dir{north}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >184 \ifnum\pgfcircmathresult <266
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{south east}\else\def\pgf@circ@dir{north west}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >265 \ifnum\pgfcircmathresult <275
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{east}\else \def\pgf@circ@dir{west}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >274 \ifnum\pgfcircmathresult <356
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{north east}\else\def\pgf@circ@dir{south west}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult <5
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{north}\else\def\pgf@circ@dir{south}
        \fi
        \fi
        \ifnum\pgfcircmathresult >355
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{north}\else\def\pgf@circ@dir{south}
        \fi
    \fi

    \ifpgf@circuit@bipole@current@below
        \def\pgf@circ@bipole@current@label@where{-90}
    \else
        \def\pgf@circ@bipole@current@label@where{+90}
    \fi
    }

    \pgfextra{\def\pgf@temp{short}\edef\pgf@circ@temp{\ctikzvalof{bipole/kind}}}
    \ifx\pgf@circ@temp\pgf@temp%draw current at a short at middle of the line
        (\tikztostart)--(\tikztotarget)
    \else% normal bipole or source
        \ifpgf@circuit@bipole@current@before
            (\tikztostart)--(anchorstartnode)
        \else
            (anchorendnode)--(\tikztotarget)
        \fi
    \fi
    \ifpgf@circuit@bipole@current@backward
        \pgfextra{
            \pgfmathsubtract{\pgf@circ@ffffff}{180}
            \edef\pgf@circ@ffffff{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
        }
    \fi
    coordinate[currarrow,pos=\ctikzvalof{current/distance},rotate=\pgf@circ@ffffff,
    anchor=center](Iarrow)
    (Iarrow.\pgf@circ@bipole@current@label@where)
    node[anchor=\pgf@circ@dir, \circuitikzbasekey/bipole current style]
    (\ctikzvalof{bipole/name}current){\pgf@circ@finallabels{current/label}}
}

\endinput


==> pgfcircflow.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% flow handling

%% styles
\ctikzset{bipole flow style/.style={}}
\tikzset{bipole flow style/.code={
        \ctikzset{bipole flow style/.style={#1}}
}}
\tikzset{bipole flow append style/.code={
        \ctikzset{bipole flow style/.append style={#1}}
}}

%% Options
\ctikzset{f^>/.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = forward,
        \circuitikzbasekey/bipole/flow/x position = after,
        \circuitikzbasekey/bipole/curflowrent/y position = above
    }
}

\ctikzset{f_>/.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = forward,
        \circuitikzbasekey/bipole/flow/x position = after,
        \circuitikzbasekey/bipole/flow/y position = below
    }
}

\ctikzset{f>^/.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = forward,
        \circuitikzbasekey/bipole/flow/x position = before,
        \circuitikzbasekey/bipole/flow/y position = above
    }
}

\ctikzset{f>_/.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = forward,
        \circuitikzbasekey/bipole/flow/x position = before,
        \circuitikzbasekey/bipole/flow/y position = below
    }
}

\ctikzset{f^</.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = backward,
        \circuitikzbasekey/bipole/flow/x position = after,
        \circuitikzbasekey/bipole/flow/y position = above
    }
}

\ctikzset{f_</.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = backward,
        \circuitikzbasekey/bipole/flow/x position = after,
        \circuitikzbasekey/bipole/flow/y position = below
    }
}

\ctikzset{f<^/.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = backward,
        \circuitikzbasekey/bipole/flow/x position = before,
        \circuitikzbasekey/bipole/flow/y position = above
    }
}

\ctikzset{f<_/.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = backward,
        \circuitikzbasekey/bipole/flow/x position = before,
        \circuitikzbasekey/bipole/flow/y position = below
    }
}

\ctikzset{f</.style = { f = #1, \circuitikzbasekey/bipole/flow/direction = backward} }
\ctikzset{f_/.style = { f = #1, \circuitikzbasekey/bipole/flow/y position = below } }
\ctikzset{f>/.style = { f = #1, \circuitikzbasekey/bipole/flow/direction = forward } }
\ctikzset{f^/.style = { f = #1, \circuitikzbasekey/bipole/flow/y position = above } }

\ctikzset{f/.code = {
        \pgfkeys{\circuitikzbasekey/bipole/flow/direction = forward,
            \circuitikzbasekey/bipole/flow/x position = after,
        \circuitikzbasekey/bipole/flow/y position = above }
        \pgfkeys{/tikz/circuitikz/bipole/flow/label/name=#1}
        \ctikzsetvalof{bipole/flow/label/unit}{}
        \ifpgf@circ@siunitx
            \pgf@circ@handleSI{#1}
            \ifpgf@circ@siunitx@res
                \edef\pgf@temp{\pgf@circ@handleSI@val}
                \pgfkeyslet{/tikz/circuitikz/bipole/flow/label/name}{\pgf@temp}
                \edef\pgf@temp{\pgf@circ@handleSI@unit}
                \pgfkeyslet{/tikz/circuitikz/bipole/flow/label/unit}{\pgf@temp}
            \else
        \fi
        \else
    \fi
}
}

%% Output routine
\def\pgf@circ@drawflow{
    \pgfextra{
        \edef\pgf@circ@ffffff{\pgf@circ@direction}
        \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@ffffff\pgf@nil}

        \ifnum\pgfcircmathresult >4 \ifnum\pgfcircmathresult <86
                \ifpgf@circuit@bipole@flow@below
                        \def\pgf@circ@dir{north west} \else \def\pgf@circ@dir{south east}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult >85 \ifnum\pgfcircmathresult <95
                \ifpgf@circuit@bipole@flow@below
                        \def\pgf@circ@dir{west} \else \def\pgf@circ@dir{east}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult >94 \ifnum\pgfcircmathresult <176
                \ifpgf@circuit@bipole@flow@below
                         \def\pgf@circ@dir{south west}\else \def\pgf@circ@dir{north east}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult >175 \ifnum\pgfcircmathresult <185
                \ifpgf@circuit@bipole@flow@below
                          \def\pgf@circ@dir{south}\else\def\pgf@circ@dir{north}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult >184 \ifnum\pgfcircmathresult <266
                \ifpgf@circuit@bipole@flow@below
                         \def\pgf@circ@dir{south east}\else\def\pgf@circ@dir{north west}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult >265 \ifnum\pgfcircmathresult <275
                \ifpgf@circuit@bipole@flow@below
                         \def\pgf@circ@dir{east}\else \def\pgf@circ@dir{west}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult >274 \ifnum\pgfcircmathresult <356
                \ifpgf@circuit@bipole@flow@below
                          \def\pgf@circ@dir{north east}\else\def\pgf@circ@dir{south west}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult <5
                \ifpgf@circuit@bipole@flow@below
                         \def\pgf@circ@dir{north}\else\def\pgf@circ@dir{south}
                \fi
        \fi
        \ifnum\pgfcircmathresult >355
                \ifpgf@circuit@bipole@flow@below
                         \def\pgf@circ@dir{north}\else\def\pgf@circ@dir{south}
                \fi
        \fi

        \ifpgf@circuit@bipole@flow@below
                \def\pgf@circ@bipole@flow@label@where{-90}
        \else
                \def\pgf@circ@bipole@flow@label@where{+90}
        \fi
    }

    \pgfextra{\def\pgf@temp{short}\edef\pgf@circ@temp{\ctikzvalof{bipole/kind}}}
    \ifx\pgf@circ@temp\pgf@temp%draw flow at a short at middle of the line
        (\tikztostart)--(\tikztotarget)
    \else% normal bipole or source
        \ifpgf@circuit@bipole@flow@before
            (\tikztostart)--(anchorstartnode)
        \else
            (anchorendnode)--(\tikztotarget)
        \fi
    \fi
    \pgfextra{
        \ifpgf@circuit@bipole@flow@backward
            \ifpgf@circuit@bipole@flow@below
                \def\flow@offset{\ctikzvalof{flow/offset}\pgf@circ@Rlen}
            \else
                \def\flow@offset{-\ctikzvalof{flow/offset}\pgf@circ@Rlen}
            \fi
            \pgfmathsubtract{\pgf@circ@ffffff}{180}
            \edef\pgf@circ@ffffff{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
            \else
            \ifpgf@circuit@bipole@flow@below
                \def\flow@offset{-\ctikzvalof{flow/offset}\pgf@circ@Rlen}
            \else
                \def\flow@offset{\ctikzvalof{flow/offset}\pgf@circ@Rlen}
            \fi
        \fi
    }
    coordinate[flowarrow,pos=\ctikzvalof{flow/distance},rotate=\pgf@circ@ffffff,yshift=\flow@offset, anchor=center](Farrowpos)
    (Farrowpos.\pgf@circ@bipole@flow@label@where) node[anchor=\pgf@circ@dir, \circuitikzbasekey/bipole flow style]
    (\ctikzvalof{bipole/name}flow){\pgf@circ@finallabels{flow/label}}
}

\endinput


==> pgfcirclabel.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Bipole label positioning

%% bipole labels and annotation extra style

\ctikzset{bipole label style/.style={}}
\tikzset{bipole label style/.code={
        \ctikzset{bipole label style/.style={#1}}
}}
\tikzset{bipole label append style/.code={
        \ctikzset{bipole label style/.append style={#1}}
}}
\ctikzset{bipole annotation style/.style={}}
\tikzset{bipole annotation style/.code={
        \ctikzset{bipole annotation style/.style={#1}}
}}
\tikzset{bipole annotation append style/.code={
        \ctikzset{bipole annotation style/.append style={#1}}
}}

%% Options
\ctikzset{label/.style = { l=#1 } }
\ctikzset{l/.code = {
        \pgfkeys{/tikz/circuitikz/bipole/label/name=#1}
        \ctikzsetvalof{bipole/label/unit}{}
        \ifpgf@circ@siunitx
            \pgf@circ@handleSI{#1}
            \ifpgf@circ@siunitx@res
                \edef\pgf@temp{\pgf@circ@handleSI@val}
                \pgfkeyslet{/tikz/circuitikz/bipole/label/name}{\pgf@temp}
                \edef\pgf@temp{\pgf@circ@handleSI@unit}
                \pgfkeyslet{/tikz/circuitikz/bipole/label/unit}{\pgf@temp}
            \else
        \fi
        \else
    \fi
}}

\ctikzset{label above/.code = {
        l=#1,
    \circuitikzbasekey/bipole/label/position=90 }
}

\ctikzset{l^/.style = {
        l=#1,
    \circuitikzbasekey/bipole/label/position=90 }
}

\ctikzset{label below/.code = {
        l=#1,
    \circuitikzbasekey/bipole/label/position=-90 }
}

\ctikzset{l_/.style = {
        l=#1,
    \circuitikzbasekey/bipole/label/position=-90 }
}

\ctikzset{annotation/.style = { a=#1 } }
\ctikzset{a/.code = {
    \pgfkeys{/tikz/circuitikz/bipole/annotation/name=#1}
    \ctikzsetvalof{bipole/annotation/unit}{}
    \ifpgf@circ@siunitx
        \pgf@circ@handleSI{#1}
        \ifpgf@circ@siunitx@res
            \edef\pgf@temp{\pgf@circ@handleSI@val}
            \pgfkeyslet{/tikz/circuitikz/bipole/annotation/name}{\pgf@temp}
            \edef\pgf@temp{\pgf@circ@handleSI@unit}
            \pgfkeyslet{/tikz/circuitikz/bipole/annotation/unit}{\pgf@temp}
        \else
        \fi
    \else
    \fi
}}

\ctikzset{annotation above/.code = {
        a=#1,
    \circuitikzbasekey/bipole/annotation/position=90 }
}

\ctikzset{a^/.style = {
        a=#1,
    \circuitikzbasekey/bipole/annotation/position=90 }
}

\ctikzset{annotation below/.code = {
        a=#1,
    \circuitikzbasekey/bipole/annotation/position=-90 }
}
\ctikzset{a_/.style = {
        a=#1,
    \circuitikzbasekey/bipole/annotation/position=-90 }
}

% This is to adjust spacing for the labels so that they are not cramped on components
\def\pgf@circ@ls{.75ex} % labelspace to have just one point to change

\def\pgf@circ@drawlabels#1{
    \pgfextra{
        % This function will be called with argument #1 equal
        % to "label" or "annotation" form pgfcircpath.tex.
        % pgf@circ@direction is the direction of the path,
        % its value is set in pgfcircpath.tex
        \pgfmathsubtract{\pgf@circ@direction}{90}
        \pgfmathround{\pgfmathresult} % avoid precision loss errors
        \edef\pgf@circ@labanc{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}

        \edef\pgf@circ@temp{\ctikzvalof{bipole/#1/position}}
        \ifnum \pgf@circ@temp < 0
                \pgfmathadd{\pgf@circ@labanc}{180}
                \edef\pgf@circ@labanc{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
        \fi
        % \typeout{INI: TEMP\space\pgf@circ@temp\space LABANC\space\pgf@circ@labanc}
        %
        % normalize the angle values
        %
        \pgfmathmod{\pgf@circ@labanc}{360}
        \edef\pgf@circ@labanc{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
        %
        \ifpgf@circuit@bipole@inverted
                \pgfmathadd{\pgf@circ@temp}{180} %If shape is inverted, use opposite anchor
                \edef\pgf@circ@temp{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
        \fi
        %
        \ifnum \ctikzvalof{mirror value} = -1
                \pgfmathadd{\pgf@circ@temp}{180} %If shape is mirrored, use opposite anchor
                \edef\pgf@circ@temp{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
        \fi
        % \typeout{FIN: TEMP\space\pgf@circ@temp\space LABANC\space\pgf@circ@labanc}
    }
    %Firstly, place a coordinate directly at the edge of the shape
    (\ctikzvalof{bipole/name}.\pgf@circ@temp) coordinate (labelcoor)
    %now decide, which labels should be drawn
    \pgfextra{
            \edef\pgf@temp{\ctikzvalof{label/align}}
            \def\pgf@circ@temp{straight}
    }
    \ifx\pgf@temp\pgf@circ@temp %straight
            \pgf@circ@drawreglabels{#1}
    \else
            \pgfextra{\def\pgf@circ@temp{rotate}}
            \ifx\pgf@temp\pgf@circ@temp %rotate
                    \pgf@circ@drawrotlabels{#1}
            \else% smart
                    \pgf@circ@drawsmartlabels{#1}
            \fi
    \fi
}


\def\pgf@circ@drawsmartlabels#1{
    \pgfextra{
        \pgfmathmod{\pgf@circ@direction}{90}
        \edef\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
    }
    \ifnum \pgfcircmathresult > 20
    \ifnum \pgfcircmathresult < 70
        \pgf@circ@drawrotlabels{#1}
    \else
        \pgf@circ@drawreglabels{#1}
    \fi
    \else
        \pgf@circ@drawreglabels{#1}
    \fi
    }


\def\pgf@circ@drawrotlabels#1{
    \pgfextra{
        % scale the distances in function of zoom, so that they are not
        % dependent on it but on font size. Thanks to @marmot
        % https://tex.stackexchange.com/a/476018/38080
        % the coeffcient is adjusted so that the distance is more or less
        % the same for rotated labels and straight ones (although it will
        % depend on the font, so it's not exact).
        \pgfgettransformentries{\tmp}{\tmp}{\tmp}{\myscale}{\tmp}{\tmp}
        \pgfmathsetlength\pgf@circ@res@temp{1.5*\pgf@circ@ls/\myscale}
        \ifnum \ctikzvalof{bipole/#1/position}>0
        %we need some more space for placement below, due to mid-anchor
            \else % we do not have <= in \ifnum...
                \pgf@circ@res@temp=1.5\pgf@circ@res@temp
        \fi
        %Calculate rotation of the label from direction and strip decimals
        \edef\pgfcirclabrot{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
        % rotate the label at second or third quadrant:
        \ifnum \pgfcirclabrot > 90 \ifnum \pgfcirclabrot < 270
                \pgfmathsubtract{\pgf@circ@direction}{180}
                \edef\pgfcirclabrot{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
                %invert the space relationships due to rotated strings
                \ifnum \ctikzvalof{bipole/#1/position}>0
                        \pgf@circ@res@temp=1.5\pgf@circ@res@temp
                \fi
        \fi\fi
        \pgfmathparse{\ctikzvalof{bipole/#1/position}>0?\pgf@circ@direction+90:\pgf@circ@direction-90}
        \edef\pgf@circ@labposangle{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
    }
    % reset cm is not working correctly here
    (labelcoor)++(\pgf@circ@labposangle:\the\pgf@circ@res@temp) coordinate(labelcoor)
    node[anchor=mid, rotate=\pgfcirclabrot, \circuitikzbasekey/bipole #1 style]
    (\ctikzvalof{bipole/name}#1){\pgf@circ@finallabels{#1}}
}

\def\pgf@circ@drawreglabels#1{
    %Now calculate all shape positions
    %Use mid-anchor at x-axis and base-anchor at y-axis, respectively.
    %All points between will be addressed by angled-anchors:
    \pgfextra{
        % scale ex-distance to make it independent on scale
        % thanks @marmot see https://tex.stackexchange.com/a/476018/38080
        \pgfgettransformentries{\tmp}{\tmp}{\tmp}{\myscale}{\tmp}{\tmp}
        \pgfmathsetlength\pgf@circ@res@temp{\pgf@circ@ls/\myscale}
        \pgfmathadd{\pgf@circ@labanc}{90}
        \pgfmathround{\pgfmathresult}
        \def\pgf@circ@labanctext{\pgf@circ@labanc}
        \edef\pgf@circ@temp{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
        \pgfmathparse{mod(\pgf@circ@temp,180)>135?mod(\pgf@circ@temp,180)-180:mod(\pgf@circ@temp,180)}
        \edef\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
    }
    %Values around 90 are at both y-axis
    \ifnum \pgfcircmathresult > 84 \ifnum \pgfcircmathresult< 96
        \pgfextra{\edef\pgf@circ@labpos{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}}
        \ifnum \pgf@circ@labpos > 180
            \ifnum \ctikzvalof{bipole/#1/position} > 0
                    \pgfextra{\def\pgf@circ@labanctext{mid west}}
            \else
                    \pgfextra{\def\pgf@circ@labanctext{mid east}}
            \fi
        \else
            \ifnum \ctikzvalof{bipole/#1/position} > 0
                    \pgfextra{\def\pgf@circ@labanctext{mid east}}
            \else
                    \pgfextra{\def\pgf@circ@labanctext{mid west}}
            \fi
        \fi
    \fi\fi
    %Values between -5 and 5 are at pos /neg x-axis
    \pgfextra{\def\uffa{}\newdimen\realshift\realshift=\dimexpr1pt\relax}
        \ifnum \pgfcircmathresult <6 \ifnum \pgfcircmathresult > -6
            \ifnum \ctikzvalof{bipole/#1/position} < 0
                \ifnum \pgf@circ@labanc > 90
                    % using base coordinate instead of south to naturally align
                    % symbols with descendants; but this invalidate the effect of
                    % the inner sep, so recover it by shifting the anchor
                    % reset cm is not working sometime, use @marmot solution
                    % see https://tex.stackexchange.com/a/476018/38080
                    (labelcoor) ++(-\pgf@circ@labanc:\pgf@circ@res@temp) coordinate(labelcoor)
                    \pgfextra{\def\pgf@circ@labanctext{base}}%base
                \else
                    \pgfextra{\def\pgf@circ@labanctext{north}}%north
                \fi
             \else
                \ifnum \pgf@circ@labanc < 90
                    % shift, as above
                    (labelcoor) ++(-\pgf@circ@labanc:\pgf@circ@res@temp) coordinate(labelcoor)
                    \pgfextra{\def\pgf@circ@labanctext{base}}%base
                \else
                    \ifnum \pgf@circ@labanc > 180
                        % this shouldn't  happen, but somehow it does (270 degree anchors)
                        % shift, as above
                        (labelcoor) ++(-\pgf@circ@labanc:\pgf@circ@res@temp) coordinate(labelcoor)
                         \pgfextra{\def\pgf@circ@labanctext{base}}%base
                    \else
                      \pgfextra{\def\pgf@circ@labanctext{north}}%north
                   \fi
                \fi
            \fi
        \fi\fi
    (labelcoor) node[anchor=\pgf@circ@labanctext,
    inner sep=0.5\pgf@circ@res@temp, outer sep=0pt, \circuitikzbasekey/bipole #1 style,
        ](\ctikzvalof{bipole/name}#1){\strut\pgf@circ@finallabels{#1}%
    }
}

\def\pgf@circ@finallabels#1{%
    \edef\pgf@temp{}%
    \edef\pgf@circ@temp{\ctikzvalof{bipole/#1/unit}}%
    \ifx\pgf@temp\pgf@circ@temp%
        \ctikzvalof{bipole/#1/name}%
    \else%
        $\SI{\ctikzvalof{bipole/#1/name}}{\ctikzvalof{bipole/#1/unit}}$%
    \fi%
}

\ctikzset{text/.style={t=#1}}
\ctikzset{t/.code={%
        \ctikzsetvalof{bipoles/twoport/text}{#1}%
}}

%%%% Stacked labels
%
% stacked labels by Romano Giannetti romano@rgtti.com
% heavily based on Claudo Fiandrinos's https://tex.stackexchange.com/a/65792/38080
% \expandafter trick inspired by Matthew Leingang's https://tex.stackexchange.com/a/12272/38080
%
% labels are in a tabular, globally aligned:
%        vertically with key l2 valign (default c)
%        c: center t: top b: bottom
%        horizontally with key l2 align (default l)
%        l: left c: centered r: right
% you can switch sides using l2_=... and l2^=...
% syntax is l2_ = line1 and line2 (same for l2^)
%
\ctikzset{%
    l2 valign/.store in=\ltwo@valign, l2 valign=c,
    l2 halign/.store in=\ltwo@halign, l2 halign=l,
}
\ctikzset{l2base/.code n args={2}{
  \pgfkeys{/tikz/circuitikz/bipole/label/name=%
        \bgroup
        \setlength{\tabcolsep}{2pt}%
        \def\ltwo@tabu{\tabular[\ltwo@valign]}%
        \expandafter\ltwo@tabu\expandafter{\ltwo@halign}%
        #1\\ #2%
        \endtabular
        \egroup
    }%
    \ctikzsetvalof{bipole/label/unit}{}
    \ifpgf@circ@siunitx
        \pgf@circ@handleSI{#2}
        \ifpgf@circ@siunitx@res
            \edef\pgf@temp{\pgf@circ@handleSI@val}
            \pgfkeyslet{/tikz/circuitikz/bipole/label/name}{\pgf@temp}
            \edef\pgf@temp{\pgf@circ@handleSI@unit}
            \pgfkeyslet{/tikz/circuitikz/bipole/label/unit}{\pgf@temp}
        \else
        \fi
    \else
    \fi
}}
\ctikzset{l2/.style args={#1 and #2}{
        l2base={#1}{#2},
    \circuitikzbasekey/bipole/label/position=90 }
}
\ctikzset{l2 above/.style args={#1 and #2}{
        l2base={#1}{#2},
    \circuitikzbasekey/bipole/label/position=90 }
}
\ctikzset{l2^/.style args={#1 and #2}{
        l2base={#1}{#2},
    \circuitikzbasekey/bipole/label/position=90 }
}
\ctikzset{l2 below/.style args={#1 and #2}{
        l2base={#1}{#2},
    \circuitikzbasekey/bipole/label/position=-90 }
}
\ctikzset{l2_/.style args={#1 and #2}{
        l2base={#1}{#2},
    \circuitikzbasekey/bipole/label/position=-90 }
}

\endinput


==> pgfcircmonopoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Monopoles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%
%% Grounds
%%%%%%%%%%%%%


%% Ground symbol
% #1 -> name
% #2 -> width
% #3 -> depth
% #4 -> code
\long\def\pgf@circ@declareground#1#2#3#4{
    \pgfdeclareshape{#1}{
        \savedmacro{\ctikzclass}{\edef\ctikzclass{grounds}}  % class of these components
        \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
        \savedanchor{\southeast}{
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@x=\ctikzvalof{monopoles/ground/width}\pgf@circ@scaled@Rlen
            \pgf@x=#2\pgf@x
            \pgf@y=\ctikzvalof{monopoles/ground/width}\pgf@circ@scaled@Rlen
            \pgf@y=-#3\pgf@y
        }
        \anchor{north}{\pgfpointorigin}
        \anchor{north east}{\southeast\pgf@y=0pt\relax}
        \anchor{east}{\southeast\pgf@y=.5\pgf@y}
        \anchor{south east}{\southeast}
        \anchor{south}{\southeast\pgf@x=0pt\relax}
        \anchor{south west}{\southeast\pgf@x=-\pgf@x}
        \anchor{west}{\southeast\pgf@y=.5\pgf@y\pgf@x=-\pgf@x}
        \anchor{north west}{\southeast\pgf@y=0pt\pgf@x=-\pgf@x}
        \anchor{left}{\pgfpointorigin}
        \anchor{right}{\pgfpointorigin}
        \anchor{center}{\pgfpointorigin}
        \behindforegroundpath{
            \pgf@circ@scaled@Rlen=\scaledRlen
            \pgf@circ@res@step=\ctikzvalof{monopoles/ground/width}\pgf@circ@scaled@Rlen
            \pgfscope
                \pgfstartlinewidth=\pgflinewidth
                #4
            \endpgfscope
        }
    }
}


\pgf@circ@declareground{ground}{0.6}{1.6}{
    \pgfsetlinewidth{\ctikzvalof{monopoles/ground/connectionthickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-1.2\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgf@circ@setlinewidth{monopoles/ground}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.4\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.25\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
    \pgfusepath{draw}
}

\pgf@circ@declareground{tlground}{0.6}{0.4}{
    \pgf@circ@setlinewidth{monopoles/ground}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{0pt}}
    \pgfpathmoveto{\pgfpoint{-.4\pgf@circ@res@step}{-0.2\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@step}{-0.2\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.25\pgf@circ@res@step}{-0.4\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@step}{-0.4\pgf@circ@res@step}}
    \pgfusepath{draw}
}


\pgf@circ@declareground{rground}{0.6}{1}{
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfstartlinewidth=\pgflinewidth
    \pgf@circ@setlinewidth{monopoles/rground}{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfsetroundcap\pgfusepath{draw}
}

\pgf@circ@declareground{tground}{0.6}{0}{
    \pgfpathmoveto{\pgfpointorigin}
    \pgfusepath{draw}

    \pgfstartlinewidth=\pgflinewidth
    \pgf@circ@setlinewidth{monopoles/tground}{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{0pt}}
    \pgfusepath{draw}
}

\pgf@circ@declareground{sground}{0.6}{1.8}{
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfstartlinewidth=\pgflinewidth
    \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0}{-1.8\pgf@circ@res@step}}
    \pgfpathclose
    \pgf@circ@draworfill
}

% noiseless ground
\pgf@circ@declareground{nground}{0.9}{1.6}{
    \pgfsetlinewidth{\ctikzvalof{monopoles/ground/connectionthickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-1.2\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgf@circ@setlinewidth{monopoles/ground}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.4\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.25\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.9\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
    \pgfpatharc{0}{180}{0.9\pgf@circ@res@step}
    \pgfusepath{draw}
}

% protective ground
\pgf@circ@declareground{pground}{0.9}{1.8}{
    \pgf@circ@setlinewidth{monopoles/ground}{\pgfstartlinewidth}
    \pgfpathcircle{\pgfpoint{0pt}{-0.9\pgf@circ@res@step}}{0.9\pgf@circ@res@step}
    \pgf@circ@draworfill
    \pgfsetlinewidth{\ctikzvalof{monopoles/ground/connectionthickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-1\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgf@circ@setlinewidth{monopoles/ground}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.4\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.25\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
    \pgfusepath{draw}
}

% chassis ground
\pgf@circ@declareground{cground}{1}{2}{
    \pgfsetlinewidth{\ctikzvalof{monopoles/ground/connectionthickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-1.5\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgf@circ@setlinewidth{monopoles/ground}{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-1.00\pgf@circ@res@step}{-2.10\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{-0.75\pgf@circ@res@step}{-1.50\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{ 0.75\pgf@circ@res@step}{-1.50\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{ 0.50\pgf@circ@res@step}{-2.10\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{ 0.00\pgf@circ@res@step}{-1.50\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{-0.25\pgf@circ@res@step}{-2.10\pgf@circ@res@step}}
    \pgfusepath{draw}
}

% Contributed by @fotesan https://github.com/fotesan
% european ground
\pgf@circ@declareground{eground}{1.1}{1.7}{
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfstartlinewidth=\pgflinewidth
    \pgf@circ@setlinewidth{monopoles/tground}{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{-1\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{1\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-1.1\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{-.6\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{-.1\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.1\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.9\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfusepath{draw}
}

\pgf@circ@declareground{eground2}{1.1}{1.7}{
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfstartlinewidth=\pgflinewidth
    \pgf@circ@setlinewidth{monopoles/tground}{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{-1\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{1\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-1.1\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{-.4\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.45\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.9\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfusepath{draw}
}

%%%%%%%%%%%%%%%%%%
%% Power supplies
%%%%%%%%%%%%%%%%%%

% Vcc
\pgfdeclareshape{vcc}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{power supplies}}  % class of these components
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \saveddimen{\scaledwidth}{% thanks to @Schrödinger's cat on https://tex.stackexchange.com/a/506249/38080
        \pgfgettransformentries{\tmpa}{\tmpb}{\tmpc}{\tmpd}{\tmp}{\tmp}%
        \pgfmathsetmacro{\gscale}{sqrt(abs(\tmpa*\tmpd-\tmpb*\tmpc))}% abs should not be needed
        \pgfmathsetlength{\pgf@x}{(\ctikzvalof{\ctikzclass/scale}*\gscale*\ctikzvalof{monopoles/vcc/width})*\pgf@circ@Rlen}%
    }
    \savedanchor{\northeast}{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@circ@res@step
        \pgf@y=3\pgf@x%
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0.5\pgf@y\relax}
    \anchor{south}{\pgfpointorigin}
    \anchor{west}{\northeast\pgf@y=0.5\pgf@y\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=0pt\relax}
    \anchor{south west}{\northeast\pgf@y=0pt\pgf@x=-\pgf@x}
    \anchor{center}{\pgfpointorigin}
    \anchor{left}{\pgfpointorigin}
    \anchor{right}{\pgfpointorigin}
    \anchor{text}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@scaled@Rlen
        \pgfpathmoveto{\pgfpoint{-.5\wd\pgfnodeparttextbox}{2\pgf@circ@res@step+2\ht\pgfnodeparttextbox}}
        \pgfpathmoveto{\pgfpoint{.5\wd\pgfnodeparttextbox}{2\pgf@circ@res@step+2\ht\pgfnodeparttextbox}}
        \pgf@x=0pt
        \pgf@y=2\pgf@circ@res@step
        \advance \pgf@y by 0.5\ht\pgfnodeparttextbox
        \pgf@x=-.5\wd\pgfnodeparttextbox
    }
    \behindforegroundpath{
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@scaled@Rlen
        \pgfscope
            \edef\pgf@circ@temp{\ctikzvalof{monopoles/vcc/arrow}}\edef\pgf@temp{legacy}
            \ifx\pgf@temp\pgf@circ@temp
                \pgfstartlinewidth=\pgflinewidth
                \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

                \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{.8\pgf@circ@res@step}}
                \pgfpathlineto{\pgfpoint{0}{1.5\pgf@circ@res@step}}
                \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{.8\pgf@circ@res@step}}
                \pgfusepath{draw}

                \pgfsetlinewidth{\pgfstartlinewidth}
            \else
            \pgfsetarrowsend{\pgf@circ@temp}
        \fi
        \pgfpathmoveto{\pgfpointorigin}
        \pgfpathlineto{\pgfpoint{0pt}{1.5\pgf@circ@res@step}}
        \pgfusepath{draw}
    \endpgfscope
    }
}

% Vee
\pgfdeclareshape{vee}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{power supplies}}  % class of these components
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \saveddimen{\scaledwidth}{% thanks to @Schrödinger's cat on https://tex.stackexchange.com/a/506249/38080
        \pgfgettransformentries{\tmpa}{\tmpb}{\tmpc}{\tmpd}{\tmp}{\tmp}%
        \pgfmathsetmacro{\gscale}{sqrt(abs(\tmpa*\tmpd-\tmpb*\tmpc))}% abs should not be needed
        \pgfmathsetlength{\pgf@x}{(\ctikzvalof{\ctikzclass/scale}*\gscale*\ctikzvalof{monopoles/vcc/width})*\pgf@circ@Rlen}%
    }
    \savedanchor{\northeast}{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@circ@res@step
        \pgf@y=-3\pgf@x%
    }
    \anchor{south}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0.5\pgf@y\relax}
    \anchor{north}{\pgfpointorigin}
    \anchor{west}{\northeast\pgf@y=0.5\pgf@y\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast}
    \anchor{south west}{\northeast\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast\pgf@y=0pt\relax}
    \anchor{north west}{\northeast\pgf@y=0pt\pgf@x=-\pgf@x}
    \anchor{center}{\pgfpointorigin}
    \anchor{left}{\pgfpointorigin}
    \anchor{right}{\pgfpointorigin}
    \anchor{text}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@scaled@Rlen
        \pgfpathmoveto{\pgfpoint{-.5\wd\pgfnodeparttextbox}{-2\pgf@circ@res@step-2\ht\pgfnodeparttextbox}}
        \pgfpathmoveto{\pgfpoint{.5\wd\pgfnodeparttextbox}{-2\pgf@circ@res@step-2\ht\pgfnodeparttextbox}}
        \pgf@x=0pt
        \pgf@y=-2\pgf@circ@res@step
        \advance \pgf@y by -1.5\ht\pgfnodeparttextbox
        \pgf@x=-.5\wd\pgfnodeparttextbox
    }

    \behindforegroundpath{
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@scaled@Rlen
        \pgfscope
            \edef\pgf@circ@temp{\ctikzvalof{monopoles/vee/arrow}}\edef\pgf@temp{legacy}
            \ifx\pgf@temp\pgf@circ@temp

                \pgfstartlinewidth=\pgflinewidth
                \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}

                \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-.8\pgf@circ@res@step}}
                \pgfpathlineto{\pgfpoint{0}{-1.5\pgf@circ@res@step}}
                \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{-.8\pgf@circ@res@step}}
                \pgfusepath{draw}
                \pgfsetlinewidth{\pgfstartlinewidth}
            \else
                \pgfsetarrowsend{\pgf@circ@temp}
            \fi
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathlineto{\pgfpoint{0pt}{-1.5\pgf@circ@res@step}}
            \pgfusepath{draw}
        \endpgfscope
    }
}

%%%%%%%%%%%%%%%%
%% RF elements
%%%%%%%%%%%%%%%%

% Legacy tlinestub
% Contributed by Leonardo Azzinnari
\pgfdeclareshape{tlinestub}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{RF}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor{\northeast}{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step = \ctikzvalof{bipoles/tline/width} \pgf@circ@scaled@Rlen
        \pgf@x=1.2\pgf@circ@res@step
        \pgf@circ@res@step = \ctikzvalof{bipoles/tline/width} \pgf@circ@scaled@Rlen
        \pgf@y=.2\pgf@circ@res@step%
    }
    % the center is on the left side of the shape for facility of usage
    \anchor{north}{\northeast\pgf@x=0.5\pgf@x\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0.5\pgf@x\relax}
    \anchor{west}{\pgfpointorigin}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=0cm\relax}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south west}{\northeast\pgf@x=0cm\pgf@y=-\pgf@y}
    \anchor{center}{\pgfpointorigin}
    \behindforegroundpath{
        \pgfstartlinewidth=\pgflinewidth

        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step=\ctikzvalof{bipoles/tline/width} \pgf@circ@scaled@Rlen
        \pgf@circ@res@step=0.6\pgf@circ@scaled@Rlen

        \pgfscope\begin{pgftransparencygroup}
            \pgfpathellipse{\pgfpoint{0.5\pgf@circ@res@step}{0\pgf@circ@res@step}}{\pgfpoint{0.125\pgf@circ@res@step}{0\pgf@circ@res@step}}{\pgfpoint{0\pgf@circ@res@step}{0.25\pgf@circ@res@step}}
            \pgf@circ@maybefill
            \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@step}{0.25\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{1.5\pgf@circ@res@step}{0.25\pgf@circ@res@step}}
            \pgfpatharc{90}{-90}{0.125\pgf@circ@res@step and 0.25\pgf@circ@res@step}
            \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{-0.25\pgf@circ@res@step}}
            \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \pgf@circ@draworfill
            \pgfpathellipse{\pgfpoint{0.5\pgf@circ@res@step}{0\pgf@circ@res@step}}{\pgfpoint{0.125\pgf@circ@res@step}{0\pgf@circ@res@step}}{\pgfpoint{0\pgf@circ@res@step}{0.25\pgf@circ@res@step}}
            \pgfusepath{draw}
        \end{pgftransparencygroup} \endpgfscope
        \pgfpathmoveto{\pgfpointorigin}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{0pt}}
        \pgfusepath{draw}
    }
}

%% New antennas without tails

% main body of antennas
\def\pgf@circ@antennabody{%
    \pgfstartlinewidth=\pgflinewidth
    \pgf@circ@scaled@Rlen=\scaledRlen
    \pgfsetcolor{\ctikzvalof{color}}
    \pgf@circ@res@step=\ctikzvalof{monopoles/bareantenna/width}\pgf@circ@scaled@Rlen
    \pgfscope
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpointorigin}
        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{2\pgf@circ@res@step}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{2\pgf@circ@res@step}}
        \pgfsetbeveljoin
        \pgfpathclose
        \pgf@circ@draworfill
    \endpgfscope
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{2\pgf@circ@res@step}}
    \pgfusepath{draw}
}

% Waves for the antennas.
\def\pgf@circ@antennawaves{%
    \pgfscope
    % define a triangle for clipping the waves
    \pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{4.2\pgf@circ@res@step}{3\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{4.2\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathclose
    \pgfusepath{clip}
    % ...and build the waves as clipped circles
    \pgf@circ@count@a=8\pgf@circ@res@other=0.5\pgf@circ@res@step
    \pgfmathloop%
    \ifnum\pgf@circ@count@a>2
        \pgfpathcircle{\pgfpoint{0pt}{\pgf@circ@res@step}}{\the\pgf@circ@count@a*\pgf@circ@res@other}
        \advance\pgf@circ@count@a-1\relax%
        \repeatpgfmathloop
        \pgfusepath{draw}
    \endpgfscope
}

% additional shape with the waves
\pgfdeclareshape{waves}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{RF}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/waves/width}\pgf@circ@scaled@Rlen
        \pgf@x=\pgf@circ@res@step
        \pgf@y=\pgf@circ@res@step
    }
    \anchor{text}{
        \northeast
        \pgf@y=\dimexpr\pgf@y+.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax
    }
    \anchor{top}{\northeast\pgf@x=0pt}
    \anchor{right}{\northeast\pgf@y=0pt}
    \anchor{left}{\northeast\pgf@x=-\pgf@x\pgf@y=0pt}
    \anchor{bottom}{\northeast\pgf@y=-\pgf@y\pgf@x=0pt}
    \anchor{north}{\northeast\pgf@x=0pt}
    \anchor{north east}{\northeast}
    \anchor{east}{\northeast\pgf@y=0pt}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south}{\northeast\pgf@y=-\pgf@y\pgf@x=0pt}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \anchor{west}{\northeast\pgf@x=-\pgf@x\pgf@y=0pt}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \behindforegroundpath{
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step=\ctikzvalof{monopoles/waves/width}\pgf@circ@scaled@Rlen
        \pgf@circ@res@step=0.5\pgf@circ@res@step
        \pgfsetcolor{\ctikzvalof{color}}
        \pgfscope
        % define a triangle for clipping the waves
        \pgfpathmoveto{\pgfpoint{-2\pgf@circ@res@step}{0pt}}
        \pgfpathlineto{\pgfpoint{2.1\pgf@circ@res@step}{2\pgf@circ@res@step}}
        \pgfpathlineto{\pgfpoint{2.1\pgf@circ@res@step}{-2\pgf@circ@res@step}}
        \pgfpathclose
        \pgfusepath{clip}
        % ...and build the waves as clipped circles
        \c@pgf@counta=8\pgf@circ@res@other=0.5\pgf@circ@res@step
        \pgfmathloop%
        \ifnum\c@pgf@counta>1
            \pgfpathcircle{\pgfpoint{-2\pgf@circ@res@step}{0pt}}{\the\c@pgf@counta*\pgf@circ@res@other}
            \advance\c@pgf@counta-1\relax%
            \repeatpgfmathloop
            \pgfusepath{draw}
        \endpgfscope
    }
}

% the three types of antennas: simple, TX, RX. Notice that you can flip them...

\pgfdeclareshape{bareantenna}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{RF}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/bareantenna/width}\pgf@circ@scaled@Rlen
        \pgf@x=\pgf@circ@res@step
        \pgf@y=2\pgf@circ@res@step
    }
    \anchor{text}{
        \northeast
        \pgf@x=\ctikzvalof{monopoles/bareantenna/label/xanchor}\pgf@x
        \pgf@y=\ctikzvalof{monopoles/bareantenna/label/yanchor}\pgf@y
        \pgf@y=\dimexpr\pgf@y+.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax
    }
    \anchor{top}{\northeast\pgf@x=0pt}
    \anchor{right}{\northeast\pgf@y=0.5\pgf@y}
    \anchor{left}{\northeast\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{bottom}{\pgfpointorigin}
    \anchor{north}{\northeast\pgf@x=0pt}
    \anchor{east}{\northeast\pgf@y=0.5\pgf@y}
    \anchor{west}{\northeast\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{south}{\pgfpointorigin}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=0pt\relax}
    \anchor{south west}{\northeast\pgf@y=0pt\pgf@x=-\pgf@x}
    \behindforegroundpath{
        \pgf@circ@antennabody
    }
}

\pgfdeclareshape{bareTXantenna}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{RF}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/bareantenna/width}\pgf@circ@scaled@Rlen
        \pgf@x=\pgf@circ@res@step
        \pgf@y=2\pgf@circ@res@step
    }
    \savedanchor{\savedwaves}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/bareantenna/width}\pgf@circ@scaled@Rlen
        \pgf@x=4.2\pgf@circ@res@step
        \pgf@y=\pgf@circ@res@step
    }
    \anchor{text}{
        \northeast
        \pgf@x=\ctikzvalof{monopoles/bareantenna/label/xanchor}\pgf@x
        \pgf@y=\ctikzvalof{monopoles/bareantenna/label/yanchor}\pgf@y
        \pgf@x=\dimexpr-\pgf@x-\wd\pgfnodeparttextbox\relax
        \pgf@y=\dimexpr\pgf@y+.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax
    }
    \anchor{waves}{\savedwaves}
    \anchor{top}{\northeast\pgf@x=0pt}
    \anchor{right}{\northeast\pgf@y=0.5\pgf@y}
    \anchor{left}{\northeast\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{bottom}{\pgfpointorigin}
    \anchor{north}{\northeast\pgf@x=0pt}
    \anchor{east}{\northeast\pgf@y=0.5\pgf@y}
    \anchor{west}{\northeast\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{south}{\pgfpointorigin}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=0pt\relax}
    \anchor{south west}{\northeast\pgf@y=0pt\pgf@x=-\pgf@x}
    \behindforegroundpath{
        \pgf@circ@antennabody
        \pgf@circ@antennawaves
    }
}

\pgfdeclareshape{bareRXantenna}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{RF}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/bareantenna/width}\pgf@circ@scaled@Rlen
        \pgf@x=\pgf@circ@res@step
        \pgf@y=2\pgf@circ@res@step
    }
    \savedanchor{\savedwaves}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/bareantenna/width}\pgf@circ@scaled@Rlen
        \pgf@x=-4.2\pgf@circ@res@step
        \pgf@y=\pgf@circ@res@step
    }
    \anchor{text}{
        \northeast
        \pgf@x=\ctikzvalof{monopoles/bareantenna/label/xanchor}\pgf@x
        \pgf@y=\ctikzvalof{monopoles/bareantenna/label/yanchor}\pgf@y
        \pgf@y=\dimexpr\pgf@y+.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax
    }
    \anchor{waves}{\savedwaves}
    \anchor{top}{\northeast\pgf@x=0pt}
    \anchor{right}{\northeast\pgf@y=0.5\pgf@y}
    \anchor{left}{\northeast\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{bottom}{\pgfpointorigin}
    \anchor{north}{\northeast\pgf@x=0pt}
    \anchor{east}{\northeast\pgf@y=0.5\pgf@y}
    \anchor{west}{\northeast\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{south}{\pgfpointorigin}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=0pt\relax}
    \anchor{south west}{\northeast\pgf@y=0pt\pgf@x=-\pgf@x}
    \behindforegroundpath{
        \pgf@circ@antennabody
        \pgftransformxshift{-5.2\pgf@circ@res@step}
        \pgf@circ@antennawaves
    }
}

% Microstrip monopoles

\pgfdeclareshape{mslstub}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{RF}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor{\southeast}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@x=\ctikzvalof{bipoles/mstline/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@y=\ctikzvalof{bipoles/mstline/height}\pgf@circ@scaled@Rlen
        \pgf@y=-.5\pgf@y
    }
    \savedanchor{\northwest}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@x=\ctikzvalof{bipoles/mstline/width}\pgf@circ@scaled@Rlen
        \pgf@x=-.5\pgf@x
        \pgf@y=\ctikzvalof{bipoles/mstline/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
    }
    \anchor{north}{\northwest\pgf@x=0pt\relax}
    \anchor{north east}{\northwest\pgf@x=-\pgf@x}
    \anchor{east}{\southeast\pgf@y=0pt\relax}
    \anchor{south east}{\southeast}
    \anchor{south}{\southeast\pgf@x=0pt\relax}
    \anchor{south west}{\southeast\pgf@x=-\pgf@x}
    \anchor{west}{\northwest\pgf@y=0pt\relax}
    \anchor{north west}{\northwest}
    %
    \anchor{center}{\northwest\pgf@y=0pt\relax}
    \anchor{left}{\northwest\pgf@y=0pt\relax}
    \anchor{right}{\southeast\pgf@y=0pt\relax}
    % put the node text above and centered
    \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
    \behindbackgroundpath{
        \pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfextractx{\pgf@circ@res@right}{\southeast}
        \pgfextractx{\pgf@circ@res@left}{\northwest}
        \pgfextracty{\pgf@circ@res@down}{\southeast}
        \pgfmathsetlength{\pgf@circ@res@step}{0.25*\pgf@circ@res@up}
        \pgfstartlinewidth=\pgflinewidth
        \pgfscope
            \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgf@circ@draworfill
        \endpgfscope
    }
}

\pgfdeclareshape{msrstub}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{RF}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor{\southeast}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@x=\ctikzvalof{monopoles/msrstub/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@y=0pt\relax
    }
    \savedanchor{\northwest}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@x=\ctikzvalof{monopoles/msrstub/width}\pgf@circ@scaled@Rlen
        \pgf@x=-.5\pgf@x
        \pgf@y=\ctikzvalof{monopoles/msrstub/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
    }
    \anchor{north}{\northwest\pgf@x=0pt\relax}
    \anchor{north east}{\northwest\pgf@x=-\pgf@x}
    \anchor{east}{\southeast\pgf@y=0pt\relax}
    \anchor{south east}{\southeast}
    \anchor{south}{\southeast\pgf@x=0pt\relax}
    \anchor{south west}{\southeast\pgf@x=-\pgf@x}
    \anchor{west}{\northwest\pgf@y=0pt\relax}
    \anchor{north west}{\northwest}
    %
    \anchor{center}{\pgfpointorigin}
    \anchor{left}{\pgfpointorigin}
    \anchor{right}{\pgfpointorigin}
    % put the node text above and centered
    \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
    \behindbackgroundpath{
        \pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfextractx{\pgf@circ@res@right}{\southeast}
        \pgfextractx{\pgf@circ@res@left}{\northwest}
        \pgfextracty{\pgf@circ@res@down}{\southeast}
        \pgfmathsetlength{\pgf@circ@res@step}{0.25*\pgf@circ@res@up}
        \pgfstartlinewidth=\pgflinewidth
        \pgfscope
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@step}}
            \pgfusepath{draw}
            \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpointpolar{135}{\pgf@circ@res@step}}
            \pgfpatharc{135}{45}{\pgf@circ@res@step}
            \pgfpathlineto{\pgfpointpolar{45}{\pgf@circ@res@up}}
            \pgfpatharc{45}{135}{\pgf@circ@res@up}
            \pgfclosepath
            \pgf@circ@draworfill
        \endpgfscope
    }
}

\pgfdeclareshape{msport}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{RF}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor{\southeast}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@x=\ctikzvalof{monopoles/msport/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@y=\ctikzvalof{bipoles/mstline/height}\pgf@circ@scaled@Rlen
        \pgf@y=-.5\pgf@y
    }
    \savedanchor{\northwest}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@x=\ctikzvalof{monopoles/msport/width}\pgf@circ@scaled@Rlen
        \pgf@x=-.5\pgf@x
        \pgf@y=\ctikzvalof{bipoles/mstline/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
    }
    \anchor{north}{\northwest\pgf@x=0pt\relax}
    \anchor{north east}{\northwest\pgf@x=-\pgf@x}
    \anchor{east}{\southeast\pgf@y=0pt\relax}
    \anchor{south east}{\southeast}
    \anchor{south}{\southeast\pgf@x=0pt\relax}
    \anchor{south west}{\southeast\pgf@x=-\pgf@x}
    \anchor{west}{\northwest\pgf@y=0pt\relax}
    \anchor{north west}{\northwest}
    %
    \anchor{center}{\northwest\pgf@y=0pt\relax}
    \anchor{left}{\northwest\pgf@y=0pt\relax}
    \anchor{right}{\southeast\pgf@y=0pt\relax}
    % put the node text above and centered
    \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{
            \dimexpr-.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax
        }
    }
    \behindbackgroundpath{
        \pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfextractx{\pgf@circ@res@right}{\southeast}
        \pgfextractx{\pgf@circ@res@left}{\northwest}
        \pgfextracty{\pgf@circ@res@down}{\southeast}
        \pgfmathsetlength{\pgf@circ@res@step}{0.5*\pgf@circ@res@up}
        \pgfstartlinewidth=\pgflinewidth
        \pgfscope
            \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@left+\pgf@circ@res@step}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@left+\pgf@circ@res@step}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope
    }
}

% Legacy antennas (with tails)
\def\pgf@circ@shift@antenna@xy#1#2{%
    \pgf@y=\dimexpr\pgf@y+#2\pgf@circ@res@step
    \pgf@x=\dimexpr\pgf@x+#1\pgf@circ@res@step
\relax}

% Legacy antenna
\pgfdeclareshape{antenna}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{RF}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/antenna/width}\pgf@circ@scaled@Rlen
        \pgf@x=\pgf@circ@res@step%-0.5\pgflinewidth
        \pgf@y=4\pgf@circ@res@step
    }
    \anchor{north}{\northeast\pgf@circ@res@step=\pgf@x\pgf@x=0cm\pgf@circ@shift@antenna@xy{0}{2}}
    \anchor{east}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=0cm\pgf@circ@shift@antenna@xy{0}{3}\relax}
    \anchor{south}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=-\pgf@y \pgf@x=0cm\pgf@circ@shift@antenna@xy{0}{4}\relax}
    \anchor{west}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=0cm\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{0}{3}}
    \anchor{north east}{\northeast\pgf@circ@res@step=\pgf@x\pgf@circ@shift@antenna@xy{0}{2}}
    \anchor{north west}{\northeast\pgf@circ@res@step=\pgf@x\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{0}{2}}
    \anchor{south east}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=-\pgf@y\pgf@circ@shift@antenna@xy{0}{4}}
    \anchor{south west}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=-\pgf@y\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{0}{4}}
    \anchor{text}{
        \northeast
        \pgf@x=\ctikzvalof{monopoles/antenna/label/xanchor}\pgf@x
        \pgf@y=\ctikzvalof{monopoles/antenna/label/yanchor}\pgf@y
    }
    \behindforegroundpath{
        \pgfstartlinewidth=\pgflinewidth
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step=\ctikzvalof{monopoles/antenna/width}\pgf@circ@scaled@Rlen

        \pgftransformxshift{ -4\pgf@circ@res@step }

        \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{0pt}}
        \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}

        \pgfusepath{draw}

        \pgfscope
            \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{5\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{4\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{3\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfsetcolor{\ctikzvalof{color}}
            \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \pgfusepath{draw}
        \endpgfscope
        \pgfsetlinewidth{\pgfstartlinewidth}

    }
}

% Legacy TX antenna
\pgfdeclareshape{txantenna}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{RF}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/antenna/width}\pgf@circ@scaled@Rlen
        \pgf@x=\pgf@circ@res@step%-0.5\pgflinewidth
        \pgf@y=4\pgf@circ@res@step
    }
    \anchor{north}{\northeast\pgf@circ@res@step=\pgf@x\pgf@x=0cm\pgf@circ@shift@antenna@xy{2}{2}}
    \anchor{east}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=0cm\pgf@circ@shift@antenna@xy{4}{3}\relax}
    \anchor{south}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=-\pgf@y \pgf@x=0cm\pgf@circ@shift@antenna@xy{2}{4}\relax}
    \anchor{west}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=0cm\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{1}{3}}
    \anchor{north east}{\northeast\pgf@circ@res@step=\pgf@x\pgf@circ@shift@antenna@xy{4}{2}}
    \anchor{north west}{\northeast\pgf@circ@res@step=\pgf@x\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{1}{2}}
    \anchor{south east}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=-\pgf@y\pgf@circ@shift@antenna@xy{4}{4}}
    \anchor{south west}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=-\pgf@y\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{1}{4}}
    \anchor{text}{
        \northeast
        \pgf@x=\ctikzvalof{monopoles/txantenna/label/xanchor}\pgf@x
        \pgf@y=\ctikzvalof{monopoles/txantenna/label/yanchor}\pgf@y
    }
    \behindforegroundpath{
        \pgfstartlinewidth=\pgflinewidth
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step=\ctikzvalof{monopoles/txantenna/width}\pgf@circ@scaled@Rlen

        \pgfpathmoveto{\pgfpointorigin}
        \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step}{0pt}}
        \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{0pt}}
        \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}

        \pgfusepath{draw}

        \pgfscope
            \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{5\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{4\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{3\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfsetcolor{\ctikzvalof{color}}
            \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \pgfusepath{draw}
        \endpgfscope
        \pgfpathmoveto{\pgfpoint{5.5\pgf@circ@res@step}{6\pgf@circ@res@step}}
        %        \pgfpatharc{60}{-60}{\pgf@circ@res@step and \pgf@circ@res@step}
        \pgfpatharc{30}{-30}{2\pgf@circ@res@step}         \pgfpathmoveto{\pgfpoint{6\pgf@circ@res@step}{6.25\pgf@circ@res@step}}
        \pgfpatharc{30}{-30}{2.5\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{6.5\pgf@circ@res@step}{6.5\pgf@circ@res@step}}
        \pgfpatharc{30}{-30}{3\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{7\pgf@circ@res@step}{6.75\pgf@circ@res@step}}
        \pgfpatharc{30}{-30}{3.5\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{7.5\pgf@circ@res@step}{7\pgf@circ@res@step}}
        \pgfpatharc{30}{-30}{4\pgf@circ@res@step}
        \pgfusepath{draw}
        \pgfsetlinewidth{\pgfstartlinewidth}

    }
}

% Legacy RX antenna
\pgfdeclareshape{rxantenna}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{RF}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step=\ctikzvalof{monopoles/antenna/width}\pgf@circ@scaled@Rlen
        \pgf@x=\pgf@circ@res@step%-0.5\pgflinewidth
        \pgf@y=4\pgf@circ@res@step
    }
    \anchor{north}{\northeast\pgf@circ@res@step=\pgf@x\pgf@x=0cm\pgf@circ@shift@antenna@xy{2}{2}}
    \anchor{east}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=0cm\pgf@circ@shift@antenna@xy{4}{3}\relax}
    \anchor{south}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=-\pgf@y \pgf@x=0cm\pgf@circ@shift@antenna@xy{2}{4}\relax}
    \anchor{west}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=0cm\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{1}{3}}
    \anchor{north east}{\northeast\pgf@circ@res@step=\pgf@x\pgf@circ@shift@antenna@xy{4}{2}}
    \anchor{north west}{\northeast\pgf@circ@res@step=\pgf@x\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{1}{2}}
    \anchor{south east}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=-\pgf@y\pgf@circ@shift@antenna@xy{4}{4}}
    \anchor{south west}{\northeast\pgf@circ@res@step=\pgf@x\pgf@y=-\pgf@y\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{1}{4}}
    \anchor{text}{
        \northeast
        \pgf@x=\ctikzvalof{monopoles/rxantenna/label/xanchor}\pgf@x
        \pgf@y=\ctikzvalof{monopoles/rxantenna/label/yanchor}\pgf@y
    }
    \behindforegroundpath{
        \pgfstartlinewidth=\pgflinewidth
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step=\ctikzvalof{monopoles/rxantenna/width}\pgf@circ@scaled@Rlen

        \pgfpathmoveto{\pgfpointorigin}
        \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step}{0pt}}
        \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{0pt}}
        \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}

        \pgfusepath{draw}

        \pgfscope
            \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{5\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{4\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{3\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfsetcolor{\ctikzvalof{color}}
            \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \pgfusepath{draw}
        \endpgfscope

        \pgfpathmoveto{\pgfpoint{6\pgf@circ@res@step}{7\pgf@circ@res@step}}
        %             \pgfpatharc{60}{-60}{\pgf@circ@res@step and \pgf@circ@res@step}
        \pgfpatharc{150}{210}{4\pgf@circ@res@step}              \pgfpathmoveto{\pgfpoint{6.5\pgf@circ@res@step}{6.75\pgf@circ@res@step}}
        \pgfpatharc{150}{210}{3.5\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{7\pgf@circ@res@step}{6.5\pgf@circ@res@step}}
        \pgfpatharc{150}{210}{3\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{7.5\pgf@circ@res@step}{6.25\pgf@circ@res@step}}
        \pgfpatharc{150}{210}{2.5\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{8\pgf@circ@res@step}{6\pgf@circ@res@step}}
        \pgfpatharc{150}{210}{2\pgf@circ@res@step}
        \pgfusepath{draw}
        \pgfsetlinewidth{\pgfstartlinewidth}
    }
}

% Legacy match
\pgfdeclareshape{match}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{RF}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor{\northeast}{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step = \ctikzvalof{monopoles/match/width} \pgf@circ@scaled@Rlen
        \pgf@x=2\pgf@circ@res@step
        \pgf@circ@res@step = \ctikzvalof{monopoles/match/width} \pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@circ@res@step%
    }
    % the center is on the left side of the shape for facility of usage
    \anchor{north}{\northeast\pgf@x=0.5\pgf@x\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=0pt\pgf@x=0.5\pgf@x\relax}
    \anchor{west}{\pgfpointorigin}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=0cm\relax}
    \anchor{south east}{\northeast\pgf@y=0pt\relax}
    \anchor{south west}{\pgfpointorigin}
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{text}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@x=\ctikzvalof{monopoles/match/width}\pgf@circ@scaled@Rlen
        \pgf@x=1.5\pgf@x
        \advance \pgf@x by -.5\wd\pgfnodeparttextbox
        \pgf@y=-1.5\ht\pgfnodeparttextbox
    }
    \behindforegroundpath{
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step=\ctikzvalof{monopoles/match/width}\pgf@circ@scaled@Rlen

        \pgfscope
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathlineto{\pgfpoint{2\pgf@circ@res@step}{0pt}}
            \pgfusepath{draw}

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{2\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{2\pgf@circ@res@step}{0}}
            \pgfusepath{fill}

            \pgfsetlinewidth{\pgfstartlinewidth}
        \endpgfscope
    }
}

\endinput


==> pgfcircmultipoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
% Copyright 2019 by Romano Giannetti
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Multipoles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%
%% Chips
%%%%%%%%%

% let's use the same shifts everywhere, no magic numbers
\def\pgf@circ@dip@pin@shift{0.5}
\def\pgf@circ@qfp@pin@shift{0.25}

% derived from https://tex.stackexchange.com/a/146753/38080
% original author Mark Wibrow
% Thanks also to John Kormylo https://tex.stackexchange.com/a/372996/38080
% a lot of thanks to @marmot  for the un-rotation hint
% https://tex.stackexchange.com/a/473571/38080

% DIP (dual in line package) chips

\pgfdeclareshape{dipchip}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{chips}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedmacro\numpins{%
            \pgf@circ@count@a=\ctikzvalof{multipoles/dipchip/num pins}%
            \def\numpins{\the\pgf@circ@count@a}
    }
    \savedanchor\centerpoint{%
        \pgf@x=-.5\wd\pgfnodeparttextbox%
        \pgf@y=-.5\ht\pgfnodeparttextbox%
        \advance\pgf@y by+.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\origin{\pgfpoint{0pt}{0pt}}
    \anchor{center}{\origin}
    \anchor{text}{\centerpoint}% to adjust text
    \saveddimen\height{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength\pgf@x{((\numpins)
        *\ctikzvalof{multipoles/dipchip/pin spacing})*\pgf@circ@scaled@Rlen/2}%
    }%
    \saveddimen{\chipspacing}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength\pgf@x{\pgf@circ@scaled@Rlen*\ctikzvalof{multipoles/dipchip/pin spacing}}}
    \saveddimen{\width}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength\pgf@x{\pgf@circ@scaled@Rlen*\ctikzvalof{multipoles/dipchip/width}}}
    \saveddimen{\extshift}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength\pgf@x{\pgf@circ@scaled@Rlen*\ctikzvalof{multipoles/external pins width}}}
    % standard anchors
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength\pgf@y{0.5*((\numpins)
        *\ctikzvalof{multipoles/dipchip/pin spacing})*\pgf@circ@scaled@Rlen/2}%
        \pgfmathsetlength\pgf@x{-0.5*\pgf@circ@scaled@Rlen*\ctikzvalof{multipoles/dipchip/width}}
    }
    \anchor{dot}{\northwest
        \pgfmathsetlength\pgf@x{\pgf@x + 0.3*\chipspacing}
        \pgfmathsetlength\pgf@y{\pgf@y - 0.3*\chipspacing}
    }
    \anchor{nw}{\northwest}
    \anchor{ne}{\northwest\pgf@x=-\pgf@x}
    \anchor{se}{\northwest\pgf@x=-\pgf@x\pgf@y=-\pgf@y}
    \anchor{sw}{\northwest\pgf@y=-\pgf@y}
    \anchor{north west}{\northwest}
    \anchor{north east}{\northwest\pgf@x=-\pgf@x}
    \anchor{south east}{\northwest\pgf@x=-\pgf@x \pgf@y=-\pgf@y}
    \anchor{south west}{\northwest\pgf@y=-\pgf@y}
    \anchor{n}{\northwest\pgf@x=0pt }
    \anchor{e}{\northwest\pgf@x=-\pgf@x\pgf@y=0pt }
    \anchor{s}{\northwest\pgf@x=0pt\pgf@y=-\pgf@y}
    \anchor{w}{\northwest\pgf@y=0pt }
    \anchor{north}{\northwest\pgf@x=0pt }
    \anchor{east}{\northwest\pgf@x=-\pgf@x\pgf@y=0pt }
    \anchor{south}{\northwest\pgf@x=0pt\pgf@y=-\pgf@y}
    \anchor{west}{\northwest\pgf@y=0pt }
    % start drawing
    \backgroundpath{%
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step = \ctikzvalof{multipoles/dipchip/pin spacing}\pgf@circ@scaled@Rlen
        \pgf@circ@res@other = \ctikzvalof{multipoles/external pins width}\pgf@circ@scaled@Rlen
        \pgfscope% (for the line width)
        \pgf@circ@setlinewidth{multipoles}{\pgflinewidth}
        \pgfpathrectanglecorners{\pgfpoint{-\width/2}{-\height/2}}{\pgfpoint{\width/2}{\height/2}}%
        \pgf@circ@draworfill
        %% upside mark
        \ifpgf@circuit@chip@topmark
            \pgfpathmoveto{\pgfpoint{0.2*\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpatharc{0}{180}{0.2*\pgf@circ@res@left}
        \fi
        \pgfusepath{stroke}%
        \pgfsetcolor{\ctikzvalof{color}}
        % Adding the pin number
        \ifpgf@circuit@chip@shownumbers
            \pgf@circ@count@a=\numpins\relax
            \divide\pgf@circ@count@a by 2 \pgf@circ@count@b=\pgf@circ@count@a
            % thanks to @marmot: https://tex.stackexchange.com/a/473571/38080
            \ifpgf@circuit@chip@straightnumbers
                \pgfgettransformentries\a\b\temp\temp\temp\temp
                \pgfmathsetmacro{\rot}{-atan2(\b,\a)}
                \pgfmathtruncatemacro{\quadrant}{mod(4+int(360+(\rot+45)/90),4)}
            \else
                \pgfmathsetmacro{\rot}{0}
                \pgfmathsetmacro{\quadrant}{0}
            \fi
            \def\pgf@circ@strut{\vrule width 0pt height 1em depth 0.4em\relax}
            \def\mytext{\ctikzvalof{multipoles/font}\space\pgf@circ@strut\the\pgf@circ@count@c\space}
            \pgfmathloop%
            \ifnum\pgf@circ@count@a>0
                \ifcase\quadrant % rotation 0
                    % left
                    \pgf@circ@count@c=\pgf@circ@count@a
                    \pgftext[left,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr2*\pgf@circ@count@b-\pgf@circ@count@a+1\relax
                    \pgftext[right,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                \or % rotation -90
                    % left
                    \pgf@circ@count@c=\pgf@circ@count@a
                    \pgftext[top,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr2*\pgf@circ@count@b-\pgf@circ@count@a+1\relax
                    \pgftext[bottom,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                \or %rotation 180
                    % left
                    \pgf@circ@count@c=\pgf@circ@count@a
                    \pgftext[right,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr2*\pgf@circ@count@b-\pgf@circ@count@a+1\relax
                    \pgftext[left,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                \or % rotation +90
                    % left
                    \pgf@circ@count@c=\pgf@circ@count@a
                    \pgftext[bottom,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr2*\pgf@circ@count@b-\pgf@circ@count@a+1\relax
                    \pgftext[top,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                \fi
                \advance\pgf@circ@count@a-1\relax%
                \repeatpgfmathloop
            \fi
            \endpgfscope
            \ifdim\pgf@circ@res@other>0pt
            \pgfscope
                \pgfsetlinewidth{\ctikzvalof{multipoles/external pins thickness}\pgflinewidth}
                \pgf@circ@count@a=\numpins\relax
                \divide\pgf@circ@count@a by 2 \pgf@circ@count@b=\pgf@circ@count@a
                \pgfmathloop%
                \ifnum\pgf@circ@count@a>0
                    \edef\padfrac{\ctikzvalof{multipoles/external pad fraction}}
                    \ifnum\padfrac>0
                        \pgf@circ@res@temp=\pgf@circ@res@step\divide\pgf@circ@res@temp by \padfrac
                        % left side pads
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@other}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@other}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        % right side pads
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgf@circ@res@other}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgf@circ@res@other}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                    \else
                        % left side pins
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@other}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        % right side pins
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgf@circ@res@other}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                    \fi
                    \advance\pgf@circ@count@a by -1\relax%
                \repeatpgfmathloop
                \pgfusepath{stroke}
            \endpgfscope
            \fi
        }%
        % \pgf@sh@s@<name of the shape here> contains all the code for the shape
        % and is executed just before a node is drawn.
        \pgfutil@g@addto@macro\pgf@sh@s@dipchip{%
            % Start with the maximum pin number and go backwards.
            \pgf@circ@count@a=\numpins\relax
            \pgfmathloop%
            \ifnum\pgf@circ@count@a>0
                % we will create two anchors per pin: the "normal one" like `pin 1` for the
                % electrical contact, and the "border one" like `bpin 1` for labels.
                % they will coincide if `external pins width` is set to 0.
                \expandafter\xdef\csname pgf@anchor@dipchip@pin\space\the\pgf@circ@count@a\endcsname{%
                    \noexpand\pgf@circ@dippinanchor{\the\pgf@circ@count@a}{1}%
                }
                \expandafter\xdef\csname pgf@anchor@dipchip@bpin\space\the\pgf@circ@count@a\endcsname{%
                    \noexpand\pgf@circ@dippinanchor{\the\pgf@circ@count@a}{0}%
                }
                \advance\pgf@circ@count@a by -1\relax%
                \repeatpgfmathloop%
            }%
        }

% QFP (quad flat package) chips

\pgfdeclareshape{qfpchip}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{chips}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedmacro\numpins{%
            \pgf@circ@count@a=\ctikzvalof{multipoles/qfpchip/num pins}%
            \def\numpins{\the\pgf@circ@count@a}
    }
    \savedanchor\centerpoint{%
        \pgf@x=-.5\wd\pgfnodeparttextbox%
        \pgf@y=-.5\ht\pgfnodeparttextbox%
        \advance\pgf@y by+.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\origin{\pgfpoint{0pt}{0pt}}
    \anchor{center}{\origin}
    \anchor{text}{\centerpoint}% to adjust text
    \saveddimen\height{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength\pgf@x{((\numpins+2)
        *\ctikzvalof{multipoles/qfpchip/pin spacing})*\pgf@circ@scaled@Rlen/4}%
    }%
    \saveddimen\width{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength\pgf@x{((\numpins+2)
        *\ctikzvalof{multipoles/qfpchip/pin spacing})*\pgf@circ@scaled@Rlen/4}%
    }%
    \saveddimen{\chipspacing}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength\pgf@x{\pgf@circ@scaled@Rlen*\ctikzvalof{multipoles/qfpchip/pin spacing}}}
    \saveddimen{\extshift}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength\pgf@x{\pgf@circ@scaled@Rlen*\ctikzvalof{multipoles/external pins width}}}
    % standard anchors
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength\pgf@y{0.5*((\numpins+2)
        *\ctikzvalof{multipoles/qfpchip/pin spacing})*\pgf@circ@scaled@Rlen/4}%
        \pgf@x=-\pgf@y
    }
    \anchor{dot}{\northwest
        \pgfmathsetlength\pgf@x{\pgf@x + 0.3*\chipspacing}
        \pgfmathsetlength\pgf@y{\pgf@y - 0.3*\chipspacing}
    }
    \anchor{nw}{\northwest}
    \anchor{ne}{\northwest\pgf@x=-\pgf@x}
    \anchor{se}{\northwest\pgf@x=-\pgf@x\pgf@y=-\pgf@y}
    \anchor{sw}{\northwest\pgf@y=-\pgf@y}
    \anchor{north west}{\northwest}
    \anchor{north east}{\northwest\pgf@x=-\pgf@x}
    \anchor{south east}{\northwest\pgf@x=-\pgf@x \pgf@y=-\pgf@y}
    \anchor{south west}{\northwest\pgf@y=-\pgf@y}
    \anchor{n}{\northwest\pgf@x=0pt }
    \anchor{e}{\northwest\pgf@x=-\pgf@x\pgf@y=0pt }
    \anchor{s}{\northwest\pgf@x=0pt\pgf@y=-\pgf@y}
    \anchor{w}{\northwest\pgf@y=0pt }
    \anchor{north}{\northwest\pgf@x=0pt }
    \anchor{east}{\northwest\pgf@x=-\pgf@x\pgf@y=0pt }
    \anchor{south}{\northwest\pgf@x=0pt\pgf@y=-\pgf@y}
    \anchor{west}{\northwest\pgf@y=0pt }
    % start drawing
    \backgroundpath{%
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step = \ctikzvalof{multipoles/qfpchip/pin spacing}\pgf@circ@scaled@Rlen
        \pgf@circ@res@other = \ctikzvalof{multipoles/external pins width}\pgf@circ@scaled@Rlen
        \pgfscope% (for the line width)
        \pgf@circ@setlinewidth{multipoles}{\pgflinewidth}
        %% upside mark
        \ifpgf@circuit@chip@topmark
            \pgfpathmoveto{\pgfpoint{-\width/2}{\height/2-\pgf@circ@res@step/2}}
            \pgfpathlineto{\pgfpoint{-\width/2+\pgf@circ@res@step/2}{\height/2}}
        \else
            \pgfpathmoveto{\pgfpoint{-\width/2}{\height/2}}
        \fi
        %% rest of the shape
        \pgfpathlineto{\pgfpoint{\width/2}{\height/2}}
        \pgfpathlineto{\pgfpoint{\width/2}{-\height/2}}
        \pgfpathlineto{\pgfpoint{-\width/2}{-\height/2}}
        \pgfpathclose
        \pgf@circ@draworfill
        % Adding the pin number
        \pgfsetcolor{\ctikzvalof{color}}
        \ifpgf@circuit@chip@shownumbers
            \pgf@circ@count@a=\numpins%
            \divide\pgf@circ@count@a by 4 \pgf@circ@count@b=\pgf@circ@count@a
            % thanks to @marmot: https://tex.stackexchange.com/a/473571/38080
            \ifpgf@circuit@chip@straightnumbers
                \pgfgettransformentries\a\b\temp\temp\temp\temp
                \pgfmathsetmacro{\rot}{-atan2(\b,\a)}
                \pgfmathtruncatemacro{\quadrant}{mod(4+int(360+(\rot+45)/90),4)}
            \else
                \pgfmathsetmacro{\rot}{0}
                \pgfmathsetmacro{\quadrant}{0}
            \fi
            \def\pgf@circ@strut{\vrule width 0pt height 1em depth 0.4em\relax}
            \def\mytext{\ctikzvalof{multipoles/font}\space\pgf@circ@strut\the\pgf@circ@count@c\space}
            \pgfmathloop%
            \ifnum\pgf@circ@count@a>0
                \ifcase\quadrant % rotation 0
                    % left
                    \pgf@circ@count@c=\pgf@circ@count@a
                    \pgftext[left,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % bottom
                    \pgf@circ@count@c=\numexpr\pgf@circ@count@b+\pgf@circ@count@a\relax
                    \pgftext[bottom,
                        at=\pgfpoint{\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@down},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b-\pgf@circ@count@a+1\relax
                    \pgftext[right,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % top
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b+\pgf@circ@count@a\relax
                    \pgftext[top,
                        at=\pgfpoint{\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@up},
                        rotate=\rot]{\mytext}
                \or % rotation -90
                    % left
                    \pgf@circ@count@c=\pgf@circ@count@a
                    \pgftext[top,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % bottom
                    \pgf@circ@count@c=\numexpr\pgf@circ@count@b+\pgf@circ@count@a\relax
                    \pgftext[left,
                        at=\pgfpoint{\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@down},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b-\pgf@circ@count@a+1\relax
                    \pgftext[bottom,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % top
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b+\pgf@circ@count@a\relax
                    \pgftext[right,
                        at=\pgfpoint{\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@up},
                        rotate=\rot]{\mytext}
                \or %rotation 180
                    % left
                    \pgf@circ@count@c=\pgf@circ@count@a
                    \pgftext[right,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % bottom
                    \pgf@circ@count@c=\numexpr\pgf@circ@count@b+\pgf@circ@count@a\relax
                    \pgftext[top,
                        at=\pgfpoint{\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@down},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b-\pgf@circ@count@a+1\relax
                    \pgftext[left,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % top
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b+\pgf@circ@count@a\relax
                    \pgftext[bottom,
                        at=\pgfpoint{\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@up},
                        rotate=\rot]{\mytext}
                \or % rotation +90
                    % left
                    \pgf@circ@count@c=\pgf@circ@count@a
                    \pgftext[bottom,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % bottom
                    \pgf@circ@count@c=\numexpr\pgf@circ@count@b+\pgf@circ@count@a\relax
                    \pgftext[right,
                        at=\pgfpoint{\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@down},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b-\pgf@circ@count@a+1\relax
                    \pgftext[top,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % top
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b+\pgf@circ@count@a\relax
                    \pgftext[left,
                        at=\pgfpoint{\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@up},
                        rotate=\rot]{\mytext}
                \fi
                \advance\pgf@circ@count@a-1\relax%
                \repeatpgfmathloop
            \fi
            \endpgfscope
            \ifdim\pgf@circ@res@other>0pt
            \pgfscope
                \pgfsetlinewidth{\ctikzvalof{multipoles/external pins thickness}\pgflinewidth}
                \pgf@circ@count@a=\numpins%
                \divide\pgf@circ@count@a by 4 \pgf@circ@count@b=\pgf@circ@count@a
                \pgfmathloop%
                \ifnum\pgf@circ@count@a>0
                    \edef\padfrac{\ctikzvalof{multipoles/external pad fraction}}
                    \ifnum\padfrac>0
                        \pgf@circ@res@temp=\pgf@circ@res@step\divide\pgf@circ@res@temp by \padfrac
                        % left side pads
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@other}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@other}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        % bottom side pads
                        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@temp+\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@down}}
                        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@temp+\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@down-\pgf@circ@res@other}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@down-\pgf@circ@res@other}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@down}}
                        % right side pads
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgf@circ@res@other}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgf@circ@res@other}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        % top side pads
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@up}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@up+\pgf@circ@res@other}}
                        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@temp+\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@up+\pgf@circ@res@other}}
                        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@temp+\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@up}}
                    \else
                        % left side pins
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@other}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        % bottom side pins
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@down}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@down-\pgf@circ@res@other}}
                        % right side pins
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgf@circ@res@other}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}}
                        % top side pins
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@up}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\pgf@circ@count@a)*\pgf@circ@res@step}{\pgf@circ@res@up+\pgf@circ@res@other}}
                    \fi
                    \advance\pgf@circ@count@a-1\relax%
                \repeatpgfmathloop
                \pgfusepath{stroke}
            \endpgfscope
            \fi
        }%
        % \pgf@sh@s@<name of the shape here> contains all the code for the shape
        % and is executed just before a node is drawn.
        \pgfutil@g@addto@macro\pgf@sh@s@qfpchip{%
            % Start with the maximum pin number and go backwards.
            \pgf@circ@count@a=\numpins%
            \pgfmathloop%
            \ifnum\pgf@circ@count@a>0
                \expandafter\xdef\csname pgf@anchor@qfpchip@pin\space\the\pgf@circ@count@a\endcsname{%
                    \noexpand\pgf@circ@qfppinanchor{\the\pgf@circ@count@a}{1}%
                }
                \expandafter\xdef\csname pgf@anchor@qfpchip@bpin\space\the\pgf@circ@count@a\endcsname{%
                    \noexpand\pgf@circ@qfppinanchor{\the\pgf@circ@count@a}{0}%
                }
                \advance\pgf@circ@count@a-1\relax%
                \repeatpgfmathloop%
            }%
        }

%% anchors for DIP
\def\pgf@circ@dippinanchor#1#2{% #1: pin number #2: 0 for border pin, 1 for external pin
    \c@pgf@countc=\numpins\relax
    \divide\c@pgf@countc by 2
    \ifnum #1 > \the\c@pgf@countc
        % right side
        \pgfpoint{\width/2+#2*\extshift}{-\height/2+(\pgf@circ@dip@pin@shift-\c@pgf@countc+#1-1)*\chipspacing}
    \else
        \pgfpoint{-\width/2-#2*\extshift}{\height/2+(\pgf@circ@dip@pin@shift-#1)*\chipspacing}
\fi
}

%% anchors for QFP
\def\pgf@circ@qfppinanchor#1#2{% #1: pin number #2: 0 for border pin, 1 for external pin
    \c@pgf@countc=\numpins\relax
    \divide\c@pgf@countc by 4
    \ifnum #1 > \the\c@pgf@countc
        \c@pgf@countb=\c@pgf@countc \multiply \c@pgf@countb by 2
        \ifnum #1 > \the\c@pgf@countb
            \c@pgf@countb=\c@pgf@countc \multiply \c@pgf@countb by 3
            \ifnum #1 > \the\c@pgf@countb
                % 3*npins/4 < pin, top side
                \pgfpoint{\width/2+(\pgf@circ@qfp@pin@shift+\c@pgf@countb-#1)*\chipspacing}{\height/2+#2*\extshift}%
            \else
                % 2*npins/4 < pin <= 3*npins/4, right side
                \pgfpoint{\width/2+#2*\extshift}{\height/2+(\pgf@circ@qfp@pin@shift-\c@pgf@countb+#1-1)*\chipspacing}%
            \fi
        \else
            %  npins/4 < pin <= 2*npins/4, bottom side
            \pgfpoint{\width/2+(\pgf@circ@qfp@pin@shift-\c@pgf@countb+#1-1)*\chipspacing}{-\height/2-#2*\extshift}%
        \fi
    \else
        % <= npins/4, left side
        \pgfpoint{-\width/2-#2*\extshift}{\height/2+(\pgf@circ@qfp@pin@shift-#1)*\chipspacing}%
    \fi
}

%%%%%%%%%%%%%%%%%
%% Rotary Switch
%%%%%%%%%%%%%%%%%

\pgfdeclareshape{rotaryswitch}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{switches}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor\northeast{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        % this strange value makes the 2-pole rotary switch equal to the 2 poles cute spdt
        % the magic number is 0.25/cos(35)
        % try to recalculate it for the actual switch
        \pgf@circ@res@temp=\ctikzvalof{tripoles/spdt/width}\pgf@circ@scaled@Rlen
        \pgf@circ@res@temp=.3052\pgf@circ@res@temp
        \edef\a{\ctikzvalof{multipoles/rotary/angle}}
        \edef\r{\ctikzvalof{nodes width}}
        \pgfmathsetlength{\pgf@y}{\r*\pgf@circ@scaled@Rlen +(\a>90 ? 2 : 2*sin(\a))*\pgf@circ@res@temp}
        \pgfmathsetlength{\pgf@x}{\r*\pgf@circ@scaled@Rlen + \pgf@circ@res@temp}
    }
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        % this strange value makes the 2-pole rotary switch equal to the 2 poles cute spdt
        % the magic number is 0.25/cos(35)
        % try to recalculate it for the actual switch
        \pgf@circ@res@temp=\ctikzvalof{tripoles/spdt/width}\pgf@circ@scaled@Rlen
        \pgf@circ@res@temp=.3052\pgf@circ@res@temp
        \edef\a{\ctikzvalof{multipoles/rotary/angle}}
        \edef\r{\ctikzvalof{nodes width}}
        \pgfmathsetlength{\pgf@y}{\r*\pgf@circ@scaled@Rlen +(\a>90 ? 2 : 2*sin(\a))*\pgf@circ@res@temp}
        \pgfmathsetlength{\pgf@x}{-\r*\pgf@circ@scaled@Rlen - (\a<90 ? 1 : 1-2*cos(\a))*\pgf@circ@res@temp}
    }
    \savedanchor\central{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        % this strange value makes the 2-pole rotary switch equal to the 2 poles cute spdt
        % the magic number is 0.25/cos(35)
        % try to recalculate it for the actual switch
        \pgf@circ@res@temp=\ctikzvalof{tripoles/spdt/width}\pgf@circ@scaled@Rlen
        \pgf@circ@res@temp=.3052\pgf@circ@res@temp
        \edef\a{\ctikzvalof{multipoles/rotary/angle}}
        \edef\r{\ctikzvalof{nodes width}}
        \pgfmathsetlength{\pgf@y}{\r*\pgf@circ@scaled@Rlen +(\a>90 ? 2 : 2*sin(\a))*\pgf@circ@res@temp}
        \pgfmathsetlength{\pgf@x}{(\a<90 ? 0 : cos(\a))*\pgf@circ@res@temp}
    }
    % external square limits
    \savedanchor\extnorthwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@x=-\ctikzvalof{tripoles/spdt/width}\pgf@circ@scaled@Rlen
        % this strange value makes the 2-pole rotary switch equal to the 2 poles cute spdt
        \pgf@x=.3052\pgf@x % the magic number is 0.25/cos(35)
        \pgf@x=2.5\pgf@x % external square size
        \pgf@y=-\pgf@x %square thing when angle=180?
    }
    \saveddimen{\width}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength\pgf@x{0.3052*\pgf@circ@scaled@Rlen*\ctikzvalof{tripoles/spdt/width}}}
    % radius of the connector
    % This is the radius of the "ocirc" shape (see pgfcircshapes.tex)
    \saveddimen{\radius}{\pgfmathsetlength\pgf@x{\pgf@circ@Rlen*\ctikzvalof{nodes width}}}
    % shapename
    \savedmacro{\thisshape}{\def\thisshape{\tikz@fig@name}}
    % shape type
    \savedmacro{\cshape}{\def\cshape{\ctikzvalof{multipoles/rotary/shape}}}
    \savedmacro{\channels}{\def\channels{\ctikzvalof{multipoles/rotary/channels}}}
    \savedmacro{\angle}{\def\angle{\ctikzvalof{multipoles/rotary/angle}}}
    \savedmacro{\wiper}{\def\wiper{\ctikzvalof{multipoles/rotary/wiper}}}
    \savedmacro{\stepa}{\pgfmathsetmacro{\stepa}{2*\ctikzvalof{multipoles/rotary/angle}/(\ctikzvalof{multipoles/rotary/channels}-1)}}
    % mid of the lever, to stack switches
    %\anchor{mid}{\midlever}
    \anchor{mid}{\northwest
        \pgf@circ@res@temp=-\pgf@x
        \pgfmathsetlength{\pgf@x}{\pgf@circ@res@temp*(-1+cos(\wiper))}
        \pgfmathsetlength{\pgf@y}{\pgf@circ@res@temp*sin(\wiper)}
    }
    % center anchors
    \anchor{cin}{ \northwest \pgf@y=0pt\advance\pgf@x by \radius}
    % horizontal angles
    \anchor{in}{ \northwest \pgf@y=0pt}
    \anchor{ain}{ \northwest \pgf@y=0pt}

    \anchor{center}{ \central \pgf@y=0pt }
    \anchor{east}{ \northeast \pgf@y=0pt }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \central \pgf@y=-\pgf@y }
    \anchor{north}{ \central }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northeast }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northeast \pgf@y=-\pgf@y }

    \anchor{ext center}{ \pgf@y=0pt \pgf@x=0pt \advance\pgf@x by -\width}
    \anchor{ext east}{ \extnorthwest \pgf@y=0pt \pgf@x=-\pgf@x \advance\pgf@x by -\width}
    \anchor{ext west}{ \extnorthwest \pgf@y=0pt \advance\pgf@x by -\width}
    \anchor{ext south}{ \extnorthwest \pgf@x=0pt \pgf@y=-\pgf@y \advance\pgf@x by -\width}
    \anchor{ext north}{ \extnorthwest \pgf@x=0pt \advance\pgf@x by -\width}
    \anchor{ext south west}{ \extnorthwest \pgf@y=-\pgf@y \advance\pgf@x by -\width}
    \anchor{ext north east}{ \extnorthwest \pgf@x=-\pgf@x \advance\pgf@x by -\width}
    \anchor{ext north west}{ \extnorthwest \advance\pgf@x by -\width}
    \anchor{ext south east}{ \extnorthwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y \advance\pgf@x by -\width}

    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        \pgf@circ@res@right = \width
        \pgf@circ@res@left = -\width

        \pgfscope %wiper
        % This is the radius of the "ocirc" shape (see pgfcircshapes.tex)
        \pgf@circ@res@temp=\radius\relax
        \pgf@circ@res@temp=\ctikzvalof{multipoles/rotary/thickness}\pgf@circ@res@temp
        \pgfsetlinewidth{2\pgf@circ@res@temp}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@circ@res@left}{0pt}}{\pgfpointpolar{\wiper}{2\pgf@circ@res@right}}}
        \pgfsetroundcap\pgfusepath{draw}
        \endpgfscope

        \ifpgf@circ@rotaryarrow
            \pgfscope % arrow
                \ifpgf@circ@rotaryarrow@ccw\pgfsetarrowsstart{latexslim}\fi
                \pgf@circ@setlinewidth{bipoles}{\pgflinewidth}
                \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}} % center of cin node
                \pgftransformrotate{\wiper}
                \pgfpathmoveto{\pgfpointpolar{50}{1.0\pgf@circ@res@right}}
                \pgfpatharc{50}{-50}{1.0\pgf@circ@res@right}
                \ifpgf@circ@rotaryarrow@cw\pgfsetarrowsend{latexslim}\fi
                \pgfusepath{draw}
            \endpgfscope
        \fi

        % \typeout{CHANNELS\space\channels\space ANGLE\space\angle STEPA\space\stepa}
        \pgf@circ@count@a=\channels\relax
        \pgfmathsetmacro{\currenta}{-\angle}
        \pgfmathloop%
        \ifnum\pgf@circ@count@a>0
            % \typeout{LOOPIN\space\space\the\pgf@circ@count@a\space CURRENTA\space\currenta\space RIGHT\space\the\pgf@circ@res@right}
            \pgfscope
                \pgftransformshift{\pgfpointadd{\pgfpoint{\pgf@circ@res@left}{0pt}}{\pgfpointpolar{\currenta}{2\pgf@circ@res@right}}}
                \pgfnode{\cshape}{center}{}{\thisshape-out \the\pgf@circ@count@a}{\pgfusepath{stroke}}
            \endpgfscope
            \pgfmathsetmacro{\currenta}{\currenta+\stepa}
            % \typeout{LOOPOUT\space\the\pgf@circ@count@a\space CURRENTA\space\currenta\space RIGHT\space\the\pgf@circ@res@right}
            \advance\pgf@circ@count@a by -1\relax%
        \repeatpgfmathloop

        \pgfscope % input
        \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfnode{\cshape}{center}{}{\thisshape-in}{\pgfusepath{stroke}}
        \endpgfscope
    }
    % \pgf@sh@s@<name of the shape here> contains all the code for the shape
    % and is executed just before a node is drawn.
    \pgfutil@g@addto@macro\pgf@sh@s@rotaryswitch{%
        % Start with the maximum pin number and go backwards.
        \pgf@circ@count@a=\channels\relax
        \pgfmathloop%
        \ifnum\pgf@circ@count@a>0
        % we will create two anchors per pin: the "normal one" like `pin 1` for the
        % electrical contact, and the "border one" like `bpin 1` for labels.
        % they will coincide if `external pins width` is set to 0.
        \expandafter\xdef\csname pgf@anchor@rotaryswitch@out\space\the\pgf@circ@count@a\endcsname{%
            \noexpand\pgf@circ@rotaryanchor{\the\pgf@circ@count@a}{1}{0}%
        }
        \expandafter\xdef\csname pgf@anchor@rotaryswitch@cout\space\the\pgf@circ@count@a\endcsname{%
            \noexpand\pgf@circ@rotaryanchor{\the\pgf@circ@count@a}{0}{0}%
        }
        \expandafter\xdef\csname pgf@anchor@rotaryswitch@aout\space\the\pgf@circ@count@a\endcsname{%
            \noexpand\pgf@circ@rotaryanchor{\the\pgf@circ@count@a}{0}{1}%
        }
        \expandafter\xdef\csname pgf@anchor@rotaryswitch@sqout\space\the\pgf@circ@count@a\endcsname{%
            \noexpand\pgf@circ@rotarysqanchor{\the\pgf@circ@count@a}{0}%
        }
        \advance\pgf@circ@count@a by -1\relax%
        \repeatpgfmathloop%
    }%
}

\def\pgf@circ@rotaryanchor#1#2#3{% #1: numero del pin; #2: 1 - x pos, 0 - center; #3 0: inner, 1 outer
    \pgf@circ@res@temp=\width
    \pgfmathsetmacro{\myangle}{\angle-(#1-1)*\stepa}
    \pgfmathsetlength{\pgf@x}{2*(\pgf@circ@res@temp+#3*\radius/2)*cos(\myangle))+#2*\radius}
    \pgfmathsetlength{\pgf@y}{2*(\pgf@circ@res@temp+#3*\radius/2)*sin(\myangle)}
    \advance\pgf@x by -\pgf@circ@res@temp
}

\def\pgf@circ@rotarysqanchor#1{% external square anchors
    \pgf@circ@res@temp=\width
    \pgfmathsetmacro{\myangle}{\angle-(#1-1)*\stepa}
    \pgfpointborderrectangle{\pgfpointpolar{\myangle}{1pt}}{\pgfpoint{2.5\pgf@circ@res@temp}{2.5\pgf@circ@res@temp}}
    \advance\pgf@x by -\pgf@circ@res@temp
}

%%%%%%%%%%%%%%%%%%%%%%%%%%
% Seven segments displays
%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfdeclareshape{bare7seg}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{displays}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedmacro{\dotstatus}{\edef\dotstatus{\pgf@circ@sevenseg@dotstate}}
    \saveddimen{\dotspace}{% the dot is on the right, and occupy the same as the thickness
        \ifpgf@circ@sevenseg@dot
            \pgfmathsetlength{\pgf@x}{\ctikzvalof{seven seg/thickness}}
        \else
            \pgf@x=0pt
        \fi
    }
    % The object extension is more or less (-width/2,-width) to (width/2,width)
    % and adjusted for line thickness (both sides) and eventually the dot
    \saveddimen{\width}{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength{\pgf@x}{\ctikzvalof{seven seg/width}*\pgf@circ@scaled@Rlen}}
    \saveddimen{\gap}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{seven seg/segment sep}}}
    \saveddimen{\boxgap}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{seven seg/box sep}}}
    \savedanchor{\southwest}{% both negative
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength{\pgf@x}{-0.5*\ctikzvalof{seven seg/width}*\pgf@circ@scaled@Rlen
        -0.5*\ctikzvalof{seven seg/thickness}-\ctikzvalof{seven seg/box sep}}
        \pgfmathsetlength{\pgf@y}{-\ctikzvalof{seven seg/width}*\pgf@circ@scaled@Rlen
        -0.5*\ctikzvalof{seven seg/thickness}-\ctikzvalof{seven seg/box sep}}
    }
    \savedanchor{\northeast}{% both positive
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \ifpgf@circ@sevenseg@dot
            \pgfmathsetlength{\pgf@circ@res@other}{\ctikzvalof{seven seg/thickness}}
        \else
            \pgf@circ@res@other=0pt
        \fi
        \pgfmathsetlength{\pgf@x}{0.5*\ctikzvalof{seven seg/width}*\pgf@circ@scaled@Rlen
        +0.5*\ctikzvalof{seven seg/thickness}+\pgf@circ@res@other+\ctikzvalof{seven seg/box sep}}
        \pgfmathsetlength{\pgf@y}{\ctikzvalof{seven seg/width}*\pgf@circ@scaled@Rlen
        +0.5*\ctikzvalof{seven seg/thickness}+\ctikzvalof{seven seg/box sep}}
    }
    \savedanchor{\topright}{% anchor without the box sep and the thickness
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgfmathsetlength{\pgf@x}{0.5*\ctikzvalof{seven seg/width}*\pgf@circ@scaled@Rlen}
        \pgfmathsetlength{\pgf@y}{\ctikzvalof{seven seg/width}*\pgf@circ@scaled@Rlen}
    }
    \anchor{center}{\pgfpointorigin}
    \anchor{north west}{\southwest\pgf@y=-\pgf@y}
    \anchor{north east}{\northeast}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south west}{\southwest}
    \anchor{north}{\northeast\pgf@x=0pt}
    \anchor{east}{\northeast\pgf@y=0pt}
    \anchor{south}{\southwest\pgf@x=0pt}
    \anchor{west}{\southwest\pgf@y=0pt}
    \anchor{a}{\topright\pgf@x=0pt}
    \anchor{b}{\topright\pgf@y=0.5\pgf@y}
    \anchor{c}{\topright\pgf@y=-0.5\pgf@y}
    \anchor{d}{\topright\pgf@y=-\pgf@y\pgf@x=0pt}
    \anchor{e}{\topright\pgf@x=-\pgf@x\pgf@y=-0.5\pgf@y}
    \anchor{f}{\topright\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{g}{\pgfpointorigin}
    \anchor{dot}{\topright\pgf@y=-\pgf@y\advance\pgf@x by \dotspace}
    \behindbackgroundpath{%
        \southwest % I do not want the dot here, it will stick out
        \pgf@circ@res@up = -\pgf@y
        \pgf@circ@res@down = \pgf@y
        \pgf@circ@res@right = \pgf@x
        \pgf@circ@res@left = -\pgf@x
        \pgfscope
        \pgf@circ@setlinewidth{multipoles}{\pgflinewidth}
        \pgfsetcolor{\ctikzvalof{color}}
        \pgfpathrectanglecorners%
        {\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        {\pgfpoint{\pgf@circ@res@left+\dotspace}{\pgf@circ@res@up}}
        \ifpgf@circ@sevenseg@box
            \pgf@circ@draworfill
        \else
            \pgf@circ@maybefill
        \fi
        \endpgfscope
        \edef\bits{\ctikzvalof{seven seg/bits}}
        \pgfscope
            \pfg@circ@sseg@drawbits{\bits}
        \endpgfscope
        \pgfscope
            \ifpgf@circ@sevenseg@dot
                \pgf@circ@sseg@drawdots
            \fi
        \endpgfscope
    }
}

\def\pgf@circ@sseg@splitbits#1#2#3#4#5#6#7\relax{%split the seven bits
    \edef\@@a{#1}\edef\@@b{#2}\edef\@@c{#3}\edef\@@d{#4}\edef\@@e{#5}\edef\@@f{#6}\edef\@@g{#7}%
}
\def\pgf@circ@sseg@drawone#1#2#3#4#5{% #1 on off the x1, y1, x2 , y2
    \ifnum #1 > 0\relax
        \pgfsetcolor{\ctikzvalof{seven seg/color on}}
    \else
        \pgfsetcolor{\ctikzvalof{seven seg/color off}}
    \fi
    \pgfpathmoveto{\pgfpoint{#2}{#3}}
    \pgfpathlineto{\pgfpoint{#4}{#5}}
    \pgfusepath{draw}
}
\def\pfg@circ@sseg@drawbits#1{% #1 must be 7 bits
    \expandafter\pgf@circ@sseg@splitbits#1\relax% a bit of magic...
    \pgfmathsetlength{\pgf@circ@res@other}{0.5*\ctikzvalof{seven seg/thickness}}
    \pgfsetlinewidth{\ctikzvalof{seven seg/thickness}}
    % \pgfsetroundcap
    \pgfsetarrowsstart{Triangle Cap[]}
    \pgfsetarrowsend{Triangle Cap[]}
    % segments
    \pgf@circ@sseg@drawone{\@@a}{-\width/2+\gap}{\width}{\width/2-\gap}{\width}
    \pgf@circ@sseg@drawone{\@@b}{\width/2}{\width-\gap}{\width/2}{0pt+\gap}
    \pgf@circ@sseg@drawone{\@@c}{\width/2}{0pt-\gap}{\width/2}{-\width+\gap}
    \pgf@circ@sseg@drawone{\@@d}{\width/2-\gap}{-\width}{-\width/2+\gap}{-\width}
    \pgf@circ@sseg@drawone{\@@e}{-\width/2}{-\width+\gap}{-\width/2}{0pt-\gap}
    \pgf@circ@sseg@drawone{\@@f}{-\width/2}{0pt+\gap}{-\width/2}{\width-\gap}
    \pgf@circ@sseg@drawone{\@@g}{-\width/2+\gap}{0pt}{\width/2-\gap}{0pt}
}
\def\pgf@circ@sseg@drawdots{% dots
    \edef\what{empty}
    \ifx\what\pgf@circ@sevenseg@dotstate
        % do nothing
    \else
        \pgfmathsetlength{\pgf@circ@res@other}{0.5*\ctikzvalof{seven seg/thickness}}
        \edef\what{off}
        \ifx\what\pgf@circ@sevenseg@dotstate
            % dot off
            \pgfsetfillcolor{\ctikzvalof{seven seg/color off}}
            \pgfsetcolor{\ctikzvalof{seven seg/color off}}
        \else
            % dot on
            \pgfsetfillcolor{\ctikzvalof{seven seg/color on}}
            \pgfsetcolor{\ctikzvalof{seven seg/color on}}
        \fi
        \pgfpathcircle{\pgfpoint{\width/2+2*\pgf@circ@res@other}{-\width}}{\pgf@circ@res@other}
        \pgfusepath{draw,fill}
    \fi
}


==> pgfcircpath.tex <==

\def\pgf@circ@direction{0.0}

% Names
\ctikzset{name/.style = { n=#1 } } %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%@@@
\ctikzset{n/.code = {
	\pgfkeys{/tikz/circuitikz/bipole/name=#1}
}}

% Reflect the node along
\ctikzset{mirrored/.is choice}
\ctikzset{mirror value/.initial=1}
\ctikzset{mirrored/true/.code = {\ctikzsetvalof{mirror value}{-1}} }
\ctikzset{mirrored/false/.code = {\ctikzsetvalof{mirror value}{1}} }
\ctikzset{mirror/.style = {/tikz/circuitikz/mirrored=true}}

% Invert node along path
\ctikzset{inverted/.is choice}
\ctikzset{invert value/.initial=1}
\ctikzset{inverted/true/.code = {\ctikzsetvalof{invert value}{-1}\pgf@circuit@bipole@invertedtrue}}
\ctikzset{inverted/false/.code = {\ctikzsetvalof{invert value}{1}\pgf@circuit@bipole@invertedfalse}}
\ctikzset{invert/.style = {/tikz/circuitikz/inverted=true}}
\newif\ifpgf@circuit@bipole@inverted
\ctikzset{bipole/inverted/.is if=pgf@circuit@bipole@inverted}

\newif\ifpgf@circuit@bipole@voltage@backward
\ctikzset{bipole/voltage/direction/.is choice}
\ctikzset{bipole/voltage/direction/forward/.code={\pgf@circuit@bipole@voltage@backwardfalse}}
\ctikzset{bipole/voltage/direction/backward/.code={\pgf@circuit@bipole@voltage@backwardtrue}}

% Initialize paths
\def\pgfcircresetpath{
    \ctikzset{bipole/name=, bipole/label/name=, bipole/label/position=90, ,bipole/annotation/name=, bipole/annotation/position=-90,
        bipole/inverted=false, bipole/kind=,
        bipole/voltage/direction=backward, bipole/voltage/label/name=, bipole/voltage/position=below,
        bipole/nodes/left=none, bipole/nodes/right=none, bipole/is voltage=false,bipole/is voltageoutsideofsymbol=false,bipole/is strokedsymbol=false,
        bipole/is current=false, bipole/current/label/name=, bipole/current/x position=after,
        bipole/current/y position=above, bipole/current/direction=forward,
        mirrored=false
    }
}

%% Helper function for path-function to ensure using anchors between nodes
\def\set@explicit@center@anchor#1{
    \pgfutil@ifundefined{pgf@sh@ns@#1}
    {
        %This coordinate is no node(but a relative position or a coordinate), no further handling needed
        }{
        \pgfutil@in@.{#1}
        \ifpgfutil@in@
            % Anchor is used, do nothing!
    \else%
        \let\tikz@moveto@waiting=\relax
        \pgfpathmoveto{\tikz@last@position}%force movement, because tikz@moveto@waiting
        \edef#1{#1.center}%ensure using center anchor
    \fi
}
}


%% Generic bipole path
%% I am not user what the second argument is needed for
\def\pgf@circ@bipole@path#1#2{

    \pgfextra{
        \set@explicit@center@anchor{\tikztostart}
        \set@explicit@center@anchor{\tikztotarget}
        \pgfsyssoftpath@getcurrentpath{\myp@th}%% save current path to extend after calculation of correct start/end coordinates
        \ctikzset{bipole/kind = #1}
        \edef\pgf@temp{\ctikzvalof{bipole/name}}
        \def\pgf@circ@temp{}
        \ifx\pgf@temp\pgf@circ@temp % if it has not a name
            \pgfmathrandominteger{\pgf@circ@rand}{1000}{9999}
            \ctikzset{bipole/name = #1\pgf@circ@rand} % create it (re-usage should not create problem, but...)
        \fi
    }

    (\tikztostart) coordinate (\ctikzvalof{bipole/name}start)%necessary to get correct coordinates in the case of relative start/end or constructions like ((node1)-|(node2))
    (\tikztotarget) coordinate (\ctikzvalof{bipole/name}end)
    \pgfextra{
        \pgfmathanglebetweenpoints{\pgfpointanchor{\ctikzvalof{bipole/name}start}{center}}
        {\pgfpointanchor{\ctikzvalof{bipole/name}end}{center}}
        \pgfmathround{\pgfmathresult}
        \edef\pgf@circ@direction{\pgfmathresult}%Calculate direction(angle) of path
        \pgfsyssoftpath@setcurrentpath{\myp@th}
    }
    \pgfextra{\def\pgf@temp{open}\def\pgf@circ@temp{#1}}
    \ifx\pgf@temp\pgf@circ@temp  % if it is an open
        \else
            --($(\ctikzvalof{bipole/name}start) ! .5\pgflinewidth ! (\ctikzvalof{bipole/name}end)$) %ugly workaround to get correct linejoins(node breaks path?)
        \fi
        ($(\tikztostart) ! .5 ! (\tikztotarget)$)%%positio of middle node
        node[#1shape, rotate=\pgf@circ@direction, yscale=\ctikzvalof{mirror value}, xscale=\ctikzvalof{invert value}]
        (\ctikzvalof{bipole/name}) {}
        \ifpgf@circuit@bipole@inverted
            \ifcsname pgf@anchor@#1shape@pathstart\endcsname%if special path-anchors are defined, use them!
                coordinate	(anchorstartnode) at (\ctikzvalof{bipole/name}.pathend)
                coordinate	(anchorendnode) at (\ctikzvalof{bipole/name}.pathstart)
            \else
                coordinate	(anchorstartnode) at (\ctikzvalof{bipole/name}.right)
                coordinate	(anchorendnode) at (\ctikzvalof{bipole/name}.left)
            \fi
            \else
            \ifcsname pgf@anchor@#1shape@pathstart\endcsname%if special path-anchors are defined, use them!
                coordinate	(anchorstartnode) at (\ctikzvalof{bipole/name}.pathstart)
                coordinate	(anchorendnode) at (\ctikzvalof{bipole/name}.pathend)
            \else
                coordinate	(anchorstartnode) at (\ctikzvalof{bipole/name}.left)
                coordinate	(anchorendnode) at (\ctikzvalof{bipole/name}.right)
            \fi
        \fi
        \pgfextra{\def\pgf@temp{open}\def\pgf@circ@temp{#1}}
        \ifx\pgf@temp\pgf@circ@temp  % if it is an open
        \else
            (\ctikzvalof{bipole/name}start.center) -- (anchorstartnode)
            (anchorendnode)  -- (\ctikzvalof{bipole/name}end.center)
        \fi

        \drawpoles
        \pgf@circ@ifkeyempty{bipole/label/name}\else\pgf@circ@drawlabels{label}\fi
        \pgf@circ@ifkeyempty{bipole/annotation/name}\else\pgf@circ@drawlabels{annotation}\fi
        \pgf@circ@ifkeyempty{bipole/voltage/label/name}\else\pgf@circ@drawvoltage\fi
        \pgf@circ@ifkeyempty{bipole/current/label/name}\else\pgf@circ@drawcurrent\fi
        \pgf@circ@ifkeyempty{bipole/flow/label/name}\else\pgf@circ@drawflow\fi
        \pgfextra{\def\pgf@temp{open}\def\pgf@circ@temp{#1}}
        \ifx\pgf@temp\pgf@circ@temp  % if it is an open
            (\ctikzvalof{bipole/name}end)%Move to end of path
        \else
            ($(\ctikzvalof{bipole/name}end) ! .5\pgflinewidth ! (\ctikzvalof{bipole/name}start)$) -- (\ctikzvalof{bipole/name}end)%ugly workaround to get correct linejoins(node breaks path?)
            %tikztostart and tikztotarget could not be used, because it would break if target coordinate is something like (node1-|node2)

        \fi
    % reset
    \pgfextra{
        \pgfcircresetpath
    }
    \tikztonodes%draw pending nodes an path
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Handling of terminals

\ctikzset{bipole/nodes/.is family}
\ctikzset{bipole/nodes/left/.initial=none}
\ctikzset{bipole/nodes/right/.initial=none}
\tikzset{bipole nodes/.style n args={2}{%
    \circuitikzbasekey/bipole/nodes/left=#1,
    \circuitikzbasekey/bipole/nodes/right=#2
    }
}

%% Easily usable styles

\ctikzset{o-o/.style = {\circuitikzbasekey/bipole/nodes/left=ocirc, \circuitikzbasekey/bipole/nodes/right=ocirc}}
\ctikzset{-o/.style = {\circuitikzbasekey/bipole/nodes/left=none, \circuitikzbasekey/bipole/nodes/right=ocirc}}
\ctikzset{o-/.style = {\circuitikzbasekey/bipole/nodes/left=ocirc, \circuitikzbasekey/bipole/nodes/right=none}}
\ctikzset{*-o/.style = {\circuitikzbasekey/bipole/nodes/left=circ, \circuitikzbasekey/bipole/nodes/right=ocirc}}
\ctikzset{o-*/.style = {\circuitikzbasekey/bipole/nodes/left=ocirc, \circuitikzbasekey/bipole/nodes/right=circ}}
\ctikzset{d-o/.style = {\circuitikzbasekey/bipole/nodes/left=diamondpole, \circuitikzbasekey/bipole/nodes/right=ocirc}}
\ctikzset{o-d/.style = {\circuitikzbasekey/bipole/nodes/left=ocirc, \circuitikzbasekey/bipole/nodes/right=diamondpole}}
\ctikzset{*-/.style = {\circuitikzbasekey/bipole/nodes/left=circ, \circuitikzbasekey/bipole/nodes/right=none}}
\ctikzset{-*/.style = {\circuitikzbasekey/bipole/nodes/left=none, \circuitikzbasekey/bipole/nodes/right=circ}}
\ctikzset{d-/.style = {\circuitikzbasekey/bipole/nodes/left=diamondpole, \circuitikzbasekey/bipole/nodes/right=none}}
\ctikzset{-d/.style = {\circuitikzbasekey/bipole/nodes/left=none, \circuitikzbasekey/bipole/nodes/right=diamondpole}}
\ctikzset{*-*/.style = {\circuitikzbasekey/bipole/nodes/left=circ, \circuitikzbasekey/bipole/nodes/right=circ}}
\ctikzset{d-*/.style = {\circuitikzbasekey/bipole/nodes/left=diamondpole, \circuitikzbasekey/bipole/nodes/right=circ}}
\ctikzset{*-d/.style = {\circuitikzbasekey/bipole/nodes/left=circ, \circuitikzbasekey/bipole/nodes/right=diamondpole}}
\ctikzset{d-d/.style = {\circuitikzbasekey/bipole/nodes/left=diamondpole, \circuitikzbasekey/bipole/nodes/right=diamondpole}}

% rectjoinfill workarounds

\ctikzset{.-/.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=none}}
\ctikzset{.-*/.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=circ}}
\ctikzset{.-o/.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=ocirc}}
\ctikzset{.-d/.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=diamondpole}}
\ctikzset{-./.style = {\circuitikzbasekey/bipole/nodes/left=none, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}
\ctikzset{o-./.style = {\circuitikzbasekey/bipole/nodes/left=ocirc, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}
\ctikzset{*-./.style = {\circuitikzbasekey/bipole/nodes/left=circ, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}
\ctikzset{d-./.style = {\circuitikzbasekey/bipole/nodes/left=diamondpole, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}
\ctikzset{.-./.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}

\tikzset{reversed/.style = {\circuitikzbasekey/bipole/inverted=true}}

\def\drawpoles{
    \pgfextra{ \edef\pgf@circ@temp{\ctikzvalof{bipole/nodes/left}} \def\pgf@temp{none}}
    \ifx\pgf@temp\pgf@circ@temp\else(\tikztostart) node[\pgf@circ@temp] {}\fi
    \pgfextra{ \edef\pgf@circ@temp{\ctikzvalof{bipole/nodes/right}} }
    \ifx\pgf@temp\pgf@circ@temp\else(\tikztotarget) node[\pgf@circ@temp] {}\fi
}

%% Path definitions
\def\pgf@circ@resistor@path#1{\ifpgf@circuit@europeanresistor\pgf@circ@bipole@path{generic}{#1}\else\pgf@circ@bipole@path{resistor}{#1}\fi}
\def\pgf@circ@vresistor@path#1{\ifpgf@circuit@europeanresistor\pgf@circ@bipole@path{tgeneric}{#1}\else\pgf@circ@bipole@path{vresistor}{#1}\fi}
\def\pgf@circ@sresistor@path#1{\ifpgf@circuit@europeanresistor\pgf@circ@bipole@path{thermistor}{#1}\else\pgf@circ@bipole@path{resistivesens}{#1}\fi}
\def\pgf@circ@potentiometer@path#1{\ifpgf@circuit@europeanresistor\pgf@circ@bipole@path{genericpotentiometer}{#1}\else\pgf@circ@bipole@path{potentiometer}{#1}\fi}
\def\pgf@circ@thermistor@path#1{\pgf@circ@bipole@path{thermistor}{#1}}
\def\pgf@circ@thermistorptc@path#1{\pgf@circ@bipole@path{thermistorptc}{#1}}
\def\pgf@circ@thermistorntc@path#1{\pgf@circ@bipole@path{thermistorntc}{#1}}
\def\pgf@circ@varistor@path#1{\pgf@circ@bipole@path{varistor}{#1}}
\def\pgf@circ@capacitor@path#1{\pgf@circ@bipole@path{capacitor}{#1}}
\def\pgf@circ@capacitivesens@path#1{\pgf@circ@bipole@path{capacitivesens}{#1}}
\def\pgf@circ@ecapacitor@path#1{\pgf@circ@bipole@path{ecapacitor}{#1}}
%% polar capacitor is deprectaed, use curved capacitor instead
\def\pgf@circ@polarcapacitor@path#1{\pgf@circ@bipole@path{polarcapacitor}{#1}}
\def\pgf@circ@ccapacitor@path#1{\pgf@circ@bipole@path{ccapacitor}{#1}}
\def\pgf@circ@vcapacitor@path#1{\pgf@circ@bipole@path{vcapacitor}{#1}}
\def\pgf@circ@piezoelectric@path#1{\pgf@circ@bipole@path{piezoelectric}{#1}}
\def\pgf@circ@battery@path#1{\pgf@circ@bipole@path{battery}{#1}}
\def\pgf@circ@batteryone@path#1{\pgf@circ@bipole@path{battery1}{#1}}
\def\pgf@circ@batterytwo@path#1{\pgf@circ@bipole@path{battery2}{#1}}
\def\pgf@circ@europeaninductor@path#1{\pgf@circ@bipole@path{fullgeneric}{#1}}
\def\pgf@circ@americaninductor@path#1{\pgf@circ@bipole@path{americaninductor}{#1}}
\def\pgf@circ@cuteinductor@path#1{\pgf@circ@bipole@path{cuteinductor}{#1}}
\def\pgf@circ@cutechoke@path#1{\pgf@circ@bipole@path{cutechoke}{#1}}
\def\pgf@circ@inductor@path#1{%
    \pgfextra{
        \edef\pgf@circ@temp{\ctikzvalof{inductor}}%
        \def\pgf@temp{european}%
    }
    \ifx\pgf@temp\pgf@circ@temp%
        \pgf@circ@europeaninductor@path{#1}%
    \else%
        \pgfextra{	\def\pgf@temp{cute} }%
        \ifx\pgf@temp\pgf@circ@temp%
            \pgf@circ@cuteinductor@path{#1}%
        \else%
            \pgf@circ@americaninductor@path{#1}%
        \fi%
    \fi%
}
\def\pgf@circ@vinductor@path#1{
    \pgfextra{
        \edef\pgf@circ@temp{\ctikzvalof{inductor}}%
        \def\pgf@temp{european}%
    }
    \ifx\pgf@temp\pgf@circ@temp%
        \pgf@circ@veuropeaninductor@path{#1}%
    \else%
        \pgfextra{	\def\pgf@temp{cute} }%
        \ifx\pgf@temp\pgf@circ@temp%
            \pgf@circ@vcuteinductor@path{#1}%
        \else%
            \pgf@circ@vamericaninductor@path{#1}%
        \fi%
    \fi%
}
\def\pgf@circ@inductivesens@path#1{%
    \pgfextra{
        \edef\pgf@circ@temp{\ctikzvalof{inductor}}%
        \def\pgf@temp{european}%
    }
    \ifx\pgf@temp\pgf@circ@temp%
        \pgf@circ@europeaninductivesens@path{#1}%
    \else%
        \pgfextra{	\def\pgf@temp{cute} }%
        \ifx\pgf@temp\pgf@circ@temp%
            \pgf@circ@cuteinductivesens@path{#1}%
        \else%
            \pgf@circ@americaninductivesens@path{#1}%
        \fi%
    \fi%
}
\def\pgf@circ@veuropeaninductor@path#1{\pgf@circ@bipole@path{tfullgeneric}{#1}}
\def\pgf@circ@vamericaninductor@path#1{\pgf@circ@bipole@path{vamericaninductor}{#1}}
\def\pgf@circ@vcuteinductor@path#1{\pgf@circ@bipole@path{vcuteinductor}{#1}}
\def\pgf@circ@europeaninductivesens@path#1{\pgf@circ@bipole@path{sfullgeneric}{#1}}
\def\pgf@circ@americaninductivesens@path#1{\pgf@circ@bipole@path{samericaninductor}{#1}}
\def\pgf@circ@cuteinductivesens@path#1{\pgf@circ@bipole@path{scuteinductor}{#1}}
\def\pgf@circ@lamp@path#1{\pgf@circ@bipole@path{lamp}{#1}}
\def\pgf@circ@bulb@path#1{\pgf@circ@bipole@path{bulb}{#1}}
\def\pgf@circ@esource@path#1{\pgf@circ@bipole@path{esource}{#1}}
\def\pgf@circ@pvsource@path#1{\pgf@circ@bipole@path{pvsource}{#1}}
\def\pgf@circ@vsource@path#1{\pgf@circ@bipole@path{vsource}{#1}}
\def\pgf@circ@dcvsource@path#1{\pgf@circ@bipole@path{dcvsource}{#1}}
\def\pgf@circ@vsourceam@path#1{\pgf@circ@bipole@path{vsourceAM}{#1}}
\def\pgf@circ@vsourcesin@path#1{\pgf@circ@bipole@path{vsourcesin}{#1}}
\def\pgf@circ@isource@path#1{\pgf@circ@bipole@path{isource}{#1}}
\def\pgf@circ@oosource@path#1{\pgf@circ@bipole@path{oosource}{#1}}
\def\pgf@circ@dcisource@path#1{\pgf@circ@bipole@path{dcisource}{#1}}
\def\pgf@circ@isourcesin@path#1{\pgf@circ@bipole@path{isourcesin}{#1}}
\def\pgf@circ@vsourcesquare@path#1{\pgf@circ@bipole@path{vsourcesquare}{#1}}
\def\pgf@circ@vsourcetri@path#1{\pgf@circ@bipole@path{vsourcetri}{#1}}
\def\pgf@circ@isourceam@path#1{\pgf@circ@bipole@path{isourceAM}{#1}}
\def\pgf@circ@ecsource@path#1{\pgf@circ@bipole@path{ecsource}{#1}}
\def\pgf@circ@cvsource@path#1{\pgf@circ@bipole@path{cvsource}{#1}}
\def\pgf@circ@cvsourceam@path#1{\pgf@circ@bipole@path{cvsourceAM}{#1}}
\def\pgf@circ@cvsourcesin@path#1{\pgf@circ@bipole@path{cvsourcesin}{#1}}
\def\pgf@circ@cisource@path#1{\pgf@circ@bipole@path{cisource}{#1}}
\def\pgf@circ@cisourceam@path#1{\pgf@circ@bipole@path{cisourceAM}{#1}}
\def\pgf@circ@cisourcesin@path#1{\pgf@circ@bipole@path{cisourcesin}{#1}}
\def\pgf@circ@short@path#1{\pgf@circ@bipole@path{short}{#1}}
\def\pgf@circ@cspst@path#1{\pgf@circ@bipole@path{cspst}{#1}}
\def\pgf@circ@ospst@path#1{\pgf@circ@bipole@path{ospst}{#1}}
\def\pgf@circ@nos@path#1{\pgf@circ@bipole@path{nos}{#1}}
\def\pgf@circ@ncs@path#1{\pgf@circ@bipole@path{ncs}{#1}}
\def\pgf@circ@pushbutton@path#1{\pgf@circ@bipole@path{pushbutton}{#1}}
\def\pgf@circ@ncpushbutton@path#1{\pgf@circ@bipole@path{ncpushbutton}{#1}}
\def\pgf@circ@open@path#1{\pgf@circ@bipole@path{open}{#1}}
\def\pgf@circ@generic@path#1{\pgf@circ@bipole@path{generic}{#1}}
\def\pgf@circ@ageneric@path#1{\pgf@circ@bipole@path{ageneric}{#1}}
\def\pgf@circ@tgeneric@path#1{\pgf@circ@bipole@path{tgeneric}{#1}}
\def\pgf@circ@fullgeneric@path#1{\pgf@circ@bipole@path{fullgeneric}{#1}}
\def\pgf@circ@tfullgeneric@path#1{\pgf@circ@bipole@path{tfullgeneric}{#1}}
\def\pgf@circ@ammeter@path#1{\pgf@circ@bipole@path{ammeter}{#1}}
\def\pgf@circ@ohmmeter@path#1{\pgf@circ@bipole@path{ohmmeter}{#1}}
\def\pgf@circ@voltmeter@path#1{\pgf@circ@bipole@path{voltmeter}{#1}}
\def\pgf@circ@oscope@path#1{\pgf@circ@bipole@path{oscope}{#1}}
\def\pgf@circ@empty@path#1{}
\def\pgf@circ@photoresistor@path#1{\pgf@circ@bipole@path{photoresistor}{#1}}
\def\pgf@circ@emptythyristor@path#1{\pgf@circ@bipole@path{emptythyristor}{#1}}
\def\pgf@circ@fullthyristor@path#1{\pgf@circ@bipole@path{fullthyristor}{#1}}
\def\pgf@circ@toggleswitch@path#1{\pgf@circ@bipole@path{toggleswitch}{#1}}
\def\pgf@circ@memristor@path#1{\pgf@circ@bipole@path{memristor}{#1}}
\def\pgf@circ@emptytriac@path#1{\pgf@circ@bipole@path{emptytriac}{#1}}
\def\pgf@circ@fulltriac@path#1{\pgf@circ@bipole@path{fulltriac}{#1}}
\def\pgf@circ@tline@path#1{\pgf@circ@bipole@path{tline}{#1}}
\def\pgf@circ@mstline@path#1{\pgf@circ@bipole@path{mstline}{#1}}
\def\pgf@circ@squid@path#1{\pgf@circ@bipole@path{squid}{#1}}
\def\pgf@circ@barrier@path#1{\pgf@circ@bipole@path{barrier}{#1}}
\def\pgf@circ@thermocouple@path#1{\pgf@circ@bipole@path{thermocouple}{#1}}
\def\pgf@circ@fuse@path#1{\pgf@circ@bipole@path{fuse}{#1}}
\def\pgf@circ@afuse@path#1{\pgf@circ@bipole@path{afuse}{#1}}

\def\pgf@circ@gfsurgearrester@path#1{\ifpgf@circuit@europeangfsurgearrester\pgf@circ@europeangfsurgearrester@path{#1}\else\pgf@circ@americangfsurgearrester@path{#1}\fi}
\def\pgf@circ@europeangfsurgearrester@path#1{\pgf@circ@bipole@path{european gas filled surge arrester}{#1}}
\def\pgf@circ@americangfsurgearrester@path#1{\pgf@circ@bipole@path{american gas filled surge arrester}{#1}}

\def\pgf@circ@twoport@path#1{\pgf@circ@bipole@path{twoport}{#1}}
\def\pgf@circ@vco@path#1{\pgf@circ@bipole@path{vco}{#1}}
\def\pgf@circ@bandpass@path#1{\pgf@circ@bipole@path{bandpass}{#1}}
\def\pgf@circ@bandstop@path#1{\pgf@circ@bipole@path{bandstop}{#1}}
\def\pgf@circ@highpass@path#1{\pgf@circ@bipole@path{highpass}{#1}}
\def\pgf@circ@lowpass@path#1{\pgf@circ@bipole@path{lowpass}{#1}}
\def\pgf@circ@adc@path#1{\pgf@circ@bipole@path{adc}{#1}}
\def\pgf@circ@dac@path#1{\pgf@circ@bipole@path{dac}{#1}}
\def\pgf@circ@dsp@path#1{\pgf@circ@bipole@path{dsp}{#1}}
\def\pgf@circ@fft@path#1{\pgf@circ@bipole@path{fft}{#1}}
\def\pgf@circ@amp@path#1{\pgf@circ@bipole@path{amp}{#1}}
\def\pgf@circ@vamp@path#1{\pgf@circ@bipole@path{vamp}{#1}}
\def\pgf@circ@piattenuator@path#1{\pgf@circ@bipole@path{piattenuator}{#1}}
\def\pgf@circ@vpiattenuator@path#1{\pgf@circ@bipole@path{vpiattenuator}{#1}}
\def\pgf@circ@tattenuator@path#1{\pgf@circ@bipole@path{tattenuator}{#1}}
\def\pgf@circ@vtattenuator@path#1{\pgf@circ@bipole@path{vtattenuator}{#1}}
\def\pgf@circ@phaseshifter@path#1{\pgf@circ@bipole@path{phaseshifter}{#1}}
\def\pgf@circ@vphaseshifter@path#1{\pgf@circ@bipole@path{vphaseshifter}{#1}}
\def\pgf@circ@detector@path#1{\pgf@circ@bipole@path{detector}{#1}}

%%Mechanical
\def\pgf@circ@spring@path#1{\pgf@circ@bipole@path{spring}{#1}}
\def\pgf@circ@mass@path#1{\pgf@circ@bipole@path{mass}{#1}}
\def\pgf@circ@damper@path#1{\pgf@circ@bipole@path{damper}{#1}}
\def\pgf@circ@viscoe@path#1{\pgf@circ@bipole@path{viscoe}{#1}}

%% Styles

\def\comnpatname{\ifpgf@circuit@compat *\else\fi}
\def\compattikzset#1{\tikzset{\comnpatname#1}}

%\def\ctikzsetbipole#1#2{%
%	\tikzset{#1/.style= {to path=#2, \circuitikzbasekey, l=##1}}%
%}

\compattikzset{spring/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@spring@path, l=#1}}
\compattikzset{mass/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@mass@path, l=#1}}
\compattikzset{damper/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@damper@path, l=#1}}
\compattikzset{viscoe/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@viscoe@path, l=#1}}
\compattikzset{resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@resistor@path, l=#1}}
\compattikzset{american resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{resistor}{#1}, l=#1}}
\compattikzset{european resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{generic}{#1}, l=#1}}
\compattikzset{potentiometer/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@potentiometer@path, l=#1}}
\compattikzset{varistor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@varistor@path, l=#1}}
\compattikzset{photoresistor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@photoresistor@path, l=#1}}
\compattikzset{thermistor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermistor@path, l=#1}}
\compattikzset{thermistor ptc/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermistorptc@path, l=#1}}
\compattikzset{thermistor ntc/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermistorntc@path, l=#1}}
\compattikzset{american potentiometer/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{potentiometer}{#1}, l=#1}}
\compattikzset{european potentiometer/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{genericpotentiometer}{#1}, l=#1}}
\compattikzset{variable resistor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vresistor@path, l=#1}}
\compattikzset{variable american resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{vresistor}{#1}, l=#1}}
\compattikzset{variable european resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{tgeneric}{#1}, l=#1}}
\compattikzset{capacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@capacitor@path, l=#1}}
\compattikzset{elko/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ecapacitor@path, l=#1}}
\compattikzset{ecapacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ecapacitor@path, l=#1}}
% polar capacitor is deprecated, use curved capacitor instead
\compattikzset{polar capacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@polarcapacitor@path, l=#1}}
\compattikzset{curved capacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ccapacitor@path, l=#1}}
\compattikzset{variable capacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vcapacitor@path, l=#1}}
\compattikzset{piezoelectric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@piezoelectric@path, l=#1}}
\compattikzset{battery/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@battery@path, \circuitikzbasekey/bipole/is voltage=true,  \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{battery1/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@batteryone@path, \circuitikzbasekey/bipole/is voltage=true,  \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{battery2/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@batterytwo@path, \circuitikzbasekey/bipole/is voltage=true,  \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@inductor@path, l=#1}}
\compattikzset{gf surge arrester/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@gfsurgearrester@path, l=#1}}
\compattikzset{american gas filled surge arrester/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@americangfsurgearrester@path, l=#1}}
\compattikzset{european gas filled surge arrester/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@europeangfsurgearrester@path, l=#1}}
\compattikzset{gas filled surge arrester/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@gfsurgearrester@path, l=#1}}
\compattikzset{american inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@americaninductor@path, l=#1}}
\compattikzset{cute inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteinductor@path, l=#1}}
\compattikzset{cute choke/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cutechoke@path, l=#1}}
\compattikzset{european inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@europeaninductor@path, l=#1}}
\compattikzset{variable inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vinductor@path, l=#1}}
\compattikzset{variable european inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@veuropeaninductor@path, l=#1}}
\compattikzset{variable american inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vamericaninductor@path, l=#1}}
\compattikzset{variable cute inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vcuteinductor@path, l=#1}}
\compattikzset{tline/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@tline@path, l=#1}}
\compattikzset{transmission line/.style = {tline = #1}}
\compattikzset{TL/.style = {tline = #1}}
\compattikzset{mstline/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@mstline@path, l=#1}}
\compattikzset{european voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsource@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{american voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourceam@path, \circuitikzbasekey/bipole/is voltage=true, v=#1}}
\compattikzset{european current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isource@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{american current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isourceam@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{empty controlled source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ecsource@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{european controlled voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cvsource@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{american controlled voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cvsourceam@path, \circuitikzbasekey/bipole/is voltage=true, v=#1}}
\compattikzset{european controlled current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cisource@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{american controlled current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cisourceam@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{sinusoidal voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourcesin@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1 }}
\compattikzset{square voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourcesquare@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1 }}
\compattikzset{triangle voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourcetri@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1 }}
\compattikzset{sinusoidal current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isourcesin@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{controlled sinusoidal voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cvsourcesin@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{controlled sinusoidal current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cisourcesin@path, \circuitikzbasekey/bipole/is current=true, i=#1}}

\compattikzset{voltage source/.style = {\comnpatname \ifpgf@circuit@europeanvoltage european \else american \fi voltage source, \circuitikzbasekey/bipole/is voltage=true, v=#1}}
\compattikzset{current source/.style = {\comnpatname \ifpgf@circuit@europeancurrent european \else american \fi current source = #1, \circuitikzbasekey/bipole/is current=true}}
\compattikzset{controlled voltage source/.style = {\comnpatname \ifpgf@circuit@europeanvoltage european \else american \fi controlled voltage source, \circuitikzbasekey/bipole/is voltage=true, v=#1}}
\compattikzset{controlled current source/.style = {\comnpatname \ifpgf@circuit@europeancurrent european \else american \fi controlled current source = #1, \circuitikzbasekey/bipole/is current=true}}


\compattikzset{generic/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@generic@path, l=#1}}
\compattikzset{ageneric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ageneric@path, l=#1}}
\compattikzset{tgeneric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@tgeneric@path, l=#1}}
\compattikzset{fullgeneric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullgeneric@path, l=#1}}
\compattikzset{tfullgeneric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@tfullgeneric@path, l=#1}}
\compattikzset{short/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@short@path}}
\compattikzset{open/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@open@path}}

\compattikzset{lamp/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@lamp@path}}
\compattikzset{bulb/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bulb@path, l=#1}}

\compattikzset{squid/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@squid@path}}
\compattikzset{barrier/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@barrier@path}}
\compattikzset{thermocouple/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermocouple@path}}
\compattikzset{fuse/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fuse@path}}
\compattikzset{asymmetric fuse/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@afuse@path}}

\compattikzset{twoport/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@twoport@path}}
\compattikzset{vco/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vco@path}}
\compattikzset{bandpass/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bandpass@path}}
\compattikzset{bandstop/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bandstop@path}}
\compattikzset{highpass/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@highpass@path}}
\compattikzset{lowpass/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@lowpass@path}}
\compattikzset{adc/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@adc@path}}
\compattikzset{dac/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@dac@path}}
\compattikzset{dsp/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@dsp@path}}
\compattikzset{fft/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fft@path}}
\compattikzset{amp/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@amp@path}}
\compattikzset{vamp/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vamp@path}}
\compattikzset{piattenuator/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@piattenuator@path}}
\compattikzset{vpiattenuator/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vpiattenuator@path}}
\compattikzset{tattenuator/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@tattenuator@path}}
\compattikzset{vtattenuator/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vtattenuator@path}}
\compattikzset{phaseshifter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@phaseshifter@path}}
\compattikzset{vphaseshifter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vphaseshifter@path}}
\compattikzset{detector/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@detector@path}}

% % % % % %
% % Begin of Diodes
% % % % % %

\def\pgf@circ@fulldiode@path#1{\pgf@circ@bipole@path{fulldiode}{#1}}
\def\pgf@circ@fullzdiode@path#1{\pgf@circ@bipole@path{fullzdiode}{#1}}
\def\pgf@circ@fullzzdiode@path#1{\pgf@circ@bipole@path{fullzzdiode}{#1}}
\def\pgf@circ@fullsdiode@path#1{\pgf@circ@bipole@path{fullsdiode}{#1}}
\def\pgf@circ@fulltdiode@path#1{\pgf@circ@bipole@path{fulltdiode}{#1}}
\def\pgf@circ@fulllediode@path#1{\pgf@circ@bipole@path{fulllediode}{#1}}
\def\pgf@circ@fullpdiode@path#1{\pgf@circ@bipole@path{fullpdiode}{#1}}
\def\pgf@circ@fullvarcap@path#1{\pgf@circ@bipole@path{fullvarcap}{#1}}
\def\pgf@circ@fullbidirectionaldiode@path#1{\pgf@circ@bipole@path{fullbidirectionaldiode}{#1}}
\def\pgf@circ@emptydiode@path#1{\pgf@circ@bipole@path{emptydiode}{#1}}
\def\pgf@circ@emptyzdiode@path#1{\pgf@circ@bipole@path{emptyzdiode}{#1}}
\def\pgf@circ@emptyzzdiode@path#1{\pgf@circ@bipole@path{emptyzzdiode}{#1}}
\def\pgf@circ@emptysdiode@path#1{\pgf@circ@bipole@path{emptysdiode}{#1}}
\def\pgf@circ@emptytdiode@path#1{\pgf@circ@bipole@path{emptytdiode}{#1}}
\def\pgf@circ@emptylediode@path#1{\pgf@circ@bipole@path{emptylediode}{#1}}
\def\pgf@circ@emptypdiode@path#1{\pgf@circ@bipole@path{emptypdiode}{#1}}
\def\pgf@circ@emptyvarcap@path#1{\pgf@circ@bipole@path{emptyvarcap}{#1}}
\def\pgf@circ@emptybidirectionaldiode@path#1{\pgf@circ@bipole@path{emptybidirectionaldiode}{#1}}

\compattikzset{full diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fulldiode@path}}
\compattikzset{full Schottky diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullsdiode@path}}
\compattikzset{full Zener diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullzdiode@path}}
\compattikzset{full ZZener diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullzzdiode@path}}
\compattikzset{full tunnel diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fulltdiode@path}}
\compattikzset{full photodiode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullpdiode@path}}
\compattikzset{full led/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fulllediode@path}}
\compattikzset{full varcap/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullvarcap@path}}
\compattikzset{full bidirectionaldiode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullbidirectionaldiode@path}}
\compattikzset{full thyristor/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullthyristor@path}}
\compattikzset{full triac/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@fulltriac@path}}

\compattikzset{empty diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptydiode@path}}
\compattikzset{empty Schottky diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptysdiode@path}}
\compattikzset{empty Zener diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptyzdiode@path}}
\compattikzset{empty ZZener diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptyzzdiode@path}}
\compattikzset{empty tunnel diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptytdiode@path}}
\compattikzset{empty photodiode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptypdiode@path}}
\compattikzset{empty led/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptylediode@path}}
\compattikzset{empty varcap/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptyvarcap@path}}
\compattikzset{empty bidirectionaldiode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptybidirectionaldiode@path}}
\compattikzset{empty thyristor/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptythyristor@path}}
\compattikzset{empty triac/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptytriac@path}}

\compattikzset{stroke diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptydiode@path}}
\compattikzset{stroke Schottky diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptysdiode@path}}
\compattikzset{stroke Zener diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptyzdiode@path}}
\compattikzset{stroke ZZener diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptyzzdiode@path}}
\compattikzset{stroke tunnel diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptytdiode@path}}
\compattikzset{stroke photodiode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptypdiode@path}}
\compattikzset{stroke led/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptylediode@path}}
\compattikzset{stroke varcap/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptyvarcap@path}}
\compattikzset{stroke thyristor/.style =  {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptythyristor@path}}
%\compattikzset{stroke triac/.style =  {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptytriac@path}}

\def\pgfcircdiodestylemacro{\ifpgf@circuit@strokediode stroke \else\ifpgf@circuit@fulldiode full \else empty \fi\fi}

\compattikzset{Schottky diode/.style = {\comnpatname \pgfcircdiodestylemacro Schottky diode}}
\compattikzset{Zener diode/.style = {\comnpatname \pgfcircdiodestylemacro Zener diode}}
\compattikzset{ZZener diode/.style = {\comnpatname \pgfcircdiodestylemacro ZZener diode}}
\compattikzset{tunnel diode/.style = {\comnpatname \pgfcircdiodestylemacro tunnel diode}}
\compattikzset{photodiode/.style = {\comnpatname \pgfcircdiodestylemacro photodiode}}
\compattikzset{led/.style = {\comnpatname \pgfcircdiodestylemacro led}}
\compattikzset{varcap/.style = {\comnpatname \pgfcircdiodestylemacro varcap}}
\compattikzset{diode/.style = {\comnpatname \pgfcircdiodestylemacro diode}}
\compattikzset{thyristor/.style =  {\comnpatname \pgfcircdiodestylemacro thyristor}}
\compattikzset{triac/.style =  {\comnpatname \ifpgf@circuit@fulldiode full \else empty \fi triac}}%no stroke triac!
\compattikzset{bidirectionaldiode/.style =  {\comnpatname \ifpgf@circuit@fulldiode full \else empty \fi bidirectionaldiode}}%no stroke bidirectionaldiode! (based on triac)

%% Define Shortcuts
\compattikzset{Do/.style = {\comnpatname empty diode}}
\compattikzset{tDo/.style = {\comnpatname empty tunnel diode}}
\compattikzset{zDo/.style = {\comnpatname empty Zener diode}}
\compattikzset{zzDo/.style = {\comnpatname empty ZZener diode}}
\compattikzset{sDo/.style = {\comnpatname empty Schottky diode}}
\compattikzset{pDo/.style = {\comnpatname empty photodiode}}
\compattikzset{leDo/.style = {\comnpatname empty led}}
\compattikzset{VCo/.style = {\comnpatname empty varcap}}
\compattikzset{biDo/.style = {\comnpatname empty bidirectionaldiode}}
\compattikzset{Tyo/.style = {\comnpatname empty thyristor}}
\compattikzset{Tro/.style = {\comnpatname empty triac}}

\compattikzset{D*/.style = {\comnpatname full diode}}
\compattikzset{tD*/.style = {\comnpatname full tunnel diode}}
\compattikzset{zD*/.style = {\comnpatname full Zener diode}}
\compattikzset{zzD*/.style = {\comnpatname full ZZener diode}}
\compattikzset{sD*/.style = {\comnpatname full Schottky diode}}
\compattikzset{pD*/.style = {\comnpatname full photodiode}}
\compattikzset{leD*/.style = {\comnpatname full led}}
\compattikzset{VC*/.style = {\comnpatname full varcap}}
\compattikzset{biD*/.style = {\comnpatname full bidirectionaldiode}}
\compattikzset{Ty*/.style = {\comnpatname full thyristor}}
\compattikzset{Tr*/.style = {\comnpatname full triac}}

\compattikzset{D/.style = {\comnpatname diode}}
\compattikzset{tD/.style = {\comnpatname tunnel diode}}
\compattikzset{zD/.style = {\comnpatname Zener diode}}
\compattikzset{zzD/.style = {\comnpatname ZZener diode}}
\compattikzset{sD/.style = {\comnpatname Schottky diode}}
\compattikzset{pD/.style = {\comnpatname photodiode}}
\compattikzset{leD/.style = {\comnpatname led}}
\compattikzset{VC/.style = {\comnpatname varcap}}
\compattikzset{biD/.style = {\comnpatname bidirectionaldiode}}
\compattikzset{Ty/.style = {\comnpatname thyristor}}
\compattikzset{Tr/.style = {\comnpatname triac}}

\compattikzset{D-/.style = {\comnpatname stroke diode}}
\compattikzset{tD-/.style = {\comnpatname stroke tunnel diode}}
\compattikzset{zD-/.style = {\comnpatname stroke Zener diode}}
\compattikzset{zzD-/.style = {\comnpatname stroke ZZener diode}}
\compattikzset{sD-/.style = {\comnpatname stroke Schottky diode}}
\compattikzset{pD-/.style = {\comnpatname stroke photodiode}}
\compattikzset{leD-/.style = {\comnpatname stroke led}}
\compattikzset{VC-/.style = {\comnpatname stroke varcap}}
\compattikzset{Ty-/.style = {\comnpatname stroke thyristor}}
\compattikzset{Tr-/.style = {\comnpatname empty triac}}%no stroke triac!
\compattikzset{biD-/.style = {\comnpatname empty bidirectionaldiode}}%no stroke bidirectionaldiode! (based on triac)

% % % % % %
% % End of Diodes
% % % % % %


\compattikzset{memristor/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@memristor@path}}
\compattikzset{closing switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cspst@path, l=#1}}
\compattikzset{opening switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ospst@path, l=#1}}
\compattikzset{ncs/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ncs@path, l=#1}}
\compattikzset{nos/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@nos@path, l=#1}}
\compattikzset{normal closed switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ncs@path, l=#1}}
\compattikzset{normal open switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@nos@path, l=#1}}
\compattikzset{switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cspst@path, l=#1}}
\compattikzset{push button/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@pushbutton@path, l=#1}}
\compattikzset{nopb/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@pushbutton@path, l=#1}}
\compattikzset{normally open push button/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@pushbutton@path, l=#1}}
\compattikzset{ncpb/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ncpushbutton@path, l=#1}}
\compattikzset{normally closed push button/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ncpushbutton@path, l=#1}}
\compattikzset{toggle switch/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@toggleswitch@path}}

\compattikzset{ammeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ammeter@path}}
\compattikzset{voltmeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@voltmeter@path}}
\compattikzset{ohmmeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ohmmeter@path}}
\tikzset{oscope/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@oscope@path, l=#1}}

% cute switches
%% closed cute switch
\def\pgf@circ@cuteclosedswitch@path#1{\pgf@circ@bipole@path{cuteclosedswitch}{#1}}
\compattikzset{cute closed switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteclosedswitch@path, l=#1}}
\compattikzset{ccsw/.style= {\comnpatname cute closed switch= #1}}

%% open cute switch
\def\pgf@circ@cuteopenswitch@path#1{\pgf@circ@bipole@path{cuteopenswitch}{#1}}
\compattikzset{cute open switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteopenswitch@path, l=#1}}
\compattikzset{cosw/.style= {\comnpatname cute open switch= #1}}

%% closing cute switch
\def\pgf@circ@cuteclosingswitch@path#1{\pgf@circ@bipole@path{cuteclosingswitch}{#1}}
\compattikzset{cute closing switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteclosingswitch@path, l=#1}}
\compattikzset{ccgsw/.style= {\comnpatname cute closing switch= #1}}

%% opening cute switch
\def\pgf@circ@cuteopeningswitch@path#1{\pgf@circ@bipole@path{cuteopeningswitch}{#1}}
\compattikzset{cute opening switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteopeningswitch@path, l=#1}}
\compattikzset{cogsw/.style= {\comnpatname cute opening switch= #1}}


% short forms
\compattikzset{esource/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@esource@path, \circuitikzbasekey/bipole/is voltage=true,\circuitikzbasekey/bipole/is voltageoutsideofsymbol=true,  v=#1}}
\compattikzset{pvsource/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@pvsource@path, \circuitikzbasekey/bipole/is voltage=true,\circuitikzbasekey/bipole/is voltageoutsideofsymbol=true,  v=#1}}
\compattikzset{dcvsource/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@dcvsource@path, \circuitikzbasekey/bipole/is voltage=true,\circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{dcisource/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@dcisource@path, \circuitikzbasekey/bipole/is current=true, l=#1}}

\compattikzset{ioosource/.style = {\circuitikzbasekey, \circuitikzbasekey/bipole/is current=true,/tikz/to path=\pgf@circ@oosource@path, i=#1}}
\compattikzset{voosource/.style = {\circuitikzbasekey, \circuitikzbasekey/bipole/is voltage=true,/tikz/to path=\pgf@circ@oosource@path, v=#1}}

\compattikzset{vsource/.style = {\comnpatname voltage source = #1}}
\compattikzset{isource/.style = {\comnpatname current source = #1}}
\compattikzset{cisource/.style = {\comnpatname controlled current source = #1}}
\compattikzset{ecsource/.style = {\comnpatname empty controlled source = #1}}
\compattikzset{cvsource/.style = {\comnpatname controlled voltage source = #1}}
\compattikzset{vsourcesin/.style = {\comnpatname sinusoidal voltage source = #1}}
\compattikzset{vsourcesquare/.style = {\comnpatname square voltage source = #1}}
\compattikzset{vsourcetri/.style = {triangle voltage source = #1}}
\compattikzset{isourcesin/.style = {\comnpatname sinusoidal current source = #1}}
\compattikzset{cisourcesin/.style = {\comnpatname controlled sinusoidal current source = #1}}
\compattikzset{cvsourcesin/.style = {\comnpatname controlled sinusoidal  voltage source = #1}}

\compattikzset{controlled vsource/.style = {\comnpatname controlled voltage source = #1}}
\compattikzset{controlled isource/.style = {\comnpatname controlled current source = #1}}
\compattikzset{controlled vsourcesin/.style = {\comnpatname controlled sinusoidal  voltage source = #1}}
\compattikzset{controlled isourcesin/.style = {\comnpatname controlled sinusoidal current source = #1}}

\compattikzset{R/.style= {\comnpatname resistor = #1}}
\compattikzset{vR/.style= {\comnpatname variable resistor = #1}}
\compattikzset{phR/.style= {\comnpatname photoresistor = #1}}
\compattikzset{thR/.style= {\comnpatname thermistor = #1}}
\compattikzset{thRp/.style= {\comnpatname thermistor ptc= #1}}
\compattikzset{thRn/.style= {\comnpatname thermistor ntc= #1}}
\compattikzset{pR/.style= {\comnpatname potentiometer = #1}}
\compattikzset{C/.style = {\comnpatname capacitor = #1}}
\compattikzset{eC/.style = {\comnpatname ecapacitor = #1}}
%% pC is deprecated, use cC instead
\compattikzset{pC/.style = {\comnpatname polar capacitor = #1}}
\compattikzset{cC/.style = {\comnpatname curved capacitor = #1}}
\compattikzset{vC/.style = {\comnpatname variable capacitor = #1}}
\compattikzset{PZ/.style = {\comnpatname piezoelectric = #1}}
\compattikzset{L/.style = {\comnpatname inductor = #1}}
\compattikzset{vL/.style = {\comnpatname variable inductor = #1}}
\compattikzset{V/.style = {\comnpatname voltage source = #1}}
\compattikzset{cV/.style = {\comnpatname controlled voltage source = #1}}
\compattikzset{sV/.style = {\comnpatname sinusoidal voltage source = #1}}
\compattikzset{sqV/.style = {\comnpatname square voltage source = #1}}
\compattikzset{tV/.style = {\comnpatname triangle voltage source = #1}}
\compattikzset{csV/.style = {\comnpatname controlled sinusoidal voltage source = #1}}
\def\pgf@temp#1{
    \compattikzset{V#1/.style = {\comnpatname voltage source, v#1=##1} }
    \compattikzset{cV#1/.style = {\comnpatname controlled  voltage source, v#1=##1} }
    \compattikzset{sV#1/.style = {\comnpatname sinusoidal  voltage source, v#1=##1} }
    \compattikzset{csV#1/.style = {\comnpatname controlled sinusoidal voltage source, v#1=##1} }
}
\pgf@temp{_>} \pgf@temp{_<} \pgf@temp{^>} \pgf@temp{^<}
\pgf@temp{>} \pgf@temp{<} \pgf@temp{^} \pgf@temp{_}

%current sources
\compattikzset{I/.style = {\comnpatname current source = #1}}
\compattikzset{cI/.style = {\comnpatname controlled current source = #1}}
\compattikzset{sI/.style = {\comnpatname sinusoidal current source = #1}}
\compattikzset{csI/.style = {\comnpatname controlled sinusoidal current source = #1}}
\def\pgf@temp#1{
    \compattikzset{I#1/.style = {\comnpatname current source, i#1=##1} }
    \compattikzset{cI#1/.style = {\comnpatname controlled current source, i#1=##1} }
    \compattikzset{sI#1/.style = {\comnpatname sinusoidal current source, i#1=##1} }
    \compattikzset{csI#1/.style = {\comnpatname controlled sinusoidal current source, i#1=##1} }
}
\pgf@temp{_>} \pgf@temp{_<} \pgf@temp{^>} \pgf@temp{^<}
\pgf@temp{>_} \pgf@temp{<_} \pgf@temp{>^} \pgf@temp{<^}
\pgf@temp{>} \pgf@temp{<} \pgf@temp{^} \pgf@temp{_}

% cute sources
\def\pgf@circ@vsourceC@path#1{\pgf@circ@bipole@path{vsourceC}{#1}}
\compattikzset{cute european voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourceC@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{vsourceC/.style= {\comnpatname cute european voltage source= #1}}
\compattikzset{ceV/.style= {\comnpatname cute european voltage source= #1}}

\def\pgf@circ@isourceC@path#1{\pgf@circ@bipole@path{isourceC}{#1}}
\compattikzset{cute european current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isourceC@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{isourceC/.style= {\comnpatname cute european current source= #1}}
\compattikzset{ceI/.style= {\comnpatname cute european current source= #1}}

\def\pgf@circ@cvsourceC@path#1{\pgf@circ@bipole@path{cvsourceC}{#1}}
\compattikzset{cute european controlled voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cvsourceC@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{cvsourceC/.style= {\comnpatname cute european controlled voltage source= #1}}
\compattikzset{cceV/.style= {\comnpatname cute european controlled voltage source= #1}}

\def\pgf@circ@cisourceC@path#1{\pgf@circ@bipole@path{cisourceC}{#1}}
\compattikzset{cute european controlled current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cisourceC@path,  \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{cisourceC/.style= {\comnpatname cute european controlled current source= #1}}
\compattikzset{cceI/.style= {\comnpatname cute european controlled current source= #1}}

% noise sources
\def\pgf@circ@vsourceN@path#1{\pgf@circ@bipole@path{vsourceN}{#1}}
\compattikzset{noise voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourceN@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{vsourceN/.style= {\comnpatname noise voltage source= #1}}
\compattikzset{nV/.style= {\comnpatname noise voltage source= #1}}

\def\pgf@circ@isourceN@path#1{\pgf@circ@bipole@path{isourceN}{#1}}
\compattikzset{noise current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isourceN@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{isourceN/.style= {\comnpatname noise current source= #1}}
\compattikzset{nI/.style= {\comnpatname noise current source= #1}}

% resistive sensor american style
\def\pgf@circ@resistivesens@path#1{\pgf@circ@bipole@path{resistivesens}{#1}}
\compattikzset{american resistive sensor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@resistivesens@path, l=#1}}
\compattikzset{european resistive sensor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermistorntc@path, l=#1}}
\compattikzset{resistive sensor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@sresistor@path, l=#1}}
\compattikzset{sR/.style= {\comnpatname resistive sensor= #1}}

\compattikzset{capacitive sensor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@capacitivesens@path, l=#1}}
\compattikzset{sC/.style= {\comnpatname capacitive sensor= #1}}

\compattikzset{cute inductive sensor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteinductivesens@path, l=#1}}
\compattikzset{european inductive sensor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@europeaninductivesens@path, l=#1}}
\compattikzset{american inductive sensor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@americaninductivesens@path, l=#1}}
\compattikzset{inductive sensor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@inductivesens@path, l=#1}}
\compattikzset{sL/.style= {\comnpatname inductive sensor= #1}}

\compattikzset{Mr/.style = {\comnpatname memristor}}

\compattikzset{cspst/.style = {\comnpatname closing switch = #1}}
\compattikzset{ospst/.style = {\comnpatname opening switch = #1}}
\compattikzset{spst/.style = {\comnpatname switch = #1}}

\compattikzset{afuse/.style = {\comnpatname asymmetric fuse=#1}}

\compattikzset{vdd/.style = {\comnpatname vcc = #1}}
\compattikzset{vss/.style = {\comnpatname vee = #1}}

% activate the to-style crossing
\def\pgf@circ@crossing@path#1{\pgf@circ@bipole@path{crossing}{#1}}
\compattikzset{crossing/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@crossing@path, l=#1}}
\compattikzset{xing/.style= {\comnpatname crossing= #1}}

%% loudspeaker and microphone

\def\pgf@circ@loudspeaker@path#1{\pgf@circ@bipole@path{loudspeaker}{#1}}
\compattikzset{loudspeaker/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@loudspeaker@path, l=#1}}

\def\pgf@circ@mic@path#1{\pgf@circ@bipole@path{mic}{#1}}
\compattikzset{mic/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@mic@path, l=#1}}

% more instrument
\def\pgf@circ@rmeter@path#1{\pgf@circ@bipole@path{rmeter}{#1}}
\compattikzset{rmeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@rmeter@path, l=#1}}
\def\pgf@circ@rmeterwa@path#1{\pgf@circ@bipole@path{rmeterwa}{#1}}
\compattikzset{rmeterwa/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@rmeterwa@path, l=#1}}
\def\pgf@circ@smeter@path#1{\pgf@circ@bipole@path{smeter}{#1}}
\compattikzset{smeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@smeter@path, l=#1}}
% current loop probes
\def\pgf@circ@iloop@path#1{\pgf@circ@bipole@path{iloop}{#1}}
\compattikzset{iloop/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@iloop@path, l=#1}}
\def\pgf@circ@iloop2@path#1{\pgf@circ@bipole@path{iloop2}{#1}}
\compattikzset{iloop2/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@iloop2@path, l=#1}}
% qucs-style probes
\def\pgf@circ@qiprobe@path#1{\pgf@circ@bipole@path{qiprobe}{#1}}
\compattikzset{qiprobe/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@qiprobe@path, l=#1}}
\def\pgf@circ@qvprobe@path#1{\pgf@circ@bipole@path{qvprobe}{#1}}
\compattikzset{qvprobe/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@qvprobe@path, l=#1}}
\def\pgf@circ@qpprobe@path#1{\pgf@circ@bipole@path{qpprobe}{#1}}
\compattikzset{qpprobe/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@qpprobe@path, l=#1}}


% Transistor like bipoles

\def\pgf@circ@trans@path#1#2{
    \pgfextra{
        \edef\pgf@temp{\ctikzvalof{bipole/name}}
        \def\pgf@circ@temp{#2}
        \ifx\pgf@temp\pgf@circ@temp % if it has not a name
            \pgfmathrandominteger{\pgf@circ@rand}{1000}{9999}
            \ctikzset{bipole/name = trans\pgf@circ@rand} % create it
        \fi
    }
    \ifpgf@circuit@bipole@inverted
        (\tikztostart) node[coordinate] (\ctikzvalof{bipole/name}end) {}
        (\tikztotarget) node[coordinate] (\ctikzvalof{bipole/name}start) {}
    \else
        (\tikztostart) node[coordinate] (\ctikzvalof{bipole/name}start) {}
        (\tikztotarget) node[coordinate] (\ctikzvalof{bipole/name}end) {}
    \fi
    \pgfextra{
        \pgfmathanglebetweenpoints{\pgfpointanchor{\ctikzvalof{bipole/name}start}{center}}
        {\pgfpointanchor{\ctikzvalof{bipole/name}end}{center}}
        \pgfmathadd{\pgfmathresult}{-90}
        \pgfmathround{\pgfmathresult}
        \edef\pgf@circ@direction{\pgfmathresult}
    }
    ($(\tikztostart) ! .5 ! (\tikztotarget)$)
    node[#1, /tikz/rotate=\pgf@circ@direction, xscale=\ctikzvalof{mirror value}]
    (\ctikzvalof{bipole/name}) {}
    node {\ctikzvalof{bipole/label/name}}
    \ifcsname pgf@anchor@#1@pathstart\endcsname%if special path-anchors are defined, use them!
        (\ctikzvalof{bipole/name}start.center) --(\ctikzvalof{bipole/name}.pathstart)
        (\ctikzvalof{bipole/name}.pathend)  -- (\ctikzvalof{bipole/name}end.center)
    \else
        (\ctikzvalof{bipole/name}start.center) --(\ctikzvalof{bipole/name}.left)
        (\ctikzvalof{bipole/name}.right)  -- (\ctikzvalof{bipole/name}end.center)
    \fi
    \drawpoles
    \pgfextra{
        \pgfcircresetpath
    }
    (\tikztotarget) 	\tikztonodes  % e si continua
}


\def\pgf@circ@definetranspath#1{
	\compattikzset{T#1/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@trans@path{#1}{}, l=##1}}
}

\pgf@circ@definetranspath{elmech}
\pgf@circ@definetranspath{nmos}
\pgf@circ@definetranspath{pmos}
\pgf@circ@definetranspath{hemt}
\pgf@circ@definetranspath{npn}
\pgf@circ@definetranspath{pnp}
\pgf@circ@definetranspath{nfet}
\pgf@circ@definetranspath{nigfete}
\pgf@circ@definetranspath{nigfetd}
\pgf@circ@definetranspath{nigfetebulk}
\pgf@circ@definetranspath{pfet}
\pgf@circ@definetranspath{pigfete}
\pgf@circ@definetranspath{pigfetd}
\pgf@circ@definetranspath{pigfetebulk}
\pgf@circ@definetranspath{njfet}
\pgf@circ@definetranspath{pjfet}
\pgf@circ@definetranspath{pigbt}
\pgf@circ@definetranspath{nigbt}
\pgf@circ@definetranspath{Lpigbt}
\pgf@circ@definetranspath{Lnigbt}


==> pgfcircquadpoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Quadripoles

\long\def\pgfcircdeclarequadpole#1#2#3{
    \pgfdeclareshape{#1}
    {
        \savedmacro{\ctikzclass}{\edef\ctikzclass{inductors}}
        \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
        % shapename
        \savedmacro{\thisshape}{\def\thisshape{\tikz@fig@name}}
        \anchor{center}{
            \northwest
            \pgf@x=0pt
            \pgf@y=0pt
        }
        \savedmacro{\stretto}{\def\stretto{\ctikzvalof{quadpoles/#1/inner}}}
        \savedanchor\northwest{%
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@y=\ctikzvalof{quadpoles/#1/height}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=.5\pgf@circ@scaled@Rlen
            \pgf@x=-\ctikzvalof{quadpoles/#1/width}\pgf@x
        }
        %% we define the upper right (positive coord) dot (which is B1)
        \savedanchor{\innerdot}{%
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@xa=.5\pgf@circ@scaled@Rlen
            \pgf@xa=-\ctikzvalof{quadpoles/#1/width}\pgf@xa
            % by default use the cute inductor size
            \pgfmathsetlength\pgf@x{-\stretto*\pgf@xa-\ctikzvalof{bipoles/cuteinductor/height}*\pgf@circ@scaled@Rlen/2}
            % check if it's american
            \edef\pgf@circ@temp{\ctikzvalof{inductor}}
            \edef\pgf@temp{american}
            \ifx\pgf@circ@temp\pgf@temp
                \pgfmathsetlength\pgf@x{-\stretto*\pgf@xa-\ctikzvalof{bipoles/americaninductor/height}*\pgf@circ@scaled@Rlen/2}
            \fi
            % check if it's european
            \edef\pgf@temp{european}
            \ifx\pgf@circ@temp\pgf@temp
                \pgfmathsetlength\pgf@x{-\stretto*\pgf@xa-\ctikzvalof{bipoles/fullgeneric/height}*\pgf@circ@scaled@Rlen/2}
            \fi
            \pgfmathsetlength\pgf@y{0.5*\pgf@circ@scaled@Rlen}
        }
        \savedanchor{\outerdot}{%
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@xa=.5\pgf@circ@scaled@Rlen
            \pgf@xa=-\ctikzvalof{quadpoles/#1/width}\pgf@xa
            % by default use the cute inductor size
            \pgfmathsetlength\pgf@x{-\stretto*\pgf@xa+\ctikzvalof{bipoles/cuteinductor/height}*\pgf@circ@scaled@Rlen/2}
            % check if it's american
            \edef\pgf@circ@temp{\ctikzvalof{inductor}}
            \edef\pgf@temp{american}
            \ifx\pgf@circ@temp\pgf@temp
                \pgfmathsetlength\pgf@x{-\stretto*\pgf@xa+\ctikzvalof{bipoles/americaninductor/height}*\pgf@circ@scaled@Rlen/2}
            \fi
            % check if it's european
            \edef\pgf@temp{european}
            \ifx\pgf@circ@temp\pgf@temp
                \pgfmathsetlength\pgf@x{-\stretto*\pgf@xa+\ctikzvalof{bipoles/fullgeneric/height}*\pgf@circ@scaled@Rlen/2}
            \fi
            \pgfmathsetlength\pgf@y{0.5*\pgf@circ@scaled@Rlen}
        }
        \anchor{A2}{
            \northwest
            \pgf@y=-\pgf@y
        }
        \anchor{B1}{
            \northwest
            \pgf@x=-\pgf@x
        }
        \anchor{A1}{
            \northwest
        }
        \anchor{B2}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=-\pgf@y
        }
        %% dot's anchors
        \anchor{inner dot A1}{\innerdot\pgf@x=-\pgf@x}
        \anchor{outer dot A1}{\outerdot\pgf@x=-\pgf@x}
        \anchor{inner dot A2}{\innerdot\pgf@x=-\pgf@x\pgf@y=-\pgf@y}
        \anchor{outer dot A2}{\outerdot\pgf@x=-\pgf@x\pgf@y=-\pgf@y}
        \anchor{inner dot B1}{\innerdot}
        \anchor{outer dot B1}{\outerdot}
        \anchor{inner dot B2}{\innerdot\pgf@y=-\pgf@y}
        \anchor{outer dot B2}{\outerdot\pgf@y=-\pgf@y}
        % geographical
        \anchor{north}{
            \northwest
            \pgf@x=0pt
        }
        \anchor{south}{
            \northwest
            \pgf@x=0pt
            \pgf@y=-\pgf@y
        }
        \anchor{west}{
            \northwest
            \pgf@y=0pt
        }
        \anchor{east}{
            \northwest
            \pgf@y=0pt
            \pgf@x=-\pgf@x
        }
        \anchor{south west}{
            \northwest
            \pgf@y=-\pgf@y
        }
        \anchor{north east}{
            \northwest
            \pgf@x=-\pgf@x
        }
        \anchor{north west}{
            \northwest
        }
        \anchor{south east}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=-\pgf@y
        }
        \anchor{base}{
            \northwest
            \pgf@x=0pt
        }
        #3
        \backgroundpath{
            \pgfsetcolor{\ctikzvalof{color}}

            \northwest
            \pgf@circ@res@up = \pgf@y
            \pgf@circ@res@down = -\pgf@y
            \pgf@circ@res@right = -\pgf@x
            \pgf@circ@res@left = \pgf@x
            #2
        }
    }
}


\def\pgf@circ@drawtransformerbasicanchor{
    \ctikzvalof{quadpoles/trans/height}
    \anchor{AA2}{
        \northwest
        \pgf@x=\ctikzvalof{quadpoles/transformer/width1}\pgf@x
        \pgf@x=.7\pgf@x
        \pgf@y=-\pgf@y
        \pgf@y=\ctikzvalof{quadpoles/transformer/height1}\pgf@y
    }
    \anchor{BB1}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@x=\ctikzvalof{quadpoles/transformer/width1}\pgf@x
        \pgf@x=.7\pgf@x
        \pgf@y=\ctikzvalof{quadpoles/transformer/height1}\pgf@y
    }
    \anchor{AA1}{
        \northwest
        \pgf@x=\ctikzvalof{quadpoles/transformer/width1}\pgf@x
        \pgf@x=.7\pgf@x
        \pgf@y=\ctikzvalof{quadpoles/transformer/height1}\pgf@y
    }
    \anchor{BB2}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@x=\ctikzvalof{quadpoles/transformer/width1}\pgf@x
        \pgf@x=.7\pgf@x
        \pgf@y=-\pgf@y
        \pgf@y=\ctikzvalof{quadpoles/transformer/height1}\pgf@y
    }
}

%% Null styles that can be used to change individually the L1 and L2
%% inductors of the transformer.

\ctikzset{transformer L1/.style={}}
\ctikzset{transformer L2/.style={}}

\def\pgf@circ@drawtransformerbasicbody{
    \pgfscope
        \pgfslopedattimetrue
        \pgfallowupsidedownattimetrue
        \pgftransformlineattime{.5}{%
            \pgfpoint%
            {\stretto\pgf@circ@res@left}%
            {\pgf@circ@res@up}%
            }{%
            \pgfpoint
            {\stretto\pgf@circ@res@left}%
            {\pgf@circ@res@down}%
        }

        \pgfkeys{\circuitikzbasekey/.cd, transformer L1}
        \edef\pgf@circ@temp{\ctikzvalof{inductor}}%
        \def\pgf@temp{european}%
        \ifx\pgf@temp\pgf@circ@temp%
            \pgfnode{fullgenericshape}{center}{}{\thisshape-L1}{\pgfusepath{stroke}}
        \else%
            \def\pgf@temp{cute}
            \ifx\pgf@temp\pgf@circ@temp%
                \pgfnode{cuteinductorshape}{center}{}{\thisshape-L1}{\pgfusepath{stroke}}
            \else%
                \pgfnode{americaninductorshape}{center}{}{\thisshape-L1}{\pgfusepath{stroke}}
            \fi%
        \fi%


    \endpgfscope
    \pgfscope
        \pgfslopedattimetrue
        \pgfallowupsidedownattimetrue
        \pgftransformlineattime{.5}{%
            \pgfpoint%
            {\stretto\pgf@circ@res@right}%
            {\pgf@circ@res@down}%
            }{%
            \pgfpoint
            {\stretto\pgf@circ@res@right}%
            {\pgf@circ@res@up}%
        }

        \pgfkeys{\circuitikzbasekey/.cd, transformer L2}
        \edef\pgf@circ@temp{\ctikzvalof{inductor}}%
        \def\pgf@temp{european}%
        \ifx\pgf@temp\pgf@circ@temp%
            \pgfnode{fullgenericshape}{center}{}{\thisshape-L2}{\pgfusepath{stroke}}
        \else%
            \def\pgf@temp{cute}
            \ifx\pgf@temp\pgf@circ@temp%
                \pgfnode{cuteinductorshape}{center}{}{\thisshape-L2}{\pgfusepath{stroke}}
            \else%
                \pgfnode{americaninductorshape}{center}{}{\thisshape-L2}{\pgfusepath{stroke}}
            \fi%
        \fi%

    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpointanchor{\thisshape-L1}{b}}

    \pgfpathmoveto{\pgfpointanchor{\thisshape-L1}{a}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpointanchor{\thisshape-L2}{a}}

    \pgfpathmoveto{\pgfpointanchor{\thisshape-L2}{b}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}

    \pgfusepath{draw}

}


\pgfcircdeclarequadpole{transformer}{
    \pgf@circ@drawtransformerbasicbody
}{\pgf@circ@drawtransformerbasicanchor}

\pgfcircdeclarequadpole{transformer core}{

    \pgf@circ@drawtransformerbasicbody

    % use the chocke line thickness
    \pgfsetlinewidth{\ctikzvalof{bipoles/cutechoke/cthick}\pgflinewidth}

    % Find the distance from center for the lines representing the core
    % the 2.5 is for backward compatibility --- the distance was calculated as a fraction
    % of the whole component, now as a fraction of the distance between coils, to be
    % compatible with the quadpoles "inner" style.
    \pgfmathsetlength{\pgf@circ@res@other}{2.5*\stretto*\ctikzvalof{quadpoles/transformer core/core width}*\pgf@circ@res@right}

    \pgfmoveto{\pgfpoint%
        {\pgf@circ@res@other}%
        {\ctikzvalof{quadpoles/transformer core/core height}\pgf@circ@res@down}%
    }
    \pgflineto{
        \pgfpoint%
        {\pgf@circ@res@other}%
        {\ctikzvalof{quadpoles/transformer core/core height}\pgf@circ@res@up}%
    }

    %% this should be just -\pgf@circ@res@other, but in case someone define an asymmetric trafo someday...
    \pgfmathsetlength{\pgf@circ@res@other}{2.5*\stretto*\ctikzvalof{quadpoles/transformer core/core width}*\pgf@circ@res@left}
    \pgfmoveto{\pgfpoint%
        {\pgf@circ@res@other}%
        {\ctikzvalof{quadpoles/transformer core/core height}\pgf@circ@res@down}%
    }
    \pgflineto{
        \pgfpoint%
        {\pgf@circ@res@other}%
        {\ctikzvalof{quadpoles/transformer core/core height}\pgf@circ@res@up}%
    }

    \pgf@circ@setlinewidth{bipoles}{\pgflinewidth}
    \pgfusepath{draw}
}{\pgf@circ@drawtransformerbasicanchor}


\pgfcircdeclarequadpole{gyrator}{

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}

    \pgfusepath{draw}

    \pgf@circ@setlinewidth{quadpoles}{\pgflinewidth}
    \pgfmathsetlength{\pgf@circ@res@other}{min(.7*\stretto*\pgf@circ@res@up, .8*\pgf@circ@res@right)} % radius
    \pgfpathmoveto{\pgfpoint{\stretto\pgf@circ@res@left}{-\pgf@circ@res@other}}
    \pgfpatharc{-90}{90}{\pgf@circ@res@other}
    \pgfpathclose
    \pgf@circ@draworfill

    \pgfpathmoveto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@other}}
    \pgfpatharc{90}{270}{\pgf@circ@res@other}
    \pgfpathclose
    \pgf@circ@draworfill
}{}

%%%%%%%%%%%%%%%%%%%%
%% Block elements
%%%%%%%%%%%%%%%%%%%%

\pgfdeclareshape{mixer}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{blocks}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor\northwest{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \ifpgf@circuit@boxed
            \pgf@y=\ctikzvalof{bipoles/twoport/width}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\ctikzvalof{bipoles/twoport/width}\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
        \else
            \pgf@y=\ctikzvalof{tripoles/mixer/width}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\ctikzvalof{tripoles/mixer/width}\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
        \fi
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{left}{%
        \northwest
        \pgf@y=0pt
    }
    \anchor{1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{2}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{3}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{4}{
        \northwest
        \pgf@y=\pgf@y
        \pgf@x=0pt
    }
    \anchor{in 1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in 2}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{in2}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{center}{
        \pgf@y=0pt
        \pgf@x=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        \pgf@circ@scaled@Rlen=\scaledRlen

        \pgf@circ@res@step=\ctikzvalof{tripoles/mixer/width}\pgf@circ@scaled@Rlen

        \pgfscope
            \pgfstartlinewidth=\pgflinewidth

            % draw outer box
            \ifpgf@circuit@boxed
                \pgfnode{blockbox}{center}{}{pgf@box}{\pgfusepath{draw}}
            \fi

            % draw outer circle
            \ifpgf@circuit@boxed
                \pgf@circ@res@step=.7\pgf@circ@res@step
                \pgfsetdash{}{0pt}	% draw solid circle if boxed
            \else
                \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \fi
            \pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
            \pgf@circ@draworfill

            % draw inner stuff
            \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
            \pgfsetlinewidth{\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathmoveto{\pgfpointpolar{135}{0.5\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpointpolar{-45}{0.5\pgf@circ@res@step}}
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathmoveto{\pgfpointpolar{45}{0.5\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpointpolar{-135}{0.5\pgf@circ@res@step}}
            \pgfusepath{draw}

        \endpgfscope
    }
}

\pgfdeclareshape{adder}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{blocks}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor\northwest{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \ifpgf@circuit@boxed
            \pgf@y=\ctikzvalof{bipoles/twoport/width}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\ctikzvalof{bipoles/twoport/width}\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
        \else
            \pgf@y=\ctikzvalof{tripoles/adder/width}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\ctikzvalof{tripoles/adder/width}\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
        \fi
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{left}{%
        \northwest
        \pgf@y=0pt
    }
    \anchor{1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{2}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{3}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{4}{
        \northwest
        \pgf@y=\pgf@y
        \pgf@x=0pt
    }
    \anchor{in 1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in 2}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{in2}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{center}{
        \pgf@y=0pt
        \pgf@x=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        \pgf@circ@scaled@Rlen=\scaledRlen

        \pgf@circ@res@step=\ctikzvalof{tripoles/adder/width}\pgf@circ@scaled@Rlen

        \pgfscope
            \pgfstartlinewidth=\pgflinewidth

            % draw outer box
            \ifpgf@circuit@boxed
                \pgfnode{blockbox}{center}{}{pgf@box}{\pgfusepath{draw}}
            \fi

            % draw outer circle
            \ifpgf@circuit@boxed
                \pgf@circ@res@step=.7\pgf@circ@res@step{}
                \pgfsetdash{}{0pt}	% draw solid circle if boxed
            \else
                \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \fi
            \pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
            \pgf@circ@draworfill

            % draw inner stuff
            \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
            \pgfsetlinewidth{\pgfstartlinewidth}

            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathmoveto{\pgfpointpolar{0}{0.3\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpointpolar{180}{0.3\pgf@circ@res@step}}
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathmoveto{\pgfpointpolar{90}{0.3\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpointpolar{270}{0.3\pgf@circ@res@step}}
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgfusepath{draw}

        \endpgfscope
    }
}

\pgfdeclareshape{oscillator}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{blocks}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor\northwest{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \ifpgf@circuit@boxed
            \pgf@y=\ctikzvalof{bipoles/twoport/width}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\ctikzvalof{bipoles/twoport/width}\pgf@circ@scaled@Rlen
        \else
            \pgf@y=\ctikzvalof{tripoles/oscillator/width}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\ctikzvalof{tripoles/oscillator/width}\pgf@circ@scaled@Rlen
        \fi
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{north}{
        \northwest
        \pgf@x=.5\pgf@x
    }
    \anchor{south}{
        \northwest
        \pgf@x=.5\pgf@x
        \pgf@y=-\pgf@y
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=0pt
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y}
    \anchor{north east}{ \northwest \pgf@x=0pt\relax}
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{text}{
        \pgf@x=-2\pgf@x
        \advance \pgf@x by -.5\wd\pgfnodeparttextbox
        \advance \pgf@y by -1.5\ht\pgfnodeparttextbox
    }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        \pgf@circ@scaled@Rlen=\scaledRlen

        \pgf@circ@res@step=\ctikzvalof{tripoles/oscillator/width}\pgf@circ@scaled@Rlen{}

        \pgfscope
            \pgfstartlinewidth=\pgflinewidth

            \pgftransformxshift{-0.5\pgf@circ@res@step} % The oscillator is shifted to the left, so a connection comes out of the anchor "east"

            % draw outer box
            \ifpgf@circuit@boxed{}
                \pgfnode{blockbox}{center}{}{pgf@box}{\pgfusepath{draw}}
            \fi

            % draw outer circle
            \ifpgf@circuit@boxed
                \pgf@circ@res@step=.7\pgf@circ@res@step{}
                \pgfsetdash{}{0pt}	% draw solid circle if boxed
            \else
                \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \fi
            \pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
            \pgf@circ@draworfill

            % draw inner sine waves
            \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
            \pgfsetlinewidth{\pgfstartlinewidth}
            \pgfsetcornersarced{\pgfpointorigin}% do not use rounded corners!
            \pgfpathmoveto{\pgfpoint{-0.3\pgf@circ@res@step}{0\pgf@circ@res@step}}
            \pgfpathsine{\pgfpoint{.15\pgf@circ@res@step}{.15\pgf@circ@res@step}}
            \pgfpathcosine{\pgfpoint{.15\pgf@circ@res@step}{-.15\pgf@circ@res@step}}
            \pgfpathsine{\pgfpoint{.15\pgf@circ@res@step}{-.15\pgf@circ@res@step}}
            \pgfpathcosine{\pgfpoint{.15\pgf@circ@res@step}{.15\pgf@circ@res@step}}

            \pgfusepath{draw}

        \endpgfscope
    }
}

\pgfdeclareshape{circulator}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{blocks}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor\northwest{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \ifpgf@circuit@boxed
            \pgf@y=\ctikzvalof{bipoles/twoport/width}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\ctikzvalof{bipoles/twoport/width}\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
        \else
            \pgf@y=\ctikzvalof{tripoles/circulator/width}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\ctikzvalof{tripoles/circulator/width}\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
        \fi
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{left}{%
        \northwest
        \pgf@y=0pt
    }
    \anchor{1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{2}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{3}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        \pgf@circ@scaled@Rlen=\scaledRlen

        \pgf@circ@res@step=\ctikzvalof{tripoles/circulator/width}\pgf@circ@scaled@Rlen

        \pgfscope
            \pgfstartlinewidth=\pgflinewidth

            % draw outer box
            \ifpgf@circuit@boxed
                \pgfnode{blockbox}{center}{}{pgf@box}{\pgfusepath{draw}}
            \fi

            % draw outer circle
            \ifpgf@circuit@boxed{}
                \pgf@circ@res@step=.7\pgf@circ@res@step{}
                \pgfsetdash{}{0pt}	% draw solid circle if boxed
            \else
                \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \fi
            \pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
            \pgf@circ@draworfill

            % inner arrow
            \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
            \pgfsetlinewidth{\pgfstartlinewidth}

            \pgfsetarrowsend{latex}
            \pgfpathmoveto{\pgfpoint{-0.25\pgf@circ@res@step}{0}}
            \pgfpatharc{180}{-90} {0.25\pgf@circ@res@step}
            \pgfpathlineto{\pgfpoint{-5pt}{-0.2\pgf@circ@res@step}}
            \pgfusepath{draw}

            \endpgfscope
        }
    }


% Wilkinson divider
\pgfdeclareshape{wilkinson}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{blocks}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/wilkinson/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x= \pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@x=-\ctikzvalof{tripoles/wilkinson/width}\pgf@x
    }
    \anchor{center}{
        \northwest
        \pgf@x=0pt
        \pgf@y=0pt
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{out1}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-0.5\pgf@y
    }
    \anchor{out2}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=0.5\pgf@y
    }
    \anchor{text}{
        \northwest
        \advance \pgf@y by 0.5\ht\pgfnodeparttextbox
        \pgf@x=-.5\wd\pgfnodeparttextbox
    }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        \pgf@circ@scaled@Rlen=\scaledRlen

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgfstartlinewidth=\pgflinewidth

        % draw outer box
        \pgf@circ@twoportbox

        % draw inner stuff
        \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
        \pgfsetarrows{-} %never draw arrows
        \pgfsetlinewidth{\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@left}{0pt}}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@down}}

        \pgfusepath{draw}

        \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
        % draw inner resisitor - european or american style is recognised
        {
            \pgftransformshift{\pgfpoint{0.5\pgf@circ@res@right}{0pt}}
            \pgftransformrotate{90}

            % calculate size of resistor
            \ifpgf@circuit@europeanresistor
                \pgfmathparse{\pgf@circ@res@up / \pgf@circ@scaled@Rlen / \ctikzvalof{bipoles/generic/width} / 2}
                \pgftransformscale{\pgfmathresult}
                \pgfnode{genericshape}{center}{}{wilk@int@R}{\pgfusepath{fill}}
            \else
                \pgfmathparse{\pgf@circ@res@up / \pgf@circ@scaled@Rlen / \ctikzvalof{bipoles/resistor/width} / 2}
                \pgftransformscale{\pgfmathresult}
                \pgfnode{resistorshape}{center}{}{wilk@int@R}{\pgfusepath{fill}}
            \fi
        }

        \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpointanchor{wilk@int@R}{right}}

        \pgfpathmoveto{\pgfpointanchor{wilk@int@R}{left}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
        \pgfusepath{draw}

    }
}

%% couplers generics
\long\def\pgfcircdeclarefourport#1#2{

    \pgfdeclareshape{#1}{
        \savedmacro{\ctikzclass}{\edef\ctikzclass{blocks}}
        \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
        \anchor{center}{
            \northwest
            \pgf@x=0pt
            \pgf@y=0pt
        }
        \savedanchor\northwest{%
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@y=\ctikzvalof{quadpoles/#1/height}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=.5\pgf@circ@scaled@Rlen
            \pgf@x=-\ctikzvalof{quadpoles/#1/width}\pgf@x
        }
        \anchor{north}{
            \northwest
            \pgf@x=0pt
        }
        \anchor{south}{
            \northwest
            \pgf@x=0pt
            \pgf@y=-\pgf@y
        }
        \anchor{west}{
            \northwest
            \pgf@y=0pt
        }
        \anchor{east}{
            \northwest
            \pgf@y=0pt
            \pgf@x=-\pgf@x
        }
        \anchor{south west}{
            \northwest
            \pgf@y=-\pgf@y
        }
        \anchor{north east}{
            \northwest
            \pgf@x=-\pgf@x
        }
        \anchor{north west}{
            \northwest
        }
        \anchor{south east}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=-\pgf@y
        }
        \anchor{port1}{
            \northwest
            \pgf@y=-0.5\pgf@y
        }
        \anchor{port2}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=-0.5\pgf@y
        }
        \anchor{port3}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=0.5\pgf@y
        }
        \anchor{port4}{
            \northwest
            \pgf@y=0.5\pgf@y
        }
        \anchor{1}{
            \northwest
            \pgf@y=-0.5\pgf@y
        }
        \anchor{2}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=-0.5\pgf@y
        }
        \anchor{3}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=0.5\pgf@y
        }
        \anchor{4}{
            \northwest
            \pgf@y=0.5\pgf@y
        }

        \anchor{text}{
            \northwest
            \advance \pgf@y by 0.5\ht\pgfnodeparttextbox
            \pgf@x=-.5\wd\pgfnodeparttextbox
        }
        \backgroundpath{
            \pgfsetcolor{\ctikzvalof{color}}

            \northwest
            \pgf@circ@res@up = \pgf@y
            \pgf@circ@res@down = -\pgf@y
            \pgf@circ@res@right = -\pgf@x
            \pgf@circ@res@left = \pgf@x
            \pgf@circ@scaled@Rlen=\scaledRlen

            \pgfstartlinewidth=\pgflinewidth

            % draw outer box
            \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgf@circ@draworfill

            % draw inner stuff
            #2

            % draw inner text
            \pgftext[center,x=-0.15\pgf@circ@res@step,y=0]{\ctikzvalof{bipoles/twoport/text}}
        }
    }
}

% four-port
\pgfcircdeclarefourport{fourport}{}

% straight coupler
\pgfcircdeclarefourport{coupler}{
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{0.7\pgf@circ@res@left}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfsetarrows{latex-latex}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.7\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.4\pgf@circ@res@down}}
    \pgfsetarrows{latex-latex}
    \pgfusepath{draw}
}

% "bended" coupler
\pgfcircdeclarefourport{coupler2}{
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
    \pgfusepath{draw}

    \pgfscope
        \pgfpathmoveto{\pgfpoint{0.1\pgf@circ@res@left}{0pt}}
        \pgfpatharc{0}{90} {0.4\pgf@circ@res@up}
        \pgfsetarrowsend{latex}
        \pgfusepath{draw}
    \endpgfscope
    \pgfscope
        \pgfpathmoveto{\pgfpoint{0.1\pgf@circ@res@left}{0pt}}
        \pgfpatharc{0}{-90} {0.4\pgf@circ@res@up}
        \pgfsetarrowsend{latex}
        \pgfusepath{draw}
    \endpgfscope
    \pgfscope
        \pgfpathmoveto{\pgfpoint{0.1\pgf@circ@res@right}{0pt}}
        \pgfpatharc{180}{90} {0.4\pgf@circ@res@up}
        \pgfsetarrowsend{latex}
        \pgfusepath{draw}
    \endpgfscope
    \pgfscope
        \pgfpathmoveto{\pgfpoint{0.1\pgf@circ@res@right}{0pt}}
        \pgfpatharc{-180}{-90} {0.4\pgf@circ@res@up}
        \pgfsetarrowsend{latex}
        \pgfusepath{draw}
    \endpgfscope
}



==> pgfcircshapes.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Other shapes

%% Nothing

\pgfdeclareshape{emptyshape}{
    \savedanchor{\northeast}{%
        \pgf@x=.5\wd\pgfnodeparttextbox%
        \pgf@y=.5\ht\pgfnodeparttextbox%
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}
    \anchor{center}{
        \pgfpointorigin
    }
}

%% Full terminal

\pgfdeclareshape{circ}{
    \anchor{center}{
        \pgfpointorigin
    }
    \savedanchor\northwest{%
        \pgf@y=\ctikzvalof{nodes width}\pgf@circ@Rlen
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchorborder{
        \pgf@circ@res@left=\pgf@x
        \pgf@circ@res@up=\pgf@y
        \pgfpointborderellipse{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}
        }{\pgfpoint{\ctikzvalof{nodes width}*\pgf@circ@Rlen}{\ctikzvalof{nodes width}*\pgf@circ@Rlen}}
    }
    \behindforegroundpath{

        \pgfscope
            \pgfpathcircle{\pgfpointorigin}{\ctikzvalof{nodes width}*\pgf@circ@Rlen}
            \pgfsetcolor{\ctikzvalof{color}}
            \pgfsetfillopacity{1.0}
            \pgfusepath{draw,fill}
        \endpgfscope

    }
}

%% Empty terminal

\pgfdeclareshape{ocirc}{
    \anchor{center}{
        \pgfpointorigin
    }
    \savedanchor\northwest{%
        \pgf@y=\ctikzvalof{nodes width}\pgf@circ@Rlen
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchorborder{
        \pgf@circ@res@left=\pgf@x
        \pgf@circ@res@up=\pgf@y
        \pgfpointborderellipse{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}
        }{\pgfpoint{\ctikzvalof{nodes width}*\pgf@circ@Rlen}{\ctikzvalof{nodes width}*\pgf@circ@Rlen}}
    }

    \behindforegroundpath{

        \pgfscope
            \pgfpathcircle{\pgfpointorigin}{\ctikzvalof{nodes width}*\pgf@circ@Rlen}
            \pgfsetcolor{\ctikzvalof{color}}
            \ifx\tikz@fillcolor\pgfutil@empty
                % set the default fill color to white
                \pgfsetfillcolor{white}
                % ...but override it if the class is defined!
                % note that this element has no class, but will inherit it when used
                % into another component
                \pgf@circ@setifdefinedfill{draw, fill}{draw, fill}
            \else
                \pgfsetfillcolor{\tikz@fillcolor}
            \fi
            \pgfsetfillopacity{1.0}
            \pgfusepath{draw,fill}
        \endpgfscope

    }
}

%% Diamond terminal

\pgfdeclareshape{diamondpole}{
    \anchor{center}{
        \pgfpointorigin
    }
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@y}{sqrt(2)*\ctikzvalof{nodes width}*\pgf@circ@Rlen}
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchorborder{
        % \typeout{IN\space X:\the\pgf@x\space Y:\the\pgf@y}
        \pgfmathsetmacro{\@@switchx}{ifthenelse(\pgf@x>0,1,-1)}
        \pgfmathsetmacro{\@@switchy}{ifthenelse(\pgf@y>0,1,-1)}
        \pgfmathsetlength{\pgf@xa}{abs(\pgf@x)}
        \pgfmathsetlength{\pgf@ya}{abs(\pgf@y)}
        \pgfextracty{\pgf@circ@res@up}{\northwest}
        % \typeout{MID\space X:\the\pgf@xa\space Y:\the\pgf@ya\space L:\the\pgf@circ@res@up}
        % \typeout{MID\space SX:\@@switchx\space SY:\@@switchy}
        \pgfpointintersectionoflines
            {\pgfpointorigin}{\pgfqpoint{\pgf@xa}{\pgf@ya}}
            {\pgfqpoint{0pt}{\pgf@circ@res@up}}{\pgfqpoint{\pgf@circ@res@up}{0pt}}
        % \typeout{CROSS \space X:\the\pgf@x\space Y:\the\pgf@y}
        \pgf@x=\@@switchx\pgf@x
        \pgf@y=\@@switchy\pgf@y
    }
    \behindforegroundpath{
        \pgfscope
            \pgfmathsetlength{\pgf@circ@res@temp}{\ctikzvalof{nodes width}*\pgf@circ@Rlen}
            \pgftransformrotate{45}
            \pgfpathrectanglecorners
            {\pgfpoint{-\pgf@circ@res@temp}{-\pgf@circ@res@temp}}
            {\pgfpoint{\pgf@circ@res@temp}{\pgf@circ@res@temp}}
            \pgfsetcolor{\ctikzvalof{color}}
            \pgfsetfillopacity{1.0}
            \pgfusepath{draw,fill}
        \endpgfscope
    }
}

%% Diamond terminal, unfilled

\pgfdeclareshape{odiamondpole}{
    \anchor{center}{
        \pgfpointorigin
    }
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@y}{sqrt(2)*\ctikzvalof{nodes width}*\pgf@circ@Rlen}
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchorborder{
        % \typeout{IN\space X:\the\pgf@x\space Y:\the\pgf@y}
        \pgfmathsetmacro{\@@switchx}{ifthenelse(\pgf@x>0,1,-1)}
        \pgfmathsetmacro{\@@switchy}{ifthenelse(\pgf@y>0,1,-1)}
        \pgfmathsetlength{\pgf@xa}{abs(\pgf@x)}
        \pgfmathsetlength{\pgf@ya}{abs(\pgf@y)}
        \pgfextracty{\pgf@circ@res@up}{\northwest}
        % \typeout{MID\space X:\the\pgf@xa\space Y:\the\pgf@ya\space L:\the\pgf@circ@res@up}
        % \typeout{MID\space SX:\@@switchx\space SY:\@@switchy}
        \pgfpointintersectionoflines
            {\pgfpointorigin}{\pgfqpoint{\pgf@xa}{\pgf@ya}}
            {\pgfqpoint{0pt}{\pgf@circ@res@up}}{\pgfqpoint{\pgf@circ@res@up}{0pt}}
        % \typeout{CROSS \space X:\the\pgf@x\space Y:\the\pgf@y}
        \pgf@x=\@@switchx\pgf@x
        \pgf@y=\@@switchy\pgf@y
    }
    \behindforegroundpath{
        \pgfscope
            \pgfmathsetlength{\pgf@circ@res@temp}{\ctikzvalof{nodes width}*\pgf@circ@Rlen}
            \pgftransformrotate{45}
            \pgfpathrectanglecorners
            {\pgfpoint{-\pgf@circ@res@temp}{-\pgf@circ@res@temp}}
            {\pgfpoint{\pgf@circ@res@temp}{\pgf@circ@res@temp}}
            \pgfsetcolor{\ctikzvalof{color}}
            \ifx\tikz@fillcolor\pgfutil@empty
                % set the default fill color to white
                \pgfsetfillcolor{white}
                % ...but override it if the class is defined!
                % note that this element has no class, but will inherit it when used
                % into another component
                \pgf@circ@setifdefinedfill{draw, fill}{draw, fill}
            \else
                \pgfsetfillcolor{\tikz@fillcolor}
            \fi
            \pgfsetfillopacity{1.0}
            \pgfusepath{draw,fill}
        \endpgfscope
    }
}

%% square terminal, filled

\pgfdeclareshape{squarepole}{
    \anchor{center}{
        \pgfpointorigin
    }
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@y}{\ctikzvalof{nodes width}*\pgf@circ@Rlen}
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchorborder{
        \pgf@xa=\pgf@x
        \pgf@ya=\pgf@y
        \pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfpointborderrectangle
            {\pgfqpoint{\pgf@xa}{\pgf@ya}}
            {\pgfqpoint{\pgf@circ@res@up}{\pgfqpoint{\pgf@circ@res@up}}}
    }
    \behindforegroundpath{
        \pgfscope
            \pgfmathsetlength{\pgf@circ@res@temp}{\ctikzvalof{nodes width}*\pgf@circ@Rlen}
            \pgfpathrectanglecorners
            {\pgfpoint{-\pgf@circ@res@temp}{-\pgf@circ@res@temp}}
            {\pgfpoint{\pgf@circ@res@temp}{\pgf@circ@res@temp}}
            \pgfsetcolor{\ctikzvalof{color}}
            \pgfsetfillopacity{1.0}
            \pgfusepath{draw,fill}
        \endpgfscope
    }
}
%% square terminal, unfilled

\pgfdeclareshape{osquarepole}{
    \anchor{center}{
        \pgfpointorigin
    }
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@y}{\ctikzvalof{nodes width}*\pgf@circ@Rlen}
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchorborder{
        \pgf@xa=\pgf@x
        \pgf@ya=\pgf@y
        \pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfpointborderrectangle
            {\pgfqpoint{\pgf@xa}{\pgf@ya}}
            {\pgfqpoint{\pgf@circ@res@up}{\pgfqpoint{\pgf@circ@res@up}}}
    }
    \behindforegroundpath{
        \pgfscope
            \pgfmathsetlength{\pgf@circ@res@temp}{\ctikzvalof{nodes width}*\pgf@circ@Rlen}
            \pgfpathrectanglecorners
            {\pgfpoint{-\pgf@circ@res@temp}{-\pgf@circ@res@temp}}
            {\pgfpoint{\pgf@circ@res@temp}{\pgf@circ@res@temp}}
            \pgfsetcolor{\ctikzvalof{color}}
            \ifx\tikz@fillcolor\pgfutil@empty
                % set the default fill color to white
                \pgfsetfillcolor{white}
                % ...but override it if the class is defined!
                % note that this element has no class, but will inherit it when used
                % into another component
                \pgf@circ@setifdefinedfill{draw, fill}{draw, fill}
            \else
                \pgfsetfillcolor{\tikz@fillcolor}
            \fi
            \pgfsetfillopacity{1.0}
            \pgfusepath{draw,fill}
        \endpgfscope
    }
}
% BNC connector

\pgfdeclareshape{bnc}{
    \anchor{center}{
        \pgfpointorigin
    }
    % BNC size is 2.5 times the size of the internal "ocirc"
    \savedanchor\northwest{%
        \pgf@y=\ctikzvalof{nodes width}\pgf@circ@Rlen
        \pgf@y=2.5\pgf@y
        \pgf@x=-\pgf@y
    }
    % center is on the opening
    \anchor{center}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{zero}{ \pgfpointorigin }
    \anchor{hot}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{shield}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    % geo-anchors
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{right}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{left}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    % put the node text above and centered
    \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
    \anchorborder{
        \pgf@circ@res@left=\pgf@x
        \pgf@circ@res@up=\pgf@y
        \pgfpointborderellipse{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}
        }{\pgfpoint{2.5*\ctikzvalof{nodes width}*\pgf@circ@Rlen}{2.5*\ctikzvalof{nodes width}*\pgf@circ@Rlen}}
    }
    \behindforegroundpath{
        \pgfextracty{\pgf@circ@res@other}{\northwest}
        \pgf@circ@res@step=\ctikzvalof{nodes width}\pgf@circ@Rlen
        \pgfscope
            \pgfstartlinewidth=\pgflinewidth
            \pgf@circ@setlinewidth{bipoles}{\pgflinewidth}
            \pgfsetcolor{\ctikzvalof{color}}
            % external circle
            \pgfscope
                % clipping path: first a rectangle bigger then the shape
                % to avoid problems with the line thickness
                \pgfpathrectanglecorners{\pgfpoint{-2\pgf@circ@res@other}{-2\pgf@circ@res@other}}
                    {\pgfpoint{2\pgf@circ@res@other}{2\pgf@circ@res@other}}
                % next the opening to the right
                \pgfpathrectanglecorners{\pgfpoint{-\pgf@circ@res@step}{-\pgf@circ@res@step}}
                    {\pgfpoint{2\pgf@circ@res@other}{\pgf@circ@res@step}}
                % do the difference and clip before drawing
                \pgfseteorule
                \pgfusepath{clip}
                \pgfpathcircle{\pgfpointorigin}{\pgf@circ@res@other}
                \pgfusepath{draw}
            \endpgfscope
            % internal circle
            \pgfpathcircle{\pgfpointorigin}{\pgf@circ@res@step}
            \pgf@circ@draworfill
            % and the contact line to the right
            \pgfsetlinewidth{\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}
            \pgfusepath{draw}
        \endpgfscope
    }
}

%% Fill for correct rectangular joins

\pgfdeclareshape{rectjoinfill}{
    \savedanchor{\northeast}{%
        \pgf@x=.5\pgflinewidth%
        \pgf@y=.5\pgflinewidth%
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \anchor{center}{
        \pgfpointorigin
    }
    \anchorborder{
        \pgf@circ@res@left=\pgf@x
        \pgf@circ@res@up=\pgf@y
    }
    \behindforegroundpath{
        \pgfscope
            \pgfpathrectanglecorners
            {\pgfpoint{0}{.5\pgflinewidth}}
            {\pgfpoint{0}{-.5\pgflinewidth}}
            \pgfsetcolor{\ctikzvalof{color}}
            \pgfusepath{draw,fill}
        \endpgfscope
    }
}

%% transistor arrow

\def\pgf@circ@find@linescale{
    % find the scale inverse of the scale factor: line width do not scale
    % with scale=..., transform shape so we have to counteract it.
    \iftikz@fullytransformed % this is true if `transform shape` is active
        % from @Circumscribe https://tex.stackexchange.com/a/474035/38080
        % Note that this trick is not working inside a `spy` environment...
        \pgfgettransformentries{\scaleA}{\scaleB}{\scaleC}{\scaleD}{\whatevs}{\whatevs}%
        \pgfmathsetmacro{\@@factor}{1.0/sqrt(abs(\scaleA*\scaleD-\scaleB*\scaleC))}%
    \else
        \pgfmathsetmacro{\@@factor}{1.0}
    \fi
}

\pgfdeclareshape{trarrow}{%
    % this arrow is only filled but grows with the linewidth, more or less
    % like currarrow do
    \savedanchor{\northeast}{%
        \pgf@circ@res@step = \pgf@circ@Rlen
        \pgf@circ@find@linescale
        \divide \pgf@circ@res@step by \ctikzvalof{current arrow scale}
        \pgfpoint{0.7*\pgf@circ@res@step +0.5*\@@factor*\pgflinewidth}
            {0.8*\pgf@circ@res@step+0.7593*\@@factor*\pgflinewidth}
    }
    % The arrow size should be more or less the same of a currarrow, which is
    % both filled and stroke, for backward output compatibility (more or less)
    %
    %      angle \beta       W is \pgf@circ@Rlen/\ctikzvalof{current arrow scale}
    %    |-\__               currarrow as the tip at (W,0)
    %    |    |              and the upper tail at (-0.7*W, 0.8*W)
    %    |    \__            it then "overshoot" do to the linew width L
    %    |       \__ xangle \alpha
    %    ---0------->
    %
    %   \beta = atan(0.7/0.8)  \alpha=atan(0.8/1.7)
    %   tip overshoot is (L/2)/sin(\alpha) = 1.743*L only in x direction
    %   tail overshoot is -(L/2) in x, and (L/2)/sin(\beta) = 0.7539*L in y
    %
    \savedanchor{\northwest}{%
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by \ctikzvalof{current arrow scale}
        \pgf@circ@find@linescale
        \pgfpoint{-0.7*\pgf@circ@res@step -0.5*\@@factor*\pgflinewidth}
            {0.8*\pgf@circ@res@step+0.7593*\@@factor*\pgflinewidth}
    }
    \savedanchor{\tip}{%
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by \ctikzvalof{current arrow scale}
        \pgf@circ@find@linescale
        \pgfpoint{\pgf@circ@res@step + 1.743*\@@factor*\pgflinewidth}{0pt}
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{tip}{
        \tip
    }
    \anchor{btip}{% this anchor is behind the tip of half a linewidth
        \tip
        \pgf@circ@find@linescale
        \pgf@circ@res@temp=\@@factor\pgflinewidth
        \advance\pgf@x by -.5\pgf@circ@res@temp
    }
    \behindforegroundpath{
        \pgfscope
            \northwest
            \pgf@circ@res@up=\pgf@y
            \pgf@circ@res@left=\pgf@x
            \tip
            \pgf@circ@res@step = \pgf@x
            %
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{1\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@up}}
            \pgfpathclose
            \pgfsetcolor{\ctikzvalof{color}}
            \pgfusepath{fill} % just fill
        \endpgfscope
    }
}

%% Current arrow

\pgfdeclareshape{currarrow}{
    \savedanchor{\northeast}{%
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by \ctikzvalof{current arrow scale}
        \pgf@x=.5\pgf@circ@res@step
        \pgf@y=\pgf@x%
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{tip}{
        \pgfpointorigin
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by \ctikzvalof{current arrow scale}
        \pgf@x	=\pgf@circ@res@step
    }
    \behindforegroundpath{
        \pgfscope
            \pgf@circ@res@step = \pgf@circ@Rlen
            \divide \pgf@circ@res@step by \ctikzvalof{current arrow scale}

            \pgfpathmoveto{\pgfpoint{-.7\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{-.7\pgf@circ@res@step}{-.8\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{1\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{-.7\pgf@circ@res@step}{.8\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{-.7\pgf@circ@res@step}{0pt}}
            \pgfsetcolor{\ctikzvalof{color}}
            \pgfusepath{draw,fill}

        \endpgfscope
    }
}

%% Flow arrow

\pgfdeclareshape{flowarrow}{
    \savedanchor{\northeast}{%
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by \ctikzvalof{current arrow scale}
        \pgf@y=.5\pgf@circ@res@step
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by 4
        \pgf@x=\pgf@circ@res@step%
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \anchor{text}{% text centered above
        \pgfpointorigin
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox}
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{tip}{
        \pgfpointorigin
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by \ctikzvalof{current arrow scale}
        \pgf@x	=\pgf@circ@res@step
    }
    \behindforegroundpath{
        \pgfscope
            \pgf@circ@res@step = \pgf@circ@Rlen
            \divide \pgf@circ@res@step by 4
            \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfsetcolor{\ctikzvalof{color}}
            \pgfusepath{draw}
            \pgftransformshift{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfnode{currarrow}{tip}{}{}{\pgfusepath{fill}}
        \endpgfscope
    }
}

%% Input arrow

\pgfdeclareshape{inputarrow}{
    \savedanchor{\northeast}{% this is really not northeast, really -northwest
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by \ctikzvalof{current arrow scale}
        \pgf@y=.5\pgf@circ@res@step
        \pgf@x=1.7\pgf@circ@res@step
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax\pgf@x=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast\pgf@x=0cm\relax}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y\pgf@x=0cm\relax}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \savedanchor{\tip}{
        \pgfpointorigin
    }
    \anchor{center}{
        \tip
    }
    \anchor{tip}{
        \tip
    }
    \behindforegroundpath{

        \pgfscope
            \pgf@circ@res@step = \pgf@circ@Rlen
            \divide \pgf@circ@res@step by 16

            \pgfpathmoveto{\pgfpoint{-1.7\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{-1.7\pgf@circ@res@step}{-.8\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{0pt}{0pt}}
            \pgfpathlineto{\pgfpoint{-1.7\pgf@circ@res@step}{.8\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{-1.7\pgf@circ@res@step}{0pt}}
            \pgfsetcolor{\ctikzvalof{color}}
            \pgfusepath{fill}

        \endpgfscope
    }
}


%% box

\pgfdeclareshape{box}{
    \anchor{center}{
        \pgfpointorigin
    }
    \behindforegroundpath{

        \pgfscope
            \pgf@circ@res@step = \ctikzvalof{bipoles/twoport/width}\pgf@circ@Rlen
            \pgf@circ@res@step = 0.5\pgf@circ@res@step
            \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \pgfpathrectanglecorners{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@step}}{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@step}}
            \pgf@circ@draworfill
        \endpgfscope
    }
}

%% box scaled with blocks

\pgfdeclareshape{blockbox}{
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{blocks/scale}\pgf@circ@Rlen}}
    \anchor{center}{
        \pgfpointorigin
    }
    \behindforegroundpath{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{blocks/scale}\pgf@circ@Rlen}
        \pgfscope
            \pgf@circ@res@step = \ctikzvalof{bipoles/twoport/width}\pgf@circ@scaled@Rlen
            \pgf@circ@res@step = 0.5\pgf@circ@res@step
            \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \pgfpathrectanglecorners{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@step}}{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@step}}
            \pgf@circ@draworfill
        \endpgfscope
    }
}

% full nodes for wire crossing

\pgfdeclareshape{jump crossing}
{
    \savedanchor\northwest{%
        \pgf@y=\ctikzvalof{bipoles/crossing/size}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \behindbackgroundpath{
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        % horizontal jumper
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{0pt}}
        \pgfpatharc{0}{-180}{0.4*\pgf@circ@res@left}
        \pgfsetbeveljoin
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        % vertical, broken path
        \pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{0.5\pgf@circ@res@up}}
        \pgfpathmoveto{\pgfpoint{0pt}{0.3\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfusepath{draw}

    }
}
\pgfdeclareshape{plain crossing}
{
    \savedanchor\northwest{%
        \pgf@y=\ctikzvalof{bipoles/crossing/size}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \behindbackgroundpath{
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        % horizontal jumper
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        % vertical, broken path
        \pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{0.1\pgf@circ@res@up}}
        \pgfpathmoveto{\pgfpoint{0pt}{0.1\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfusepath{draw}

    }
}

\endinput


==> pgfcirctripoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tripoles

%%%%%%%%%%%%%
%% switches
%%%%%%%%%%%%%

% Legacy spdt
\pgfdeclareshape{spdt}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{switches}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/spdt/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/spdt/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{left}{%
        \northwest
        \pgf@y=0pt
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{out 1}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{out 2}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \anchor{center}{
        \pgf@y=0pt
        \pgf@x=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@res@other = \ctikzvalof{tripoles/spdt/margin}\pgf@circ@res@left


        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}

        \pgfusepath{draw}

        \pgfscope
            \pgftransformshift{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
            \pgfnode{ocirc}{center}{}{spdt1}{\pgfusepath{stroke}}
        \endpgfscope
        \pgfscope
            \pgftransformshift{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}
            \pgfnode{ocirc}{center}{}{}{\pgfusepath{stroke}}
        \endpgfscope
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@other}{0pt}}
            \pgfnode{ocirc}{center}{}{spdt2}{\pgfusepath{stroke}}
        \endpgfscope

        \pgfscope
            \pgfpathmoveto{\pgfpointshapeborder{spdt2}{\pgfpointorigin}}
            \pgfpathlineto{
                \pgfpointadd{\pgfpointshapeborder{spdt1}{\pgfpoint{-\pgf@circ@res@other}{-100pt}}}
                {\pgfpoint{-.05\pgf@circ@res@up}{-.05\pgf@circ@res@up}}
            }
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgfusepath{draw}
        \endpgfscope
    }
}


% cute switch "node" shapes, matching with cute "to" shapes
% #1 -> name
% #2 -> barposition
% #3 -> arrowcode
\long\def\pgfcircdeclarecutespdt#1#2#3{
    \pgfdeclareshape{#1}
    {
        \savedmacro{\ctikzclass}{\edef\ctikzclass{switches}}
        \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
        \savedanchor\northwest{%
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@y=\ctikzvalof{bipoles/cuteswitch/height}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\ctikzvalof{tripoles/spdt/width}\pgf@circ@scaled@Rlen
            \pgf@x=.25\pgf@x
        }
        \savedanchor\midlever{
            % these values are calculated when we create the definition of the shape.
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@y=\ctikzvalof{bipoles/cuteswitch/height}\pgf@circ@scaled@Rlen
            \pgf@circ@res@temp=\ctikzvalof{nodes width}\pgf@circ@scaled@Rlen
            \pgf@circ@res@temp=\ctikzvalof{bipoles/cuteswitch/thickness}\pgf@circ@res@temp
            \pgf@circ@res@down = -.5\pgf@y
            \pgf@circ@res@up = .5\pgf@y
            \pgfextracty{\pgf@circ@res@other}{#2}
            \pgf@x=0pt
            \pgf@y=.5\pgf@circ@res@other
        }
        % radius of the connector
        % This is the radius of the "ocirc" shape (see pgfcircshapes.tex)
        \saveddimen{\radius}{\pgfmathsetlength\pgf@x{\pgf@circ@Rlen*\ctikzvalof{nodes width}}}
        % shapename
        \savedmacro{\thisshape}{\def\thisshape{\tikz@fig@name}}
        % shape type
        \savedmacro{\cshape}{\def\cshape{\ctikzvalof{bipoles/cuteswitch/shape}}}
        % mid of the lever, to stack switches
        \anchor{mid}{\midlever}
        % center anchors
        \anchor{cin}{ \northwest \pgf@y=0pt}
        \anchor{cout 1}{ \northwest \pgf@x=-\pgf@x }
        \anchor{cout 2}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
        % horizontal angles
        \anchor{in}{ \northwest \pgf@y=0pt\advance\pgf@x by -\radius}
        \anchor{out 1}{ \northwest \pgf@x=-\pgf@x \advance\pgf@x by \radius}
        \anchor{out 2}{ \northwest \pgf@x=-\pgf@x \advance\pgf@x by \radius \pgf@y=-\pgf@y }

        \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
        \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
        \anchor{west}{ \northwest \pgf@y=0pt }
        \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
        \anchor{north}{ \northwest \pgf@x=0pt }
        \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
        \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
        \anchor{north west}{ \northwest }
        \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }

        \backgroundpath{
            \pgfsetcolor{\ctikzvalof{color}}
            \northwest
            \pgf@circ@res@up = \pgf@y
            \pgf@circ@res@down = -\pgf@y
            \pgf@circ@res@right = -\pgf@x
            \pgf@circ@res@left = \pgf@x

            \pgfscope
            % This is the radius of the "ocirc" shape (see pgfcircshapes.tex)
            \pgf@circ@res@temp=\radius\relax
            \pgf@circ@res@temp=\ctikzvalof{bipoles/cuteswitch/thickness}\pgf@circ@res@temp
            \pgfsetlinewidth{2\pgf@circ@res@temp}
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfpathlineto{#2}
            \pgfsetroundcap\pgfusepath{draw}
            \endpgfscope
            \pgfscope % arrow
            #3
            \endpgfscope
            % terminals
            \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
            \pgfnode{\cshape}{center}{}{\thisshape-out 1}{\pgfusepath{stroke}}
            \endpgfscope
            \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgfnode{\cshape}{center}{}{\thisshape-out 2}{\pgfusepath{stroke}}
            \endpgfscope
            \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{\cshape}{center}{}{\thisshape-in}{\pgfusepath{stroke}}
            \endpgfscope

        }
    }
}

\pgfcircdeclarecutespdt{cute spdt up}
{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up-1.5\pgf@circ@res@temp}}
{}

\pgfcircdeclarecutespdt{cute spdt mid}
{\pgfpoint{\pgf@circ@res@right}{0pt}}
{}

\pgfcircdeclarecutespdt{cute spdt down}
{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down+1.5\pgf@circ@res@temp}}
{}

\pgfcircdeclarecutespdt{cute spdt up arrow}
{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up-1.5\pgf@circ@res@temp}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgflinewidth}
    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}} % in node
    \pgfpathmoveto{\pgfpointpolar{70}{1.5\pgf@circ@res@right}}
    \pgfpatharc{70}{-50}{1.5\pgf@circ@res@right}
    \pgfsetarrowsend{latexslim}
    \pgfusepath{draw}
}

\pgfcircdeclarecutespdt{cute spdt mid arrow}
{\pgfpoint{\pgf@circ@res@right}{0pt}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgflinewidth}
    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}} % in node
    \pgfsetarrowsstart{latexslim}
    \pgfpathmoveto{\pgfpointpolar{-60}{1.5\pgf@circ@res@right}}
    \pgfpatharc{-60}{60}{1.5\pgf@circ@res@right}
    \pgfsetarrowsend{latexslim}
    \pgfusepath{draw}
}

\pgfcircdeclarecutespdt{cute spdt down arrow}
{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down+1.5\pgf@circ@res@temp}}
{
    \pgf@circ@setlinewidth{bipoles}{\pgflinewidth}
    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}} % in node
    \pgfpathmoveto{\pgfpointpolar{-50}{1.5\pgf@circ@res@right}}
    \pgfpatharc{-50}{70}{1.5\pgf@circ@res@right}
    \pgfsetarrowsend{latexslim}
    \pgfusepath{draw}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%       Logic ports
%%
%% Code from John Kormylo at tex.stackexchange.com
%% See https://tex.stackexchange.com/questions/372993/is-it-possible-to-implement-multiple-input-logic-ports-with-circuitikz
%% Integration and fixes from Romano Giannetti and TheTeXnician <38565529+TheTeXnician@users.noreply.github.com>
%%

\newcount\pgf@circ@res@count% reserve global register

\def\pgf@circ@logicport@input#1% #1 = \pgfmathcounter
{%
    \pgfextracty{\pgf@circ@res@up}{\northeast}%
    \step
    \pgf@circ@res@step=\dimexpr 2\pgf@y -2\pgf@circ@res@up\relax
    \advance\pgf@y by -#1\pgf@circ@res@step\relax
}%

% #1 = \pgfmathcounter #2=type #3 specificic port
% type is 1 for and,nand; 2 for or,nor; 3 for xor,xnor, 4 for european.
\def\pgf@circ@logicport@baseinput#1#2#3%
{%
    % and and nand
    \ifnum #2=1\relax
        \pgfextracty{\pgf@circ@res@up}{\northeast}%
        \pgfextractx{\pgf@circ@res@left}{\southwest}%
        \step
        \pgf@circ@res@step=\dimexpr 2\pgf@y -2\pgf@circ@res@up\relax
        \advance\pgf@y by -#1\pgf@circ@res@step\relax
        \pgf@x=\ctikzvalof{tripoles/american #3 port/port width}\pgf@circ@res@left
    \fi
    % or and nor
    \ifnum #2=2\relax
        \pgfextracty{\pgf@circ@res@up}{\northeast}%
        \pgfextractx{\pgf@circ@res@left}{\southwest}%
        \pgfextractx{\pgf@circ@res@right}{\northeast}%
        \step
        \pgf@circ@res@step=\dimexpr 2\pgf@y -2\pgf@circ@res@up\relax
        \advance\pgf@y by -#1\pgf@circ@res@step\relax
        \edef\pgf@circ@math@angle{\ctikzvalof{tripoles/american #3 port/angle}}%
        \pgf@circ@res@other=\ctikzvalof{tripoles/american #3 port/inner}\pgf@circ@res@right
        \pgfmathsetlengthmacro{\pgf@circ@math@xradius}{\pgf@circ@res@other /(1 - cos(\pgf@circ@math@angle)}%
        \pgfmathsetlengthmacro{\pgf@circ@math@yradius}{\pgf@circ@res@up /sin(\pgf@circ@math@angle)}%
        \pgf@circ@res@other=\ctikzvalof{tripoles/american #3 port/port width}\pgf@circ@res@right
        \pgfmathsetlengthmacro{\pgf@circ@math@xorigin}{\pgf@circ@res@other + \pgf@circ@math@xradius*cos(\pgf@circ@math@angle)}%
        \pgf@circ@res@temp=\pgf@y
        \pgfmathsetmacro{\pgf@circ@math@angle}{asin(\pgf@circ@res@temp/\pgf@circ@math@yradius)}%
        \pgfmathsetlength{\pgf@circ@res@other}{\pgf@circ@math@xradius*cos(\pgf@circ@math@angle)-\pgf@circ@math@xorigin}%
        \pgf@x=\pgf@circ@res@other
    \fi
    % xor and xnor
    \ifnum #2=3\relax
        \pgfextracty{\pgf@circ@res@up}{\northeast}%
        \pgfextractx{\pgf@circ@res@left}{\southwest}%
        \pgfextractx{\pgf@circ@res@right}{\northeast}%
        \pgfkeysgetvalue{/tikz/circuitikz/tripoles/american #3 port/angle}{\pgf@circ@math@angle}%
        \pgf@circ@res@other=\ctikzvalof{tripoles/american #3 port/inner}\pgf@circ@res@right
        \pgfmathsetlengthmacro{\pgf@circ@math@xradius}{\pgf@circ@res@other /(1 - cos(\pgf@circ@math@angle)}%
        \pgfmathsetlengthmacro{\pgf@circ@math@yradius}{\pgf@circ@res@up / sin(\pgf@circ@math@angle))}%
        \pgf@circ@res@other=\ctikzvalof{tripoles/american #3 port/port width}\pgf@circ@res@right
        \pgfmathsetlengthmacro{\pgf@circ@math@xorigin}{\pgf@circ@res@other + \pgf@circ@math@xradius*cos(\pgf@circ@math@angle)}%
        \pgf@circ@res@temp=\ctikzvalof{tripoles/american #3 port/distance}\pgf@circ@res@right
        \pgfmathsetlengthmacro{\pgf@circ@math@distance}{\pgf@circ@res@temp}
        % this compensates for the effect of the line width on the gap between the arcs
        \pgfmathsetlengthmacro{\pgf@circ@math@yradiusA}{\pgf@circ@math@yradius -2\pgflinewidth}%
        \pgfmathsetlengthmacro{\pgf@circ@math@xradiusA}{\pgf@circ@math@xradius -2\pgflinewidth}%

        \step
        \pgf@circ@res@step=\dimexpr 2\pgf@y -2\pgf@circ@res@up\relax
        \advance\pgf@y by -#1\pgf@circ@res@step\relax
         \pgf@circ@res@temp=\pgf@y
            \pgfmathsetmacro{\pgf@circ@math@angle}{asin(\pgf@circ@res@temp  / \pgf@circ@math@yradiusA)}%
        \pgfmathsetlength{\pgf@circ@res@other}{\pgf@circ@math@xradiusA*cos(\pgf@circ@math@angle)-\pgf@circ@math@xorigin}%
        \advance\pgf@circ@res@other by -\pgf@circ@math@distance
        \pgf@x=\pgf@circ@res@other
    \fi
    % european
    \ifnum #2=4\relax
        \pgfextracty{\pgf@circ@res@up}{\northeast}%
        \pgfextractx{\pgf@circ@res@other}{\left}%
        \step
        \pgf@circ@res@step=\dimexpr 2\pgf@y -2\pgf@circ@res@up\relax
        \advance\pgf@y by -#1\pgf@circ@res@step\relax
        \pgf@x=\pgf@circ@res@other
    \fi
}%

%%% american
\long\def\pgfcircdeclarelogicport#1#2#3{%
    \pgfdeclareshape{american #1 port}%
    {%
        \savedmacro{\ctikzclass}{\edef\ctikzclass{logic ports}}
        \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
        \savedmacro\resize{% automatic
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@circ@res@up = \ctikzvalof{tripoles/american #1 port/height}\pgf@circ@scaled@Rlen
            \pgf@circ@res@up = .5\pgf@circ@res@up
            \pgf@circ@res@down = -\pgf@circ@res@up
            \pgf@circ@res@right = \ctikzvalof{tripoles/american #1 port/width}\pgf@circ@scaled@Rlen
            \pgf@circ@res@right = .5\pgf@circ@res@right
            \pgf@circ@res@left = -\pgf@circ@res@right
    }%
    \savedmacro\inputs{% get number of inputs
        \pgf@circ@res@count=\pgfkeysvalueof{/tikz/number inputs}\relax%
        \ifnum\pgf@circ@res@count=0
            \pgf@circ@res@count=\ctikzvalof{tripoles/american #1 port/inputs}\relax%
        \fi
        \ifnum\pgf@circ@res@count<2 \pgf@circ@res@count=2\fi
        \ifnum\pgf@circ@res@count>16 \pgf@circ@res@count=16\fi
        \def\inputs{\the\pgf@circ@res@count}%
    }%
    \savedanchor\step{% 1/2 gap at edges
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step = \ctikzvalof{tripoles/american #1 port/height}\pgf@circ@scaled@Rlen
        \divide\pgf@circ@res@step by \pgf@circ@res@count
        \pgfpoint{\pgf@circ@res@left}{\dimexpr\pgf@circ@res@up+0.5\pgf@circ@res@step}%
    }%
    \savedanchor\northeast{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \savedanchor\southwest{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \savedanchor\left{\pgfpoint{\ctikzvalof{tripoles/american #1 port/port width}\pgf@circ@res@left}{0pt}}
    \savedanchor\right{\pgfpoint{\ctikzvalof{tripoles/american #1 port/port width}\pgf@circ@res@right}{0pt}}
    \savedanchor\origin{\pgfpoint{\ctikzvalof{tripoles/american #1 port/origin}\pgf@circ@res@right}{0pt}}

    \anchor{center}{\origin}% for backwards compatibility
    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    % create input anchors
    \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@american #1 port\endcsname{%
        \pgfmathloop%
        \ifnum\pgfmathcounter>\pgf@circ@res@count%
    \else%
        %\pgfutil@ifundefined{pgf@anchor@american #1 port@in \pgfmathcounter}{%
        \expandafter\xdef\csname pgf@anchor@american #1 port@in \pgfmathcounter\endcsname{%
            \noexpand\pgf@circ@logicport@input{\pgfmathcounter}% defined above
        }%
        \expandafter\xdef\csname pgf@anchor@american #1 port@bin \pgfmathcounter\endcsname{%
            \noexpand\pgf@circ@logicport@baseinput{\pgfmathcounter}{#2}{#1}% defined above
        }%
        %}{}%
        \repeatpgfmathloop%
    }

    \anchor{out}{\northeast\pgf@y=0pt}
    \anchor{bout}{\right\pgf@y=0pt}


    \anchor{left}{\left}% edges of component mius leads
    \anchor{right}{\right}

    \anchor{north east}{\northeast}% see \Compass macro
    \anchor{south west}{\southwest}
    \anchor{north}{\pgfextracty{\pgf@circ@res@up}{\northeast}%
    \pgfpoint{0cm}{\pgf@circ@res@up}}
    \anchor{north west}{\pgfextracty{\pgf@circ@res@up}{\northeast}%
        \pgfextractx{\pgf@circ@res@left}{\southwest}%
    \pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \anchor{west}{\pgfextractx{\pgf@circ@res@left}{\southwest}%
    \pgfpoint{\pgf@circ@res@left}{0cm}}
    \anchor{south}{\pgfextracty{\pgf@circ@res@down}{\southwest}%
    \pgfpoint{0cm}{\pgf@circ@res@down}}
    \anchor{south east}{\pgfextracty{\pgf@circ@res@down}{\southwest}%
        \pgfextractx{\pgf@circ@res@right}{\northeast}%
    \pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \anchor{east}{\pgfextractx{\pgf@circ@res@right}{\northeast}%
    \pgfpoint{\pgf@circ@res@right}{0cm}}

    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        #3
    }
}
}
%%% american and %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfcircdeclarelogicport{and}{1}{
    \pgfextracty{\pgf@circ@res@temp}{\step}%
    \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
    \pgf@circ@res@count = \inputs\relax
    \loop\ifnum\pgf@circ@res@count>0
        \advance\pgf@circ@res@temp by -\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/american and port/port width}\pgf@circ@res@left}
        {\pgf@circ@res@temp}}
        \advance\pgf@circ@res@count by -1
        \repeat

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint
        {\ctikzvalof{tripoles/american and port/port width}\pgf@circ@res@right}
    {0pt}}

    \pgfusepath{draw}

    \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
    \pgf@circ@res@other=\ctikzvalof{tripoles/american and port/port width}\pgf@circ@res@left

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
    \pgfpatharc{-90}{90}{-2\pgf@circ@res@other and \pgf@circ@res@up}
    \pgfpathclose
    \pgf@circ@draworfill
    }
%%% american nand %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgfcircdeclarelogicport{nand}{1}{
    \pgfextracty{\pgf@circ@res@temp}{\step}%
    \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
    \pgf@circ@res@count = \inputs\relax
    \loop\ifnum\pgf@circ@res@count>0
        \advance\pgf@circ@res@temp by -\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/american nand port/port width}\pgf@circ@res@left}
        {\pgf@circ@res@temp}}
        \advance\pgf@circ@res@count by -1
    \repeat

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint
        {\ctikzvalof{tripoles/american nand port/port width}\pgf@circ@res@right} {0pt}}

    \pgfusepath{draw}

    \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
    \pgf@circ@res@step = \ctikzvalof{tripoles/american nand port/circle width}\pgf@circ@res@right
    \pgf@circ@res@other = \ctikzvalof{tripoles/american nand port/port width}\pgf@circ@res@right
    \pgf@circ@res@temp = \dimexpr 2\pgf@circ@res@other - \pgf@circ@res@step\relax

    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}
    \pgfpatharc{-90}{90}{\pgf@circ@res@temp and \pgf@circ@res@up}
    \pgfpathclose

    \pgfpathellipse
    {\pgfpoint{\pgf@circ@res@other-.5\pgf@circ@res@step}{0pt}}
    {\pgfpoint{.5\pgf@circ@res@step}{0pt}}
    {\pgfpoint{0pt}{.5\pgf@circ@res@step}}

    \pgf@circ@draworfill
}
%%% american nor %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfcircdeclarelogicport{nor}{2}{
    \edef\pgf@circ@math@angle{\ctikzvalof{tripoles/american nor port/angle}}%
    \pgf@circ@res@other=\ctikzvalof{tripoles/american nor port/inner}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xradius}{\pgf@circ@res@other /(1 - cos(\pgf@circ@math@angle)}%
    \pgfmathsetlengthmacro{\pgf@circ@math@yradius}{\pgf@circ@res@up /sin(\pgf@circ@math@angle)}%
    \pgf@circ@res@other=\ctikzvalof{tripoles/american nor port/port width}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xorigin}{\pgf@circ@res@other + \pgf@circ@math@xradius*cos(\pgf@circ@math@angle)}%

    \pgfextracty{\pgf@circ@res@temp}{\step}%
    \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
    \pgf@circ@res@count = \inputs\relax
    \loop\ifnum\pgf@circ@res@count>0
        \advance\pgf@circ@res@temp by -\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
        \pgfmathsetmacro{\pgf@circ@math@angle}{asin(\pgf@circ@res@temp/\pgf@circ@math@yradius)}%
        \pgfmathsetlength{\pgf@circ@res@other}{\pgf@circ@math@xradius*cos(\pgf@circ@math@angle)-\pgf@circ@math@xorigin}%
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@temp}}%
        \advance\pgf@circ@res@count by -1
    \repeat

    \pgf@circ@res@other=\ctikzvalof{tripoles/american nor port/port width}\pgf@circ@res@right
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}

    \pgfusepath{draw}

    \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}

    \edef\pgf@circ@math@angle{\ctikzvalof{tripoles/american nor port/angle}}%
    \pgf@circ@res@step = \ctikzvalof{tripoles/american nor port/circle width}\pgf@circ@res@right
    \pgf@circ@res@temp = \dimexpr 2\pgf@circ@res@other - \pgf@circ@res@step\relax
    \advance\pgf@circ@res@other by -\pgf@circ@res@step

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}% for symmetry
    \pgfpatharc{0}{90}{\pgf@circ@res@temp and \pgf@circ@res@up}%
    \pgfpatharc{\pgf@circ@math@angle}{-\pgf@circ@math@angle}{\pgf@circ@math@xradius and \pgf@circ@math@yradius}%
    \pgfpatharc{-90}{0}{\pgf@circ@res@temp and \pgf@circ@res@up}%
    \pgfpathclose

    \pgfpathellipse
    {\pgfpoint{\pgf@circ@res@other+.5\pgf@circ@res@step}{0pt}}
    {\pgfpoint{.5\pgf@circ@res@step}{0pt}}
    {\pgfpoint{0pt}{.5\pgf@circ@res@step}}

    \pgf@circ@draworfill
}
%%% american or %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfcircdeclarelogicport{or}{2}{
    \edef\pgf@circ@math@angle{\ctikzvalof{tripoles/american or port/angle}}%
    \pgf@circ@res@other=\ctikzvalof{tripoles/american or port/inner}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xradius}{\pgf@circ@res@other /(1 - cos(\pgf@circ@math@angle)}%
    \pgfmathsetlengthmacro{\pgf@circ@math@yradius}{\pgf@circ@res@up /sin(\pgf@circ@math@angle)}%
    \pgf@circ@res@other=\ctikzvalof{tripoles/american or port/port width}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xorigin}{\pgf@circ@res@other + \pgf@circ@math@xradius*cos(\pgf@circ@math@angle)}%

    \pgfextracty{\pgf@circ@res@temp}{\step}%
    \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
    \pgf@circ@res@count = \inputs\relax
    \loop\ifnum\pgf@circ@res@count>0
        \advance\pgf@circ@res@temp by -\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
        \pgfmathsetmacro{\pgf@circ@math@angle}{asin(\pgf@circ@res@temp/\pgf@circ@math@yradius)}%
        \pgfmathsetlength{\pgf@circ@res@other}{\pgf@circ@math@xradius*cos(\pgf@circ@math@angle)-\pgf@circ@math@xorigin}%
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@temp}}%
        \advance\pgf@circ@res@count by -1
    \repeat

    \pgf@circ@res@other=\ctikzvalof{tripoles/american or port/port width}\pgf@circ@res@right
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}

    \pgfusepath{draw}

    \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}

    \edef\pgf@circ@math@angle{\ctikzvalof{tripoles/american or port/angle}}%

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}% for symmetry
    \pgfpatharc{0}{90}{2\pgf@circ@res@other and \pgf@circ@res@up}%
    \pgfpatharc{\pgf@circ@math@angle}{-\pgf@circ@math@angle}{\pgf@circ@math@xradius and \pgf@circ@math@yradius}%
    \pgfpatharc{-90}{0}{2\pgf@circ@res@other and \pgf@circ@res@up}%
    \pgfpathclose

    \pgf@circ@draworfill
}
%%% american xor %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfcircdeclarelogicport{xor}{3}{
    \pgfkeysgetvalue{/tikz/circuitikz/tripoles/american xor port/angle}{\pgf@circ@math@angle}%
    \pgf@circ@res@other=\ctikzvalof{tripoles/american xor port/inner}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xradius}{\pgf@circ@res@other /(1 - cos(\pgf@circ@math@angle)}%
    \pgfmathsetlengthmacro{\pgf@circ@math@yradius}{\pgf@circ@res@up / sin(\pgf@circ@math@angle))}%
    \pgf@circ@res@other=\ctikzvalof{tripoles/american xor port/port width}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xorigin}{\pgf@circ@res@other + \pgf@circ@math@xradius*cos(\pgf@circ@math@angle)}%
    \pgf@circ@res@temp=\ctikzvalof{tripoles/american xor port/distance}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@distance}{\pgf@circ@res@temp}
    % this compensates for the effect of the line width on the gap between the arcs
    \pgfmathsetlengthmacro{\pgf@circ@math@yradiusA}{\pgf@circ@math@yradius -2\pgflinewidth}%
    \pgfmathsetlengthmacro{\pgf@circ@math@xradiusA}{\pgf@circ@math@xradius -2\pgflinewidth}%

    \pgfextracty{\pgf@circ@res@temp}{\step}%
    \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
    \pgf@circ@res@count = \inputs\relax
    \loop\ifnum\pgf@circ@res@count>0
        \advance\pgf@circ@res@temp by -\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
        \pgfmathsetmacro{\pgf@circ@math@angle}{asin(\pgf@circ@res@temp  / \pgf@circ@math@yradiusA)}%
        \pgfmathsetlength{\pgf@circ@res@other}{\pgf@circ@math@xradiusA*cos(\pgf@circ@math@angle)-\pgf@circ@math@xorigin}%
        \advance\pgf@circ@res@other by -\pgf@circ@math@distance
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@temp}}%
        \advance\pgf@circ@res@count by -1
    \repeat

    \pgf@circ@res@other=\ctikzvalof{tripoles/american xor port/port width}\pgf@circ@res@right
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}

    \pgfusepath{draw}

    \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}

    \edef\pgf@circ@math@angle{\ctikzvalof{tripoles/american xor port/angle}}%

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}% for symmetry
    \pgfpatharc{0}{90}{2\pgf@circ@res@other and \pgf@circ@res@up}%
    \pgfpatharc{\pgf@circ@math@angle}{-\pgf@circ@math@angle}{\pgf@circ@math@xradius and \pgf@circ@math@yradius}%
    \pgfpatharc{-90}{0}{2\pgf@circ@res@other and \pgf@circ@res@up}%
    \pgfpathclose
    \pgf@circ@draworfill

    \pgfmathsetlength{\pgf@circ@res@temp}{(\pgf@circ@math@yradiusA)*sin(\pgf@circ@math@angle)}%

    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other-\pgf@circ@math@distance}{\pgf@circ@res@temp}}% first arc
    \pgfpatharc{\pgf@circ@math@angle}{-\pgf@circ@math@angle}{\pgf@circ@math@xradiusA and \pgf@circ@math@yradiusA}%

    \pgfusepath{draw}
}
%%% american xnor %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfcircdeclarelogicport{xnor}{3}{
    \pgfkeysgetvalue{/tikz/circuitikz/tripoles/american xnor port/angle}{\pgf@circ@math@angle}%
    \pgf@circ@res@other=\ctikzvalof{tripoles/american xnor port/inner}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xradius}{\pgf@circ@res@other /(1 - cos(\pgf@circ@math@angle)}%
    \pgfmathsetlengthmacro{\pgf@circ@math@yradius}{\pgf@circ@res@up / sin(\pgf@circ@math@angle))}%
    \pgf@circ@res@other=\ctikzvalof{tripoles/american xnor port/port width}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xorigin}{\pgf@circ@res@other + \pgf@circ@math@xradius*cos(\pgf@circ@math@angle)}%
    \pgf@circ@res@temp=\ctikzvalof{tripoles/american xor port/distance}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@distance}{\pgf@circ@res@temp}
    % this compensates for the effect of the line width on the gap between the arcs
    \pgfmathsetlengthmacro{\pgf@circ@math@yradiusA}{\pgf@circ@math@yradius -2\pgflinewidth}%
    \pgfmathsetlengthmacro{\pgf@circ@math@xradiusA}{\pgf@circ@math@xradius -2\pgflinewidth}%

    \pgfextracty{\pgf@circ@res@temp}{\step}%
    \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
    \pgf@circ@res@count = \inputs\relax
    \loop\ifnum\pgf@circ@res@count>0
        \advance\pgf@circ@res@temp by -\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
        \pgfmathsetmacro{\pgf@circ@math@angle}{asin(\pgf@circ@res@temp  / \pgf@circ@math@yradiusA)}%
        \pgfmathsetlength{\pgf@circ@res@other}{\pgf@circ@math@xradiusA*cos(\pgf@circ@math@angle)-\pgf@circ@math@xorigin}%
        \advance\pgf@circ@res@other by -\pgf@circ@math@distance
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@temp}}%
        \advance\pgf@circ@res@count by -1
    \repeat

    \pgf@circ@res@other=\ctikzvalof{tripoles/american xnor port/port width}\pgf@circ@res@right
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}

    \pgfusepath{draw}

    \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}

    \edef\pgf@circ@math@angle{\ctikzvalof{tripoles/american xnor port/angle}}%
    \pgf@circ@res@step = \ctikzvalof{tripoles/american xnor port/circle width}\pgf@circ@res@right
    \pgf@circ@res@temp = \dimexpr 2\pgf@circ@res@other - \pgf@circ@res@step\relax
    \advance\pgf@circ@res@other by -\pgf@circ@res@step

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}% for symmetry
    \pgfpatharc{0}{90}{\pgf@circ@res@temp and \pgf@circ@res@up}%
    \pgfpatharc{\pgf@circ@math@angle}{-\pgf@circ@math@angle}{\pgf@circ@math@xradius and \pgf@circ@math@yradius}%
    \pgfpatharc{-90}{0}{\pgf@circ@res@temp and \pgf@circ@res@up}%
    \pgfpathclose

    \pgfpathellipse
    {\pgfpoint{\pgf@circ@res@other+.5\pgf@circ@res@step}{0pt}}
    {\pgfpoint{.5\pgf@circ@res@step}{0pt}}
    {\pgfpoint{0pt}{.5\pgf@circ@res@step}}
    \pgf@circ@draworfill

    \pgf@circ@res@other=\ctikzvalof{tripoles/american xnor port/port width}\pgf@circ@res@left
    \pgfmathsetlength{\pgf@circ@res@temp}{(\pgf@circ@math@yradiusA)*sin(\pgf@circ@math@angle)}%

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other-\pgf@circ@math@distance}{\pgf@circ@res@temp}}% first arc
    \pgfpatharc{\pgf@circ@math@angle}{-\pgf@circ@math@angle}{\pgf@circ@math@xradiusA and \pgf@circ@math@yradiusA}%

    \pgfusepath{draw}
}

%%% Original one-input ports

\pgfdeclareshape{american not port}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{logic ports}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{bipoles/not port/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{bipoles/not port/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in 1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{bin}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{bin 1}{
        \northwest
        \pgf@y=0pt
        \pgf@x=0.7\pgf@x
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{bout}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-0.7\pgf@x
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgf@circ@res@other = \ctikzvalof{bipoles/not port/circle width}\pgf@circ@res@right

        \pgfscope
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
            \pgf@circ@draworfill
            \pgfpathellipse
            {\pgfpoint{\pgf@circ@res@step-.5\pgf@circ@res@other}{0pt}}
            {\pgfpoint{.5\pgf@circ@res@other}{0pt}}
            {\pgfpoint{0pt}{.5\pgf@circ@res@other}}
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}

        \pgfusepath{draw}
    }
}

\pgfdeclareshape{american buffer port}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{logic ports}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{bipoles/not port/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{bipoles/not port/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in 1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{bin}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{bin 1}{
        \northwest
        \pgf@y=0pt
        \pgf@x=0.7\pgf@x
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{bout}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-0.7\pgf@x
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgfscope
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}

        \pgfusepath{draw}
    }
}
\pgfdeclareshape{invschmitt}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{logic ports}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{bipoles/not port/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{bipoles/not port/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in 1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{bin 1}{
        \northwest
        \pgf@y=0pt
        \pgf@x=0.7\pgf@x
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{bout}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-0.7\pgf@x
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgf@circ@res@other = \ctikzvalof{bipoles/not port/circle width}\pgf@circ@res@right

        \pgfscope
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
            \pgfpathellipse
            {\pgfpoint{\pgf@circ@res@step-.5\pgf@circ@res@other}{0pt}}
            {\pgfpoint{.5\pgf@circ@res@other}{0pt}}
            {\pgfpoint{0pt}{.5\pgf@circ@res@other}}
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
        \pgfusepath{draw}
        %draw inner shape

        \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}

        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.05\pgf@circ@res@left}{.3\pgf@circ@res@up}}
        \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.3\pgf@circ@res@up}}
        \pgfusepath{draw}

    }
}

\pgfdeclareshape{schmitt}{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{logic ports}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{bipoles/not port/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{bipoles/not port/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in 1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{bin 1}{
        \northwest
        \pgf@y=0pt
        \pgf@x=0.7\pgf@x
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{bout}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-.7\pgf@x
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}


        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgfscope
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right-\pgf@circ@res@other}{0pt}}
        \pgfusepath{draw}
        %draw inner shape

        \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}

        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.05\pgf@circ@res@left}{.3\pgf@circ@res@up}}
        \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.3\pgf@circ@res@up}}
        \pgfusepath{draw}

    }
}


%%% start european logic ports, from John Kormylo
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%

% #1 - name
% #2 - text inside
% #3 - number of inputs
% #4 = is it a not?

\long\def\pgfcircdeclareeurologicport#1#2#3#4{
    \pgfdeclareshape{european #1 port}
    {
        \savedmacro{\ctikzclass}{\edef\ctikzclass{logic ports}}
        \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
        \savedmacro\resize{% automatic
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@circ@res@up = \ctikzvalof{tripoles/european #1 port/height}\pgf@circ@scaled@Rlen
            \pgf@circ@res@up = .5\pgf@circ@res@up
            \pgf@circ@res@down = -\pgf@circ@res@up
            \pgf@circ@res@right = \ctikzvalof{tripoles/european #1 port/width}\pgf@circ@scaled@Rlen
            \pgf@circ@res@right = .5\pgf@circ@res@right
            \pgf@circ@res@left = -\pgf@circ@res@right
        }%
        \savedmacro\inputs{% get number of inputs
            \pgf@circ@res@count=\pgfkeysvalueof{/tikz/number inputs}\relax%
            \ifnum\pgf@circ@res@count=0
                \pgf@circ@res@count=\ctikzvalof{tripoles/european #1 port/inputs}\relax%
            \fi
        \ifnum\pgf@circ@res@count<2 \pgf@circ@res@count=2\fi
    \ifnum\pgf@circ@res@count>16 \pgf@circ@res@count=16\fi
        \def\inputs{\the\pgf@circ@res@count}%
    }%
    \savedanchor\step{% 1/2 gap at edges
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@circ@res@step = \ctikzvalof{tripoles/european #1 port/height}\pgf@circ@scaled@Rlen
        \divide\pgf@circ@res@step by #3
        \pgfpoint{\pgf@circ@res@left}{\dimexpr\pgf@circ@res@up+0.5\pgf@circ@res@step}%
    }%
    \savedanchor\northeast{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}%
    \savedanchor\southwest{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}%
    \savedanchor\left{\pgfpoint{\ctikzvalof{tripoles/european #1 port/reserved}\pgf@circ@res@left}{0pt}}%
    \savedanchor\right{\pgfpoint{\ctikzvalof{tripoles/european #1 port/reserved}\pgf@circ@res@right}{0pt}}%
    \savedanchor\origin{\pgfpoint{\ctikzvalof{tripoles/european #1 port/origin}\pgf@circ@res@right}{0pt}}%

    \anchor{center}{\origin}% for backwards compatibility
    % the text anchor overlaps the logic symbol
    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}%
    % create input anchors
    \ifnum#3=1\relax
        \anchor{in}{\southwest\pgfpoint{\pgf@x}{0pt}}% or \step
        \anchor{in 1}{\southwest\pgfpoint{\pgf@x}{0pt}}% or \step
        \anchor{bin}{\left\pgfpoint{\pgf@x}{0pt}}% or \step
        \anchor{bin 1}{\left\pgfpoint{\pgf@x}{0pt}}% or \step
    \else
        \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@european #1 port\endcsname{%
            \pgfmathloop%
            \ifnum\pgfmathcounter>#3%
        \else%
            %\pgfutil@ifundefined{pgf@anchor@european #1 port@in \pgfmathcounter}{% redundant
            \expandafter\xdef\csname pgf@anchor@european #1 port@in \pgfmathcounter\endcsname{%
                \noexpand\pgf@circ@logicport@input{\pgfmathcounter}% defined above
            }%
            \expandafter\xdef\csname pgf@anchor@european #1 port@bin \pgfmathcounter\endcsname{%
                \noexpand\pgf@circ@logicport@baseinput{\pgfmathcounter}{4}{#1}% defined above
            }%
            %}{}%
            \repeatpgfmathloop%
        }
    \fi
    \anchor{out}{\northeast\pgf@y=0pt}
    \anchor{bout}{\right\pgf@y=0pt}

    \anchor{left}{\left}% edges of component minus leads
    \anchor{right}{\right}

    \anchor{north east}{\northeast}% see \Compass macro
    \anchor{south west}{\southwest}
    \anchor{north}{\pgfextracty{\pgf@circ@res@up}{\northeast}%
    \pgfpoint{0cm}{\pgf@circ@res@up}}
    \anchor{north west}{\pgfextracty{\pgf@circ@res@up}{\northeast}%
        \pgfextractx{\pgf@circ@res@left}{\southwest}%
    \pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \anchor{west}{\pgfextractx{\pgf@circ@res@left}{\southwest}%
    \pgfpoint{\pgf@circ@res@left}{0cm}}
    \anchor{south}{\pgfextracty{\pgf@circ@res@down}{\southwest}%
    \pgfpoint{0cm}{\pgf@circ@res@down}}
    \anchor{south east}{\pgfextracty{\pgf@circ@res@down}{\southwest}%
        \pgfextractx{\pgf@circ@res@right}{\northeast}%
    \pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \anchor{east}{\pgfextractx{\pgf@circ@res@right}{\northeast}%
    \pgfpoint{\pgf@circ@res@right}{0cm}}

    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        \pgfscope
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgfpathrectanglecorners
            {\pgfpoint{\ctikzvalof{tripoles/european #1 port/reserved}\pgf@circ@res@left}{\pgf@circ@res@up}}
            {\pgfpoint{\ctikzvalof{tripoles/european #1 port/reserved}\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgf@circ@draworfill
        \endpgfscope
        \ifnum#3=1\relax
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}%
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/european #1 port/reserved}\pgf@circ@res@left}{0pt}}%
        \else
            \pgfextracty{\pgf@circ@res@temp}{\step}%
            \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
            %\pgf@circ@res@count = #3\relax% redundant
            \loop\ifnum\pgf@circ@res@count>0
                \advance\pgf@circ@res@temp by -\pgf@circ@res@step
                \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
                \pgfpathlineto{\pgfpoint
                    {\ctikzvalof{tripoles/european #1 port/reserved}\pgf@circ@res@left}
                {\pgf@circ@res@temp}}
                \advance\pgf@circ@res@count by -1
                \repeat
            \fi
            %
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
            \pgfpathlineto{%
            \pgfpoint{\ctikzvalof{tripoles/european #1 port/reserved}\pgf@circ@res@right}{0pt}}
            %
            \edef\pgf@temp{not}
            \edef\pgf@circ@temp{#4}
            \ifx\pgf@temp\pgf@circ@temp % is a not
                \pgfpathmoveto{\pgfpoint{\ctikzvalof{tripoles/european #1 port/not width}\pgf@circ@res@right}{0pt}}
                \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/european #1 port/reserved}\pgf@circ@res@right}%
                {\ctikzvalof{tripoles/european #1 port/not height}\pgf@circ@res@up}}
            \fi
            %
            \pgfusepath{draw}
            %
            \pgfpathmoveto{\pgfpointorigin}
            \pgftext{#2}
        }
    }
}
\pgfcircdeclareeurologicport{and}{\&}{\pgf@circ@res@count}{}
\pgfcircdeclareeurologicport{or}{$\ge 1$}{\pgf@circ@res@count}{}
\pgfcircdeclareeurologicport{xor}{$=1$}{\pgf@circ@res@count}{}
\pgfcircdeclareeurologicport{not}{$1$}{1}{not}
\pgfcircdeclareeurologicport{buffer}{$1$}{1}{}
\pgfcircdeclareeurologicport{nand}{\&}{\pgf@circ@res@count}{not}
\pgfcircdeclareeurologicport{nor}{$\ge 1$}{\pgf@circ@res@count}{not}
\pgfcircdeclareeurologicport{xnor}{$=1$}{\pgf@circ@res@count}{not}

%% end european logic ports

%%%%%%%%%%%%%%%%%%%%%%%%
%% Transistors
%%%%%%%%%%%%%%%%%%%%%%%%


\long\def\pgfcircdeclaretransistor#1#2#3{
    \pgfdeclareshape{#1}
    {
        \savedmacro{\ctikzclass}{\edef\ctikzclass{transistors}}
        \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
        \anchor{center}{
            \pgfpointorigin
        }
        \savedanchor\northeast{% upper right
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@y=\ctikzvalof{tripoles/#1/height}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=0pt
        }
        \savedanchor\left{%center left
            \pgf@y=0pt
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@x=-\ctikzvalof{tripoles/#1/width}\pgf@circ@scaled@Rlen
        }
        \savedanchor\right{%center right -- added by Burak Kelleci % this is really 0,0
            \pgf@y=0pt
            \pgf@x=0pt
        }
        \anchor{text}{
            \northeast
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \ifpgf@circuit@transisors@fixlabels
                \ifpgf@circuit@fet@bodydiode
                    % try to put the text to the right of the flyback diode
                    \pgfmathsetlength{\pgf@circ@res@other}{(
                        \ctikzvalof{tripoles/#1/bodydiode distance}*
                        \ctikzvalof{tripoles/#1/width} +
                        \ctikzvalof{tripoles/#1/bodydiode scale}*
                        \ctikzvalof{bipoles/diode/height}/2
                        )*\pgf@circ@scaled@Rlen}
                    \advance\pgf@x by \pgf@circ@res@other
                \fi
                % add a bit of space to avoid central (substrate) terminal if drawn
                \advance\pgf@x by 0.05\pgf@circ@scaled@Rlen\relax
                \pgf@y=\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax
            \else
                \pgf@y=.7\pgf@y
                \pgf@x= \pgf@circ@scaled@Rlen
                \pgf@x=0.1\pgf@x
            \fi
        }
        \anchor{pathstart}{ % south
            \northeast
            \pgf@y=-\pgf@y
        }
        \anchor{pathend}{
            \northeast
        }
        \anchor{north}{
            \northeast
            \pgf@circ@res@step=\pgf@y
            \left
            \pgf@y=\pgf@circ@res@step
            \pgf@x=.5\pgf@x
        }
        \anchor{west}{
            \left
        }
        \anchor{east}{
            \northeast
            \pgf@y=0pt
        }
        \anchor{south}{
            \northeast
            \pgf@circ@res@step=\pgf@y
            \left
            \pgf@y=-\pgf@circ@res@step
            \pgf@x=.5\pgf@x
        }
        \anchor{south west}{
            \northeast
            \pgf@circ@res@step=\pgf@y
            \left
            \pgf@y=-\pgf@circ@res@step
        }
        \anchor{north east}{
            \northeast
        }
        \anchor{north west}{
            \northeast
            \pgf@circ@res@step=\pgf@y
            \left
            \pgf@y=\pgf@circ@res@step
        }
        \anchor{south east}{
            \northeast
            \pgf@y=-\pgf@y
        }
        \anchor{B}{
            \northeast
            \pgf@circ@res@step=\ctikzvalof{tripoles/#1/conn height}\pgf@y
            \left
            \pgf@y=-\ctikzvalof{tripoles/#1/curr direction}\pgf@circ@res@step
        }
        \anchor{base}{
            \northeast
            \pgf@circ@res@step=\ctikzvalof{tripoles/#1/conn height}\pgf@y
            \left
            \pgf@y=-\ctikzvalof{tripoles/#1/curr direction}\pgf@circ@res@step
        }
        \anchor{bulk}{ %added by Burak Kelleci
            \northeast
            \pgf@circ@res@step=\ctikzvalof{tripoles/#1/conn height}\pgf@y
            \right
            \pgf@y=-\ctikzvalof{tripoles/#1/curr direction}\pgf@circ@res@step
        }
        \anchor{nobulk}{ %added by Burak Kelleci
            \left
            \pgf@x=\ctikzvalof{tripoles/#1/base width}\pgf@x
        }
        \anchor{G}{
            \northeast
            \pgf@circ@res@step=\ctikzvalof{tripoles/#1/conn height}\pgf@y
            \left
            \pgf@y=-\ctikzvalof{tripoles/#1/curr direction}\pgf@circ@res@step
        }
        \anchor{gate}{
            \northeast
            \pgf@circ@res@step=\ctikzvalof{tripoles/#1/conn height}\pgf@y
            \left
            \pgf@y=-\ctikzvalof{tripoles/#1/curr direction}\pgf@circ@res@step
        }
        \anchor{nobase}{
            \left
            \pgf@x=\ctikzvalof{tripoles/#1/base width}\pgf@x
        }
        \anchor{nogate}{
            \left
            \pgf@x=\ctikzvalof{tripoles/#1/gate width}\pgf@x
        }
        \anchor{E}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/#1/curr direction}\pgf@y
        }
        \anchor{emitter}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/#1/curr direction}\pgf@y
        }
        \anchor{C}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/#1/curr direction}\pgf@y
        }
        \anchor{collector}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/#1/curr direction}\pgf@y
        }
        \anchor{S}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/#1/curr direction}\pgf@y
        }
        \anchor{source}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/#1/curr direction}\pgf@y
        }
        \anchor{D}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/#1/curr direction}\pgf@y
        }
        \anchor{drain}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/#1/curr direction}\pgf@y
        }
        \anchor{body C in}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/#1/curr direction}\pgf@y
            \pgf@y=\ctikzvalof{tripoles/#1/bodydiode conn}\pgf@y
        }
        \anchor{body E in}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/#1/curr direction}\pgf@y
            \pgf@y=\ctikzvalof{tripoles/#1/bodydiode conn}\pgf@y
        }
        \anchor{body C out}{
            \northeast
            \pgf@ya=\ctikzvalof{tripoles/#1/curr direction}\pgf@y
            \pgf@ya=\ctikzvalof{tripoles/#1/bodydiode conn}\pgf@ya
            \pgf@y=\pgf@ya
            \left
            \pgf@x=-\ctikzvalof{tripoles/#1/bodydiode distance}\pgf@x
            \pgf@y=\pgf@ya
        }
        \anchor{body E out}{
            \northeast
            \pgf@ya=-\ctikzvalof{tripoles/#1/curr direction}\pgf@y
            \pgf@ya=\ctikzvalof{tripoles/#1/bodydiode conn}\pgf@ya
            \pgf@y=\pgf@ya
            \left
            \pgf@x=-\ctikzvalof{tripoles/#1/bodydiode distance}\pgf@x
            \pgf@y=\pgf@ya
        }
        #2
        \backgroundpath{
            \pgftransformationadjustments
            \pgfsetcolor{\ctikzvalof{color}}
            %
            \ifnum \ctikzvalof{tripoles/#1/curr direction} > 0
            \pgf@circuit@trans@ntypetrue
            \else
            \pgf@circuit@trans@ntypefalse
        \fi
        \northeast
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = \pgf@x
        \left
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@scaled@Rlen=\scaledRlen
        %
        #3
        % BODY DIODE
        \ifpgf@circuit@fet@bodydiode
            \drawbodydiode{#1}
        \fi
        %
    }
}
}

\long\def\drawbodydiode#1{
    \pgfscope
        \pgftransformshift{\pgfpoint{-\ctikzvalof{tripoles/#1/bodydiode distance}\pgf@circ@res@left}{\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgftransformrotate{90}
        % diode scale and bodydiode scale interacts. We want the size of the diode
        % proportional to the transistor, so we will:
        % 1) undo diode scale 2) apply transistor scale (using the current class) 3) apply bodydiode scale
        \pgfmathsetmacro{\@@BDscale}{\ctikzvalof{tripoles/#1/bodydiode scale}* \ctikzvalof{\ctikzclass/scale}/\ctikzvalof{diodes/scale}}
        \pgftransformscale{\@@BDscale}
        \ifpgf@circuit@fulldiode
            \pgfnode{fulldiodeshape}{center}{}{pgf@bodydiode}{\pgfusepath{fill}}
        \else
            \pgfnode{emptydiodeshape}{center}{}{pgf@bodydiode}{\pgfusepath{fill}}
        \fi
    \endpgfscope
    % Draw stroke line
    \ifpgf@circuit@strokediode
        \pgfpathmoveto{\pgfpointanchor{pgf@bodydiode}{west}}
        \pgfpathlineto{\pgfpointanchor{pgf@bodydiode}{east}}
        \pgfusepath{stroke}
    \fi
    %Draw upper connection to body diode
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/#1/bodydiode conn}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{-\ctikzvalof{tripoles/#1/bodydiode distance}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/#1/bodydiode conn}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpointanchor{pgf@bodydiode}{east}}
    \pgfusepath{draw}
    \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@right}
        {\ctikzvalof{tripoles/#1/bodydiode conn}\pgf@circ@res@up}}
        \pgftransformscale{0.5}
        \pgfnode{circ}{center}{}{}{\pgfusepath{fill}}
    \endpgfscope{}
    %Draw lower connection to body diode
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/#1/bodydiode conn}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{-\ctikzvalof{tripoles/#1/bodydiode distance}\pgf@circ@res@left}{\ctikzvalof{tripoles/#1/bodydiode conn}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpointanchor{pgf@bodydiode}{west}}
    \pgfusepath{draw}
    \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@right}		        	       {\ctikzvalof{tripoles/#1/bodydiode conn}\pgf@circ@res@down}}
        \pgftransformscale{0.5}
        \pgfnode{circ}{center}{}{}{\pgfusepath{fill}}
    \endpgfscope
}

\long\def\declarebpt#1{
    \pgfcircdeclaretransistor{#1}{
        \anchor{inner up}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/#1/base height}\pgf@y
        }
        \anchor{inner down}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/#1/base height}\pgf@y
        }
        }{
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
        {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/#1/base height 2}\pgf@circ@res@up}}
        \pgfusepath{draw}

        \pgfscope
            \pgfpathmoveto{\pgfpoint
                {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint
                {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@down}}
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgfusepath{draw}
        \endpgfscope

        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/#1/base height 2}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
        {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
        \pgfusepath{draw}
        %draw arrow depending on type of transistor
        \pgfscope
            \pgfslopedattimetrue
            \pgfallowupsidedownattimetrue
            \pgfresetnontranslationattimefalse
            \edef\@@anchor{center}
            \ifpgf@circuit@trans@ntype
                \ifpgf@circuit@trans@arrowatend
                    \edef\@@anchor{btip}
                    \pgftransformlineattime{1.0}{%
                        \pgfpoint%
                        {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}%
                        {\ctikzvalof{tripoles/#1/base height 2}\pgf@circ@res@down}%
                        }{%
                        \pgfpoint{\pgf@circ@res@right}%
                        {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@down}%
                    }
                \else
                    \pgftransformlineattime{\ctikzvalof{tripoles/#1/arrow pos}}{%
                        \pgfpoint%
                        {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}%
                        {\ctikzvalof{tripoles/#1/base height 2}\pgf@circ@res@down}%
                        }{%
                        \pgfpoint{\pgf@circ@res@right}%
                        {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@down}%
                    }
                \fi
            \else % p-type
                \ifpgf@circuit@trans@arrowatend
                    \edef\@@anchor{tip}
                    \pgftransformlineattime{1.0}{%
                        \pgfpoint{\pgf@circ@res@right}%
                        {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@up}%
                        }{%
                        \pgfpoint{\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}%
                        {\ctikzvalof{tripoles/#1/base height 2}\pgf@circ@res@up}%
                    }
                \else
                    \pgftransformlineattime{\ctikzvalof{tripoles/#1/arrow pos}}{%
                        \pgfpoint{\pgf@circ@res@right}%
                        {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@up}%
                        }{%
                        \pgfpoint{\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}%
                        {\ctikzvalof{tripoles/#1/base height 2}\pgf@circ@res@up}%
                    }
                \fi
            \fi
            \pgfnode{trarrow}{\@@anchor}{}{}{\pgfusepath{stroke}}
        \endpgfscope

        \ifpgf@circuit@bpt@drawphoto
            \pgfscope
                \pgfsetarrowsstart{latexslim}
                \pgfpathmoveto{\pgfpointadd{\pgfpoint
                        {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
                    {\pgf@circ@res@up+\pgf@circ@res@down}}
                {\pgfpoint{0.05\pgf@circ@res@left}{0.1\pgf@circ@res@up}}}
                \pgfpathlineto{\pgfpointadd{\pgfpoint
                        {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
                    {\pgf@circ@res@up+\pgf@circ@res@down}}
                {\pgfpoint{0.5\pgf@circ@res@left}{0.3\pgf@circ@res@up}}}
                \pgfusepath{draw}
                \pgfpathmoveto{\pgfpointadd{\pgfpoint
                        {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
                    {\pgf@circ@res@up+\pgf@circ@res@down}}
                {\pgfpoint{0.05\pgf@circ@res@left}{-0.1\pgf@circ@res@up}}}
                \pgfpathlineto{\pgfpointadd{\pgfpoint
                        {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
                    {\pgf@circ@res@up+\pgf@circ@res@down}}
                {\pgfpoint{0.5\pgf@circ@res@left}{0.1\pgf@circ@res@up}}}
                \pgfusepath{draw}
            \endpgfscope
            \else
            \ifpgf@circuit@bpt@drawbase
                \pgfpathmoveto{\pgfpoint
                    {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
                {\pgf@circ@res@up+\pgf@circ@res@down}}
                \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgf@circ@res@up+\pgf@circ@res@down}}
                \pgfusepath{draw}
            \fi
        \fi
    }
}

\declarebpt{npn}
\declarebpt{pnp}
%
% multi-emitter and multi-collector BJTs by Romano Giannetti
%
\def\pgf@circ@bjt@C@anchor#1{% #1: collector number
    \pgfextractx{\pgf@circ@res@temp}{\basedimension}
    \pgfextracty{\pgf@circ@res@other}{\basedimension}
    \ifnum\cdir>0 % NPN, above
        \pgfpoint{\pgf@circ@res@temp}{%
        \pgf@circ@res@other+\pgfverticaltransformationadjustment*.5*\pgflinewidth+(#1-1)*\multistep}
    \else % PNP, below
        \pgfpoint{\pgf@circ@res@temp}{%
        -\pgf@circ@res@other-\pgfverticaltransformationadjustment*.5*\pgflinewidth-(#1-1)*\multistep}
    \fi
}
\def\pgf@circ@bjt@E@anchor#1{% #1: collector number
    \pgfextractx{\pgf@circ@res@temp}{\basedimension}
    \pgfextracty{\pgf@circ@res@other}{\basedimension}
    \ifnum\cdir<0 % PNP, above
        \pgfpoint{\pgf@circ@res@temp}{%
        \pgf@circ@res@other+\pgfverticaltransformationadjustment*.5*\pgflinewidth+(#1-1)*\multistep}
    \else % PNP, below
        \pgfpoint{\pgf@circ@res@temp}{%
        -\pgf@circ@res@other-\pgfverticaltransformationadjustment*.5*\pgflinewidth-(#1-1)*\multistep}
    \fi
}

\long\def\declarebjt#1{
    \pgfdeclareshape{bjt#1}{
        \savedmacro{\ctikzclass}{\edef\ctikzclass{transistors}}
        \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
        % \cdir is 1 for npn, -1 for pnp
        \savedmacro{\cdir}{\edef\cdir{\ctikzvalof{tripoles/bjt/#1/curr direction}}}
        \savedmacro{\numE}{\edef\numE{\ctikzvalof{tripoles/bjt/emitters}}}
        \savedmacro{\numC}{\edef\numC{\ctikzvalof{tripoles/bjt/collectors}}}
        % step up or down for the additional C/Es
        \saveddimen{\multistep}{\pgfmathsetlength{\pgf@x}{%
            \ctikzvalof{tripoles/bjt/height}*\ctikzvalof{tripoles/bjt/multi height}*
            \ctikzvalof{\ctikzclass/scale}*\pgf@circ@Rlen}}
        \saveddimen{\external}{\pgfmathsetlength{\pgf@x}{%
            \ctikzvalof{tripoles/bjt/pins width}*\ctikzvalof{\ctikzclass/scale}*\pgf@circ@Rlen}}
        \savedanchor\basedimension{% these are the dimensions if nC=1 y nE=1
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@y=\ctikzvalof{tripoles/bjt/height}\pgf@circ@scaled@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=\ctikzvalof{tripoles/bjt/width}\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
        }
        \savedanchor\northeast{% upper right
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgfmathsetlength{\pgf@circ@res@step}{%
                \ctikzvalof{tripoles/bjt/height}*\ctikzvalof{tripoles/bjt/multi height}*
                \ctikzvalof{\ctikzclass/scale}*\pgf@circ@Rlen}
            \ifnum\cdir> 0
                \edef\numup{\numC}\edef\numdown{\numE}
            \else
                \edef\numup{\numE}\edef\numdown{\numC}
            \fi
            \pgfmathsetlength{\pgf@y}{0.5*\ctikzvalof{tripoles/bjt/height}\pgf@circ@scaled@Rlen
                + (\numup-1)*\pgf@circ@res@step+\pgfverticaltransformationadjustment*.5*\pgflinewidth
                + \ctikzvalof{tripoles/bjt/pins width}*\ctikzvalof{\ctikzclass/scale}*\pgf@circ@Rlen}
            \pgf@x=\ctikzvalof{tripoles/bjt/width}\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
        }
        \savedanchor\southeast{% lower right
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgfmathsetlength{\pgf@circ@res@step}{%
                \ctikzvalof{tripoles/bjt/height}*\ctikzvalof{tripoles/bjt/multi height}*
                \ctikzvalof{\ctikzclass/scale}*\pgf@circ@Rlen}
            \ifnum\cdir> 0
                \edef\numup{\numC}\edef\numdown{\numE}
            \else
                \edef\numup{\numE}\edef\numdown{\numC}
            \fi
            \pgfmathsetlength{\pgf@y}{-0.5*\ctikzvalof{tripoles/bjt/height}\pgf@circ@scaled@Rlen
                - (\numdown-1)*\pgf@circ@res@step-\pgfverticaltransformationadjustment*.5*\pgflinewidth
                - \ctikzvalof{tripoles/bjt/pins width}*\ctikzvalof{\ctikzclass/scale}*\pgf@circ@Rlen}
            \pgf@x=\ctikzvalof{tripoles/bjt/width}\pgf@circ@scaled@Rlen
            \pgf@x=.5\pgf@x
        }
        \savedanchor\southwest{% lower left
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgfmathsetlength{\pgf@circ@res@step}{%
                \ctikzvalof{tripoles/bjt/height}*\ctikzvalof{tripoles/bjt/multi height}*
                \ctikzvalof{\ctikzclass/scale}*\pgf@circ@Rlen}
            \ifnum\cdir> 0
                \edef\numup{\numC}\edef\numdown{\numE}
            \else
                \edef\numup{\numE}\edef\numdown{\numC}
            \fi
            \pgfmathsetlength{\pgf@y}{-0.5*\ctikzvalof{tripoles/bjt/height}\pgf@circ@scaled@Rlen
                - (\numdown-1)*\pgf@circ@res@step-\pgfverticaltransformationadjustment*.5*\pgflinewidth
                - \ctikzvalof{tripoles/bjt/pins width}*\ctikzvalof{\ctikzclass/scale}*\pgf@circ@Rlen}
            \pgfmathsetlength{\pgf@x}{-0.5*\ctikzvalof{tripoles/bjt/width}*\pgf@circ@scaled@Rlen
                - \ctikzvalof{tripoles/bjt/pins width}*\ctikzvalof{\ctikzclass/scale}*\pgf@circ@Rlen}
        }
        \anchor{center}{\pgfpointorigin}
        \anchor{north}{\northeast\pgf@x=0cm\relax}
        \anchor{east}{\northeast\pgf@y=0cm\relax}
        \anchor{south}{\southwest\pgf@x=0cm\relax}
        \anchor{west}{\southwest\pgf@y=0cm}
        \anchor{north east}{\northeast}
        \anchor{north west}{\northeast\pgf@ya=\pgf@y\southwest\pgf@y=\pgf@ya}
        \anchor{south west}{\southwest}
        \anchor{south east}{\southeast}

        \anchor{text}{\northeast\pgf@y=\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax}
        \anchor{B}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x\advance\pgf@x by -\external}
        \anchor{base}{\basedimension\pgf@y=0cm\pgf@x=-\pgf@x\advance\pgf@x by -\external}
        \anchor{nobase}{\basedimension\pgf@y=0cm\pgf@x=-\pgf@x}
        % center of the base "bar"
        \anchor{cbase}{\basedimension\pgf@x=-\pgf@x
            \pgfmathsetlength{\pgf@y}{\cdir*(\numC-\numE)*\multistep/2}%
        }
        % geometrical centers
        \anchor{vcenter}{\pgf@x=0cm\relax
            \pgfmathsetlength{\pgf@y}{\cdir*(\numC-\numE)*\multistep/2}%
        }
        \anchor{gcenter}{%
            \northeast\pgf@xa=0.5\pgf@x
            \southwest\advance\pgf@xa by 0.5\pgf@x
            \pgf@x=\pgf@xa
            \pgfmathsetlength{\pgf@y}{\cdir*(\numC-\numE)*\multistep/2}%
        }
        % external connections
        \anchor{E}{
            \ifnum\cdir>0% npn, emitter down
            \southeast
            \else
            \northeast
            \fi
        }% first emitter
        \anchor{emitter}{\ifnum\cdir>0\southeast\else\northeast\fi}% first emitter
        \anchor{C}{\ifnum\cdir<0\southeast\else\northeast\fi}
        \anchor{collector}{\ifnum\cdir<0\southeast\else\northeast\fi}

        \backgroundpath{
            \pgftransformationadjustments
            \pgfsetcolor{\ctikzvalof{color}}
            %
            % set the type and up and down number of connections
            %
            \ifnum\cdir> 0
                \pgf@circuit@trans@ntypetrue
                \edef\numup{\numC}
                \edef\numdown{\numE}
            \else
                \pgf@circuit@trans@ntypefalse
                \edef\numup{\numE}
                \edef\numdown{\numC}
            \fi
            \basedimension
            \pgf@circ@res@up = \pgf@y
            \pgf@circ@res@down = -\pgf@y
            \pgf@circ@res@right = \pgf@x
            \pgf@circ@res@left = -\pgf@x
            \pgf@circ@scaled@Rlen=\scaledRlen
            \pgf@circ@res@step=\multistep
            %
            % set arrow positions options
            %
            \edef\@@anchor{center}\edef\@@pos{\ctikzvalof{tripoles/#1/arrow pos}}
            \ifpgf@circuit@trans@arrowatend
                \edef\@@pos{1.0}
                \ifpgf@circuit@trans@ntype % arrow is toward outside, push it a bit
                    \edef\@@anchor{btip}
                \else
                    \edef\@@anchor{tip}
                \fi
            \fi
            %
            % Drawing upper connections
            %
            \pgfscope
            \pgf@circ@count@a=\numup\relax
            \pgfmathloop%
            \ifnum\pgf@circ@count@a>0
            \advance\pgf@circ@count@a-1\relax
            \pgfmathsetlength{\pgf@circ@res@other}{\the\pgf@circ@count@a*\multistep}%
            \ifnum\pgf@circ@count@a=\numexpr\numup-1\relax % draw the external pin connection
            \pgfpathmoveto{\pgfpoint
                {\pgf@circ@res@right}%
                {\pgf@circ@res@up+\external+\pgfverticaltransformationadjustment*.5*\pgflinewidth+\pgf@circ@res@other}}%
            \pgfpathlineto{\pgfpoint
                {\pgf@circ@res@right}%
                {\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth+\pgf@circ@res@other}}%
            \else
            \pgfpathmoveto{\pgfpoint
                {\pgf@circ@res@right}%
                {\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth+\pgf@circ@res@other}}%
            \fi
            \pgfpathlineto{\pgfpoint
                {\ctikzvalof{tripoles/bjt/base width}\pgf@circ@res@left}%
                {\ctikzvalof{tripoles/bjt/base height 2}\pgf@circ@res@up+\pgf@circ@res@other}}%
            \pgfsetroundcap % better when connecting to sloped lines
            \pgfusepath{draw}
            \ifpgf@circuit@trans@ntype\else % it's a PNP; draw arrow
            \pgfscope
                \pgfslopedattimetrue
                \pgfallowupsidedownattimetrue
                \pgfresetnontranslationattimefalse
                \pgftransformlineattime{\@@pos}{%
                    \pgfpoint
                        {\pgf@circ@res@right}%
                        {\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth+\pgf@circ@res@other}%
                    }{\pgfpoint
                        {\ctikzvalof{tripoles/bjt/base width}\pgf@circ@res@left}%
                        {\ctikzvalof{tripoles/bjt/base height 2}\pgf@circ@res@up+\pgf@circ@res@other}%
                    }
                    \pgfnode{trarrow}{\@@anchor}{}{}{\pgfusepath{stroke}}
            \endpgfscope
            \fi
            \repeatpgfmathloop
            \endpgfscope
            %
            % Drawing base
            %
            \pgfscope
                \pgfpathmoveto{\pgfpoint
                    {\ctikzvalof{tripoles/bjt/base width}\pgf@circ@res@left}
                    {\ctikzvalof{tripoles/bjt/base height}\pgf@circ@res@up+(\numup-1)*\multistep}}
                \pgfpathlineto{\pgfpoint
                    {\ctikzvalof{tripoles/bjt/base width}\pgf@circ@res@left}
                    {\ctikzvalof{tripoles/bjt/base height}\pgf@circ@res@down-(\numdown-1)*\multistep}}
                \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
                \pgfsetroundcap % I like it more...
                \pgfusepath{draw}
            \endpgfscope
            %
            % draw base external connection
            %
            \pgfpathmoveto{\pgfpoint{\ctikzvalof{tripoles/bjt/base width}\pgf@circ@res@left}{0pt}}
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/bjt/base width}\pgf@circ@res@left-\external}{0pt}}
            \pgfusepath{draw}
            %
            % Drawing lower connections
            %
            \pgfscope
            \pgf@circ@count@a=\numdown\relax
            \pgfmathloop%
            \ifnum\pgf@circ@count@a>0
            \advance\pgf@circ@count@a-1\relax
            \pgfmathsetlength{\pgf@circ@res@other}{\the\pgf@circ@count@a*\multistep}%
            \pgfpathmoveto{\pgfpoint
                {\ctikzvalof{tripoles/bjt/base width}\pgf@circ@res@left}
                {\ctikzvalof{tripoles/bjt/base height 2}\pgf@circ@res@down-\pgf@circ@res@other}}
            \pgfpathlineto{\pgfpoint
                {\pgf@circ@res@right}
                {\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth-\pgf@circ@res@other}}
            \ifnum\pgf@circ@count@a=\numexpr\numdown-1\relax % draw the external pin connection
            \pgfpathlineto{\pgfpoint
                {\pgf@circ@res@right}
                {\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth-\pgf@circ@res@other-\external}}
            \fi
            \pgfsetroundcap % better when connecting to sloped lines
            \pgfusepath{draw}
            \ifpgf@circuit@trans@ntype % it's a NPN; draw arrow
            \pgfscope
                \pgfslopedattimetrue
                \pgfallowupsidedownattimetrue
                \pgfresetnontranslationattimefalse
                \pgftransformlineattime{\@@pos}{%
                    \pgfpoint
                        {\ctikzvalof{tripoles/bjt/base width}\pgf@circ@res@left}%
                        {\ctikzvalof{tripoles/bjt/base height 2}\pgf@circ@res@down-\pgf@circ@res@other}%
                    }{\pgfpoint
                        {\pgf@circ@res@right}%
                        {\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth-\pgf@circ@res@other}%
                    }
                    \pgfnode{trarrow}{\@@anchor}{}{}{\pgfusepath{stroke}}
            \endpgfscope
            \fi
            \repeatpgfmathloop
            \endpgfscope
        }
        % \pgf@sh@s@<name of the shape here> contains all the code for the shape
        % and is executed just before a node is drawn.
        \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@bjt#1\endcsname{%
            % Start with the maximum collector number and go backwards.
            \pgf@circ@count@a=\numC\relax
            \pgfmathloop%
            \ifnum\pgf@circ@count@a>0
                % we will create two anchors per pin: the "normal one" like `pin 1` for the
                % electrical contact, and the "border one" like `bpin 1` for labels.
                % they will coincide if `external pins width` is set to 0.
                \expandafter\xdef\csname pgf@anchor@bjt#1@C\the\pgf@circ@count@a\endcsname{%
                    \noexpand\pgf@circ@bjt@C@anchor{\the\pgf@circ@count@a}%
                }
            \advance\pgf@circ@count@a by -1\relax%
            \repeatpgfmathloop%
            % and emitters
            \pgf@circ@count@a=\numE\relax
            \pgfmathloop%
            \ifnum\pgf@circ@count@a>0
                % we will create two anchors per pin: the "normal one" like `pin 1` for the
                % electrical contact, and the "border one" like `bpin 1` for labels.
                % they will coincide if `external pins width` is set to 0.
                \expandafter\xdef\csname pgf@anchor@bjt#1@E\the\pgf@circ@count@a\endcsname{%
                    \noexpand\pgf@circ@bjt@E@anchor{\the\pgf@circ@count@a}%
                }
            \advance\pgf@circ@count@a by -1\relax%
            \repeatpgfmathloop%
            }%
    }
}

\declarebjt{npn}
\declarebjt{pnp}

% end of multi-bjts

\long\def\declareigbt#1{
    \pgfcircdeclaretransistor{#1}{
        \anchor{inner up}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/#1/gate height}\pgf@y
        }
        \anchor{inner down}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/#1/gate height}\pgf@y
        }
    }
    {
        %draw upper connection
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
        {\ctikzvalof{tripoles/#1/gate height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/#1/gate height 2}\pgf@circ@res@up}}
        \pgfusepath{draw}

        %draw thicker gate lines
        \pgfscope
            \pgfpathmoveto{\pgfpoint
                {\ctikzvalof{tripoles/#1/gate width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5\pgflinewidth}}
            \pgfpathlineto{\pgfpoint
                {\ctikzvalof{tripoles/#1/gate width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5\pgflinewidth}}
            \pgfpathmoveto{\pgfpoint
                {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5\pgflinewidth}}
            \pgfpathlineto{\pgfpoint
                {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5\pgflinewidth}}
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgfusepath{draw}
        \endpgfscope
        %draw lower connection
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/#1/gate height 2}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
        {\ctikzvalof{tripoles/#1/gate height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
        \pgfusepath{draw}
        %draw arrow depending on type of transistor
        \pgfscope
            \pgfslopedattimetrue
            \pgfallowupsidedownattimetrue
            \pgfresetnontranslationattimefalse
            \ifpgf@circuit@trans@arrowatend
                \ifpgf@circuit@trans@ntype
                    \edef\@@anchor{btip}\edef\@@pos{1.0}
                \else
                    \edef\@@anchor{tip}\edef\@@pos{1.0}
                \fi
            \else
                \edef\@@anchor{center}\edef\@@pos{0.5}
            \fi
            \ifpgf@circuit@trans@ntype
                \pgftransformlineattime{\@@pos}{%
                    \pgfpoint%
                    {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}%
                    {\ctikzvalof{tripoles/#1/gate height 2}\pgf@circ@res@down}%
                    }{%
                    \pgfpoint{\pgf@circ@res@right}%
                    {\ctikzvalof{tripoles/#1/gate height}\pgf@circ@res@down}%
                }
            \else
                \pgftransformlineattime{\@@pos}{%
                    \pgfpoint{\pgf@circ@res@right}%
                    {\ctikzvalof{tripoles/#1/gate height}\pgf@circ@res@up}%
                    }{%
                    \pgfpoint{\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}%
                    {\ctikzvalof{tripoles/#1/gate height 2}\pgf@circ@res@up}%
                }
            \fi
            \pgfnode{trarrow}{\@@anchor}{}{}{\pgfusepath{stroke}}
        \endpgfscope
        %draw gate
        \ifpgf@circuit@trans@ntype
            \pgfpathmoveto{\pgfpoint
                {\ctikzvalof{tripoles/#1/gate width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/conn height}\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}%
            {\ctikzvalof{tripoles/#1/conn height}\pgf@circ@res@down}}
        \else
            \pgfpathmoveto{\pgfpoint
                {\ctikzvalof{tripoles/#1/gate width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/conn height}\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}%
            {\ctikzvalof{tripoles/#1/conn height}\pgf@circ@res@up}}
        \fi
        \pgfusepath{draw}
    }
}

\declareigbt{pigbt}
\declareigbt{nigbt}
\declareigbt{Lnigbt}
\declareigbt{Lpigbt}

\pgfcircdeclaretransistor{nmos}{
        \anchor{inner up}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/nmos/gate height}\pgf@y
        }
        \anchor{inner down}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/nmos/gate height}\pgf@y
        }
    }{%
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/nmos/gate height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint
        {\ctikzvalof{tripoles/nmos/base width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/nmos/gate height}\pgf@circ@res@up}}

    \pgfpathmoveto{\pgfpoint
        {\ctikzvalof{tripoles/nmos/base width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/nmos/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/nmos/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfusepath{draw}

    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/nmos/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/nmos/base height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/nmos/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/nmos/base height}\pgf@circ@res@down}}
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/nmos/gate width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/nmos/gate height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/nmos/gate width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/nmos/gate height}\pgf@circ@res@down}}
        \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope
    \ifpgf@circuit@mos@arrows
        \pgfscope
            \ifpgf@circuit@trans@arrowatend
                \pgftransformshift{\pgfpoint
                    {\pgf@circ@res@right}%
                    {\ctikzvalof{tripoles/pmos/gate height}\pgf@circ@res@down}%
                }
                \pgfnode{trarrow}{btip}{}{}{\pgfusepath{stroke}}
            \else
                \pgfslopedattimetrue
                \pgfallowupsidedownattimetrue
                \pgfresetnontranslationattimefalse
                \pgftransformlineattime{\ctikzvalof{tripoles/nmos/arrow pos}}{%
                    \pgfpoint%
                    {\ctikzvalof{tripoles/nmos/gate width}\pgf@circ@res@left}%
                    {\ctikzvalof{tripoles/nmos/gate height}\pgf@circ@res@down}%
                    }{%
                    \pgfpoint
                    {\pgf@circ@res@right}%
                    {\ctikzvalof{tripoles/nmos/gate height}\pgf@circ@res@down}%
                }
                \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
            \fi
        \endpgfscope
    \fi

    \ifpgf@circuit@bpt@drawgate
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/nmos/gate width}\pgf@circ@res@left}
        {\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgfusepath{draw}
    \fi

    \ifpgf@circuit@bpt@drawbulk % added by Burak Kelleci
        \pgfpathmoveto{\pgfpoint{\ctikzvalof{tripoles/nmos/base width}\pgf@circ@res@left}
                {\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}
                {\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgfusepath{draw}
    \fi
}

\pgfcircdeclaretransistor{pmos}{
        \anchor{inner up}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/pmos/gate height}\pgf@y
        }
        \anchor{inner down}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/pmos/gate height}\pgf@y
        }
    }{%
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/pmos/gate height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint
        {\ctikzvalof{tripoles/pmos/base width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/pmos/gate height}\pgf@circ@res@up}}
    \pgfusepath{draw}

    \ifpgf@circuit@mos@arrows
        \pgfscope
            \ifpgf@circuit@trans@arrowatend
                \pgftransformshift{\pgfpoint
                    {\ctikzvalof{tripoles/pmos/base width}\pgf@circ@res@left}%
                    {\ctikzvalof{tripoles/pmos/gate height}\pgf@circ@res@up}%
                }
                \pgftransformrotate{180}
                \pgfnode{trarrow}{tip}{}{}{\pgfusepath{stroke}}
            \else
                \pgfslopedattimetrue
                \pgfallowupsidedownattimetrue
                \pgfresetnontranslationattimefalse
                \pgftransformlineattime{\ctikzvalof{tripoles/pmos/arrow pos}}{%
                    \pgfpoint%
                    {\pgf@circ@res@right}%
                    {\ctikzvalof{tripoles/pmos/gate height}\pgf@circ@res@up}%
                    }{%
                    \pgfpoint
                    {\ctikzvalof{tripoles/pmos/gate width}\pgf@circ@res@left}%
                    {\ctikzvalof{tripoles/pmos/gate height}\pgf@circ@res@up}%
                }
                \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
            \fi
        \endpgfscope
    \fi

    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/pmos/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/pmos/base height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/pmos/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/pmos/base height}\pgf@circ@res@down}}
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/pmos/gate width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/pmos/gate height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/pmos/gate width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/pmos/gate height}\pgf@circ@res@down}}
        \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint
        {\ctikzvalof{tripoles/pmos/base width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/pmos/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/pmos/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}


    \pgfusepath{draw}
    \ifpgf@circuit@bpt@drawgate
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/pmos/gate width}\pgf@circ@res@left}
        {\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgfusepath{draw}
    \fi

    \ifpgf@circuit@bpt@drawbulk % added by Burak Kelleci
        \pgfpathmoveto{\pgfpoint{\ctikzvalof{tripoles/pmos/base width}\pgf@circ@res@left}
                {\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}
                {\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgfusepath{draw}
    \fi

    \ifpgf@circuit@pmos@nocircle\else
        % we are not scaling the circle with the MOS --- I think it's better to have it
        % coherent with the poles/nodes of the rest of the circuit.
        \pgfpathcircle{\pgfpoint
            {\ctikzvalof{tripoles/pmos/gate width}\pgf@circ@res@left - \ctikzvalof{nodes width}*\pgf@circ@Rlen}
        {\pgf@circ@res@up+\pgf@circ@res@down}}{\ctikzvalof{nodes width}*\pgf@circ@Rlen}
        \ifpgf@circuit@pmos@emptycircle
            \pgfsetfillcolor{white}
        \fi
        \pgfusepath{draw,fill}
    \fi
}

%% HEMT FET Transistor
\pgfcircdeclaretransistor{hemt}{
        \anchor{inner up}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/hemt/gate height}\pgf@y
        }
        \anchor{inner down}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/hemt/gate height}\pgf@y
        }
    }{%
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/hemt/gate height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint
        {\ctikzvalof{tripoles/hemt/base width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/hemt/gate height}\pgf@circ@res@up}}

    \pgfpathmoveto{\pgfpoint
        {\ctikzvalof{tripoles/hemt/base width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/hemt/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/hemt/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfusepath{draw}

    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/hemt/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/hemt/base height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/hemt/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/hemt/base height}\pgf@circ@res@down}}
        \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint
        {\ctikzvalof{tripoles/hemt/base width}\pgf@circ@res@left}
    {\pgf@circ@res@up+\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgf@circ@res@up+\pgf@circ@res@down}}
    \pgfusepath{draw}
}

\long\def\drawfetcore#1{
    \pgftransformationadjustments
    %top connection
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/#1/gate height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint
        {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/#1/gate height}\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@up}}
        \ifpgf@circuit@trans@depletiontype
            \pgfpathlineto{\pgfpoint
                {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@down}}
        \else

            \pgfpathlineto{\pgfpoint
                {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@up*0.45}}
            \pgfpathmoveto{\pgfpoint
                {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@up*0.25}}
            \pgfpathlineto{\pgfpoint
                {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@down*0.25}}
            \pgfpathmoveto{\pgfpoint
                {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/nfet/base height}\pgf@circ@res@down*0.45}}
            \pgfpathlineto{\pgfpoint
                {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/#1/base height}\pgf@circ@res@down}}
        \fi
        \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope
    %Bulk connection line
    \pgfpathmoveto{\pgfpoint
        {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
    {\pgf@circ@res@up+\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}
    {\pgf@circ@res@up+\pgf@circ@res@down}}

    %bottom connection
    \pgfpathmoveto{\pgfpoint
        {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/#1/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/#1/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfusepath{draw}

    %draw thick gate line
    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/#1/gate width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/#1/gate height}\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/#1/gate width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/#1/gate height}\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
        \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope

    % arrows
    \pgfscope
        \pgfslopedattimetrue
        \pgfallowupsidedownattimetrue
        \pgfresetnontranslationattimefalse
        \ifpgf@circuit@trans@arrowatend
                \ifpgf@circuit@trans@ntype
                    \edef\@@anchor{tip}
                    \edef\@@pos{1.0}
                \else
                    \edef\@@anchor{btip}
                    \edef\@@pos{0.0}
                \fi
        \else
            \edef\@@anchor{center}\edef\@@pos{0.6}
        \fi
        \pgftransformlineattime{\@@pos}{%
            \pgfpoint
            {\pgf@circ@res@right}%
            {\pgf@circ@res@up+\pgf@circ@res@down}%
            }{%
            \pgfpoint%
            {\ctikzvalof{tripoles/#1/base width}\pgf@circ@res@left}%
            {\pgf@circ@res@up+\pgf@circ@res@down}%
        }
        \ifpgf@circuit@trans@ntype
        \else
            \pgftransformrotate{180}
        \fi
        \pgfnode{trarrow}{\@@anchor}{}{}{\pgfusepath{stroke}}
    \endpgfscope

% GATE CONNECTION
\ifpgf@circuit@bpt@drawgate
    \ifpgf@circuit@trans@ntype
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/#1/gate width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/#1/conn height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\ctikzvalof{tripoles/#1/conn height}\pgf@circ@res@down}}
    \else
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/#1/gate width}\pgf@circ@res@left}
        {-\ctikzvalof{tripoles/#1/conn height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{-\ctikzvalof{tripoles/#1/conn height}\pgf@circ@res@down}}
    \fi
    \pgfusepath{draw}
\fi

}

\long\def\pgfdeclaretransistorwrapperaddbulk#1#2#3
{\pgfcircdeclaretransistor{#1}{
        \anchor{bulk}{\left\pgf@x=0pt}
        \anchor{B}{\left\pgf@x=0pt}%override Base anchor from npn&igbt
        \anchor{inner up}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/#1/gate height}\pgf@y
        }
        \anchor{inner down}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/#1/gate height}\pgf@y
        }
        #2
    }
    {#3}
}

\pgfdeclaretransistorwrapperaddbulk{nfet}{}{%
	\pgf@circuit@trans@depletiontypefalse
	\drawfetcore{nfet}
}

\pgfdeclaretransistorwrapperaddbulk{pfet}{}{%
    \pgf@circuit@trans@depletiontypefalse
    \drawfetcore{pfet}
}

% N-CHANNEL IGFET ENHANCEMENT TYPE
\pgfdeclaretransistorwrapperaddbulk{nigfete}{}{%
    \pgf@circuit@trans@depletiontypefalse
    \drawfetcore{nigfete}

    % SOURCE CONNECTION
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}

    % SOLDER DOT at source-bulk connection
    \ifpgf@circuit@fet@solderdot
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
            \ctikzvalof{tripoles/nigfete/gate height}\pgf@circ@res@down}}
            \pgfnode{circ}{center}{}{}{}
    \endpgfscope{}
\fi
}

% N-CHANNEL IGFET ENHANCEMENT TYPE with Bulk connector
\pgfdeclaretransistorwrapperaddbulk{nigfetebulk}{}{%
    \pgf@circuit@trans@depletiontypefalse
    \drawfetcore{nigfetebulk}
    % SOLDER DOT at source-bulk connection
    \ifpgf@circuit@fet@solderdot
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
            \ctikzvalof{tripoles/nigfetebulk/gate height}\pgf@circ@res@down}}
            \pgfnode{circ}{center}{}{}{}
        \endpgfscope{}
    \fi
}

% N-CHANNEL IGFET DEPLETION TYPE
\pgfdeclaretransistorwrapperaddbulk{nigfetd}{}{%
    \pgf@circuit@trans@depletiontypetrue
    \drawfetcore{nigfetd}

    % SOURCE CONNECTION
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}

    % SOLDER DOT at source-bulk connection
    \ifpgf@circuit@fet@solderdot
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
            \ctikzvalof{tripoles/nigfete/gate height}\pgf@circ@res@down}}
            \pgfnode{circ}{center}{}{}{}
        \endpgfscope{}
    \fi
}

% P-CHANNEL IGFET ENHANCEMENT TYPE
\pgfdeclaretransistorwrapperaddbulk{pigfete}{}{%
    \pgf@circuit@trans@depletiontypefalse
    \drawfetcore{pigfete}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}

    % SOURCE CONNECTION
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}


    % SOLDER DOT at source-bulk connection
    \ifpgf@circuit@fet@solderdot
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
            \ctikzvalof{tripoles/pigfete/gate height}\pgf@circ@res@up}}
            \pgfnode{circ}{center}{}{}{}
        \endpgfscope
    \fi
}

% P-CHANNEL IGFET ENHANCEMENT TYPE with bulk connector
\pgfdeclaretransistorwrapperaddbulk{pigfetebulk}{}{%
    \pgf@circuit@trans@depletiontypefalse
    \drawfetcore{pigfetebulk}
}

% P-CHANNEL IGFET DEPLETION TYPE
\pgfdeclaretransistorwrapperaddbulk{pigfetd}{}{%
    \pgf@circuit@trans@depletiontypetrue
    \drawfetcore{pigfetd}

    % SOURCE CONNECTION
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}


    % SOLDER DOT at source-bulk connection
    \ifpgf@circuit@fet@solderdot
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
            \ctikzvalof{tripoles/nigfete/gate height}\pgf@circ@res@up}}
            \pgfnode{circ}{center}{}{}{}
        \endpgfscope{}
    \fi
}

\pgfcircdeclaretransistor{njfet}{
        \anchor{inner up}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/njfet/gate height 2}\pgf@y
        }
        \anchor{inner down}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/njfet/gate height 2}\pgf@y
        }
    }{%
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/njfet/gate height 2}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint
        {\ctikzvalof{tripoles/njfet/gate width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/njfet/gate height 2}\pgf@circ@res@up}}

    \pgfpathmoveto{\pgfpoint
        {\ctikzvalof{tripoles/njfet/gate width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/njfet/gate height 2}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/njfet/gate height 2}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfusepath{draw}

    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/njfet/gate width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/njfet/gate height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/njfet/gate width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/njfet/gate height}\pgf@circ@res@down}}
        \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope

    % arrow
    \pgfscope
        \pgfslopedattimetrue
        \pgfallowupsidedownattimetrue
        \pgfresetnontranslationattimefalse
        \ifpgf@circuit@trans@arrowatend
            \edef\@@anchor{tip}\edef\@@pos{1.0}
        \else
            \edef\@@anchor{center}\edef\@@pos{0.6}
        \fi
        \pgftransformlineattime{\@@pos}{%
            \pgfpoint{\pgf@circ@res@left}%
            {\ctikzvalof{tripoles/njfet/gate height 2}\pgf@circ@res@down}%
            }{%
            \pgfpoint
            {\ctikzvalof{tripoles/njfet/gate width}\pgf@circ@res@left}%
            {\ctikzvalof{tripoles/njfet/gate height 2}\pgf@circ@res@down}%
        }
        \pgfnode{trarrow}{\@@anchor}{}{}{\pgfusepath{stroke}}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint
        {\ctikzvalof{tripoles/njfet/gate width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/njfet/gate height 2}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}
    {\ctikzvalof{tripoles/njfet/gate height 2}\pgf@circ@res@down}}
    \pgfusepath{draw}
}

\pgfcircdeclaretransistor{pjfet}{
        \anchor{inner up}{
            \northeast
            \pgf@y=\ctikzvalof{tripoles/pjfet/gate height 2}\pgf@y
        }
        \anchor{inner down}{
            \northeast
            \pgf@y=-\ctikzvalof{tripoles/pjfet/gate height 2}\pgf@y
        }
    }{%
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/pjfet/gate height 2}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint
        {\ctikzvalof{tripoles/pjfet/gate width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/pjfet/gate height 2}\pgf@circ@res@up}}

    \pgfpathmoveto{\pgfpoint
        {\ctikzvalof{tripoles/pjfet/gate width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/pjfet/gate height 2}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/pjfet/gate height 2}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfusepath{draw}

    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/pjfet/gate width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/pjfet/gate height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/pjfet/gate width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/pjfet/gate height}\pgf@circ@res@down}}
        \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope

    \pgfscope
        \pgfslopedattimetrue
        \pgfallowupsidedownattimetrue
        \pgfresetnontranslationattimefalse
        \ifpgf@circuit@trans@arrowatend
            \edef\@@anchor{btip}\edef\@@pos{1.0}
        \else
            \edef\@@anchor{center}\edef\@@pos{0.4}
        \fi
        \pgftransformlineattime{\@@pos}{%
            \pgfpoint%
            {\ctikzvalof{tripoles/pjfet/gate width}\pgf@circ@res@left}%
            {\ctikzvalof{tripoles/pjfet/gate height 2}\pgf@circ@res@up}%
            }{%
            \pgfpoint{\pgf@circ@res@left}%
            {\ctikzvalof{tripoles/pjfet/gate height 2}\pgf@circ@res@up}%
        }
        \pgfnode{trarrow}{\@@anchor}{}{}{\pgfusepath{stroke}}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint
        {\ctikzvalof{tripoles/pjfet/gate width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/pjfet/gate height 2}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}
    {\ctikzvalof{tripoles/pjfet/gate height 2}\pgf@circ@res@up}}
    \pgfusepath{draw}
}

\pgfdeclaretransistorwrapperaddbulk{isfet}{}{%
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    % DRAIN CONNECTION
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/isfet/gate height}\pgf@circ@res@up}}
    % DRAIN
    \pgfpathlineto{\pgfpoint
        {\ctikzvalof{tripoles/isfet/base width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/isfet/gate height}\pgf@circ@res@up}}
    \pgfusepath{draw}

    % GATE, DEPLETION TYPE
    \pgfscope %% added
        \pgfpathmoveto{\pgfpoint
            {\ctikzvalof{tripoles/isfet/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/isfet/base height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/isfet/base width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/isfet/base height}\pgf@circ@res@down}}
        \pgf@circ@setlinewidth{tripoles}{\pgflinewidth} %% added
        \pgfusepath{draw} %% added
    \endpgfscope %% added

    % BULK
    \pgfpathmoveto{\pgfpoint
        {\ctikzvalof{tripoles/isfet/base width}\pgf@circ@res@left}
    {\pgf@circ@res@up+\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+.5\pgflinewidth}
    {\pgf@circ@res@up+\pgf@circ@res@down}}

    % SOURCE
    \pgfpathmoveto{\pgfpoint
        {\ctikzvalof{tripoles/isfet/base width}\pgf@circ@res@left}
    {\ctikzvalof{tripoles/isfet/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\ctikzvalof{tripoles/isfet/gate height}\pgf@circ@res@down}}
    % SOURCE CONNECTION
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfusepath{draw}

    % SOLDER DOT at source-bulk connection
    \ifpgf@circuit@fet@solderdot
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
            \ctikzvalof{tripoles/nigfete/gate height}\pgf@circ@res@down}}
            \pgfnode{circ}{center}{}{}{}
        \endpgfscope{}
    \fi
    % ARROW
    \pgfscope
        \pgfslopedattimetrue
        \pgfallowupsidedownattimetrue
        \pgfresetnontranslationattimefalse
        \ifpgf@circuit@trans@arrowatend
            \edef\@@anchor{tip}\edef\@@pos{1.0}
        \else
            \edef\@@anchor{center}\edef\@@pos{0.6}
        \fi
        \pgftransformlineattime{\@@pos}{%
            \pgfpoint
            {\pgf@circ@res@right}%
            {\pgf@circ@res@up+\pgf@circ@res@down}%
            }{%
            \pgfpoint%
            {\ctikzvalof{tripoles/isfet/base width}\pgf@circ@res@left}%
            {\pgf@circ@res@up+\pgf@circ@res@down}%
        }
        \pgfnode{trarrow}{\@@anchor}{}{}{\pgfusepath{stroke}}
    \endpgfscope
    \pgfusepath{draw}

    % Wavy lines
    \pgfscope
        \pgfpathmoveto{\pgfpoint{-\ctikzvalof{tripoles/isfet/waves x sep}\pgf@circ@res@up}{\ctikzvalof{tripoles/isfet/waves y sep}\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{-\ctikzvalof{tripoles/isfet/wave width}\pgf@circ@res@up}{-\ctikzvalof{tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{-\ctikzvalof{tripoles/isfet/wave width}\pgf@circ@res@up}{\ctikzvalof{tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{-\ctikzvalof{tripoles/isfet/wave width}\pgf@circ@res@up}{\ctikzvalof{tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{-\ctikzvalof{tripoles/isfet/wave width}\pgf@circ@res@up}{-\ctikzvalof{tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfusepath{draw}

        \pgfpathmoveto{\pgfpoint{-\ctikzvalof{tripoles/isfet/waves x sep}\pgf@circ@res@up}{0cm}}
        \pgfpathsine{\pgfpoint{-\ctikzvalof{tripoles/isfet/wave width}\pgf@circ@res@up}{-\ctikzvalof{tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{-\ctikzvalof{tripoles/isfet/wave width}\pgf@circ@res@up}{\ctikzvalof{tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{-\ctikzvalof{tripoles/isfet/wave width}\pgf@circ@res@up}{\ctikzvalof{tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{-\ctikzvalof{tripoles/isfet/wave width}\pgf@circ@res@up}{-\ctikzvalof{tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfusepath{draw}

        \pgfpathmoveto{\pgfpoint{-\ctikzvalof{tripoles/isfet/waves x sep}\pgf@circ@res@up}{-\ctikzvalof{tripoles/isfet/waves y sep}\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{-\ctikzvalof{tripoles/isfet/wave width}\pgf@circ@res@up}{-\ctikzvalof{tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{-\ctikzvalof{tripoles/isfet/wave width}\pgf@circ@res@up}{\ctikzvalof{tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{-\ctikzvalof{tripoles/isfet/wave width}\pgf@circ@res@up}{\ctikzvalof{tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{-\ctikzvalof{tripoles/isfet/wave width}\pgf@circ@res@up}{-\ctikzvalof{tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

% end of transistors

%%%%%%%%%%%%%
%% Switches
%%%%%%%%%%%%%

\pgfcircdeclarebipole{
	\anchor{out 1}{
		\northeast
		\pgf@y=0cm
	}
	\anchor{out 2}{
		\northeast
		\pgf@y=.8\pgf@y
	}
}
{\ctikzvalof{tripoles/toggleswitch/height 2}}
{toggleswitch}
{\ctikzvalof{tripoles/toggleswitch/height}}
{\ctikzvalof{tripoles/toggleswitch/width}}
{

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.3\pgf@circ@res@left}{0pt}}
    \pgfusepath{draw}
    \pgfscope
        \pgfpathmoveto{\pgfpoint{.3\pgf@circ@res@left}{0pt}}
        \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{.5\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{0}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{.15\pgf@circ@res@up}}
    \pgfusepath{draw}


    \pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetdash{{.08\pgf@circ@res@up}{.04\pgf@circ@res@up}{.7\pgf@circ@res@up}{.04\pgf@circ@res@up}{.8\pgf@circ@res@up}}{0cm}
    \pgfpathmoveto{\pgfpoint{0}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0}{.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@left}{.6\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0}{.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0}{.2\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfsetdash{}{0cm}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% operational and instrumentation amplifiers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfdeclareshape{op amp}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{amplifiers}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/op amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/op amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {\left
        \pgf@x = \ctikzvalof{tripoles/op amp/port width}\pgf@x
    }
    \savedanchor\inOneFixed{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/op amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/op amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/op amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/op amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/op amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/op amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \savedanchor\up{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/op amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/op amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \ctikzvalof{tripoles/op amp/up pos}}{
            \pgfpoint{
            \ctikzvalof{tripoles/op amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{\ctikzvalof{tripoles/op amp/port width}\pgf@circ@res@right}{0pt}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }

    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }

    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@scaled@Rlen=\scaledRlen

				% Triangle
        \pgfscope
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgftransformxshift{\ctikzvalof{tripoles/op amp/port width}\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=\ctikzvalof{tripoles/op amp/port width}\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

				% Negative input terminal
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\ctikzvalof{tripoles/op amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/op amp/port width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/op amp/input height}\pgf@circ@res@up}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/op amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/op amp/input height}\pgf@circ@res@up}]{\ctikzvalof{tripoles/op amp/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}

				% Positive input terminal
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\ctikzvalof{tripoles/op amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/op amp/port width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/op amp/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/op amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/op amp/input height}\pgf@circ@res@down}]{\ctikzvalof{tripoles/op amp/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}

        % Output terminal
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/op amp/port width}\pgf@circ@res@right}{0pt}}
        \pgfsetrectcap
        \pgfusepath{draw}
    }
}

% Op amp shape as in european standard EN 60617
\pgfdeclareshape{en amp}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{amplifiers}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/en amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/en amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {
        \left
        \pgf@x = \ctikzvalof{tripoles/en amp/port width}\pgf@x
    }
    \savedanchor\inOneFixed{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/en amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/en amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/en amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/en amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/en amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/en amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \anchor{up}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{down}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@scaled@Rlen=\scaledRlen

        \pgfscope
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgfpathmoveto{\pgfpoint{\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@left}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@right}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\ctikzvalof{tripoles/en amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/en amp/input height}\pgf@circ@res@up}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/en amp/input height}\pgf@circ@res@up}]{\ctikzvalof{tripoles/en amp/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}

        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\ctikzvalof{tripoles/en amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/en amp/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/en amp/input height}\pgf@circ@res@down}]{\ctikzvalof{tripoles/en amp/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
        \pgfsetrectcap
        \pgfusepath{draw}


        \pgftext[top, y=-.5ex, at=\pgfpoint{0pt}{\pgf@circ@res@up}]{\hbox{\ctikzvalof{tripoles/en amp/font2}\ctikzvalof{tripoles/en amp/text}}}
        % \pgftext[top, y=-.5ex, at=\pgfpoint{0pt}{\pgf@circ@res@up}]{\ctikzvalof{tripoles/en amp/font2}$\mathstrut{\triangleright}\,\mathrm{A}$}
    }
}

% Fully differential output op amp
% Contributed by Kristofer M. Monisit
\pgfdeclareshape{fd op amp}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{amplifiers}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/fd op amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd op amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \savedanchor\outline{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/fd op amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd op amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    \ifpgf@circuit@oa@oplusup\else\pgf@y=-\pgf@y\fi
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y\pgf@x=0pt\relax
    }
    \anchor{north}{
        \northwest\pgf@x=0pt\relax
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \savedanchor\inOneFixed{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/fd op amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/fd op amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd op amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/fd op amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/fd op amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd op amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \savedanchor\up{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/fd op amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd op amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \ctikzvalof{tripoles/fd op amp/up pos}}{
            \pgfpoint{
            \ctikzvalof{tripoles/fd op amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{\ctikzvalof{tripoles/fd op amp/port width}\pgf@circ@res@right}{0pt}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    \anchor{out up}{
        \northwest
        \pgf@y=\ctikzvalof{tripoles/fd op amp/output height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd op amp/port width}\pgf@x
    }
    \anchor{out down}{
        \northwest
        \pgf@y=-\ctikzvalof{tripoles/fd op amp/output height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd op amp/port width}\pgf@x
    }
    \anchor{out +}{
        \outline
        \pgf@y=\ctikzvalof{tripoles/fd op amp/output height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd op amp/port width}\pgf@x
    }
    \anchor{out -}{
        \outline
        \pgf@y=-\ctikzvalof{tripoles/fd op amp/output height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd op amp/port width}\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\ctikzvalof{tripoles/fd op amp/port width}\pgf@x
    }
    \anchor{out}{% should not be used
        \left
        \pgf@x=-\ctikzvalof{tripoles/fd op amp/port width}\pgf@x
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\ctikzvalof{tripoles/fd op amp/port width}\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\ctikzvalof{tripoles/fd op amp/port width}\pgf@x \pgf@y=-\pgf@y }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@scaled@Rlen=\scaledRlen

        % Triangle
        % Includes output terminals to ensure that diagonal joins are properly displayed
        \pgfscope
            \pgf@circ@setlinewidth{quadpoles}{\pgflinewidth}
            \pgftransformxshift{\ctikzvalof{tripoles/fd op amp/port width}\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=\ctikzvalof{tripoles/fd op amp/port width}\pgf@circ@res@step

            % Initial point (right vertex)
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}

            % Negative output terminal
            \pgfpathlineto{\pgfpointlineattime{\ctikzvalof{tripoles/fd op amp/output height}}{\pgfpoint{\pgf@circ@res@step}{0pt}}{\pgfpoint{0pt}{\pgf@circ@res@up}}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{\ctikzvalof{tripoles/fd op amp/output height}\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpointlineattime{\ctikzvalof{tripoles/fd op amp/output height}}{\pgfpoint{\pgf@circ@res@step}{0pt}}{\pgfpoint{0pt}{\pgf@circ@res@up}}}

            % Top vertex
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}

            % Bottom vertex
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}

            % Positive output terminal
            \pgfpathlineto{\pgfpointlineattime{\ctikzvalof{tripoles/fd op amp/output height}}{\pgfpoint{\pgf@circ@res@step}{0pt}}{\pgfpoint{0pt}{\pgf@circ@res@down}}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{\ctikzvalof{tripoles/fd op amp/output height}\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpointlineattime{\ctikzvalof{tripoles/fd op amp/output height}}{\pgfpoint{\pgf@circ@res@step}{0pt}}{\pgfpoint{0pt}{\pgf@circ@res@down}}}

            % Right vertex
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}

            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        % Negative input terminal
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\ctikzvalof{tripoles/fd op amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/fd op amp/port width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/fd op amp/input height}\pgf@circ@res@up}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/fd op amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/fd op amp/input height}\pgf@circ@res@up}]{\ctikzvalof{tripoles/fd op amp/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}

        % Positive input terminal
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\ctikzvalof{tripoles/fd op amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/fd op amp/port width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/fd op amp/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/fd op amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/fd op amp/input height}\pgf@circ@res@down}]{\ctikzvalof{tripoles/fd op amp/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}

        % Negative output terminal label
        \pgftext[right, bottom, x=3pt, y=1pt, at=\pgfpoint{0pt}{0.425\pgf@circ@res@down}]{\ctikzvalof{tripoles/fd op amp/font} \ifpgf@circuit@oa@oplusup$-$\else$+$\fi}

        % Positive output terminal label
        \pgftext[right, top, x=3pt, y=-1pt, at=\pgfpoint{0pt}{0.425\pgf@circ@res@up}]{\ctikzvalof{tripoles/fd op amp/font} \ifpgf@circuit@oa@oplusup$+$\else$-$\fi}

        \pgfsetrectcap
        \pgfusepath{draw}
    }
}


% Instrumentation amplifier with differential output
\pgfdeclareshape{fd inst amp}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{amplifiers}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    % when tikz calls the anchor it wants the relative position in the lengths
    % \pgf@x  \pgf@y
    % \pgfpoint* functions set that variables
    % anchors are visible outside and run on use
    \anchor{center}{\pgfpointorigin}
    % savedanchors are internals and run on node creation (not use)
    % bounding-box top left
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/fd inst amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd inst amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{nw}{
        \northwest
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y\pgf@x=0pt\relax
    }
    \anchor{north}{
        \northwest\pgf@x=0pt\relax
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {\left
        \pgf@x = \ctikzvalof{tripoles/fd inst amp/port width}\pgf@x
    }
    \savedanchor\inOneFixed{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
          \pgf@y=\ctikzvalof{tripoles/fd inst amp/height}\pgf@circ@scaled@Rlen
          \pgf@y=.5\pgf@y
          \pgf@y=\ctikzvalof{tripoles/fd inst amp/input height}\pgf@y
          \pgf@x=-\ctikzvalof{tripoles/fd inst amp/width}\pgf@circ@scaled@Rlen
          \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/fd inst amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/fd inst amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd inst amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \savedanchor\up{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/fd inst amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd inst amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \ctikzvalof{tripoles/fd inst amp/up pos}}{
            \pgfpoint{
            \ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/fd inst amp/height 2}\pgf@circ@res@up}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    % reference voltage input anchors.
    \savedanchor\refv{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/fd inst amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd inst amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \ctikzvalof{tripoles/fd inst amp/refv pos}}{
            \pgfpoint{
            \ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/fd inst amp/height 2}\pgf@circ@res@up}}
    }
    % we need both because they are normally drawn under the amp, and if you
    % mirror it vertically you need them
    \anchor{refv up}{
        \refv
    }
    \anchor{refv down}{
        \refv
        \pgf@y=-\pgf@y
    }
    \savedanchor\outport{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/fd inst amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/fd inst amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd inst amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=-.5\pgf@x
        \ifpgf@circuit@oa@oplusup\else\pgf@y=-\pgf@y\fi
    }
    \anchor{out}{
        \outport
        \pgf@y=0pt
    }
    \anchor{out +}{
        \outport
    }
    \anchor{out -}{
        \outport
        \pgf@y=-\pgf@y
    }
    \savedanchor\outportfixed{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/fd inst amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/fd inst amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/fd inst amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=-.5\pgf@x
    }
    \anchor{out up}{
        \outportfixed
    }
    \anchor{out down}{
        \outportfixed
        \pgf@y=-\pgf@y
    }
    %
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    % let's start drawing the component
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        %
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@scaled@Rlen=\scaledRlen
        % main component, normally in thicker lines
        \pgfscope
            \newdimen\pgf@circ@res@right@double
						\pgf@circ@res@right@double=2\pgf@circ@res@right

            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgftransformxshift{\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@step
            %first point (near output)
            \pgfpathmoveto{\pgfpoint{\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@right@double}{0}}
            %from the exit to the top (short side)... (note that the .6 must be copied in \up and \refv anchors
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@right@double}{\ctikzvalof{tripoles/fd inst amp/height 2}\pgf@circ@res@up}}
            % and then to the input "front up", "down", to the output short side "down"
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@right@double}{\ctikzvalof{tripoles/fd inst amp/height 2}\pgf@circ@res@down}}
            % ...and close
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        % input terminal up
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\ctikzvalof{tripoles/fd inst amp/input height}\pgf@circ@res@up}}
        %
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/fd inst amp/input height}\pgf@circ@res@up}}
        %
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/fd inst amp/input height}\pgf@circ@res@up}]{\ctikzvalof{tripoles/fd inst amp/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}

        % input terminal down
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\ctikzvalof{tripoles/fd inst amp/input height}\pgf@circ@res@down}}
        %
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/fd inst amp/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/fd inst amp/input height}\pgf@circ@res@down}]{\ctikzvalof{tripoles/fd inst amp/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}

        % output leads down and up
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\ctikzvalof{tripoles/fd inst amp/output height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/fd inst amp/output height}\pgf@circ@res@down}} %
        \pgftext[right, at=\pgfpoint{\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/fd inst amp/output height}\pgf@circ@res@down}]{\ctikzvalof{tripoles/fd inst amp/font}\ifpgf@circuit@oa@oplusup$-\;$\else$+\;$\fi}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\ctikzvalof{tripoles/fd inst amp/output height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/fd inst amp/output height}\pgf@circ@res@up}} %
        \pgftext[right, at=\pgfpoint{\ctikzvalof{tripoles/fd inst amp/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/fd inst amp/output height}\pgf@circ@res@up}]{\ctikzvalof{tripoles/fd inst amp/font}\ifpgf@circuit@oa@oplusup$+\;$\else$-\;$\fi}
        %
        \pgfsetrectcap
        \pgfusepath{draw}
    }
}

% Transconductance amplifier (Transkonduktanzverstärker)
\pgfdeclareshape{gm amp}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{amplifiers}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/gm amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/gm amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {\left
        \pgf@x = \ctikzvalof{tripoles/op amp/port width}\pgf@x
    }
    \savedanchor\inOneFixed{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/gm amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/gm amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/gm amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/gm amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/gm amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/gm amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
        \savedanchor\up{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/gm amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/gm amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \ctikzvalof{tripoles/gm amp/up pos}}{
            \pgfpoint{
            \ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/gm amp/height 2}\pgf@circ@res@up}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }

    \anchor{text}{\northwest
        \pgf@x=\ctikzvalof{tripoles/op amp/port width}\pgf@x
    \pgfpoint{-.5\wd\pgfnodeparttextbox+.25\pgf@x}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@scaled@Rlen=\scaledRlen

        \pgfscope
            \newdimen\pgf@circ@res@right@double
						\pgf@circ@res@right@double=2\pgf@circ@res@right

            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgftransformxshift{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@step
            %Umrandung:
            \pgfpathmoveto{\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@right@double}{0}} %geändert startpunkt neu am ausgangsstrich
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@right@double}{\ctikzvalof{tripoles/gm amp/height 2}\pgf@circ@res@up}}%vom Ausgang nach oben
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}} %neu ecke links oben nach rechts oben
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}} %bei deneigängen runter
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@right@double}{\ctikzvalof{tripoles/gm amp/height 2}\pgf@circ@res@down}}%ecke links unten nach rechts unten
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\ctikzvalof{tripoles/gm amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/gm amp/input height}\pgf@circ@res@up}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/gm amp/input height}\pgf@circ@res@up}]{\ctikzvalof{tripoles/gm amp/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}


        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\ctikzvalof{tripoles/gm amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/gm amp/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/gm amp/input height}\pgf@circ@res@down}]{\ctikzvalof{tripoles/gm amp/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@right}{0pt}} %
        \pgfsetrectcap
        \pgfusepath{draw}

    }
}

% Instrumentation amplifier
\pgfdeclareshape{inst amp}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{amplifiers}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    % when tikz calls the anchor it wants the relative position in the lengths
    % \pgf@x  \pgf@y
    % \pgfpoint* functions set that variables
    % anchors are visible outside and run on use
    \anchor{center}{\pgfpointorigin}
    % savedanchors are internals and run on node creation (not use)
    % bounding-box top left
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/inst amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/inst amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{nw}{
        \northwest
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {\left
        \pgf@x = \ctikzvalof{tripoles/op amp/port width}\pgf@x
    }
    \savedanchor\inOneFixed{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
          \pgf@y=\ctikzvalof{tripoles/inst amp/height}\pgf@circ@scaled@Rlen
          \pgf@y=.5\pgf@y
          \pgf@y=\ctikzvalof{tripoles/inst amp/input height}\pgf@y
          \pgf@x=-\ctikzvalof{tripoles/inst amp/width}\pgf@circ@scaled@Rlen
          \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/inst amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/inst amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/inst amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \savedanchor\up{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/inst amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/inst amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \ctikzvalof{tripoles/inst amp/up pos}}{
            \pgfpoint{
            \ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{\ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/inst amp/height 2}\pgf@circ@res@up}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    % reference voltage input anchors.
    \savedanchor\refv{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/inst amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/inst amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \ctikzvalof{tripoles/inst amp/refv pos}}{
            \pgfpoint{
            \ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{\ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/inst amp/height 2}\pgf@circ@res@up}}
    }
    % we need both because they are normally drawn under the amp, and if you
    % mirror it vertically you need them
    \anchor{refv up}{
        \refv
    }
    \anchor{refv down}{
        \refv
        \pgf@y=-\pgf@y
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }

    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    % let's start drawing the component
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        %
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@scaled@Rlen=\scaledRlen

        % main component, normally in thicker lines
        \pgfscope
            \newdimen\pgf@circ@res@right@double
						\pgf@circ@res@right@double=2\pgf@circ@res@right

            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgftransformxshift{\ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=\ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@step
            %first point (near output)
            \pgfpathmoveto{\pgfpoint{\ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@right@double}{0}}
            %from the exit to the top (short side)... (note that the .6 must be copied in \up and \refv anchors
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@right@double}{\ctikzvalof{tripoles/inst amp/height 2}\pgf@circ@res@up}}
            % and then to the input "front up", "down", to the output short side "down"
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@right@double}{\ctikzvalof{tripoles/inst amp/height 2}\pgf@circ@res@down}}
            % ...and close
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        % Negative input terminal
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\ctikzvalof{tripoles/inst amp/input height}\pgf@circ@res@up}}
        %
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/inst amp/input height}\pgf@circ@res@up}}
        %
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/inst amp/input height}\pgf@circ@res@up}]{\ctikzvalof{tripoles/inst amp/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}

        % Positive input terminal
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\ctikzvalof{tripoles/inst amp/input height}\pgf@circ@res@down}}
        %
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/inst amp/input height}\pgf@circ@res@down}}
    \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/inst amp/input height}\pgf@circ@res@down}]{\ctikzvalof{tripoles/inst amp/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}

        % Output terminal
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/inst amp/port width}\pgf@circ@res@right}{0pt}} %
        %
        \pgfsetrectcap
        \pgfusepath{draw}
    }
}

% Instrumentation amplifier with terminals for gain resistance between inputs
\pgfdeclareshape{inst amp ra}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{amplifiers}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    % bounding-box top left
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/inst amp ra/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/inst amp ra/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{nw}{
        \northwest
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y\pgf@x=0pt\relax
    }
    \anchor{north}{
        \northwest\pgf@x=0pt\relax
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {\left
        \pgf@x = \ctikzvalof{tripoles/op amp/port width}\pgf@x
    }
    % inputs (+-)
    \savedanchor\inOneFixed{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
          \pgf@y=\ctikzvalof{tripoles/inst amp ra/height}\pgf@circ@scaled@Rlen
          \pgf@y=.5\pgf@y
          \pgf@y=\ctikzvalof{tripoles/inst amp ra/input height}\pgf@y
          \pgf@x=-\ctikzvalof{tripoles/inst amp ra/width}\pgf@circ@scaled@Rlen
          \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/inst amp ra/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/inst amp ra/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/inst amp ra/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    % R ampli anchors. They are by default at 20% more than R-length distance
    % you can change that with the `ra pos` key (use 0.5 for one-R).
    \savedanchor\raOneFixed{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
          \pgf@y=\ctikzvalof{tripoles/inst amp ra/height}\pgf@circ@scaled@Rlen
          \pgf@y=.5\pgf@y
          \pgf@y=\ctikzvalof{tripoles/inst amp ra/input height}\pgf@y
          \pgf@x=-\ctikzvalof{tripoles/inst amp ra/width}\pgf@circ@scaled@Rlen
          \pgf@x=.5\pgf@x
    }
    \anchor{ra up}{
        \inOneFixed
    }
    \anchor{ra down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\raOne{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\pgf@circ@scaled@Rlen
        \pgf@y=\ctikzvalof{tripoles/inst amp ra/ra pos}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/inst amp ra/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{ra-}{
        \raOne
    }
    \anchor{ra+}{
        \raOne
        \pgf@y=-\pgf@y
    }
    % power supplies
    \savedanchor\up{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/inst amp ra/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/inst amp ra/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \ctikzvalof{tripoles/inst amp ra/up pos}}{
            \pgfpoint{
            \ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/inst amp ra/height 2}\pgf@circ@res@up}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    % reference voltage input anchors.
    \savedanchor\refv{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/inst amp ra/height}\pgf@circ@scaled@Rlen
        \pgf@y=0.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/inst amp ra/width}\pgf@circ@scaled@Rlen
        \pgf@x=0.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \ctikzvalof{tripoles/inst amp ra/refv pos}}{
            \pgfpoint{
            \ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/inst amp ra/height 2}\pgf@circ@res@up}}
    }
    % we need both because they are normally drawn under the amp, and if you
    % mirror it vertically you need them
    \anchor{refv up}{
        \refv
    }
    \anchor{refv down}{
        \refv
        \pgf@y=-\pgf@y
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }

    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    % drawing of the component
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@scaled@Rlen=\scaledRlen

        \newdimen\pgf@circ@res@right@double
				\pgf@circ@res@right@double=2\pgf@circ@res@right

        % main component, normally in thicker lines
        \pgfscope
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgftransformxshift{\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@step
            %primer punto: la linea de salida (lado componente)
            \pgfpathmoveto{\pgfpoint{\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@right@double}{0}}
            %from the exit to the top (short side)... (note that the .6 must be copied in \up anchor
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@right@double}{\ctikzvalof{tripoles/inst amp ra/height 2}\pgf@circ@res@up}}
            % and then to the input "front up", "down", to the output short side "down"
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@right@double}{\ctikzvalof{tripoles/inst amp ra/height 2}\pgf@circ@res@down}}
            % ...and close
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        % ra terminal -
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\ctikzvalof{tripoles/inst amp ra/ra pos}\pgf@circ@Rlen}}
        %
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/inst amp ra/ra pos}\pgf@circ@Rlen}}
        % ra terminal +
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {-\ctikzvalof{tripoles/inst amp ra/ra pos}\pgf@circ@Rlen}}
        %
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@left}
        {-\ctikzvalof{tripoles/inst amp ra/ra pos}\pgf@circ@Rlen}}

        % Negative input terminal
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\ctikzvalof{tripoles/inst amp ra/input height}\pgf@circ@res@up}}
        %
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/inst amp ra/input height}\pgf@circ@res@up}}
        %
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/inst amp ra/input height}\pgf@circ@res@up}]{\ctikzvalof{tripoles/inst amp ra/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}

        % Positive input terminal
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\ctikzvalof{tripoles/inst amp ra/input height}\pgf@circ@res@down}}
        %
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/inst amp ra/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/inst amp ra/input height}\pgf@circ@res@down}]{\ctikzvalof{tripoles/inst amp ra/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}

        % Output terminal
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/inst amp ra/port width}\pgf@circ@res@right}{0pt}} %
        %
        \pgfsetrectcap
        \pgfusepath{draw}
    }
}

% Buffer
% Contributed by Danilo Piazzalunga
\pgfdeclareshape{buffer}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{amplifiers}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{bipoles/buffer/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{bipoles/buffer/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }

    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgfscope
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}

        \pgfusepath{draw}
    }
}

% plain amplifier, no symbols
\pgfdeclareshape{plain amp}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{amplifiers}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/plain amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/plain amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \savedanchor\inOne{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/plain amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/plain amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/plain amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \anchor{in up}{
        \inOne
    }
    \anchor{in down}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \savedanchor\up{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/plain amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/plain amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \ctikzvalof{tripoles/plain amp/up pos}}{
            \pgfpoint{
            \ctikzvalof{tripoles/plain amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{\ctikzvalof{tripoles/plain amp/port width}\pgf@circ@res@right}{0pt}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }

    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgfscope
            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgftransformxshift{\ctikzvalof{tripoles/plain amp/port width}\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=\ctikzvalof{tripoles/plain amp/port width}\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\ctikzvalof{tripoles/plain amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/plain amp/port width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/plain amp/input height}\pgf@circ@res@up}}


        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\ctikzvalof{tripoles/plain amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/plain amp/port width}\pgf@circ@res@left}
        {\ctikzvalof{tripoles/plain amp/input height}\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/plain amp/port width}\pgf@circ@res@right}{0pt}}

        \pgfusepath{draw}
    }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% electromechanical device (motor/generator)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfdeclareshape{elmech}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{electromechanicals}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor\northwest{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/elmech/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/elmech/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{text}{
        \pgfpointorigin
        \advance \pgf@x by -.5\wd\pgfnodeparttextbox
        \advance \pgf@y by -.5\ht\pgfnodeparttextbox
    }
    \anchor{left}{%
        \northwest
        \pgf@y=0pt
    }
    \anchor{right}{%
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{top}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{pathstart}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{pathend}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{bottom}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{center}{
        \pgf@y=0pt
        \pgf@x=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchorborder{%
        \@tempdima=\pgf@x\@tempdimb=\pgf@y
        \northwest\pgf@circ@res@other=-\pgf@x
        \pgfpointborderellipse{\pgfqpoint{\@tempdima}{\@tempdimb}}{\pgfqpoint{\pgf@circ@res@other}{\pgf@circ@res@other}}
    }
    \anchor{block north west}{\northwest\pgf@x=0.5\pgf@x}
    \anchor{block south west}{\northwest\pgf@x=0.5\pgf@x\pgf@y=-\pgf@y}
    \anchor{block north east}{\northwest\pgf@x=-0.5\pgf@x}
    \anchor{block south east}{\northwest\pgf@x=-0.5\pgf@x\pgf@y=-\pgf@y}
    \anchor{block up right}{
        \northwest
        % remember that pgf@x is negative
        % center of the block is at 0.5*H+W*cos(30)/2
        \pgf@y=\dimexpr0.5\pgf@y - 0.433\pgf@x\relax
        \pgf@x=-0.5\pgf@x
    }
    \anchor{block up left}{
        \northwest
        % remember that pgf@x is negative
        % center of the block is at 0.5*H+W*cos(30)/2
        \pgf@y=\dimexpr0.5\pgf@y - 0.433\pgf@x\relax
        \pgf@x=0.5\pgf@x
    }
    \anchor{block down right}{
        \northwest
        % remember that pgf@x is negative
        % center of the block is at 0.5*H+W*cos(30)/2
        \pgf@y=\dimexpr0.5\pgf@y - 0.433\pgf@x\relax
        \pgf@y=-\pgf@y
        \pgf@x=-0.5\pgf@x
    }
    \anchor{block down left}{
        \northwest
        % remember that pgf@x is negative
        % center of the block is at 0.5*H+W*cos(30)/2
        \pgf@y=\dimexpr0.5\pgf@y - 0.433\pgf@x\relax
        \pgf@y=-\pgf@y
        \pgf@x=0.5\pgf@x
    }
    \behindbackgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step=\ctikzvalof{tripoles/elmech/width}\pgf@circ@scaled@Rlen
        \pgf@circ@res@up=\ctikzvalof{tripoles/elmech/height}\pgf@circ@scaled@Rlen
        \pgfscope
            \pgfstartlinewidth=\pgflinewidth
            \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            \pgfscope % clip the bar: whole size minus the circle
                \pgfpathrectanglecorners{\pgfpoint{-.5\pgf@circ@res@step}{-.5\pgf@circ@res@up}}{\pgfpoint{.5\pgf@circ@res@step}{.5\pgf@circ@res@up}}
                \pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
                \pgfseteorule
                \pgfusepath{clip}
                \pgfpathrectangle{\pgfpoint{-.25\pgf@circ@res@step}{-.5\pgf@circ@res@up}}{\pgfpoint{.5\pgf@circ@res@step}{\pgf@circ@res@up}}
                \pgfsetfillcolor{\ctikzvalof{color}}
                \pgfusepath{fill, draw}
            \endpgfscope
            \pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
            \ifx\tikz@fillcolor\pgfutil@empty
                % set the default fill color to white
                \pgfsetfillcolor{white}
                % ...but override it if the class is defined!
                \pgf@circ@setifdefinedfill{draw, fill}{draw, fill}
            \else
                \pgfsetfillcolor{\tikz@fillcolor}
                \pgfusepath{draw, fill}
            \fi
        \endpgfscope
    }
}

%%%%%%%%%%%%%%%%%%%
%% Magnetron
%%%%%%%%%%%%%%%%%%%

\pgfdeclareshape{magnetron}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{tubes}}  % class of these components
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \savedanchor\northwest{
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/magnetron/width}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/magnetron/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{anode}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{cathode1}{
        \northwest
        \pgf@circ@res@step=\pgf@y
        \pgfmathparse{cos(105)}
        \pgf@x=\pgfmathresult\pgf@circ@res@step
        \pgfmathparse{sin(105)}
        \pgf@y=\pgfmathresult\pgf@circ@res@step
        %\pgfpointorigin
        %\pgfpathmoveto{\pgfpointpolar{105}{\pgf@circ@res@step}}%not working in a scaled tikzpicture
    }
    \anchor{cathode2}{
        \northwest
        \pgf@circ@res@step=\pgf@y
        \pgfmathparse{cos(75)}
        \pgf@x=\pgfmathresult\pgf@circ@res@step
        \pgfmathparse{sin(75)}
        \pgf@y=\pgfmathresult\pgf@circ@res@step
        %\pgfpointorigin
        %\pgfpathmoveto{\pgfpointpolar{75}{\pgf@circ@res@step}}%not working in a scaled tikzpicture
    }
    \anchor{text}{
        \pgfpointorigin
        \advance \pgf@x by -.5\wd\pgfnodeparttextbox
        \advance \pgf@y by -.5\ht\pgfnodeparttextbox
    }
    \anchor{left}{%
        \northwest
        \pgf@y=0pt
    }
    \anchor{right}{%
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{top}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{pathstart}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{pathend}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{bottom}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{center}{
        \pgf@y=0pt
        \pgf@x=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}
        \pgf@circ@scaled@Rlen=\scaledRlen
        \pgf@circ@res@step=\ctikzvalof{tripoles/magnetron/width}\pgf@circ@scaled@Rlen
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfmathsetlength{\pgf@circ@res@other}{sin(15)*\pgf@circ@res@up}

        \pgfscope
            \pgfstartlinewidth=\pgflinewidth
            \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
            %create outer circle
            \pgfpathcircle{\pgfpoint{0}{0}} {\pgf@circ@res@right}
            \pgf@circ@draworfill
            %create chambers
            \foreach \angle in {45,135,225,315}{
                \pgfpathmoveto{ \pgfpointpolar{\angle}{0.6\pgf@circ@res@right}}
                \pgfpathlineto{ \pgfpointpolar{\angle}{\pgf@circ@res@right}}
            }
            \pgfsetroundcap
            \pgfusepath{draw}
            \pgfscope
                %draw connection from outside
                %anode
                \pgfsetlinewidth{\pgfstartlinewidth}
                \pgfpathmoveto{\pgfpoint{0\pgf@circ@res@left}{\pgf@circ@res@down}}
                \pgfpathlineto{\pgfpoint{0\pgf@circ@res@right}{.5\pgf@circ@res@down}}
                %cathodes
                \pgfpathmoveto{\pgfpointpolar{105}{\pgf@circ@res@up}}
                \pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{.5\pgf@circ@res@up}}
                \pgfpathmoveto{\pgfpointpolar{75}{\pgf@circ@res@up}}
                \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
                \pgfsetbuttcap
                \pgfusepath{draw}
            \endpgfscope
            %create cathode
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0}{.15\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{.5\pgf@circ@res@up}}
            \pgfusepath{draw}
            %create anode
            \pgfpathmoveto{\pgfpoint{0.3\pgf@circ@res@left}{.5\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{0.3\pgf@circ@res@right}{.5\pgf@circ@res@down}}

            \pgfsetbuttcap
            \pgfusepath{draw}
        \endpgfscope
    }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Electronic tubes, submitted by J. op den Brouw
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Draw tube outline
\def\pgf@circ@tubes@drawtube{%
	\ifdim\ctikzvalof{tubes/width}pt>\ctikzvalof{tubes/height}pt\relax
	\pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@up}}
	\pgfutil@tempdima=\pgf@circ@res@right
	\advance\pgfutil@tempdima by -\pgf@circ@res@up
	\pgfpathlineto{\pgfpoint{\pgfutil@tempdima}{\pgf@circ@res@up}}
	\pgfpatharc{90}{-90}{\pgf@circ@res@up}
	\pgfpathlineto{\pgfpoint{-\pgfutil@tempdima}{-\pgf@circ@res@up}}
	\pgfpatharc{270}{90}{\pgf@circ@res@up}
	\else
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@right}{0pt}}
	\pgfutil@tempdima=\pgf@circ@res@up
	\advance\pgfutil@tempdima by -\pgf@circ@res@right
	\pgfpathlineto{\pgfpoint{-\pgf@circ@res@right}{\pgfutil@tempdima}}
	\pgfpatharc{180}{0}{\pgf@circ@res@right}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-\pgfutil@tempdima}}
	\pgfpatharc{180}{0}{-\pgf@circ@res@right}
	\fi
	\pgfpathclose
}

%% The diode (tube), triode, tetrode and pentode only differ in the
%% number of grids. So we construct a generic declare function in
%% which we can put code for the grid anchors and grid drawing code
%% \pgfcircdeclaretube{tube name}{grid anchors}{grid drawing code}
\long\def\pgfcircdeclaretube#1#2#3{%
    \pgfdeclareshape{#1}{
        \savedmacro{\ctikzclass}{\edef\ctikzclass{tubes}}
        \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
        \anchor{center}{
            \pgfpointorigin
        }
        \savedanchor\northwest{%
            \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            \pgf@circ@res@up=\ctikzvalof{tubes/height}\pgf@circ@scaled@Rlen
            \pgf@circ@res@right=\ctikzvalof{tubes/width}\pgf@circ@scaled@Rlen
            % x and y should be half the Rlen
            \pgf@y=\pgf@circ@res@up
            \pgf@y=.5\pgf@y
            \pgf@x=-\pgf@circ@res@right
            \pgf@x=.5\pgf@x
        }
        \anchor{north} {%
            \northwest
            \pgf@x=0pt
        }
        \anchor{east}{%
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=0pt
        }
        \anchor{south}{%
            \northwest
            \pgf@y=-\pgf@y
            \pgf@x=0pt
        }
        \anchor{west}{%
            \northwest
            \pgf@y=0pt
        }
        \anchor{north west}{%
            \northwest
        }
        \anchor{north east}{%
            \northwest
            \pgf@x=-\pgf@x
        }
        \anchor{south east}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=-\pgf@y
        }
        \anchor{south west}{
            \northwest
            \pgf@y=-\pgf@y
        }
        \anchor{anode} {%
            \northwest
            \pgf@x=0pt
        }
        \anchor{cathode}{%
            \northwest
            \pgf@y=-\pgf@y
            \pgf@x=\ctikzvalof{tubes/cathode width}\pgf@x
        }
        \anchor{cathode 1}{%
            \northwest
            \pgf@y=-\pgf@y
            \pgf@x=\ctikzvalof{tubes/cathode width}\pgf@x
        }
        \anchor{cathode 2}{%
            \northwest
            \pgf@y=-\pgf@y
            \pgf@x=-\ctikzvalof{tubes/cathode width}\pgf@x
        }
        \anchor{filament 1}{%
            \northwest
            \pgfmathparse{(\ctikzvalof{tubes/tube radius}*sin(\ctikzvalof{tubes/filament angle})}
            \pgf@x=\pgfmathresult\pgf@x
            \pgf@y=-\pgf@y
        }
        \anchor{filament 2}{%
            \northwest
            \pgfmathparse{(\ctikzvalof{tubes/tube radius}*sin(\ctikzvalof{tubes/filament angle})}
            \pgf@x=-\pgfmathresult\pgf@x
            \pgf@y=-\pgf@y
        }

        % Extra anchors
        #2

        \backgroundpath{
            \pgfscope
                % Line width for tripoles
                \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
                \pgf@circ@scaled@Rlen=\scaledRlen

                % Setup to draw tube
                \pgf@circ@res@up=\ctikzvalof{tubes/height}\pgf@circ@scaled@Rlen
                \pgf@circ@res@right=\ctikzvalof{tubes/width}\pgf@circ@scaled@Rlen
                \pgf@circ@res@up=\ctikzvalof{tubes/tube radius}\pgf@circ@res@up
                \pgf@circ@res@right=\ctikzvalof{tubes/tube radius}\pgf@circ@res@right

                % Tube outline
                \pgf@circ@tubes@drawtube

                % Setup to draw grid, filament, anode and cathode
                \pgf@circ@res@up=\ctikzvalof{tubes/height}\pgf@circ@scaled@Rlen
                \pgf@circ@res@right=\ctikzvalof{tubes/width}\pgf@circ@scaled@Rlen
                \pgf@circ@res@up=0.5\pgf@circ@res@up
                \pgf@circ@res@right=0.5\pgf@circ@res@right

                % Tube fill color (if any)
                \pgf@circ@draworfill

                % Grid drawing
                #3

                % Filament (is not drawn by default)
                \ifpgf@circuit@tubes@filament
                    \pgf@circ@res@temp=-\ctikzvalof{tubes/cathode distance}\pgf@circ@res@up
                    \advance\pgf@circ@res@temp by -\ctikzvalof{tubes/filament distance}\pgf@circ@res@up
                    \pgfmathparse{(\ctikzvalof{tubes/tube radius}*sin(\ctikzvalof{tubes/filament angle})}
                    \pgf@xa=\pgfmathresult\pgf@circ@res@right
                    \pgfmathparse{\ctikzvalof{tubes/tube radius}+\ctikzvalof{tubes/tube radius}*cos(\ctikzvalof{tubes/filament angle}}
                    \pgf@ya=\pgfmathresult\pgf@circ@res@up
                    \pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@temp}}
                    \pgfpathlineto{\pgfpoint{-\pgf@xa}{-\pgf@ya}}
                    \pgfpathlineto{\pgfpoint{-\pgf@xa}{-\pgf@circ@res@up}}
                    \pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@temp}}
                    \pgfpathlineto{\pgfpoint{\pgf@xa}{-\pgf@ya}}
                    \pgfpathlineto{\pgfpoint{\pgf@xa}{-\pgf@circ@res@up}}
                    \pgf@circuit@tubes@filamentfalse
                \fi

                % Anode (or plate)
                \pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@up}} % north
                \pgfpathlineto{\pgfpoint{0pt}{\ctikzvalof{tubes/anode distance}\pgf@circ@res@up}}
                \pgfpathmoveto{\pgfpoint{-\ctikzvalof{tubes/anode width}\pgf@circ@res@right}{\ctikzvalof{tubes/anode distance}\pgf@circ@res@up}}
                \pgfpathlineto{\pgfpoint{\ctikzvalof{tubes/anode width}\pgf@circ@res@right}{\ctikzvalof{tubes/anode distance}\pgf@circ@res@up}}

                % Cathode
                \ifpgf@circuit@tubes@nocathode
                    \pgf@circuit@tubes@nocathodefalse
                \else
                    \pgfsetcornersarced{\pgfpoint{\ctikzvalof{tubes/cathode corners}\pgf@circ@res@up}{\ctikzvalof{tubes/cathode corners}\pgf@circ@res@up}}
                    \pgfpathmoveto{\pgfpoint{-\ctikzvalof{tubes/cathode width}\pgf@circ@res@right}{-\pgf@circ@res@up}}
                    \pgfpathlineto{\pgfpoint{-\ctikzvalof{tubes/cathode width}\pgf@circ@res@right}{-\ctikzvalof{tubes/cathode distance}\pgf@circ@res@up}}
                    \pgfpathlineto{\pgfpoint{\ctikzvalof{tubes/cathode width}\pgf@circ@res@right}{-\ctikzvalof{tubes/cathode distance}\pgf@circ@res@up}}
                    \ifpgf@circuit@tubes@fullcathode
                        \pgfpathlineto{\pgfpoint{\ctikzvalof{tubes/cathode width}\pgf@circ@res@right}{-\pgf@circ@res@up}}
                        \pgf@circuit@tubes@fullcathodefalse
                    \else
                        \pgfpathlineto{\pgfpoint{\ctikzvalof{tubes/cathode width}\pgf@circ@res@right}{-\ctikzvalof{tubes/cathode distance}\pgf@circ@res@up-\ctikzvalof{tubes/cathode right extend}\pgf@circ@res@up}}
                    \fi
                \fi

                % Draw the background
                \pgfusepath{draw}
            \endpgfscope
        }
    }
}

\pgfcircdeclaretube{diodetube}{}{} % shape diode already exists

\pgfcircdeclaretube{triode}
{
	\anchor{grid} {% should not be used
		\northwest
		\pgf@y=\ctikzvalof{tubes/grid shift}\pgf@y
	}
	\anchor{control} {%
		\northwest
		\pgf@y=\ctikzvalof{tubes/grid shift}\pgf@y
	}
}
{
	% Grid protrusion
	\pgf@xa=-\ctikzvalof{tubes/tube radius}\pgf@circ@res@right
	\advance\pgf@xa by -\ctikzvalof{tubes/grid protrusion}\pgf@circ@res@right
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@right}{\ctikzvalof{tubes/grid shift}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\pgf@xa}{\ctikzvalof{tubes/grid shift}\pgf@circ@res@up}}
	% Grid dashes: calculations
	\pgf@xb=2\pgf@circ@res@right
	\pgf@circ@res@step=\ctikzvalof{tubes/tube radius}\pgf@xb
	\pgf@circ@count@a=\ctikzvalof{tubes/grid dashes}  % dashes*2+1
	\multiply\pgf@circ@count@a by 2\relax
	\advance\pgf@circ@count@a by 1\relax
	\advance\pgf@circ@res@step by -\pgf@xa
	\divide\pgf@circ@res@step by \pgf@circ@count@a
	% Grid dashes: draw
	\pgf@circ@res@temp=\pgf@xa
	\pgf@circ@count@a=\ctikzvalof{tubes/grid dashes}
	\loop
	\advance\pgf@circ@res@temp by\pgf@circ@res@step
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@temp}{\ctikzvalof{tubes/grid shift}\pgf@circ@res@up}}
	\advance\pgf@circ@res@temp by\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@temp}{\ctikzvalof{tubes/grid shift}\pgf@circ@res@up}}
	\advance\pgf@circ@count@a by-1
	\ifnum\pgf@circ@count@a>0\relax
	\repeat
}

\pgfcircdeclaretube{tetrode}
{
	\anchor{grid} {% should not be used
		\northwest
		\pgfutil@tempdima=\pgf@y
		\pgf@y=-\ctikzvalof{tubes/grid separation}\pgf@y
		\pgf@y=0.5\pgf@y
		\advance\pgf@y by \ctikzvalof{tubes/grid shift}\pgfutil@tempdima
	}
	\anchor{control} {%
		\northwest
		\pgfutil@tempdima=\pgf@y
		\pgf@y=-\ctikzvalof{tubes/grid separation}\pgf@y
		\pgf@y=0.5\pgf@y
		\advance\pgf@y by \ctikzvalof{tubes/grid shift}\pgfutil@tempdima
	}
	\anchor{screen} {%
		\northwest
		\pgfutil@tempdima=\pgf@y
		\pgf@y=\ctikzvalof{tubes/grid separation}\pgf@y
		\pgf@y=0.5\pgf@y
		\advance\pgf@y by \ctikzvalof{tubes/grid shift}\pgfutil@tempdima
	}
}
{
	% Grid x/y points
	\pgf@xa=-\ctikzvalof{tubes/tube radius}\pgf@circ@res@right
	\advance\pgf@xa by -\ctikzvalof{tubes/grid protrusion}\pgf@circ@res@right
	\pgfutil@tempdima=\ctikzvalof{tubes/grid separation}\pgf@circ@res@up
	\pgfutil@tempdimb=-\pgfutil@tempdima
	\pgfutil@tempdima=0.5\pgfutil@tempdima
	\advance\pgfutil@tempdima by \ctikzvalof{tubes/grid shift}\pgf@circ@res@up
	\pgfutil@tempdimb=0.5\pgfutil@tempdimb
	\advance\pgfutil@tempdimb by \ctikzvalof{tubes/grid shift}\pgf@circ@res@up
	% Grid protrusion
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@right}{\pgfutil@tempdimb}}
	\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgfutil@tempdimb}}
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@right}{\pgfutil@tempdima}}
	\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgfutil@tempdima}}
	% Grid dashes: calculations
	\pgf@xb=2\pgf@circ@res@right
	\pgf@circ@res@step=\ctikzvalof{tubes/tube radius}\pgf@xb
	\pgf@circ@count@a=\ctikzvalof{tubes/grid dashes}  % dashes*2+1
	\multiply\pgf@circ@count@a by 2\relax
	\advance\pgf@circ@count@a by 1\relax
	\advance\pgf@circ@res@step by -\pgf@xa
	\divide\pgf@circ@res@step by \pgf@circ@count@a
	% Grid dashes: draw
	\pgf@circ@res@temp=\pgf@xa
	\pgf@circ@count@a=\ctikzvalof{tubes/grid dashes}
	\loop
	\advance\pgf@circ@res@temp by\pgf@circ@res@step
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@temp}{\pgfutil@tempdima}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@step}{\pgfutil@tempdima}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@temp}{\pgfutil@tempdimb}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@step}{\pgfutil@tempdimb}}
	\advance\pgf@circ@res@temp by\pgf@circ@res@step
	\advance\pgf@circ@count@a by-1
	\ifnum\pgf@circ@count@a>0\relax
	\repeat
}

\pgfcircdeclaretube{pentode}
{
	\anchor{grid} {% should not be used
		\northwest
		\pgfutil@tempdima=\pgf@y
		\pgf@y=-\ctikzvalof{tubes/grid separation}\pgf@y
		\advance\pgf@y by \ctikzvalof{tubes/grid shift}\pgfutil@tempdima
	}
	\anchor{control} {%
		\northwest
		\pgfutil@tempdima=\pgf@y
		\pgf@y=-\ctikzvalof{tubes/grid separation}\pgf@y
		\advance\pgf@y by \ctikzvalof{tubes/grid shift}\pgfutil@tempdima
	}
	\anchor{screen} {%
		\northwest
		\pgf@y=\ctikzvalof{tubes/grid shift}\pgf@y
	}
	\anchor{suppressor} {%
		\northwest
		\pgfutil@tempdima=\pgf@y
		\pgf@y=\ctikzvalof{tubes/grid separation}\pgf@y
		\advance\pgf@y by \ctikzvalof{tubes/grid shift}\pgfutil@tempdima
	}
}
{
	% Grid x/y points
	\pgf@xa=-\ctikzvalof{tubes/tube radius}\pgf@circ@res@right
	\advance\pgf@xa by -\ctikzvalof{tubes/grid protrusion}\pgf@circ@res@right
	\pgfutil@tempdima=\ctikzvalof{tubes/grid separation}\pgf@circ@res@up
	\pgfutil@tempdimb=-\pgfutil@tempdima
	\advance\pgfutil@tempdima by \ctikzvalof{tubes/grid shift}\pgf@circ@res@up
	\advance\pgfutil@tempdimb by \ctikzvalof{tubes/grid shift}\pgf@circ@res@up
	\pgf@circ@res@other=\ctikzvalof{tubes/grid shift}\pgf@circ@res@up
	% Grid protrusion
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@right}{\pgfutil@tempdimb}}
	\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgfutil@tempdimb}}
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@right}{\pgfutil@tempdima}}
	\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgfutil@tempdima}}
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@right}{\pgf@circ@res@other}}
	\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@circ@res@other}}
	% Grid dashes: calculations
	\pgf@xb=2\pgf@circ@res@right
	\pgf@circ@res@step=\ctikzvalof{tubes/tube radius}\pgf@xb
	\pgf@circ@count@a=\ctikzvalof{tubes/grid dashes}  % dashes*2+1
	\multiply\pgf@circ@count@a by 2\relax
	\advance\pgf@circ@count@a by 1\relax
	\advance\pgf@circ@res@step by -\pgf@xa
	\divide\pgf@circ@res@step by \pgf@circ@count@a
	% Grid dashes: draw
	\pgf@circ@res@temp=\pgf@xa
	\pgf@circ@count@a=\ctikzvalof{tubes/grid dashes}
	\loop
	\advance\pgf@circ@res@temp by\pgf@circ@res@step
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@temp}{\pgfutil@tempdima}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@step}{\pgfutil@tempdima}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@temp}{\pgfutil@tempdimb}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@step}{\pgfutil@tempdimb}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@temp}{\pgf@circ@res@other}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@step}{\pgf@circ@res@other}}
	\advance\pgf@circ@res@temp by\pgf@circ@res@step
	\advance\pgf@circ@count@a by-1
	\ifnum\pgf@circ@count@a>0\relax
	\repeat
}

\pgfcircdeclaretube{pentode suppressor to cathode}
{
	\anchor{grid} {% should not be used
		\northwest
		\pgfutil@tempdima=\pgf@y
		\pgf@y=-\ctikzvalof{tubes/grid separation}\pgf@y
		\advance\pgf@y by \ctikzvalof{tubes/grid shift}\pgfutil@tempdima
	}
	\anchor{control} {%
		\northwest
		\pgfutil@tempdima=\pgf@y
		\pgf@y=-\ctikzvalof{tubes/grid separation}\pgf@y
		\advance\pgf@y by \ctikzvalof{tubes/grid shift}\pgfutil@tempdima
	}
	\anchor{screen} {%
		\northwest
		\pgf@y=\ctikzvalof{tubes/grid shift}\pgf@y
	}
}
{
	% Grid x/y points
	\pgf@xa=-\ctikzvalof{tubes/tube radius}\pgf@circ@res@right
	\advance\pgf@xa by -\ctikzvalof{tubes/grid protrusion}\pgf@circ@res@right
	\pgfutil@tempdima=\ctikzvalof{tubes/grid separation}\pgf@circ@res@up
	\pgfutil@tempdimb=-\pgfutil@tempdima
	\advance\pgfutil@tempdima by \ctikzvalof{tubes/grid shift}\pgf@circ@res@up
	\advance\pgfutil@tempdimb by \ctikzvalof{tubes/grid shift}\pgf@circ@res@up
	\pgf@circ@res@other=\ctikzvalof{tubes/grid shift}\pgf@circ@res@up
	% Grid protrusion
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@right}{\pgfutil@tempdimb}}
	\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgfutil@tempdimb}}
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@right}{\pgf@circ@res@other}}
	\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@circ@res@other}}
	% Grid dashes: calculations
	\pgf@xb=2\pgf@circ@res@right
	\pgf@circ@res@step=\ctikzvalof{tubes/tube radius}\pgf@xb
	\pgf@circ@count@a=\ctikzvalof{tubes/grid dashes}  % dashes*2+1
	\multiply\pgf@circ@count@a by 2\relax
	\advance\pgf@circ@count@a by 1\relax
	\advance\pgf@circ@res@step by -\pgf@xa
	\divide\pgf@circ@res@step by \pgf@circ@count@a
	% Grid dashes: draw
	\pgf@circ@res@temp=\pgf@xa
	\pgf@circ@count@a=\ctikzvalof{tubes/grid dashes}
	\loop
	\advance\pgf@circ@res@temp by\pgf@circ@res@step
	\ifnum\pgf@circ@count@a>1\relax
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@temp}{\pgfutil@tempdimb}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@step}{\pgfutil@tempdimb}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@temp}{\pgf@circ@res@other}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@step}{\pgf@circ@res@other}}
	\fi
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@temp}{\pgfutil@tempdima}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@step}{\pgfutil@tempdima}}
	\advance\pgf@circ@res@temp by\pgf@circ@res@step
	\advance\pgf@circ@count@a by-1
	\ifnum\pgf@circ@count@a>0\relax
	\repeat
	% Grid: connection from suppressor to cathode
	\pgfsetcornersarced{\pgfpoint{\ctikzvalof{tubes/cathode corners}\pgf@circ@res@up}{\ctikzvalof{tubes/cathode corners}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@temp}{\pgfutil@tempdima-2*\ctikzvalof{tubes/grid separation}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\ctikzvalof{tubes/cathode width}\pgf@circ@res@right-0.4142136*\ctikzvalof{tubes/cathode corners}\pgf@circ@res@right}{-\ctikzvalof{tubes/cathode distance}\pgf@circ@res@up-0.4142136*\ctikzvalof{tubes/cathode corners}\pgf@circ@res@up}}

}

\endinput


==> pgfcircutils.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%\def\pgf@circ@handleSI#1{%
 % \pgf@circ@siunitx@resfalse
%
 % \edef\len{\stringlength[e]{#1}}
  %\testmatchingchar[e]{#1}{\len}{>}%
  %\ifmatchingchar%
  %  \ifnum\findchars{#1}{<}=0
	%  \def\pgf@circ@handleSI@val{\substring{#1}{1}{\findchars{#1}{<}-1}}
	  %\def\pgf@circ@handleSI@unit{\substring{#1}{\findchars{#1}{<}-1}+1}{\stringlength{#1}}
	  %\pgf@circ@siunitx@restrue
%	\else
%	\fi
  %\else
  %\fi
%}

\def\pgf@circ@handleSI#1{
    \noexpandarg
    \def\pgf@temp{}
    \StrBetween{#1}{<}{>}[\pgf@circ@handleSI@unit]
    \StrLen{\pgf@circ@handleSI@unit}[\pgf@circ@handleSI@unit@len]

    \ifnum\pgf@circ@handleSI@unit@len=0
    \pgf@circ@siunitx@resfalse
    \else
    \IfEndWith{#1}{>}{
        \pgf@circ@siunitx@restrue
        \noexpandarg
        \StrBefore{#1}{<}[\pgf@circ@handleSI@val]
        %\typeout{si |#1|}
        }{
        \pgf@circ@siunitx@resfalse
        %\typeout{no si |#1|}
    }
\fi
}

\def\pgf@circ@ifkeyempty#1{
    \pgfextra{
        \ctikzset{#1/.get=\pgf@circ@temp}
        \edef\pgf@temp{}
    }
    \ifx\pgf@circ@temp\pgf@temp
    }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%    Math routines

\def\pgf@circ@stripdecimals#1.#2\pgf@nil{#1}

%%%%%%%
%% flipping text

\def\ctikzflipx#1{\scalebox{-1}[1]{#1}}
\def\ctikzflipy#1{\scalebox{1}[-1]{#1}}
\def\ctikzflipxy#1{\scalebox{-1}[-1]{#1}}

\endinput


==> pgfcircvoltage.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Voltage management

%% styles
\ctikzset{bipole voltage style/.style={}}
\tikzset{bipole voltage style/.code={
        \ctikzset{bipole voltage style/.style={#1}}
}}
\tikzset{bipole voltage append style/.code={
        \ctikzset{bipole voltage style/.append style={#1}}
}}

\ctikzset{v^>/.style = {
        v = #1,
        \circuitikzbasekey/bipole/voltage/direction = forward,
        \circuitikzbasekey/bipole/voltage/position = above
    }
}

\ctikzset{v^</.style = {
        v = #1,
        \circuitikzbasekey/bipole/voltage/direction = backward,
        \circuitikzbasekey/bipole/voltage/position = above
    }
}

\ctikzset{v_>/.style = {
        v = #1,
        \circuitikzbasekey/bipole/voltage/direction = forward,
        \circuitikzbasekey/bipole/voltage/position = below
    }
}

\ctikzset{v_</.style = {
        v = #1,
        \circuitikzbasekey/bipole/voltage/direction = backward,
        \circuitikzbasekey/bipole/voltage/position = below
    }
}

\ctikzset{v_/.style = {v = #1, \circuitikzbasekey/bipole/voltage/position = below} }
\ctikzset{v^/.style = {v = #1, \circuitikzbasekey/bipole/voltage/position  = above} }
\ctikzset{v>/.style = {v = #1, \circuitikzbasekey/bipole/voltage/direction = forward} }
\ctikzset{v</.style = {v = #1, \circuitikzbasekey/bipole/voltage/direction = backward} }

% Default position varies whether the component is a voltage source
% or not
\ctikzset{v/.code = {
        \ifpgf@circuit@bipole@isvoltage
            \pgfkeys{\circuitikzbasekey/bipole/voltage/position=above,
            \circuitikzbasekey/bipole/voltage/direction=forward}
        \else
            \ifpgf@circ@oldvoltagedirection
                \pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
                \circuitikzbasekey/bipole/voltage/direction=backward}
            \else
                \pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
                \circuitikzbasekey/bipole/voltage/direction=forward}
            \fi
        \fi
        \ifpgf@circ@oldvoltagedirection
            \ifpgf@circuit@bipole@iscurrent\ifpgf@circ@fixbatteries
                \pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
                \circuitikzbasekey/bipole/voltage/direction=forward}
        \fi\fi
        \else
        \ifpgf@circuit@bipole@iscurrent
            \ifpgf@circuit@bipole@current@backward
                \pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
                \circuitikzbasekey/bipole/voltage/direction=forward}
            \else
                \pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
                \circuitikzbasekey/bipole/voltage/direction=backward}
            \fi\fi\fi
            \pgfkeys{/tikz/circuitikz/bipole/voltage/label/name=#1}
            \ctikzsetvalof{bipole/voltage/label/unit}{}
            \ifpgf@circ@siunitx
                \pgf@circ@handleSI{#1}
                \ifpgf@circ@siunitx@res
                    \edef\pgf@temp{\pgf@circ@handleSI@val}
                    \pgfkeyslet{/tikz/circuitikz/bipole/voltage/label/name}{\pgf@temp}
                    \edef\pgf@temp{\pgf@circ@handleSI@unit}
                    \pgfkeyslet{/tikz/circuitikz/bipole/voltage/label/unit}{\pgf@temp}
                \else
            \fi
            \else
        \fi
    }
}

% american voltage font selection and symbol definition
% the default font command is {} --- nothing
\def\pgf@circ@avfont{\ctikzvalof{voltage/american font}}
%
% plus and minus symbols (default is $+$ and $-$, see pgfcirc.defines.tex)
%
\def\pgf@circ@avplus{\ctikzvalof{voltage/american plus}}
\def\pgf@circ@avminus{\ctikzvalof{voltage/american minus}}

%%
\def\setscaledRlenforclass{%
    \csname pgf@sh@ma@\ctikzvalof{bipole/name}\endcsname
    \ifdefined\ctikzclass
        \edef\pgf@temp{/tikz/circuitikz/\ctikzclass/scale}
        \pgfkeysifdefined{\pgf@temp}
            {\pgf@circ@scaled@Rlen=\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
            {\pgf@circ@scaled@Rlen=\pgf@circ@Rlen}
    \else
        \pgf@circ@scaled@Rlen=\pgf@circ@Rlen
    \fi
}

%% Output routine for generic bipoles

\def\pgf@circ@drawvoltagegeneric{
    \pgfextra{
        % \typeout{NAME:\ctikzvalof{bipole/name}}
        \edef\pgf@temp{/tikz/circuitikz/bipoles/\ctikzvalof{bipole/kind}/voltage/straight label distance}
        \pgfkeysifdefined{\pgf@temp}
        {
            \edef\partheight{\ctikzvalof{bipoles/\ctikzvalof{bipole/kind}/voltage/straight label distance}}
            \edef\tmpdistfromline{(\partheight\pgf@circ@scaled@Rlen)}
        }
        {
            \pgfkeysifdefined{/tikz/circuitikz/bipoles/voltage/straight label distance}
            {
                \edef\partheight{\ctikzvalof{bipoles/voltage/straight label distance}}
                \edef\tmpdistfromline{(\partheight\pgf@circ@scaled@Rlen)}
            }
            {%calculate default value from part height
                \edef\pgf@temp{/tikz/circuitikz/bipoles/\ctikzvalof{bipole/kind}/height}
                \pgfkeysifdefined{\pgf@temp}
                {
                    \edef\partheight{0.5*\ctikzvalof{bipoles/\ctikzvalof{bipole/kind}/height}}
                    \edef\tmpdistfromline{(\partheight\pgf@circ@scaled@Rlen+0.2\pgf@circ@scaled@Rlen)}
                }
                {
                    \edef\tmpdistfromline{(.5\pgf@circ@scaled@Rlen)} %fallback to fixed value
                }
            }
        }
        % \typeout{KIND:\ctikzvalof{bipole/kind}\space RLEN:\the\pgf@circ@Rlen\space SCALED:\the\pgf@circ@scaled@Rlen}
        \ifnum \ctikzvalof{mirror value}=-1
        \ifpgf@circuit@bipole@inverted
            \ifpgf@circuit@bipole@voltage@straight
                \def\distfromline{\tmpdistfromline}
            \else
                \def\distfromline{\ctikzvalof{voltage/distance from line}\pgf@circ@scaled@Rlen}
            \fi
            \else
            \ifpgf@circuit@bipole@voltage@straight
                \def\distfromline{-\tmpdistfromline}
            \else
                \def\distfromline{-\ctikzvalof{voltage/distance from line}\pgf@circ@scaled@Rlen}
            \fi
        \fi
        \else
            \ifpgf@circuit@bipole@inverted
                \ifpgf@circuit@bipole@voltage@straight
                    \def\distfromline{-\tmpdistfromline}
                \else
                    \def\distfromline{-\ctikzvalof{voltage/distance from line}\pgf@circ@scaled@Rlen}
                \fi
                \else
                \ifpgf@circuit@bipole@voltage@straight
                    \def\distfromline{\tmpdistfromline}
                \else
                    \def\distfromline{\ctikzvalof{voltage/distance from line}\pgf@circ@scaled@Rlen}
                \fi
            \fi
        \fi
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@voltage@angle{90}
        \else
            \def\pgf@circ@voltage@angle{-90}
        \fi
        \edef\pgf@temp{/tikz/circuitikz/bipoles/\ctikzvalof{bipole/kind}/voltage/distance from node}
        \pgfkeysifdefined{\pgf@temp}
            { \edef\distancefromnode{\ctikzvalof{bipoles/\ctikzvalof{bipole/kind}/voltage/distance from node}} }
            { \edef\distancefromnode{\ctikzvalof{voltage/distance from node}} }
        \edef\pgf@temp{/tikz/circuitikz/bipoles/\ctikzvalof{bipole/kind}/voltage/bump b}
        \pgfkeysifdefined{\pgf@temp}
            { \edef\bumpb{\ctikzvalof{bipoles/\ctikzvalof{bipole/kind}/voltage/bump b}} }
            { \edef\bumpb{\ctikzvalof{voltage/bump b}} }
        \edef\shiftv{\ctikzvalof{voltage/shift}}
        \newdimen{\absvshift}
        \pgfmathsetlength{\absvshift}{\shiftv*\distfromline+\distfromline}
        % put this to true to see the voltage label coordinate anchors
        \newif\ifpgf@circ@debugv\pgf@circ@debugvfalse
    }
    % %\pgf@circ@Rlen/\ctikzvalof{current arrow scale} is equal to the length of the currarrow
    coordinate (pgfcirc@midtmp) at ($(\tikztostart) ! \pgf@circ@Rlen/\ctikzvalof{current arrow scale} ! (anchorstartnode)$) %absolute move, minimum space is length of arrowhead
    coordinate (pgfcirc@midtmp) at ($(pgfcirc@midtmp) ! \distancefromnode ! (anchorstartnode)$)
    coordinate (pgfcirc@Vfrom@flat) at (pgfcirc@midtmp)
    coordinate (pgfcirc@Vfrom) at ($(pgfcirc@midtmp) ! -\distfromline ! \pgf@circ@voltage@angle:(anchorstartnode)$)

    coordinate (pgfcirc@midtmp) at ($(\tikztotarget) ! \pgf@circ@Rlen/\ctikzvalof{current arrow scale} ! (anchorendnode)$)%absolute move, minimum space is length of arrowhead
    coordinate (pgfcirc@midtmp) at ($(pgfcirc@midtmp) ! \distancefromnode ! (anchorendnode)$)
    coordinate (pgfcirc@Vto@flat) at (pgfcirc@midtmp)
    coordinate (pgfcirc@Vto) at ($(pgfcirc@midtmp) ! \distfromline ! \pgf@circ@voltage@angle : (anchorendnode)$)

    \ifpgf@circuit@bipole@voltage@below
        \ifpgf@circ@debugv
            node [ocirc, fill=red] at (anchorstartnode) {}
            node [ocirc, fill=blue] at (anchorendnode) {}
            node [ocirc, fill=green] at (pgfcirc@Vto) {}
            node [ocirc, fill=yellow] at (pgfcirc@Vfrom) {}
            node [odiamondpole, fill=green] at (pgfcirc@Vto@flat) {}
            node [odiamondpole, fill=yellow] at (pgfcirc@Vfrom@flat) {}
        \fi
        coordinate (pgfcirc@Vto) at ($(pgfcirc@Vto@flat) ! \absvshift!90 :  (anchorendnode)$)
        coordinate (pgfcirc@Vfrom) at ($(pgfcirc@Vfrom@flat) ! \absvshift!-90 :  (anchorstartnode)$)
        coordinate (pgfcirc@Vcont1t) at ($(\ctikzvalof{bipole/name}.center) ! \bumpb ! (\ctikzvalof{bipole/name}.-110)$)
        coordinate (pgfcirc@Vcont2t) at ($(\ctikzvalof{bipole/name}.center) ! \bumpb ! (\ctikzvalof{bipole/name}.-70)$)
        coordinate (pgfcirc@Vcont1) at ($(pgfcirc@Vcont1t) ! -\absvshift!90 : (pgfcirc@Vcont2t)$)
        coordinate (pgfcirc@Vcont2) at ($(pgfcirc@Vcont2t) ! -\absvshift!-90 : (pgfcirc@Vcont1t)$)
        \ifpgf@circ@debugv
            node [odiamondpole, fill=green] at (pgfcirc@Vto) {}
            node [odiamondpole, fill=yellow] at (pgfcirc@Vfrom) {}
            node [osquarepole, fill=red] at (pgfcirc@Vcont1) {}
            node [osquarepole, fill=blue] at (pgfcirc@Vcont2) {}
        \fi
    \else
        \ifpgf@circ@debugv
            node [ocirc, fill=red] at (anchorstartnode) {}
            node [ocirc, fill=blue] at (anchorendnode) {}
            node [ocirc, fill=green] at (pgfcirc@Vto) {}
            node [ocirc, fill=yellow] at (pgfcirc@Vfrom) {}
            node [odiamondpole, fill=green] at (pgfcirc@Vto@flat) {}
            node [odiamondpole, fill=yellow] at (pgfcirc@Vfrom@flat) {}
        \fi
        coordinate (pgfcirc@Vto) at ($(pgfcirc@Vto@flat) ! -\absvshift!90 :  (anchorendnode)$)
        coordinate (pgfcirc@Vfrom) at ($(pgfcirc@Vfrom@flat) ! -\absvshift!-90 :  (anchorstartnode)$)
        coordinate (pgfcirc@Vcont1t) at ($(\ctikzvalof{bipole/name}.center) ! \bumpb ! (\ctikzvalof{bipole/name}.110)$)
        coordinate (pgfcirc@Vcont2t) at ($(\ctikzvalof{bipole/name}.center) ! \bumpb ! (\ctikzvalof{bipole/name}.70)$)
        coordinate (pgfcirc@Vcont1) at ($(pgfcirc@Vcont1t) ! \absvshift!90 : (pgfcirc@Vcont2t)$)
        coordinate (pgfcirc@Vcont2) at ($(pgfcirc@Vcont2t) ! \absvshift!-90 : (pgfcirc@Vcont1t)$)
        \ifpgf@circ@debugv
            node [odiamondpole, fill=green] at (pgfcirc@Vto) {}
            node [odiamondpole, fill=yellow] at (pgfcirc@Vfrom) {}
            node [osquarepole, fill=red] at (pgfcirc@Vcont1) {}
            node [osquarepole, fill=blue] at (pgfcirc@Vcont2) {}
        \fi
    \fi

    \ifpgf@circuit@europeanvoltage
        \ifpgf@circuit@bipole@voltage@straight
            \ifpgf@circuit@bipole@voltage@backward
                (pgfcirc@Vto) --(pgfcirc@Vfrom) node[currarrow, sloped,  allow upside down, pos=1,anchor=tip] {}
            \else
                (pgfcirc@Vfrom) --(pgfcirc@Vto) node[currarrow, sloped,  allow upside down, pos=1,anchor=tip] {}
            \fi
            \else
            \ifpgf@circuit@bipole@voltage@backward
                (pgfcirc@Vto) .. controls (pgfcirc@Vcont2)  and (pgfcirc@Vcont1) ..
                node[currarrow, sloped,  allow upside down, pos=1, anchor=tip] {}
                (pgfcirc@Vfrom)
            \else
                (pgfcirc@Vfrom) .. controls (pgfcirc@Vcont1)  and (pgfcirc@Vcont2) ..
                node[currarrow, sloped,  allow upside down, pos=1, anchor=tip] {}
                (pgfcirc@Vto)
            \fi
        \fi
        \else
        \ifpgf@circuit@bipole@voltage@backward
            \ifpgf@circ@oldvoltagedirection
                (pgfcirc@Vfrom) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avplus}
                (pgfcirc@Vto) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avminus}
            \else
                (pgfcirc@Vfrom) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avminus}
                (pgfcirc@Vto) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avplus}
            \fi
            \else
            \ifpgf@circ@oldvoltagedirection
                (pgfcirc@Vfrom) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avminus}
                (pgfcirc@Vto) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avplus}
            \else
                (pgfcirc@Vfrom) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avplus}
                (pgfcirc@Vto) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avminus}
            \fi
        \fi
    \fi
}

%% Output routine for voltage sources
\def\pgf@circ@drawvoltagegenerator{
    % the following is affected indirectly by voltage/shift, you can move the arrow with voltage/bump a.
    % it's not perfect, but I can't find the way to do it correctly...
    \pgfextra{
        \edef\shiftv{\ctikzvalof{voltage/shift}}
        \edef\bumpa{\ctikzvalof{voltage/bump a}}
        \pgfmathsetmacro{\bumpaplus}{\bumpa + 0.5*\shiftv} % coefficient added "by feel". Sorry.
    }
    \ifpgf@circuit@bipole@voltage@below
        coordinate (pgfcirc@Vfrom) at ($(\ctikzvalof{bipole/name}.center) ! \bumpaplus ! (\ctikzvalof{bipole/name}.-120)$)
        coordinate (pgfcirc@Vto) at ($(\ctikzvalof{bipole/name}.center) ! \bumpaplus ! (\ctikzvalof{bipole/name}.-60)$)
    \else
        coordinate (pgfcirc@Vfrom) at ($ (\ctikzvalof{bipole/name}.center) ! \bumpaplus ! (\ctikzvalof{bipole/name}.120)$)
        coordinate (pgfcirc@Vto) at ($ (\ctikzvalof{bipole/name}.center) ! \bumpaplus ! (\ctikzvalof{bipole/name}.60)$)
    \fi
    % fix the (unused in this case) Vcont1/2 coords for label placement along the line
    coordinate (pgfcirc@Vcont1) at (pgfcirc@Vto)
    coordinate (pgfcirc@Vcont2) at (pgfcirc@Vfrom)
    \ifpgf@circuit@europeanvoltage
        \ifpgf@circuit@bipole@voltage@backward
            (pgfcirc@Vto)  -- node[currarrow, sloped,  allow upside down, pos=1, anchor=tip] {} (pgfcirc@Vfrom)
        \else
            (pgfcirc@Vfrom)  -- node[currarrow, sloped,  allow upside down, pos=1, anchor=tip] {} (pgfcirc@Vto)
        \fi
        \else% american voltage
        \ifpgf@circuit@bipole@voltageoutsideofsymbol
            % if it is a battery, must put + and -

            \ifpgf@circ@fixbatteries
                \ifpgf@circuit@bipole@voltage@backward
                    (pgfcirc@Vfrom)  node[node font=\pgf@circ@avfont] {\pgf@circ@avplus}
                    (pgfcirc@Vto) node[node font=\pgf@circ@avfont] {\pgf@circ@avminus}
                \else
                    (pgfcirc@Vfrom)  node[node font=\pgf@circ@avfont] {\pgf@circ@avminus}
                    (pgfcirc@Vto) node[node font=\pgf@circ@avfont] {\pgf@circ@avplus}
                \fi
                \else
                \ifpgf@circuit@bipole@voltage@backward
                    (pgfcirc@Vfrom)  node[node font=\pgf@circ@avfont] {\pgf@circ@avminus}
                    (pgfcirc@Vto) node[node font=\pgf@circ@avfont] {\pgf@circ@avplus}
                \else
                    (pgfcirc@Vfrom)  node[node font=\pgf@circ@avfont] {\pgf@circ@avplus}
                    (pgfcirc@Vto) node[node font=\pgf@circ@avfont] {\pgf@circ@avminus}
                \fi
            \fi
        \fi
    \fi
}

%% Output routine
\def\pgf@circ@drawvoltage{% node name
    \pgfextra{ %WARNING: indentation is probably wrong
        \edef\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
        \ifnum\pgfcircmathresult >4 \ifnum\pgfcircmathresult <86
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{north west}
        \else
            \def\pgf@circ@bipole@voltage@label@anchor{south east}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >85 \ifnum\pgfcircmathresult <95
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{west}
        \else
            \def\pgf@circ@bipole@voltage@label@anchor{east}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >94 \ifnum\pgfcircmathresult <176
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{south west}
        \else \def\pgf@circ@bipole@voltage@label@anchor{north east}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >175 \ifnum\pgfcircmathresult <185
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{south}
        \else\def\pgf@circ@bipole@voltage@label@anchor{north}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >184 \ifnum\pgfcircmathresult <266
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{south east}
        \else\def\pgf@circ@bipole@voltage@label@anchor{north west}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >265 \ifnum\pgfcircmathresult <275
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{east}
        \else \def\pgf@circ@bipole@voltage@label@anchor{west}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >274 \ifnum\pgfcircmathresult <356
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{north east}
        \else\def\pgf@circ@bipole@voltage@label@anchor{south west}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >-1 \ifnum\pgfcircmathresult <5
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{north}
        \else\def\pgf@circ@bipole@voltage@label@anchor{south}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >355 \ifnum\pgfcircmathresult <361
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{north}
        \else\def\pgf@circ@bipole@voltage@label@anchor{south}
        \fi
        \fi\fi

        % this must be set *before* changing for mirroring and inverting; in that case
        % the xscale/yscale parameters take it into account
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@where{-90}
        \else
            \def\pgf@circ@bipole@voltage@label@where{90}
        \fi

        % magic to counteract the scale and yscale effects (there should be a better way...)
        \ifnum \ctikzvalof{mirror value}=-1
            \ifpgf@circuit@bipole@voltage@below
                \pgf@circuit@bipole@voltage@belowfalse
            \else
                \pgf@circuit@bipole@voltage@belowtrue
            \fi
        \fi

        \ifpgf@circuit@bipole@inverted
            \ifpgf@circuit@bipole@voltage@below
                \pgf@circuit@bipole@voltage@belowfalse
            \else
                \pgf@circuit@bipole@voltage@belowtrue
            \fi
        \fi

        % take into account scaling
        \setscaledRlenforclass

        \edef\pgf@temp{/tikz/circuitikz/bipoles/\ctikzvalof{bipole/kind}/voltage/european label distance}
        \pgfkeysifdefined{\pgf@temp}
            { \edef\eudist{\ctikzvalof{bipoles/\ctikzvalof{bipole/kind}/voltage/european label distance}} }
            { \edef\eudist{\ctikzvalof{voltage/european label distance}} }
        % find the height of the bipole or use a default value
        \edef\pgf@temp{/tikz/circuitikz/bipoles/\ctikzvalof{bipole/kind}/height}
        \pgfkeysifdefined{\pgf@temp}
            {\pgfmathsetmacro{\partheightf}{0.5*\ctikzvalof{bipoles/\ctikzvalof{bipole/kind}/height}}
             \edef\partheight{\partheightf\pgf@circ@scaled@Rlen}}
            {\edef\partheight{(.5\pgf@circ@scaled@Rlen)}} %fallback to fixed value
        \newdimen{\alshift}
        % this is more or less the same of the legacy code; we shift the american label a bit
        % outside the (+) -- (-) line
        \pgfmathsetlength{\alshift}{(\ctikzvalof{voltage/american label distance}-0.6)*\partheight}
        \pgfsetcornersarced{\pgfpointorigin}% do not use rounded corners!
    }%end pgfextra

    \ifpgf@circuit@bipole@isvoltage
        \pgf@circ@drawvoltagegenerator
    \else
        \pgf@circ@drawvoltagegeneric
    \fi

    \ifpgf@circuit@bipole@voltage@straight
        coordinate (Vlab) at ($(pgfcirc@Vto)!0.5!(pgfcirc@Vfrom) $)
        node [anchor=\pgf@circ@bipole@voltage@label@anchor, inner sep=2pt,
        \circuitikzbasekey/bipole voltage style](\ctikzvalof{bipole/name}voltage)
        at (Vlab) {\pgf@circ@finallabels{voltage/label}}
    \else
        \ifpgf@circuit@europeanvoltage
            coordinate (Vlab) at ($(pgfcirc@Vcont1)!0.5!(pgfcirc@Vcont2)$)
        \else
            coordinate (Vlab) at ($(pgfcirc@Vfrom)!0.5!(pgfcirc@Vto)$)
            \ifpgf@circuit@bipole@isvoltage\else
            % add a bit of space for american labels above their symbols in the normal case. You can avoid that
            % with voltage/american label distance=0.5 (it's measured from the center of the component, in heights)
                coordinate (Vlab) at ($(Vlab) ! \alshift ! \pgf@circ@bipole@voltage@label@where :(pgfcirc@Vto)$)
            \fi
        \fi
        node [anchor=\pgf@circ@bipole@voltage@label@anchor, inner sep=2pt,
        \circuitikzbasekey/bipole voltage style](\ctikzvalof{bipole/name}voltage)
        at (Vlab) {\pgf@circ@finallabels{voltage/label}}
    \fi
}%end drawvoltages
\endinput

